An Estimate of the Binary Star Fraction Among Young Stars at the Galactic Center: Possible Evidence of a Radial Dependence

We present the first estimate of the intrinsic binary fraction of young stars across the central $\approx$ 0.4 pc surrounding the supermassive black hole (SMBH) at the Milky Way Galactic center (GC). This experiment searched for photometric variability in 102 young stars, using 119 nights of 10"-wide adaptive optics imaging observations taken at Keck Observatory over 16 years in the K'- and H-bands. We photometrically detected three binary stars, all of which are situated more than 1" (0.04 pc) from the SMBH and one of which, S2-36, is newly reported here with spectroscopic confirmation. To convert the observed binary fraction into an estimate of the underlying binary fraction, we determined experiment sensitivity through detailed light curve simulations, incorporating photometric effects of eclipses, irradiation, and tidal distortion in binaries. The simulations assumed a population of young binaries, with stellar ages (4 Myr) and masses matched to the most probable values measured for the GC young star population and underlying binary system parameters similar to those of local massive stars. The detections and simulations imply young, massive stars in the GC have a stellar binary fraction $\geq$ 71% (68% confidence), or $\geq$ 42% (95% confidence). This inferred GC young star binary fraction is consistent with that typically seen in young stellar populations in the solar neighborhood. Furthermore, our measured binary fraction is significantly higher than that recently reported by Chu et al. (2023) based on RV measurements of young stars <~1" of the SMBH. Constrained with these two studies, the probability that the same underlying young binary fraction extends across the entire region is <1.4%. This tension provides support for a radial dependence of the binary star fraction and, therefore, for the dynamical predictions of binary merger and evaporation events close to the SMBH.

==> Sections/PhotCal.tex <==
\begin{deluxetable*}{ll|lll|lll}[t]
    \tablewidth{0pt}
    \tablecolumns{8}
    \tablecaption{Photometric Calibrator Star Bandpass Corrected Reference Fluxes\label{tab:bandpass_corr}}
    \tablehead{
        \colhead{Star Name}     &
        \colhead{Spectral Type} &
        \colhead{$K$s$_{\text{S10}}$}                        &
		\colhead{$K$s$_{\text{S10}} - K'_{\text{NIRC2}}$}    &
        \colhead{$K'_{\text{NIRC2}}$}                                   &
        \colhead{$H_{\text{S10}}$}                        &
		\colhead{$H_{\text{S10}} - H_{\text{NIRC2}}$}    &
        \colhead{$H_{\text{NIRC2}}$}
    }
    \startdata
    IRS 16NW    & Wolf-Rayet    & $10.14 \pm 0.06$   & $-0.05$          & $10.19 \pm 0.06$  & $12.03 \pm 0.06$  & $-0.15 \pm 0.01$  & $12.18 \pm 0.07$  \\
    S3-22       & Late-Type     & $11.03 \pm 0.06$   & $-0.05$          & $11.08 \pm 0.06$  & $13.16 \pm 0.07$  & $-0.18$           & $13.34 \pm 0.07$  \\
    S2-22       & Early-Type    & $12.98 \pm 0.09$   & $-0.05$          & $13.03 \pm 0.09$  & $14.75 \pm 0.08$  & $-0.14 \pm 0.01$  & $14.89 \pm 0.09$  \\
    S4-3        & Late-Type     & $12.91 \pm 0.07$   & $-0.05$          & $12.96 \pm 0.07$  & $14.86 \pm 0.07$  & $-0.16 \pm 0.01$  & $15.02 \pm 0.08$  \\
    S1-1        & Early-Type    & $13.09 \pm 0.07$   & $-0.05$          & $13.04 \pm 0.07$  & $14.95 \pm 0.07$  & $-0.15 \pm 0.01$  & $15.10 \pm 0.08$  \\
    S1-21       & Early-Type    & $13.26 \pm 0.06$   & $-0.07 \pm 0.01$ & $13.33 \pm 0.07$  & $15.60 \pm 0.07$  & $-0.20 \pm 0.01$  & $15.80 \pm 0.08$  \\
    S1-12       & Early-Type    & $13.52 \pm 0.07$   & $-0.05 \pm 0.01$ & $13.57 \pm 0.07$  & $15.41 \pm 0.08$  & $-0.15 \pm 0.01$  & $15.56 \pm 0.09$  \\
    S2-2        & Late-Type     & $13.97 \pm 0.06$   & $-0.04$          & $14.01 \pm 0.06$  & $15.51 \pm 0.06$  & $-0.13 \pm 0.01$  & $15.64 \pm 0.07$  \\
    S3-88       & Late-Type     & $14.23 \pm 0.06$   & $-0.05$          & $14.28 \pm 0.06$  & $16.24 \pm 0.07$  & $-0.17 \pm 0.01$  & $16.41 \pm 0.08$  \\
    S2-75       & Late-Type     & $14.38 \pm 0.08$   & $-0.05$          & $14.43 \pm 0.08$  & $16.46 \pm 0.08$  & $-0.18 \pm 0.01$  & $16.64 \pm 0.09$  \\
    S3-36       & Late-Type     & $14.61 \pm 0.09$   & $-0.05$          & $14.66 \pm 0.09$  & $16.49 \pm 0.09$  & $-0.16 \pm 0.01$  & $16.65 \pm 0.10$  \\
    S1-33       & Early-Type    & $14.96 \pm 0.07$   & $-0.05$          & $15.01 \pm 0.07$  & $16.84 \pm 0.08$  & $-0.15 \pm 0.01$  & $15.01 \pm 0.09$  \\
    \enddata   
    \tablerefs{S10: \cite{Schodel:2010}}
\end{deluxetable*}

\section{Photometric Calibration Details} % (fold)
\label{sec:phot_calibration_details}
Table~\ref{tab:bandpass_corr} collects the bandpass corrections for the calibrator stars from the \citet{Schodel:2010} catalog measurements to the respective NIRC2 bandpasses. The bandpass corrected $K'_{\text{NIRC2}}$ and $H_{\text{NIRC2}}$ are the reference calibrator magnitudes used for the absolute photometric calibration step used in this work.

% The absolute photometric uncertainty is contributed by the uncertainty in zero-point correction during the initial, absolute photometric calibration. In \citetalias{2019ApJ...871..103K}, the median zero-point uncertainty across all their observations during absolute photometric calibration was 0.179 magnitudes. The median zero-point uncertainty across all $K'$-band observations during absolute photometric calibration in this work is 0.060 magnitudes, or 0.056 magnitudes when only considering the same observations as used in \citetalias{2019ApJ...871..103K}. The lower absolute photometry zero-point correction uncertainty in this work compared to \citetalias{2019ApJ...871..103K} is a result of our revised calculation of calibrator star reference fluxes (detailed in Section~\ref{sub:photometric_measurement_and_calibration}), derived from the high resolution  \citet{Schodel:2010} catalog. The median zero-point uncertainty across all $H$-band observations during absolute photometric calibration in this work is 0.2215 magnitudes.
%
% The final photometric uncertainty is largely contributed by the uncertainty in zero-point correction during the final (relative) photometric calibration step. This quantity is shown for all our observations in Figure~\ref{fig:zeropointsErrs}. Across all observations in this work, the median zero-point correction error is 0.032 mag in $K'$-band and 0.034 mag in $H$-band. In \citetalias{2019ApJ...871..103K}, the median zero-point correction error was 0.027 mag. The difference largely originates from this work including observations in 2018 and 2019, several of which were derived from fewer frames leading to poorer image quality and higher uncertainty in the zero-point correction. When comparing the same observations as were used in \citetalias{2019ApJ...871..103K}, the calibration procedure used in this work leads to a median zero-point correction error of 0.029 mag. The remaining difference is small and is a consequence of the differences in photometric calibration that are detailed in Section~\ref{sub:photometric_measurement_and_calibration}.

==> Tables/Sample/samp_cat.tex <==
%    /\_/\
%   ( o.o )
%    > ^ <
% Samp Cat (Sample Catalog)

\begin{longrotatetable}
\begin{deluxetable}{l|DD|r|rr|DD|cc|D|DDD}
    \tablehead{
        \colhead{Star} &
        \multicolumn2c{$\overline{m}_{K'}$} & \multicolumn2c{$\overline{m}_{H}$} &
        \colhead{Star Age} &
        \colhead{$K'$} & \colhead{$H$} &
        \multicolumn2c{$\chi^2_{\text{red, }K'}$} & \multicolumn2c{$\chi^2_{\text{red, }H}$} &
        \colhead{$K'$} & \colhead{$H$} &
        \multicolumn2c{Injected Binary} &
        \multicolumn2c{$x_0$} & \multicolumn2c{$y_0$} & \multicolumn2c{$t_0$} \\
        \colhead{} &
        \multicolumn2c{} & \multicolumn2c{} &
        \colhead{} &
        \colhead{Nights} & \colhead{Nights} &
        \multicolumn2c{} & \multicolumn2c{} &
        \colhead{Var.?} & \colhead{Var.?} &
        \multicolumn2c{Recovery Fraction} &
        \multicolumn2c{($''$ E of}  & \multicolumn2c{($''$ N of}    & \multicolumn2c{}  \\
        \colhead{}  &
        \multicolumn2c{} & \multicolumn2c{} &
        \colhead{}  &
        \colhead{}  & \colhead{}    &
        \multicolumn2c{}    & \multicolumn2c{}  &
        \colhead{}  & \colhead{}    &
        \multicolumn2c{}    &
        \multicolumn2c{Sgr A*)} & \multicolumn2c{Sgr A*)}   & \multicolumn2c{}
    }
    \tablecaption{Stellar sample\label{tab:stellar_sample}}
\decimals
\startdata
IRS 16C & 10.03 & 12.07 & Known Young & 100 & 19 & 4.20 & 3.48 & Yes & No & 0.11 & 1.05 & 0.55 & 2009.989 \\
IRS 16SW & 10.08 & 12.16 & Known Young & 100 & 19 & 16.02 & 26.02 & Yes & Yes & 0.02 & 1.11 & -0.95 & 2009.820 \\
IRS 16NW & 10.28 & 12.34 & Known Young & 100 & 19 & 1.89 & 0.71 & Yes & No & 0.06 & 0.08 & 1.22 & 2010.047 \\
IRS 33E & 10.29 & 12.51 & Known Young & 100 & 19 & 1.22 & 0.61 & No & No & 0.10 & 0.71 & -3.14 & 2010.182 \\
S2-17 & 10.69 & 12.74 & Known Young & 100 & 19 & 1.10 & 2.48 & No & No & 0.01 & 1.34 & -1.88 & 2010.154 \\
S5-89 & 10.90 & 13.30 & Known Old & 99 & 19 & 1.23 & 1.27 & No & No & 0.04 & -0.79 & -5.25 & 2010.162 \\
IRS 16CC & 10.99 & 13.46 & Known Young & 100 & 19 & 80.36 & 67.19 & Yes & Yes & 0.00 & 1.98 & 0.60 & 2010.135 \\
S3-22 & 11.12 & 13.46 & Known Old & 100 & 19 & 0.38 & 0.53 & No & No & 0.09 & -0.34 & -3.21 & 2010.201 \\
IRS 16SW-E & 11.22 & 14.36 & Known Young & 92 & 19 & 5.61 & 12.51 & Yes & Yes & 0.00 & 1.90 & -1.12 & 2010.045 \\
S6-12 & 11.27 & 13.74 & Unknown Age & 93 & 19 & 3.49 & 3.39 & Yes & No & 0.01 & -0.21 & -6.08 & 2010.161 \\
IRS 33N & 11.29 & 13.48 & Known Young & 100 & 19 & 3.59 & 3.98 & Yes & Yes & 0.04 & -0.03 & -2.24 & 2010.161 \\
S6-63 & 11.31 & 13.44 & Known Young & 87 & 17 & 2.06 & 2.26 & Yes & No & 0.03 & 1.87 & -6.31 & 2011.057 \\
S4-207 & 11.32 & 14.31 & Known Old & 99 & 18 & 6.32 & 10.38 & Yes & Yes & 0.02 & -4.05 & -2.08 & 2009.835 \\
IRS 29S & 11.38 & 13.75 & Known Old & 100 & 19 & 0.60 & 1.05 & No & No & 0.04 & -1.84 & 0.96 & 2010.201 \\
S1-24 & 11.42 & 13.62 & Known Young & 73 & 19 & 1.78 & 4.01 & No & Yes & 0.02 & 0.74 & -1.65 & 2010.125 \\
S5-183 & 11.59 & 13.49 & Known Young & 100 & 19 & 1.13 & 0.39 & No & No & 0.01 & 4.59 & -3.44 & 2010.024 \\
S1-23 & 11.67 & 14.01 & Known Old & 100 & 19 & 2.66 & 2.04 & Yes & No & 0.02 & -0.90 & -1.50 & 2010.144 \\
IRS 34W & 11.67 & 14.85 & Known Young & 70 & 8 & 18.46 & 38.68 & Yes & Yes & 0.00 & -4.07 & 1.55 & 2010.189 \\
S2-11 & 11.78 & 13.88 & Known Old & 100 & 19 & 1.83 & 1.14 & No & No & 0.03 & 1.97 & -0.61 & 2009.813 \\
S6-343 & 11.81 & 14.10 & Unknown Age & 63 & 15 & 2.27 & 4.23 & Yes & Yes & 0.01 & -1.80 & -6.41 & 2017.086 \\
S2-6 & 11.90 & 14.11 & Known Young & 100 & 19 & 6.59 & 7.16 & Yes & Yes & 0.03 & 1.66 & -1.33 & 2010.067 \\
S3-5 & 11.93 & 14.25 & Known Young & 100 & 19 & 1.81 & 1.02 & No & No & 0.02 & 2.96 & -1.15 & 2009.910 \\
S2-4 & 12.04 & 14.39 & Known Young & 99 & 19 & 7.85 & 5.77 & Yes & Yes & 0.00 & 1.52 & -1.46 & 2010.007 \\
S4-129 & 12.06 & 14.42 & Known Old & 100 & 18 & 17.20 & 1.35 & Yes & No & 0.00 & 3.69 & -2.22 & 2009.999 \\
S3-291 & 12.12 & \text{---} & Known Old & 31 & 0 & 2.10 & \text{---} & No & \text{---} & 0.02 & -3.53 & -1.25 & 2010.064 \\
S3-10 & 12.13 & 14.09 & Known Young & 100 & 19 & 0.74 & 0.41 & No & No & 0.01 & 3.34 & -1.11 & 2009.944 \\
S4-4 & 12.13 & 14.90 & Known Old & 100 & 19 & 15.81 & 7.07 & Yes & Yes & 0.01 & 3.61 & -2.44 & 2009.973 \\
S3-2 & 12.16 & 14.36 & Known Young & 100 & 19 & 3.90 & 7.86 & Yes & Yes & 0.01 & 3.09 & 0.55 & 2010.014 \\
IRS 9W & 12.19 & 14.59 & Known Young & 99 & 19 & 3.74 & 4.63 & Yes & Yes & 0.03 & 2.90 & -5.59 & 2010.247 \\
S1-3 & 12.20 & 14.31 & Known Young & 98 & 19 & 1.13 & 0.82 & No & No & 0.03 & 0.32 & 0.88 & 2010.207 \\
S2-8 & 12.23 & 14.09 & Known Old & 96 & 17 & 1.01 & 0.35 & No & No & 0.01 & -1.96 & 0.89 & 2010.183 \\
S1-17 & 12.24 & 14.67 & Known Old & 85 & 13 & 1.19 & 2.00 & No & No & 0.01 & 0.48 & -1.53 & 2010.070 \\
S6-89 & 12.30 & 14.61 & Known Young & 44 & 9 & 5.49 & 3.22 & Yes & No & 0.02 & 5.45 & 3.00 & 2009.877 \\
S2-32 & 12.32 & 14.49 & Known Old & 100 & 18 & 1.03 & 0.57 & No & No & 0.01 & 1.13 & 2.78 & 2009.937 \\
S7-5 & 12.33 & 14.63 & Known Young & 99 & 18 & 4.13 & 4.43 & Yes & Yes & 0.00 & 4.86 & -5.52 & 2010.523 \\
S6-27 & 12.33 & 14.60 & Known Old & 100 & 19 & 0.32 & 0.74 & No & No & 0.02 & 4.08 & -4.68 & 2010.175 \\
S2-16 & 12.34 & 15.76 & Known Young & 100 & 19 & 13.35 & 4.92 & Yes & Yes & 0.00 & -1.07 & 2.06 & 2010.201 \\
S4-71 & 12.38 & 14.57 & Known Young & 100 & 19 & 0.80 & 0.49 & No & No & 0.01 & 0.77 & -4.09 & 2010.194 \\
S3-26 & 12.38 & 14.48 & Known Young & 100 & 19 & 2.31 & 2.77 & Yes & No & 0.00 & -2.57 & -2.07 & 2010.133 \\
S2-85 & 12.40 & 15.42 & Known Old & 84 & 18 & 30.39 & 121.75 & Yes & Yes & 0.01 & -1.29 & 2.67 & 2010.210 \\
S6-35 & 12.43 & 14.95 & Known Old & 85 & 16 & 3.23 & 2.99 & Yes & No & 0.02 & -4.91 & -3.96 & 2009.226 \\
S1-20 & 12.43 & 14.73 & Known Old & 100 & 19 & 32.68 & 10.65 & Yes & Yes & 0.00 & 0.45 & 1.60 & 2010.147 \\
S3-30 & 12.46 & 14.74 & Known Young & 69 & 19 & 2.64 & 3.75 & Yes & Yes & 0.01 & 1.66 & -2.94 & 2010.064 \\
S8-11 & 12.50 & 15.00 & Unknown Age & 77 & 17 & 14.35 & 39.61 & Yes & Yes & 0.01 & 5.38 & -5.97 & 2011.241 \\
S3-374 & 12.55 & 15.23 & Known Young & 100 & 19 & 19.80 & 75.68 & Yes & Yes & 0.00 & -2.76 & -2.85 & 2010.080 \\
S1-4 & 12.57 & 14.77 & Known Young & 100 & 19 & 2.99 & 1.91 & Yes & No & 0.01 & 0.88 & -0.66 & 2010.057 \\
S1-5 & 12.58 & 14.98 & Known Old & 80 & 18 & 2.37 & 8.23 & Yes & Yes & 0.00 & 0.32 & -0.89 & 2010.094 \\
S1-22 & 12.62 & 14.73 & Known Young & 51 & 19 & 0.85 & 4.41 & No & Yes & 0.01 & -1.57 & -0.52 & 2010.135 \\
S5-233 & 12.64 & 14.73 & Known Young & 33 & 10 & 2.20 & 4.55 & No & No & 0.00 & 5.59 & 0.67 & 2010.312 \\
S4-344 & 12.65 & 15.13 & Known Old & 100 & 19 & 0.80 & 2.64 & No & No & 0.03 & -1.43 & -4.72 & 2010.131 \\
S4-2 & 12.67 & 15.03 & Known Old & 100 & 19 & 1.37 & 2.30 & No & No & 0.04 & 3.76 & 1.65 & 2009.789 \\
S2-19 & 12.71 & 14.83 & Known Young & 100 & 19 & 1.85 & 3.76 & No & Yes & 0.00 & 0.38 & 2.31 & 2010.075 \\
S4-6 & 12.73 & 15.25 & Known Old & 100 & 19 & 4.67 & 17.15 & Yes & Yes & 0.01 & 3.28 & -2.75 & 2010.123 \\
S5-234 & 12.79 & \text{---} & Known Old & 34 & 0 & 2.59 & \text{---} & No & \text{---} & 0.01 & 5.71 & 0.56 & 2010.134 \\
S1-14 & 12.80 & 14.78 & Known Young & 84 & 18 & 0.96 & 3.43 & No & No & 0.02 & -1.32 & -0.37 & 2009.666 \\
S3-6 & 12.81 & 15.22 & Known Old & 42 & 19 & 0.65 & 3.42 & No & No & 0.04 & 3.23 & -0.05 & 2010.040 \\
S4-36 & 12.82 & 15.29 & Known Young & 83 & 11 & 5.93 & 5.13 & Yes & Yes & 0.00 & -3.69 & 1.78 & 2009.810 \\
S5-213 & 12.86 & 15.07 & Known Old & 99 & 19 & 0.86 & 1.38 & No & No & 0.01 & 4.98 & -3.26 & 2010.066 \\
S5-191 & 12.87 & 14.91 & Known Young & 100 & 19 & 0.58 & 1.15 & No & No & 0.03 & 3.18 & -4.89 & 2010.357 \\
S2-22 & 12.96 & 15.01 & Known Young & 100 & 19 & 0.85 & 1.43 & No & No & 0.03 & 2.30 & -0.21 & 2010.168 \\
S4-3 & 12.99 & 15.15 & Known Old & 100 & 18 & 0.16 & 0.38 & No & No & 0.01 & 4.22 & 0.12 & 2009.959 \\
S2-31 & 12.99 & 15.44 & Known Old & 100 & 18 & 3.93 & 5.61 & Yes & Yes & 0.03 & 2.76 & -0.19 & 2010.061 \\
S3-34 & 13.00 & 15.09 & Known Old & 100 & 19 & 179.80 & 30.85 & Yes & Yes & 0.00 & 3.24 & -1.26 & 2010.374 \\
S1-34 & 13.00 & 14.74 & Known Old & 94 & 19 & 0.35 & 0.15 & No & No & 0.02 & 0.87 & -0.99 & 2010.145 \\
S3-178 & 13.06 & 15.36 & Known Old & 31 & 19 & 0.53 & 1.79 & No & No & 0.04 & -0.51 & -3.39 & 2009.953 \\
S1-1 & 13.10 & 15.11 & Known Young & 100 & 19 & 0.67 & 0.33 & No & No & 0.03 & 1.04 & 0.03 & 2009.895 \\
S4-258 & 13.11 & 16.37 & Known Young & 91 & 18 & 142.99 & 398.75 & Yes & Yes & 0.00 & -4.40 & -1.63 & 2009.761 \\
S2-18 & 13.18 & 15.70 & Known Old & 100 & 19 & 17.33 & 92.74 & Yes & Yes & 0.01 & -1.00 & -2.15 & 2010.123 \\
S4-180 & 13.19 & 15.87 & Known Young & 41 & 18 & 2.59 & 1.57 & Yes & No & 0.01 & -4.29 & -1.33 & 2011.094 \\
IRS 7SE & 13.24 & 15.91 & Known Young & 99 & 18 & 34.40 & 3.84 & Yes & Yes & 0.00 & 2.99 & 3.46 & 2009.595 \\
S2-5 & 13.27 & 15.39 & Known Young & 99 & 19 & 1.36 & 0.90 & No & No & 0.00 & 1.94 & -0.79 & 2010.021 \\
S3-149 & 13.27 & 15.74 & Known Old & 100 & 19 & 7.03 & 4.10 & Yes & Yes & 0.01 & -2.90 & 1.71 & 2010.286 \\
S6-58 & 13.28 & 15.68 & Unknown Age & 99 & 19 & 1.38 & 4.32 & No & Yes & 0.02 & 3.22 & -5.65 & 2010.151 \\
S5-237 & 13.28 & 15.33 & Known Young & 63 & 14 & 8.20 & 2.40 & Yes & No & 0.00 & 5.49 & 1.02 & 2012.046 \\
S5-187 & 13.29 & 15.27 & Known Young & 99 & 19 & 1.79 & 1.64 & No & No & 0.03 & -1.71 & -5.55 & 2009.655 \\
S4-1 & 13.29 & 15.59 & Known Old & 100 & 19 & 0.61 & 0.78 & No & No & 0.02 & 4.00 & -0.36 & 2009.980 \\
S1-68 & 13.30 & 15.55 & Known Old & 99 & 19 & 1.04 & 1.73 & No & No & 0.00 & 1.83 & -0.65 & 2010.023 \\
S2-74 & 13.30 & 15.59 & Known Young & 100 & 18 & 4.26 & 3.25 & Yes & No & 0.01 & 0.11 & 2.78 & 2010.109 \\
S5-211 & 13.30 & 15.00 & Known Old & 100 & 19 & 0.29 & 0.39 & No & No & 0.02 & 4.46 & -3.90 & 2010.061 \\
S1-21 & 13.31 & 15.32 & Known Young & 100 & 19 & 0.96 & 0.60 & No & No & 0.02 & -1.64 & 0.09 & 2010.177 \\
S2-21 & 13.33 & 15.42 & Known Young & 100 & 19 & 1.40 & 0.89 & No & No & 0.00 & -1.62 & -1.67 & 2010.222 \\
S5-95 & 13.33 & 15.63 & Known Old & 86 & 16 & 1.99 & 1.05 & Yes & No & 0.01 & -1.94 & -4.99 & 2010.143 \\
S0-13 & 13.33 & 15.48 & Known Old & 49 & 13 & 0.57 & 1.46 & No & No & 0.01 & 0.56 & -0.41 & 2010.122 \\
S1-25 & 13.39 & 15.69 & Known Old & 97 & 19 & 0.64 & 0.46 & No & No & 0.01 & 1.68 & -0.61 & 2010.098 \\
S5-134 & 13.39 & 15.80 & Known Old & 94 & 18 & 3.64 & 2.21 & Yes & No & 0.00 & -0.53 & -5.46 & 2009.951 \\
S2-67 & 13.40 & 15.79 & Known Old & 98 & 19 & 3.37 & 2.23 & Yes & No & 0.01 & -2.47 & -0.88 & 2010.171 \\
S2-36 & 13.43 & 15.61 & Known Young & 98 & 19 & 8.85 & 9.81 & Yes & Yes & 0.00 & 1.99 & 0.44 & 2009.947 \\
S4-143 & 13.47 & 16.03 & Known Old & 94 & 18 & 0.39 & 0.41 & No & No & 0.01 & 2.90 & -3.25 & 2010.331 \\
S1-12 & 13.53 & 15.58 & Known Young & 100 & 19 & 0.50 & 0.75 & No & No & 0.01 & -0.75 & -1.03 & 2010.234 \\
S2-78 & 13.55 & 16.01 & Known Old & 89 & 13 & 1.74 & 2.93 & No & No & 0.00 & -2.82 & -0.28 & 2010.204 \\
S3-13 & 13.57 & 15.86 & Known Old & 100 & 19 & 0.64 & 0.79 & No & No & 0.01 & 3.84 & 0.98 & 2009.952 \\
S2-77 & 13.58 & 15.85 & Known Old & 36 & 19 & 1.57 & 11.95 & No & Yes & 0.02 & -1.76 & -2.21 & 2008.709 \\
S1-19 & 13.58 & 15.68 & Known Young & 83 & 13 & 0.93 & 0.64 & No & No & 0.00 & 0.43 & -1.64 & 2010.024 \\
S3-39 & 13.59 & 15.91 & Known Old & 99 & 18 & 1.23 & 1.37 & No & No & 0.02 & 3.56 & 1.08 & 2009.733 \\
S3-7 & 13.61 & 16.02 & Known Old & 100 & 19 & 1.91 & 6.93 & Yes & Yes & 0.02 & 1.92 & -2.61 & 2010.088 \\
S3-29 & 13.61 & 15.67 & Known Old & 97 & 19 & 2.58 & 1.14 & Yes & No & 0.00 & 1.44 & -3.08 & 2010.219 \\
S3-370 & 13.63 & 15.84 & Known Old & 95 & 19 & 0.47 & 0.19 & No & No & 0.03 & -0.29 & -3.91 & 2010.136 \\
S4-169 & 13.64 & 15.57 & Known Young & 100 & 12 & 0.43 & 0.36 & No & No & 0.00 & 4.41 & 0.28 & 2009.872 \\
S2-24 & 13.67 & 16.08 & Known Old & 94 & 17 & 0.71 & 1.06 & No & No & 0.00 & -2.34 & -0.89 & 2009.893 \\
S6-76 & 13.68 & 16.02 & Known Old & 100 & 19 & 0.91 & 1.27 & No & No & 0.00 & 5.18 & -4.52 & 2010.291 \\
S0-14 & 13.69 & 15.73 & Known Young & 96 & 18 & 0.98 & 2.41 & No & No & 0.00 & -0.76 & -0.29 & 2010.316 \\
S0-15 & 13.70 & 15.86 & Known Young & 56 & 17 & 9.32 & 49.61 & Yes & Yes & 0.00 & -0.97 & 0.18 & 2009.722 \\
IRS 34NW & 13.71 & 16.90 & Known Young & 90 & 18 & 29.56 & 40.95 & Yes & Yes & 0.00 & -3.78 & 2.83 & 2010.283 \\
S3-198 & 13.71 & 16.36 & Unknown Age & 99 & 18 & 3.87 & 10.81 & Yes & Yes & 0.01 & 0.65 & 3.45 & 2009.959 \\
S4-287 & 13.73 & 15.87 & Known Young & 100 & 19 & 0.42 & 0.25 & No & No & 0.01 & 0.13 & -4.77 & 2010.188 \\
S7-27 & 13.73 & 16.05 & Unknown Age & 77 & 17 & 2.06 & 3.41 & Yes & No & 0.01 & 3.26 & -6.36 & 2011.875 \\
S5-34 & 13.73 & 16.18 & Known Young & 89 & 18 & 1.46 & 2.76 & No & No & 0.01 & -4.33 & -2.74 & 2010.071 \\
S2-26 & 13.74 & 16.11 & Known Old & 100 & 19 & 59.39 & 6.19 & Yes & Yes & 0.00 & 0.79 & 2.31 & 2010.167 \\
S4-161 & 13.74 & 16.18 & Known Old & 100 & 19 & 0.50 & 1.17 & No & No & 0.01 & 4.42 & -0.26 & 2009.943 \\
S3-331 & 13.75 & 15.85 & Known Young & 95 & 18 & 2.16 & 1.82 & Yes & No & 0.00 & -1.22 & 3.65 & 2010.150 \\
S6-25 & 13.77 & 16.10 & Unknown Age & 92 & 18 & 1.23 & 4.21 & No & Yes & 0.02 & 0.71 & -6.17 & 2010.070 \\
S2-25 & 13.78 & 16.17 & Known Old & 100 & 19 & 1.14 & 1.23 & No & No & 0.01 & 0.76 & -2.42 & 2010.330 \\
S5-185 & 13.79 & 16.08 & Unknown Age & 100 & 18 & 1.55 & 1.46 & No & No & 0.01 & 3.00 & -4.92 & 2010.475 \\
S4-112 & 13.79 & 16.15 & Known Old & 96 & 19 & 4.35 & 5.04 & Yes & Yes & 0.01 & 2.24 & -3.61 & 2010.251 \\
S3-134 & 13.79 & 16.10 & Known Old & 100 & 19 & 0.36 & 0.28 & No & No & 0.00 & -1.39 & -3.01 & 2010.208 \\
S5-115 & 13.80 & 16.54 & Unknown Age & 68 & 8 & 4.45 & 3.25 & Yes & No & 0.02 & -5.17 & -1.55 & 2010.148 \\
S3-17 & 13.81 & 16.43 & Known Young & 34 & 18 & 8.09 & 63.40 & Yes & Yes & 0.00 & -1.41 & 2.85 & 2009.185 \\
S3-14 & 13.84 & 16.41 & Known Old & 79 & 18 & 11.05 & 28.40 & Yes & Yes & 0.00 & 0.18 & 3.07 & 2009.981 \\
S4-59 & 13.84 & 15.93 & Known Old & 72 & 7 & 0.82 & 0.32 & No & No & 0.02 & -3.15 & 2.65 & 2010.023 \\
S3-35 & 13.87 & 16.60 & Unknown Age & 99 & 18 & 3.71 & 2.72 & Yes & No & 0.00 & -1.21 & 3.28 & 2010.167 \\
S5-71 & 13.88 & 16.12 & Known Old & 100 & 19 & 0.44 & 0.25 & No & No & 0.02 & -1.75 & -4.94 & 2009.691 \\
S6-31 & 13.88 & 16.21 & Known Old & 93 & 18 & 1.23 & 0.46 & No & No & 0.03 & -2.12 & -5.85 & 2010.015 \\
S2-7 & 13.91 & 16.17 & Known Young & 100 & 18 & 46.48 & 12.53 & Yes & Yes & 0.00 & 0.93 & 1.85 & 2010.257 \\
S4-342 & 13.92 & 16.39 & Unknown Age & 74 & 14 & 16.73 & 6.33 & Yes & Yes & 0.01 & 3.07 & 3.86 & 2010.650 \\
S3-28 & 13.93 & 16.40 & Unknown Age & 99 & 18 & 2.68 & 1.06 & Yes & No & 0.00 & -0.83 & 3.23 & 2010.134 \\
S3-27 & 13.96 & 16.33 & Unknown Age & 99 & 18 & 9.21 & 0.76 & Yes & No & 0.00 & -0.33 & 3.32 & 2010.092 \\
S3-284 & 13.97 & 17.13 & Known Old & 100 & 18 & 9.82 & 8.53 & Yes & Yes & 0.00 & -2.57 & 2.71 & 2010.347 \\
S4-84 & 13.99 & 16.80 & Known Old & 35 & 9 & 4.39 & 7.07 & Yes & Yes & 0.00 & -3.36 & 2.52 & 2009.984 \\
S5-145 & 13.99 & 15.96 & Unknown Age & 90 & 18 & 1.61 & 0.93 & No & No & 0.00 & -0.57 & -5.54 & 2010.081 \\
S4-24 & 14.02 & 16.75 & Unknown Age & 68 & 5 & 5.63 & 6.02 & Yes & No & 0.01 & -0.72 & 4.00 & 2010.423 \\
S3-25 & 14.04 & 16.13 & Known Young & 100 & 18 & 1.76 & 3.76 & No & Yes & 0.00 & 1.41 & 2.95 & 2009.923 \\
S0-6 & 14.04 & 16.32 & Known Old & 100 & 19 & 1.27 & 6.06 & No & Yes & 0.03 & 0.02 & -0.36 & 2010.779 \\
S2-58 & 14.05 & 16.27 & Known Young & 94 & 18 & 3.12 & 6.02 & Yes & Yes & 0.01 & 2.14 & -1.13 & 2010.157 \\
S6-66 & 14.06 & 16.59 & Known Old & 39 & 15 & 2.52 & 2.24 & No & No & 0.00 & -4.71 & -4.66 & 2009.332 \\
S3-207 & 14.06 & 16.33 & Unknown Age & 99 & 18 & 0.61 & 0.53 & No & No & 0.00 & 1.55 & 3.21 & 2009.989 \\
S2-2 & 14.06 & 15.78 & Known Old & 100 & 19 & 0.20 & 0.24 & No & No & 0.01 & -0.52 & 2.09 & 2010.141 \\
S4-158 & 14.08 & 16.20 & Known Old & 100 & 19 & 0.40 & 0.92 & No & No & 0.02 & -0.86 & -4.33 & 2010.174 \\
S1-13 & 14.08 & 16.41 & Known Old & 76 & 19 & 0.82 & 3.02 & No & No & 0.01 & -1.14 & -0.97 & 2010.185 \\
S4-197 & 14.09 & 16.62 & Known Old & 100 & 19 & 2.12 & 3.62 & Yes & Yes & 0.01 & -2.55 & -3.71 & 2010.272 \\
S5-205 & 14.09 & 16.39 & Known Old & 93 & 19 & 3.42 & 10.93 & Yes & Yes & 0.00 & -0.91 & -5.81 & 2010.004 \\
S7-29 & 14.12 & 16.58 & Known Old & 72 & 16 & 1.98 & 2.34 & No & No & 0.00 & -3.66 & -6.38 & 2010.986 \\
S0-2 & 14.12 & 16.13 & Known Young & 89 & 18 & 1.92 & 3.86 & No & Yes & 0.02 & -0.01 & 0.17 & 2007.893 \\
S6-39 & 14.13 & 16.47 & Unknown Age & 93 & 18 & 5.95 & 2.93 & Yes & No & 0.00 & 2.51 & -5.79 & 2009.801 \\
S5-202 & 14.14 & 16.12 & Unknown Age & 93 & 19 & 0.74 & 2.76 & No & No & 0.00 & -0.51 & -5.85 & 2010.094 \\
S5-199 & 14.16 & 16.68 & Known Old & 83 & 18 & 1.34 & 4.54 & No & Yes & 0.01 & -4.20 & -4.08 & 2009.569 \\
S3-146 & 14.17 & 16.38 & Unknown Age & 89 & 17 & 5.50 & 6.03 & Yes & Yes & 0.00 & -0.29 & -3.35 & 2010.110 \\
S4-319 & 14.17 & 16.42 & Known Old & 86 & 19 & 1.29 & 0.88 & No & No & 0.00 & 4.68 & -1.38 & 2010.042 \\
S0-32 & 14.19 & 15.05 & Unknown Age & 90 & 18 & 0.81 & 0.26 & No & No & 0.02 & 0.32 & 0.79 & 2010.090 \\
S4-229 & 14.20 & 17.03 & Unknown Age & 66 & 10 & 4.28 & 13.93 & Yes & Yes & 0.00 & -4.19 & 1.94 & 2010.123 \\
S2-57 & 14.22 & 16.47 & Known Old & 71 & 14 & 1.71 & 0.89 & No & No & 0.00 & -1.15 & -2.09 & 2010.273 \\
S4-170 & 14.22 & 16.40 & Known Old & 99 & 19 & 1.57 & 0.49 & No & No & 0.01 & -0.57 & -4.41 & 2010.181 \\
S1-8 & 14.22 & 16.48 & Known Young & 99 & 19 & 2.86 & 2.68 & Yes & No & 0.00 & -0.58 & -0.92 & 2010.185 \\
S0-4 & 14.23 & 16.25 & Known Young & 39 & 13 & 2.14 & 1.31 & No & No & 0.00 & 0.45 & -0.33 & 2010.008 \\
S2-3 & 14.23 & 16.63 & Known Old & 58 & 18 & 0.74 & 1.26 & No & No & 0.00 & -1.51 & -1.41 & 2010.300 \\
S3-88 & 14.24 & 16.42 & Known Old & 100 & 19 & 0.36 & 0.11 & No & No & 0.00 & -0.85 & -3.00 & 2010.102 \\
S2-344 & 14.25 & 16.57 & Unknown Age & 36 & 9 & 1.74 & 1.05 & No & No & 0.01 & -1.73 & -2.20 & 2012.518 \\
S5-43 & 14.26 & 16.79 & Known Old & 100 & 19 & 3.54 & 5.42 & Yes & Yes & 0.00 & 1.84 & -4.80 & 2010.260 \\
S5-240 & 14.26 & 16.45 & Unknown Age & 76 & 16 & 1.78 & 1.27 & No & No & 0.01 & 5.36 & 0.08 & 2011.220 \\
S2-47 & 14.26 & 16.61 & Known Old & 100 & 19 & 1.39 & 1.27 & No & No & 0.01 & 2.19 & -0.52 & 2010.214 \\
S4-221 & 14.27 & 16.70 & Known Old & 100 & 19 & 2.83 & 9.74 & Yes & Yes & 0.00 & 2.69 & -3.77 & 2010.222 \\
S0-9 & 14.28 & 16.27 & Known Young & 82 & 18 & 3.21 & 6.85 & Yes & Yes & 0.00 & 0.22 & -0.60 & 2009.769 \\
S7-3 & 14.30 & 16.63 & Unknown Age & 87 & 18 & 0.84 & 1.87 & No & No & 0.02 & 4.17 & -5.80 & 2010.379 \\
S6-49 & 14.31 & 16.67 & Known Old & 88 & 19 & 1.30 & 3.37 & No & No & 0.00 & -2.85 & -5.77 & 2010.422 \\
S4-196 & 14.32 & 16.56 & Known Young & 100 & 19 & 5.62 & 7.76 & Yes & Yes & 0.00 & 2.24 & -3.93 & 2010.135 \\
S3-288 & 14.32 & 17.58 & Known Old & 100 & 18 & 11.95 & 6.10 & Yes & Yes & 0.00 & -2.77 & 2.54 & 2010.339 \\
S3-190 & 14.33 & 17.12 & Known Young & 100 & 19 & 11.22 & 22.72 & Yes & Yes & 0.00 & -3.19 & 1.41 & 2010.223 \\
S5-170 & 14.33 & 16.54 & Unknown Age & 34 & 16 & 16.45 & 2.76 & Yes & No & 0.00 & 4.23 & 3.84 & 2009.509 \\
S5-174 & 14.37 & 16.84 & Known Old & 90 & 18 & 1.61 & 2.80 & No & No & 0.00 & -4.16 & -3.94 & 2010.073 \\
S6-77 & 14.38 & 16.60 & Known Old & 78 & 15 & 1.53 & 1.75 & No & No & 0.00 & 5.06 & -4.75 & 2010.476 \\
S0-12 & 14.39 & 16.66 & Known Old & 100 & 19 & 1.29 & 2.14 & No & No & 0.00 & -0.55 & 0.41 & 2009.012 \\
S4-168 & 14.40 & 16.90 & Unknown Age & 76 & 9 & 4.20 & 1.57 & Yes & No & 0.00 & -1.91 & 3.97 & 2010.678 \\
S4-139 & 14.41 & 16.65 & Known Old & 99 & 18 & 5.03 & 1.77 & Yes & No & 0.00 & 2.40 & -3.62 & 2010.074 \\
S1-49 & 14.41 & 16.46 & Unknown Age & 98 & 19 & 5.57 & 5.68 & Yes & Yes & 0.01 & -1.72 & 0.15 & 2010.287 \\
S2-75 & 14.43 & 16.73 & Known Old & 100 & 19 & 0.43 & 0.91 & No & No & 0.00 & 2.63 & -0.85 & 2010.082 \\
S2-70 & 14.45 & 17.25 & Known Old & 100 & 19 & 14.15 & 103.90 & Yes & Yes & 0.00 & -2.68 & 0.39 & 2010.154 \\
S3-20 & 14.45 & 16.97 & Known Old & 98 & 19 & 3.04 & 8.68 & Yes & Yes & 0.00 & 1.58 & -2.79 & 2009.965 \\
S3-208 & 14.47 & 16.36 & Known Young & 100 & 19 & 1.41 & 1.54 & No & No & 0.00 & -0.98 & -3.41 & 2010.198 \\
S2-23 & 14.47 & 17.07 & Known Old & 100 & 19 & 2.50 & 8.38 & Yes & Yes & 0.00 & 1.65 & 1.74 & 2010.053 \\
S4-352 & 14.48 & 17.34 & Unknown Age & 90 & 16 & 4.87 & 8.33 & Yes & Yes & 0.00 & -4.88 & -0.88 & 2009.519 \\
S6-70 & 14.49 & 16.88 & Known Old & 84 & 19 & 1.44 & 3.29 & No & No & 0.01 & -2.80 & -6.15 & 2011.881 \\
S5-168 & 14.51 & 16.96 & Unknown Age & 52 & 8 & 1.61 & 1.56 & No & No & 0.00 & 4.37 & 3.62 & 2010.149 \\
S6-64 & 14.53 & 16.34 & Known Young & 74 & 18 & 1.28 & 0.69 & No & No & 0.00 & -3.05 & -5.86 & 2010.405 \\
S3-187 & 14.55 & 17.09 & Known Old & 100 & 19 & 7.19 & 7.15 & Yes & Yes & 0.00 & -3.40 & -0.75 & 2010.032 \\
S3-96 & 14.56 & 17.14 & Known Young & 68 & 12 & 1.15 & 1.45 & No & No & 0.01 & -3.13 & -0.63 & 2010.217 \\
S3-364 & 14.59 & 16.72 & Unknown Age & 86 & 14 & 3.04 & 7.10 & Yes & Yes & 0.00 & -0.96 & 3.80 & 2010.143 \\
S4-236 & 14.59 & 16.84 & Known Old & 65 & 19 & 0.43 & 0.76 & No & No & 0.01 & -1.91 & -4.22 & 2009.747 \\
S3-36 & 14.62 & 16.70 & Known Old & 100 & 19 & 0.20 & 0.73 & No & No & 0.01 & 3.47 & -0.81 & 2010.145 \\
S5-198 & 14.62 & 16.85 & Unknown Age & 93 & 19 & 0.91 & 2.28 & No & No & 0.00 & 0.51 & -5.82 & 2010.297 \\
S3-4 & 14.63 & 17.76 & Unknown Age & 98 & 19 & 9.62 & 5.09 & Yes & Yes & 0.00 & 3.07 & -0.48 & 2010.182 \\
S0-3 & 14.65 & 16.74 & Known Young & 98 & 19 & 1.46 & 5.31 & No & Yes & 0.00 & 0.34 & 0.12 & 2008.393 \\
S5-83 & 14.69 & 16.86 & Known Old & 100 & 19 & 0.60 & 0.89 & No & No & 0.01 & 5.20 & -0.94 & 2010.125 \\
S6-62 & 14.71 & 17.12 & Known Old & 36 & 15 & 3.51 & 3.65 & Yes & No & 0.00 & -4.70 & -4.60 & 2009.407 \\
S2-277 & 14.73 & 16.86 & Unknown Age & 100 & 18 & 1.25 & 2.06 & No & No & 0.00 & -2.44 & -1.44 & 2010.286 \\
S4-46 & 14.76 & 16.61 & Known Old & 99 & 19 & 0.82 & 0.32 & No & No & 0.01 & 3.84 & -1.48 & 2010.066 \\
S1-10 & 14.77 & 16.57 & Known Old & 89 & 15 & 0.43 & 1.06 & No & No & 0.00 & -1.10 & -0.02 & 2010.139 \\
S1-2 & 14.78 & 16.82 & Known Young & 100 & 19 & 2.06 & 1.22 & Yes & No & 0.00 & 0.08 & -1.02 & 2009.985 \\
S0-1 & 14.78 & 16.92 & Known Young & 67 & 18 & 9.03 & 7.40 & Yes & Yes & 0.00 & 0.04 & -0.26 & 2006.300 \\
S3-249 & 14.80 & 18.51 & Known Old & 100 & 13 & 60.47 & 278.63 & Yes & Yes & 0.00 & -3.38 & 1.28 & 2010.016 \\
S4-98 & 14.80 & 17.13 & Unknown Age & 94 & 12 & 5.64 & 2.98 & Yes & No & 0.00 & -4.12 & -0.90 & 2009.807 \\
S5-12 & 14.82 & 17.45 & Known Old & 88 & 18 & 0.55 & 1.07 & No & No & 0.00 & -4.28 & -2.63 & 2010.189 \\
S2-69 & 14.82 & 17.84 & Unknown Age & 99 & 18 & 13.76 & 90.06 & Yes & Yes & 0.00 & -0.88 & 2.56 & 2010.273 \\
S5-112 & 14.83 & \text{---} & Unknown Age & 40 & 0 & 7.99 & \text{---} & Yes & \text{---} & 0.00 & -5.27 & 1.23 & 2009.265 \\
S4-12 & 14.83 & 17.45 & Known Young & 70 & 18 & 18.53 & 20.45 & Yes & Yes & 0.00 & -2.86 & 2.84 & 2010.034 \\
S5-133 & 14.83 & 16.85 & Unknown Age & 88 & 16 & 9.58 & 3.50 & Yes & No & 0.00 & -0.75 & -5.45 & 2009.873 \\
S3-403 & 14.84 & 17.10 & Unknown Age & 57 & 16 & 4.07 & 5.30 & Yes & Yes & 0.00 & -0.12 & -3.38 & 2009.561 \\
S2-72 & 14.84 & 17.22 & Known Old & 56 & 12 & 2.95 & 4.99 & Yes & Yes & 0.00 & -1.50 & -2.24 & 2010.007 \\
S6-123 & 14.84 & 17.13 & Unknown Age & 47 & 15 & 1.11 & 3.35 & No & No & 0.00 & -0.11 & -6.45 & 2010.778 \\
S7-43 & 14.86 & 17.42 & Unknown Age & 72 & 15 & 2.44 & 3.44 & Yes & No & 0.01 & 4.09 & -6.40 & 2011.383 \\
S1-18 & 14.87 & 17.13 & Known Young & 69 & 19 & 2.98 & 4.90 & Yes & Yes & 0.00 & -0.79 & 1.50 & 2009.682 \\
S5-243 & 14.90 & 17.21 & Known Old & 48 & 10 & 3.80 & 5.61 & Yes & Yes & 0.00 & 5.52 & 1.45 & 2007.596 \\
S2-73 & 14.91 & 17.13 & Known Old & 100 & 19 & 2.04 & 5.56 & Yes & Yes & 0.00 & 2.13 & -1.66 & 2009.926 \\
S5-99 & 14.91 & 17.15 & Known Old & 100 & 19 & 0.53 & 0.77 & No & No & 0.02 & 4.61 & -2.74 & 2010.082 \\
S3-223 & 14.92 & 17.37 & Unknown Age & 63 & 12 & 4.18 & 14.31 & Yes & Yes & 0.00 & 1.28 & -3.37 & 2009.821 \\
S6-37 & 14.96 & 17.58 & Known Old & 93 & 19 & 3.89 & 0.92 & Yes & No & 0.00 & -2.31 & -5.87 & 2010.256 \\
S3-11 & 14.99 & 17.46 & Known Old & 91 & 18 & 2.30 & 5.57 & Yes & Yes & 0.00 & 2.96 & -1.90 & 2011.181 \\
S1-51 & 15.01 & 17.29 & Unknown Age & 100 & 19 & 1.35 & 0.44 & No & No & 0.00 & -1.66 & -0.17 & 2010.270 \\
S5-31 & 15.02 & 16.95 & Unknown Age & 43 & 10 & 1.30 & 1.27 & No & No & 0.00 & -4.34 & 2.65 & 2011.201 \\
S0-5 & 15.03 & 17.13 & Known Young & 72 & 12 & 4.49 & 1.31 & Yes & No & 0.00 & 0.17 & -0.36 & 2009.636 \\
S0-53 & 15.03 & \text{---} & Unknown Age & 81 & 0 & 37.75 & \text{---} & Yes & \text{---} & 0.00 & 0.35 & 0.20 & 2005.892 \\
S1-33 & 15.04 & 17.13 & Known Young & 100 & 19 & 1.01 & 0.65 & No & No & 0.00 & -1.25 & -0.00 & 2009.977 \\
S3-16 & 15.04 & 17.27 & Known Old & 93 & 17 & 9.38 & 3.57 & Yes & No & 0.00 & 2.97 & -0.95 & 2009.811 \\
S6-128 & 15.06 & 17.59 & Known Old & 38 & 8 & 2.86 & 2.16 & Yes & No & 0.00 & 5.70 & -2.54 & 2010.873 \\
S3-438 & 15.06 & 17.16 & Unknown Age & 31 & 8 & 4.23 & 3.45 & Yes & No & 0.00 & -0.52 & -3.41 & 2016.818 \\
S4-172 & 15.08 & 17.39 & Known Old & 92 & 17 & 16.83 & 22.94 & Yes & Yes & 0.00 & 3.09 & -3.17 & 2010.358 \\
S2-62 & 15.08 & 17.43 & Known Old & 99 & 19 & 0.92 & 2.03 & No & No & 0.00 & -1.03 & -2.32 & 2010.009 \\
S3-37 & 15.09 & 16.96 & Known Old & 95 & 17 & 1.14 & 1.45 & No & No & 0.01 & 3.42 & 1.36 & 2010.050 \\
S3-216 & 15.10 & 17.16 & Unknown Age & 72 & 18 & 0.55 & 0.94 & No & No & 0.00 & -3.14 & 1.67 & 2009.725 \\
S0-31 & 15.10 & 17.10 & Known Young & 88 & 11 & 2.41 & 8.33 & Yes & Yes & 0.00 & 0.57 & 0.45 & 2009.906 \\
S5-193 & 15.11 & 16.84 & Unknown Age & 59 & 19 & 0.77 & 1.09 & No & No & 0.01 & -1.16 & -5.73 & 2009.874 \\
S3-3 & 15.13 & 17.20 & Known Young & 100 & 19 & 1.27 & 2.23 & No & No & 0.00 & 3.09 & -0.64 & 2010.081 \\
S0-18 & 15.14 & 17.34 & Known Old & 32 & 19 & 1.29 & 4.82 & No & Yes & 0.00 & -0.12 & -0.42 & 2009.454 \\
S5-159 & 15.15 & 17.31 & Unknown Age & 98 & 19 & 0.54 & 0.60 & No & No & 0.01 & 0.43 & -5.60 & 2010.221 \\
S0-7 & 15.17 & 17.26 & Known Young & 97 & 17 & 3.42 & 3.53 & Yes & No & 0.00 & 0.51 & 0.10 & 2010.379 \\
S4-315 & 15.18 & 17.40 & Known Old & 85 & 16 & 6.00 & 1.77 & Yes & No & 0.00 & 4.81 & 0.85 & 2009.738 \\
S3-155 & 15.18 & 17.03 & Known Young & 99 & 18 & 0.47 & 0.41 & No & No & 0.00 & -1.84 & -2.83 & 2010.185 \\
S2-12 & 15.18 & 17.39 & Known Old & 99 & 18 & 1.79 & 1.57 & No & No & 0.00 & 1.64 & 1.14 & 2010.272 \\
S0-11 & 15.19 & 17.27 & Known Young & 98 & 18 & 1.68 & 1.03 & No & No & 0.00 & 0.49 & -0.06 & 2010.011 \\
S2-55 & 15.19 & 17.48 & Known Old & 98 & 17 & 2.30 & 1.87 & Yes & No & 0.00 & 0.90 & -2.19 & 2009.600 \\
S2-50 & 15.20 & 17.34 & Known Young & 85 & 16 & 5.50 & 7.82 & Yes & Yes & 0.00 & 1.70 & -1.51 & 2009.533 \\
S4-188 & 15.20 & 17.80 & Unknown Age & 91 & 17 & 24.07 & 18.82 & Yes & Yes & 0.00 & -4.14 & -1.77 & 2010.496 \\
S2-49 & 15.20 & 17.41 & Known Old & 100 & 19 & 1.60 & 1.41 & No & No & 0.00 & -0.80 & -2.14 & 2010.126 \\
S2-71 & 15.21 & 17.35 & Known Old & 100 & 19 & 0.79 & 0.96 & No & No & 0.01 & -0.88 & -2.52 & 2010.060 \\
S3-262 & 15.22 & 18.78 & Known Old & 100 & 16 & 27.50 & 158.86 & Yes & Yes & 0.00 & -2.35 & 2.81 & 2010.084 \\
S4-277 & 15.22 & 17.38 & Known Old & 75 & 16 & 1.46 & 1.71 & No & No & 0.01 & 4.75 & 0.21 & 2009.665 \\
S5-98 & 15.22 & 17.32 & Unknown Age & 99 & 18 & 0.59 & 0.53 & No & No & 0.01 & 1.04 & -5.24 & 2010.354 \\
S5-156 & 15.22 & 17.54 & Known Old & 98 & 19 & 1.91 & 2.33 & Yes & No & 0.00 & -1.42 & -5.45 & 2010.209 \\
S6-44 & 15.22 & 17.43 & Known Young & 92 & 19 & 5.26 & 6.17 & Yes & Yes & 0.00 & -2.15 & -6.00 & 2010.113 \\
S3-227 & 15.22 & 17.45 & Unknown Age & 98 & 17 & 1.63 & 0.54 & No & No & 0.00 & 0.03 & -3.60 & 2010.028 \\
S1-53 & 15.22 & 17.42 & Known Old & 98 & 19 & 1.58 & 1.76 & No & No & 0.00 & 1.67 & -0.10 & 2009.524 \\
S3-51 & 15.23 & 17.34 & Unknown Age & 99 & 18 & 0.64 & 0.84 & No & No & 0.01 & -0.15 & 3.02 & 2010.104 \\
S3-385 & 15.24 & 17.36 & Known Old & 90 & 16 & 0.84 & 0.94 & No & No & 0.00 & 3.69 & -1.46 & 2009.997 \\
S3-32 & 15.24 & 17.48 & Known Old & 99 & 19 & 2.23 & 5.08 & Yes & Yes & 0.00 & 2.87 & -1.77 & 2010.163 \\
S6-14 & 15.25 & 17.61 & Known Old & 85 & 19 & 1.30 & 0.33 & No & No & 0.01 & -3.24 & -5.16 & 2009.107 \\
S2-84 & 15.25 & 17.54 & Unknown Age & 99 & 18 & 1.56 & 1.50 & No & No & 0.00 & 1.66 & -2.47 & 2010.187 \\
S3-192 & 15.25 & 17.55 & Unknown Age & 94 & 10 & 1.93 & 3.78 & Yes & No & 0.02 & 0.50 & -3.47 & 2009.890 \\
S1-39 & 15.25 & 17.53 & Known Old & 76 & 19 & 1.50 & 1.82 & No & No & 0.01 & -0.54 & -1.38 & 2009.934 \\
S4-86 & 15.25 & 17.32 & Known Old & 100 & 19 & 0.65 & 0.28 & No & No & 0.00 & -0.66 & -4.12 & 2009.691 \\
S1-32 & 15.27 & 17.55 & Known Old & 71 & 11 & 1.33 & 1.98 & No & No & 0.00 & -0.99 & -0.66 & 2010.144 \\
S1-63 & 15.27 & 17.94 & Unknown Age & 66 & 11 & 7.08 & 54.15 & Yes & Yes & 0.00 & -1.22 & 1.41 & 2008.658 \\
S2-316 & 15.27 & 17.77 & Unknown Age & 54 & 18 & 7.66 & 3.52 & Yes & No & 0.00 & -2.43 & 1.64 & 2009.665 \\
S2-306 & 15.28 & 17.89 & Known Young & 52 & 11 & 6.16 & 9.79 & Yes & Yes & 0.00 & -0.49 & -2.89 & 2010.382 \\
S1-52 & 15.28 & 17.36 & Unknown Age & 38 & 6 & 0.97 & 4.88 & No & No & 0.00 & 0.01 & 1.68 & 2007.924 \\
S2-29 & 15.29 & 17.43 & Known Young & 87 & 17 & 2.30 & 1.68 & Yes & No & 0.00 & 1.95 & -2.16 & 2010.009 \\
S2-82 & 15.29 & 17.53 & Unknown Age & 36 & 17 & 1.92 & 7.18 & No & Yes & 0.00 & 2.86 & 0.06 & 2009.160 \\
S4-375 & 15.29 & 17.58 & Unknown Age & 47 & 13 & 3.02 & 3.29 & Yes & No & 0.00 & 3.94 & 1.62 & 2010.282 \\
S3-268 & 15.29 & 17.56 & Known Young & 87 & 19 & 1.44 & 2.20 & No & No & 0.00 & -2.15 & -3.03 & 2010.422 \\
S3-43 & 15.29 & 17.44 & Unknown Age & 84 & 13 & 3.01 & 1.43 & Yes & No & 0.00 & -0.16 & -3.02 & 2009.661 \\
S3-344 & 15.29 & 17.47 & Unknown Age & 100 & 18 & 1.24 & 0.81 & No & No & 0.00 & 3.07 & 2.41 & 2010.234 \\
S4-45 & 15.29 & 17.57 & Unknown Age & 93 & 18 & 0.97 & 0.57 & No & No & 0.02 & 4.11 & -0.41 & 2009.981 \\
S3-348 & 15.30 & 17.42 & Unknown Age & 95 & 18 & 0.63 & 0.26 & No & No & 0.00 & 3.91 & 0.23 & 2009.944 \\
S3-286 & 15.30 & 17.44 & Known Old & 100 & 19 & 0.78 & 0.59 & No & No & 0.00 & 3.41 & -1.52 & 2010.090 \\
S3-327 & 15.30 & 17.40 & Known Old & 45 & 16 & 9.07 & 5.17 & Yes & Yes & 0.00 & 2.50 & -2.92 & 2010.243 \\
S2-345 & 15.30 & 17.68 & Unknown Age & 32 & 6 & 13.10 & 12.32 & Yes & Yes & 0.00 & 1.78 & -1.18 & 2015.482 \\
S6-78 & 15.31 & 17.56 & Unknown Age & 88 & 18 & 1.07 & 3.76 & No & Yes & 0.00 & 4.38 & -5.38 & 2009.990 \\
S2-61 & 15.31 & 17.47 & Known Old & 65 & 13 & 4.60 & 1.45 & Yes & No & 0.00 & 2.36 & -0.65 & 2009.705 \\
S6-135 & 15.31 & 17.67 & Unknown Age & 54 & 14 & 5.75 & 2.17 & Yes & No & 0.00 & 5.49 & 2.56 & 2008.759 \\
S5-60 & 15.32 & 17.45 & Unknown Age & 86 & 15 & 2.44 & 2.43 & Yes & No & 0.00 & 5.22 & 0.12 & 2009.817 \\
S3-33 & 15.33 & 17.53 & Unknown Age & 36 & 17 & 1.66 & 4.75 & No & Yes & 0.01 & 3.32 & -0.83 & 2010.120 \\
S0-35 & 15.33 & 17.61 & Unknown Age & 39 & 16 & 3.13 & 5.86 & Yes & Yes & 0.00 & 0.02 & 0.88 & 2009.499 \\
S1-29 & 15.34 & 17.63 & Known Young & 82 & 11 & 2.63 & 3.98 & Yes & No & 0.00 & 1.07 & 0.16 & 2010.071 \\
S4-312 & 15.34 & 17.56 & Known Old & 99 & 19 & 0.74 & 0.67 & No & No & 0.00 & 4.60 & -1.54 & 2010.231 \\
S6-4 & 15.35 & 17.57 & Unknown Age & 92 & 18 & 1.52 & 2.03 & No & No & 0.01 & 1.72 & -5.79 & 2010.138 \\
S1-48 & 15.35 & 17.56 & Known Old & 96 & 17 & 4.20 & 2.39 & Yes & No & 0.00 & -0.63 & -1.55 & 2009.947 \\
S3-319 & 15.35 & 17.48 & Unknown Age & 98 & 19 & 0.67 & 1.08 & No & No & 0.01 & 3.57 & -1.44 & 2010.045 \\
S3-62 & 15.35 & 17.56 & Unknown Age & 33 & 11 & 0.78 & 1.20 & No & No & 0.00 & 2.70 & -1.53 & 2011.039 \\
S4-8 & 15.35 & 17.54 & Known Young & 99 & 19 & 0.64 & 1.44 & No & No & 0.00 & -0.45 & -3.97 & 2010.186 \\
S4-176 & 15.36 & 17.55 & Unknown Age & 100 & 18 & 1.02 & 1.03 & No & No & 0.01 & 4.26 & 1.40 & 2010.293 \\
S5-113 & 15.36 & 17.66 & Known Old & 100 & 19 & 1.19 & 1.07 & No & No & 0.00 & -2.55 & -4.80 & 2009.454 \\
S5-178 & 15.37 & 17.54 & Known Old & 98 & 17 & 1.39 & 4.17 & No & Yes & 0.00 & 4.85 & -3.04 & 2010.330 \\
S2-41 & 15.37 & 17.58 & Known Old & 99 & 19 & 3.35 & 2.36 & Yes & No & 0.00 & -0.47 & -2.09 & 2010.303 \\
S5-212 & 15.37 & 17.50 & Known Old & 95 & 18 & 3.23 & 1.50 & Yes & No & 0.01 & 4.03 & -4.39 & 2010.182 \\
S2-59 & 15.37 & 17.79 & Known Old & 74 & 14 & 2.50 & 4.83 & Yes & Yes & 0.00 & 0.82 & -2.33 & 2009.842 \\
S3-31 & 15.38 & 17.40 & Unknown Age & 59 & 17 & 2.25 & 2.43 & Yes & No & 0.00 & 3.39 & 0.39 & 2009.878 \\
S5-141 & 15.38 & 17.50 & Unknown Age & 96 & 15 & 1.63 & 4.30 & No & Yes & 0.00 & 4.34 & -3.41 & 2010.171 \\
S4-279 & 15.38 & 17.65 & Unknown Age & 40 & 18 & 0.52 & 1.68 & No & No & 0.01 & 4.00 & 2.59 & 2010.027 \\
S3-21 & 15.38 & 17.58 & Unknown Age & 39 & 9 & 8.06 & 58.05 & Yes & Yes & 0.00 & 3.20 & -0.21 & 2009.590 \\
S6-80 & 15.38 & 17.68 & Known Old & 72 & 18 & 1.54 & 2.20 & No & No & 0.00 & 5.03 & -4.86 & 2010.739 \\
S1-45 & 15.38 & 17.83 & Unknown Age & 40 & 1 & 4.65 & \text{---} & Yes & No & 0.00 & -1.28 & 1.10 & 2009.660 \\
S5-131 & 15.39 & 17.76 & Known Old & 98 & 18 & 1.47 & 2.90 & No & No & 0.00 & 4.87 & -2.55 & 2010.240 \\
S3-159 & 15.39 & 17.85 & Unknown Age & 96 & 18 & 2.66 & 1.03 & Yes & No & 0.00 & -1.29 & 3.13 & 2010.052 \\
S3-23 & 15.39 & 17.77 & Unknown Age & 68 & 12 & 1.90 & 2.09 & No & No & 0.00 & 2.91 & -1.37 & 2009.964 \\
S2-81 & 15.39 & 17.78 & Known Old & 98 & 17 & 2.49 & 1.97 & Yes & No & 0.00 & 1.98 & -2.04 & 2010.068 \\
S2-68 & 15.40 & 18.12 & Unknown Age & 97 & 18 & 12.94 & 4.92 & Yes & Yes & 0.00 & -1.81 & 1.95 & 2010.217 \\
S4-314 & 15.41 & 17.60 & Known Young & 99 & 19 & 0.59 & 1.97 & No & No & 0.02 & 4.41 & -2.03 & 2010.075 \\
S6-48 & 15.42 & 17.67 & Known Old & 46 & 10 & 2.18 & 3.41 & No & No & 0.01 & 4.88 & -4.16 & 2009.975 \\
S1-50 & 15.42 & 17.73 & Unknown Age & 88 & 7 & 4.67 & 9.32 & Yes & Yes & 0.00 & 1.48 & 0.66 & 2009.664 \\
S0-19 & 15.43 & 17.52 & Known Young & 79 & 17 & 5.90 & 5.08 & Yes & Yes & 0.00 & -0.01 & 0.40 & 2009.642 \\
S0-28 & 15.43 & \text{---} & Known Old & 45 & 0 & 12.00 & \text{---} & Yes & \text{---} & 0.00 & -0.14 & -0.49 & 2007.822 \\
S5-165 & 15.44 & 17.65 & Known Old & 100 & 18 & 0.59 & 0.80 & No & No & 0.01 & 4.88 & -2.86 & 2010.181 \\
S2-40 & 15.44 & 17.62 & Known Young & 34 & 18 & 1.06 & 1.24 & No & No & 0.00 & 1.74 & 1.27 & 2009.828 \\
S1-175 & 15.46 & 17.66 & Unknown Age & 82 & 16 & 4.53 & 7.59 & Yes & Yes & 0.00 & -1.41 & -0.34 & 2014.063 \\
S3-314 & 15.46 & 17.56 & Known Young & 79 & 19 & 1.39 & 1.82 & No & No & 0.01 & 3.84 & -0.09 & 2010.262 \\
S4-295 & 15.46 & 17.92 & Unknown Age & 51 & 12 & 1.59 & 4.17 & No & No & 0.01 & -3.09 & 3.67 & 2010.626 \\
S0-62 & 15.46 & 17.69 & Known Old & 80 & 17 & 2.42 & 4.70 & Yes & Yes & 0.00 & 0.16 & -0.54 & 2010.228 \\
S1-6 & 15.46 & 17.77 & Known Old & 37 & 15 & 2.97 & 3.22 & Yes & No & 0.00 & -0.96 & 0.74 & 2008.886 \\
S3-383 & 15.47 & 17.74 & Known Old & 99 & 19 & 1.08 & 1.79 & No & No & 0.00 & 3.92 & -0.56 & 2010.082 \\
S2-63 & 15.47 & 17.73 & Unknown Age & 100 & 18 & 1.92 & 2.44 & Yes & No & 0.00 & -0.65 & 2.47 & 2010.227 \\
S3-437 & 15.47 & 17.82 & Unknown Age & 51 & 17 & 1.38 & 1.02 & No & No & 0.00 & 2.69 & -1.38 & 2013.944 \\
S1-64 & 15.47 & 17.90 & Unknown Age & 97 & 16 & 7.18 & 31.30 & Yes & Yes & 0.00 & 0.66 & 1.82 & 2010.079 \\
S6-142 & 15.47 & 17.75 & Known Old & 63 & 15 & 1.32 & 2.37 & No & No & 0.01 & 5.47 & -3.56 & 2011.172 \\
S1-66 & 15.47 & 17.72 & Known Old & 68 & 12 & 6.18 & 2.69 & Yes & No & 0.02 & -0.81 & -1.74 & 2009.970 \\
S2-308 & 15.48 & 17.64 & Known Old & 36 & 12 & 1.13 & 1.00 & No & No & 0.00 & -0.64 & -2.85 & 2010.059 \\
S5-24 & 15.48 & 18.27 & Unknown Age & 79 & 10 & 3.47 & 2.57 & Yes & No & 0.00 & -5.00 & -0.89 & 2010.110 \\
S1-26 & 15.49 & 17.71 & Known Old & 98 & 18 & 2.34 & 0.46 & Yes & No & 0.01 & -0.88 & 0.39 & 2010.306 \\
S1-62 & 15.49 & 17.88 & Unknown Age & 98 & 13 & 6.02 & 9.08 & Yes & Yes & 0.01 & 0.44 & 1.80 & 2010.021 \\
S2-34 & 15.49 & 17.81 & Known Old & 95 & 16 & 1.07 & 1.60 & No & No & 0.01 & 1.84 & 1.00 & 2009.058 \\
S2-134 & 15.49 & 17.69 & Known Old & 70 & 14 & 2.98 & 3.18 & Yes & No & 0.00 & -0.99 & -2.00 & 2010.568 \\
S2-46 & 15.49 & 17.71 & Unknown Age & 94 & 17 & 1.69 & 5.30 & No & Yes & 0.00 & 2.17 & -0.71 & 2010.099 \\
S3-209 & 15.50 & 17.23 & Unknown Age & 90 & 17 & 1.71 & 1.83 & No & No & 0.00 & -2.93 & -1.98 & 2010.310 \\
S5-123 & 15.50 & 18.29 & Known Old & 63 & 14 & 7.77 & 2.09 & Yes & No & 0.01 & -4.34 & -3.30 & 2009.664 \\
S1-56 & 15.50 & 18.00 & Known Old & 85 & 14 & 28.05 & 16.48 & Yes & Yes & 0.00 & -1.11 & 1.32 & 2009.763 \\
S7-2 & 15.51 & 17.81 & Unknown Age & 74 & 14 & 4.55 & 5.41 & Yes & Yes & 0.00 & 3.37 & -6.31 & 2010.793 \\
S1-55 & 15.51 & 17.89 & Unknown Age & 95 & 15 & 2.51 & 7.28 & Yes & Yes & 0.00 & 1.59 & 0.64 & 2008.856 \\
S5-252 & 15.51 & 17.77 & Known Old & 80 & 15 & 3.19 & 1.33 & Yes & No & 0.01 & 5.50 & -1.23 & 2012.288 \\
S4-105 & 15.51 & 18.24 & Known Old & 100 & 18 & 1.39 & 2.26 & No & No & 0.00 & -2.82 & -3.18 & 2010.228 \\
S4-56 & 15.52 & 17.88 & Unknown Age & 71 & 10 & 1.95 & 3.62 & No & No & 0.00 & -0.99 & 3.99 & 2010.465 \\
S3-24 & 15.52 & 17.82 & Unknown Age & 59 & 6 & 3.65 & 1.14 & Yes & No & 0.00 & 3.29 & 0.45 & 2009.493 \\
S3-109 & 15.52 & 17.89 & Known Old & 65 & 11 & 1.76 & 4.19 & No & No & 0.02 & -3.19 & 0.42 & 2010.197 \\
S1-47 & 15.52 & 17.74 & Unknown Age & 99 & 18 & 1.85 & 9.55 & No & Yes & 0.00 & -1.61 & 0.43 & 2010.417 \\
S1-67 & 15.53 & 17.85 & Known Old & 91 & 17 & 1.64 & 3.15 & No & No & 0.00 & -1.43 & -1.32 & 2010.456 \\
S3-125 & 15.53 & 18.05 & Unknown Age & 35 & 6 & 2.02 & 0.57 & No & No & 0.00 & -3.07 & -1.22 & 2010.010 \\
S5-106 & 15.53 & 17.96 & Known Young & 86 & 18 & 3.68 & 1.16 & Yes & No & 0.02 & -4.35 & -3.20 & 2010.067 \\
S2-198 & 15.54 & 17.90 & Known Old & 96 & 17 & 2.25 & 4.93 & Yes & Yes & 0.01 & 0.41 & -2.48 & 2009.978 \\
S3-377 & 15.54 & 18.01 & Unknown Age & 85 & 16 & 107.61 & 51.03 & Yes & Yes & 0.00 & 2.56 & -3.03 & 2008.170 \\
S0-67 & 15.54 & 17.79 & Known Old & 79 & 17 & 3.45 & 5.77 & Yes & Yes & 0.00 & 0.25 & -0.54 & 2009.197 \\
S5-288 & 15.55 & 17.73 & Unknown Age & 68 & 15 & 2.36 & 2.70 & Yes & No & 0.00 & 5.33 & 0.16 & 2011.188 \\
S0-29 & 15.56 & 17.60 & Known Old & 34 & 12 & 1.23 & 3.35 & No & No & 0.02 & 0.37 & -0.44 & 2009.722 \\
S3-169 & 15.56 & 17.86 & Unknown Age & 100 & 18 & 0.69 & 0.87 & No & No & 0.03 & -3.39 & 0.37 & 2010.038 \\
S5-124 & 15.56 & 17.76 & Unknown Age & 50 & 10 & 1.53 & 0.96 & No & No & 0.01 & -1.85 & -5.16 & 2009.615 \\
S3-92 & 15.56 & 18.11 & Unknown Age & 34 & 5 & 10.00 & 12.80 & Yes & Yes & 0.00 & -1.35 & 2.88 & 2009.116 \\
S6-8 & 15.57 & 17.81 & Known Old & 91 & 18 & 1.03 & 3.75 & No & Yes & 0.00 & -0.76 & -6.01 & 2009.881 \\
S5-94 & 15.57 & 18.01 & Unknown Age & 83 & 18 & 1.39 & 1.69 & No & No & 0.02 & 4.92 & 2.12 & 2008.726 \\
S1-36 & 15.57 & 17.79 & Known Old & 49 & 18 & 2.40 & 4.63 & Yes & Yes & 0.00 & -0.53 & -1.21 & 2010.227 \\
S2-83 & 15.57 & 17.89 & Known Old & 68 & 10 & 2.00 & 3.61 & No & No & 0.01 & 2.86 & -0.69 & 2009.982 \\
S2-175 & 15.58 & 18.03 & Unknown Age & 51 & 13 & 10.83 & 4.06 & Yes & No & 0.00 & 2.07 & -1.21 & 2009.495 \\
S2-212 & 15.58 & 17.81 & Known Old & 95 & 17 & 2.65 & 5.41 & Yes & Yes & 0.00 & 0.17 & -2.59 & 2009.949 \\
S6-28 & 15.58 & 17.80 & Known Old & 58 & 14 & 1.02 & 0.98 & No & No & 0.02 & 5.01 & -3.66 & 2010.052 \\
S5-210 & 15.58 & 17.76 & Unknown Age & 95 & 15 & 5.88 & 8.72 & Yes & Yes & 0.00 & -1.82 & -5.66 & 2009.694 \\
S4-97 & 15.58 & 17.68 & Known Old & 100 & 19 & 0.74 & 0.41 & No & No & 0.02 & -0.95 & -4.12 & 2010.207 \\
S4-67 & 15.58 & 18.30 & Unknown Age & 89 & 14 & 5.36 & 9.74 & Yes & Yes & 0.00 & 2.82 & -3.04 & 2010.016 \\
S0-27 & 15.58 & 17.79 & Known Old & 84 & 13 & 1.40 & 2.90 & No & No & 0.00 & 0.15 & 0.55 & 2009.841 \\
S5-6 & 15.58 & 18.35 & Unknown Age & 89 & 16 & 3.31 & 3.84 & Yes & No & 0.00 & -4.81 & -1.46 & 2009.544 \\
S2-80 & 15.58 & 17.78 & Known Old & 98 & 18 & 1.74 & 1.42 & No & No & 0.02 & 2.20 & 1.81 & 2010.224 \\
S6-55 & 15.58 & 17.81 & Known Old & 61 & 10 & 1.45 & 1.07 & No & No & 0.00 & 5.00 & -4.11 & 2010.196 \\
S5-80 & 15.59 & 17.78 & Unknown Age & 55 & 18 & 0.87 & 1.73 & No & No & 0.02 & 0.24 & -5.30 & 2009.782 \\
S4-280 & 15.59 & 18.05 & Unknown Age & 56 & 18 & 2.28 & 1.94 & Yes & No & 0.00 & 1.23 & -4.60 & 2010.339 \\
S2-64 & 15.59 & 17.80 & Known Old & 91 & 12 & 2.05 & 4.74 & Yes & Yes & 0.01 & 2.63 & 0.25 & 2010.053 \\
S3-50 & 15.59 & 17.85 & Unknown Age & 98 & 19 & 2.60 & 9.46 & Yes & Yes & 0.00 & -1.88 & -2.33 & 2010.312 \\
S2-205 & 15.59 & 17.81 & Known Old & 98 & 17 & 22.28 & 18.23 & Yes & Yes & 0.00 & 0.48 & 2.49 & 2010.052 \\
S3-108 & 15.60 & 17.80 & Unknown Age & 96 & 18 & 1.72 & 1.45 & No & No & 0.01 & -0.89 & 3.12 & 2010.133 \\
S2-317 & 15.60 & 17.89 & Known Old & 62 & 14 & 3.47 & 12.80 & Yes & Yes & 0.01 & -0.71 & -2.87 & 2010.148 \\
S4-107 & 15.60 & 17.68 & Unknown Age & 44 & 13 & 2.04 & 3.46 & No & No & 0.01 & 3.93 & 1.54 & 2011.962 \\
S1-54 & 15.61 & 18.03 & Unknown Age & 89 & 15 & 4.20 & 2.64 & Yes & No & 0.01 & -1.51 & 0.75 & 2009.661 \\
S2-195 & 15.61 & 18.07 & Unknown Age & 92 & 16 & 9.66 & 2.90 & Yes & No & 0.01 & -2.03 & 1.45 & 2008.883 \\
S2-42 & 15.61 & 17.98 & Unknown Age & 60 & 17 & 5.04 & 3.21 & Yes & No & 0.00 & 0.49 & 2.15 & 2009.692 \\
S1-59 & 15.61 & 17.17 & Unknown Age & 38 & 10 & 5.87 & 11.57 & Yes & Yes & 0.00 & 0.02 & 1.78 & 2007.241 \\
S4-40 & 15.62 & 17.93 & Known Old & 100 & 18 & 1.19 & 1.70 & No & No & 0.00 & -1.97 & -3.61 & 2010.232 \\
S1-58 & 15.62 & 17.99 & Unknown Age & 76 & 15 & 3.62 & 3.77 & Yes & No & 0.01 & -1.49 & 0.97 & 2010.095 \\
S1-65 & 15.62 & 17.71 & Unknown Age & 97 & 16 & 1.49 & 1.66 & No & No & 0.02 & 1.48 & 1.28 & 2009.943 \\
S2-76 & 15.62 & 18.18 & Known Young & 68 & 17 & 11.59 & 21.94 & Yes & Yes & 0.01 & -0.22 & 2.81 & 2011.550 \\
S5-44 & 15.62 & 17.83 & Known Old & 99 & 19 & 0.95 & 0.38 & No & No & 0.00 & 3.52 & -3.74 & 2010.094 \\
S4-273 & 15.62 & 17.88 & Unknown Age & 100 & 19 & 1.08 & 0.71 & No & No & 0.03 & -1.15 & -4.61 & 2009.965 \\
S5-203 & 15.62 & 17.92 & Unknown Age & 50 & 10 & 4.75 & 6.71 & Yes & Yes & 0.00 & -0.23 & -5.87 & 2009.735 \\
S5-126 & 15.64 & 16.81 & Unknown Age & 98 & 19 & 1.43 & 0.80 & No & No & 0.02 & -0.04 & -5.47 & 2009.751 \\
S4-167 & 15.64 & 17.91 & Unknown Age & 96 & 18 & 1.74 & 3.14 & No & No & 0.00 & 3.73 & 2.42 & 2010.133 \\
S6-40 & 15.64 & 17.90 & Unknown Age & 79 & 14 & 3.84 & 4.12 & Yes & No & 0.01 & 0.09 & -6.34 & 2009.538 \\
S6-33 & 15.64 & 18.01 & Unknown Age & 90 & 15 & 2.92 & 4.49 & Yes & Yes & 0.02 & -3.61 & -5.09 & 2009.762 \\
S0-16 & 15.64 & 17.75 & Known Young & 44 & 11 & 19.66 & 6.28 & Yes & Yes & 0.00 & 0.23 & 0.17 & 2007.593 \\
S3-91 & 15.64 & 17.87 & Unknown Age & 95 & 16 & 4.75 & 4.14 & Yes & Yes & 0.02 & -1.71 & -2.67 & 2010.365 \\
S6-53 & 15.65 & \text{---} & Unknown Age & 42 & 0 & 3.53 & \text{---} & Yes & \text{---} & 0.00 & -3.69 & -5.33 & 2009.250 \\
S3-229 & 15.65 & 18.33 & Unknown Age & 84 & 16 & 5.98 & 3.84 & Yes & No & 0.00 & 1.56 & -3.22 & 2010.224 \\
S5-25 & 15.65 & 17.98 & Unknown Age & 100 & 18 & 0.54 & 0.47 & No & No & 0.01 & -2.58 & -4.37 & 2010.133 \\
S3-160 & 15.66 & \text{---} & Unknown Age & 36 & 0 & 3.22 & \text{---} & Yes & \text{---} & 0.00 & 3.30 & 0.79 & 2009.133 \\
S4-140 & 15.66 & 17.97 & Unknown Age & 100 & 18 & 0.66 & 0.31 & No & No & 0.00 & 3.17 & 2.98 & 2010.071 \\
S6-181 & 15.66 & 17.93 & Known Old & 94 & 16 & 1.98 & 3.17 & Yes & No & 0.02 & 5.31 & -4.21 & 2010.492 \\
S5-209 & 15.66 & 17.87 & Unknown Age & 74 & 18 & 0.77 & 0.82 & No & No & 0.02 & -2.93 & -5.15 & 2008.589 \\
S0-24 & 15.66 & 17.75 & Known Old & 71 & 17 & 5.62 & 1.68 & Yes & No & 0.00 & 0.20 & 0.09 & 2008.557 \\
S4-31 & 15.67 & 17.93 & Unknown Age & 100 & 18 & 7.92 & 0.99 & Yes & No & 0.01 & -2.21 & -3.43 & 2010.415 \\
S3-263 & 15.67 & 17.85 & Unknown Age & 94 & 15 & 2.41 & 0.95 & Yes & No & 0.01 & -0.40 & -3.64 & 2010.140 \\
S6-30 & 15.67 & 17.90 & Unknown Age & 82 & 16 & 1.78 & 10.22 & No & Yes & 0.03 & 0.58 & -6.20 & 2009.828 \\
S4-51 & 15.67 & 17.78 & Unknown Age & 43 & 18 & 2.68 & 8.71 & Yes & Yes & 0.01 & 3.17 & 2.63 & 2011.116 \\
S3-225 & 15.67 & 18.02 & Unknown Age & 94 & 16 & 2.14 & 2.43 & Yes & No & 0.01 & 1.45 & -3.26 & 2009.856 \\
S1-40 & 15.68 & \text{---} & Unknown Age & 43 & 0 & 5.89 & \text{---} & Yes & \text{---} & 0.00 & -1.41 & -0.61 & 2010.207 \\
S2-268 & 15.69 & 18.17 & Unknown Age & 83 & 14 & 9.64 & 22.18 & Yes & Yes & 0.01 & -2.78 & 0.48 & 2010.071 \\
S2-319 & 15.69 & \text{---} & Known Old & 89 & 0 & 2.51 & \text{---} & Yes & \text{---} & 0.01 & 0.99 & -2.78 & 2009.644 \\
S3-256 & 15.70 & 18.19 & Unknown Age & 73 & 18 & 9.27 & 12.65 & Yes & Yes & 0.00 & -1.85 & -3.18 & 2009.353 \\
S5-160 & 15.70 & \text{---} & Unknown Age & 34 & 0 & 132.84 & \text{---} & Yes & \text{---} & 0.00 & 4.23 & 3.76 & 2009.530 \\
S1-31 & 15.70 & 18.00 & Known Old & 83 & 17 & 2.00 & 3.38 & Yes & No & 0.01 & -0.99 & 0.54 & 2010.569 \\
S5-127 & 15.70 & 17.78 & Known Old & 93 & 18 & 0.81 & 1.29 & No & No & 0.03 & 4.79 & -2.64 & 2010.228 \\
S4-262 & 15.71 & 17.77 & Known Young & 98 & 18 & 11.27 & 5.79 & Yes & Yes & 0.01 & 4.28 & -1.96 & 2010.562 \\
S3-65 & 15.71 & 18.01 & Known Young & 98 & 16 & 1.27 & 2.30 & No & No & 0.03 & -1.24 & -2.80 & 2009.687 \\
S1-170 & 15.71 & \text{---} & Unknown Age & 64 & 0 & 3.67 & \text{---} & Yes & \text{---} & 0.00 & 1.57 & -1.19 & 2009.609 \\
S2-86 & 15.71 & 18.09 & Unknown Age & 55 & 13 & 4.87 & 6.67 & Yes & Yes & 0.00 & 2.66 & -1.36 & 2007.744 \\
S2-208 & 15.72 & 18.44 & Unknown Age & 75 & 13 & 12.12 & 10.31 & Yes & Yes & 0.00 & -2.05 & 1.58 & 2010.131 \\
S2-200 & 15.72 & 18.06 & Unknown Age & 36 & 18 & 2.84 & 0.94 & Yes & No & 0.02 & -2.53 & 0.01 & 2009.425 \\
S3-59 & 15.72 & 17.89 & Unknown Age & 94 & 15 & 4.12 & 1.83 & Yes & No & 0.01 & -2.42 & -1.88 & 2010.347 \\
S0-108 & 15.72 & 17.76 & Unknown Age & 54 & 10 & 3.04 & 3.77 & Yes & No & 0.00 & 0.45 & -0.90 & 2015.921 \\
S2-261 & 15.72 & 18.22 & Unknown Age & 99 & 18 & 3.52 & 1.36 & Yes & No & 0.01 & -2.60 & 1.01 & 2009.671 \\
S6-36 & 15.73 & 18.18 & Known Old & 66 & 11 & 1.70 & 3.69 & No & No & 0.00 & -4.60 & -4.28 & 2009.482 \\
S6-52 & 15.74 & 17.94 & Unknown Age & 83 & 14 & 3.73 & 3.93 & Yes & No & 0.00 & -1.61 & -6.24 & 2012.171 \\
S2-51 & 15.74 & 18.12 & Known Old & 99 & 18 & 2.09 & 3.34 & Yes & No & 0.02 & 0.74 & 2.14 & 2009.837 \\
S4-123 & 15.75 & 18.10 & Unknown Age & 98 & 18 & 1.10 & 2.07 & No & No & 0.03 & 2.27 & 3.63 & 2010.065 \\
S2-128 & 15.75 & 18.16 & Unknown Age & 81 & 6 & 4.47 & 13.89 & Yes & Yes & 0.00 & 1.09 & -1.89 & 2010.052 \\
S2-44 & 15.75 & 18.17 & Unknown Age & 98 & 16 & 3.20 & 16.43 & Yes & Yes & 0.01 & 0.52 & -2.14 & 2009.503 \\
S5-162 & 15.75 & 17.98 & Unknown Age & 99 & 19 & 1.88 & 1.84 & Yes & No & 0.03 & 5.17 & -2.25 & 2010.076 \\
S3-151 & 15.75 & 18.06 & Known Old & 93 & 16 & 3.29 & 4.46 & Yes & Yes & 0.01 & 1.91 & -2.78 & 2009.954 \\
S3-104 & 15.75 & 18.43 & Unknown Age & 68 & 12 & 11.56 & 44.77 & Yes & Yes & 0.00 & -3.17 & -0.66 & 2010.439 \\
S3-215 & 15.76 & 18.18 & Unknown Age & 63 & 12 & 1.72 & 4.97 & No & Yes & 0.00 & 1.33 & -3.30 & 2010.030 \\
S2-89 & 15.76 & 18.27 & Unknown Age & 90 & 9 & 4.13 & 3.38 & Yes & No & 0.02 & 1.06 & -1.69 & 2010.077 \\
S1-41 & 15.76 & 17.95 & Unknown Age & 74 & 6 & 3.47 & 4.13 & Yes & No & 0.00 & 0.96 & 1.14 & 2010.300 \\
S3-176 & 15.78 & \text{---} & Unknown Age & 65 & 0 & 3.62 & \text{---} & Yes & \text{---} & 0.00 & 3.09 & 1.43 & 2009.859 \\
S1-42 & 15.78 & 18.10 & Unknown Age & 74 & 8 & 4.70 & 4.94 & Yes & No & 0.00 & 0.92 & 1.23 & 2010.216 \\
S5-217 & 15.78 & 18.13 & Unknown Age & 97 & 17 & 0.81 & 0.82 & No & No & 0.02 & 2.45 & -5.46 & 2010.004 \\
S3-123 & 15.79 & 17.97 & Unknown Age & 99 & 17 & 0.93 & 0.87 & No & No & 0.01 & -1.14 & -3.10 & 2009.922 \\
S0-8 & 15.79 & 17.81 & Known Young & 88 & 16 & 8.72 & 5.25 & Yes & Yes & 0.00 & -0.23 & 0.16 & 2008.370 \\
S5-150 & 15.79 & 18.22 & Known Old & 91 & 18 & 4.80 & 2.96 & Yes & No & 0.02 & -3.91 & -4.02 & 2009.922 \\
S2-14 & 15.79 & 18.16 & Unknown Age & 75 & 13 & 3.59 & 2.81 & Yes & No & 0.02 & -1.56 & -1.41 & 2010.393 \\
S4-66 & 15.79 & 18.24 & Unknown Age & 80 & 15 & 8.64 & 19.29 & Yes & Yes & 0.03 & 2.73 & -3.13 & 2010.371 \\
S3-294 & 15.79 & 18.22 & Unknown Age & 87 & 13 & 2.75 & 3.51 & Yes & No & 0.01 & 0.52 & 3.75 & 2010.542 \\
S6-50 & 15.80 & 18.13 & Unknown Age & 62 & 18 & 1.51 & 1.29 & No & No & 0.02 & -3.13 & -5.61 & 2008.044 \\
S4-23 & 15.80 & 18.17 & Unknown Age & 98 & 18 & 4.79 & 4.60 & Yes & Yes & 0.01 & 1.47 & -3.78 & 2009.563 \\
S5-250 & 15.80 & 18.17 & Unknown Age & 43 & 7 & 3.90 & 2.14 & Yes & No & 0.01 & 5.65 & -1.08 & 2011.116 \\
S5-137 & 15.80 & \text{---} & Unknown Age & 33 & 0 & 5.90 & \text{---} & Yes & \text{---} & 0.00 & 3.59 & 4.19 & 2009.603 \\
S5-216 & 15.80 & 18.22 & Unknown Age & 72 & 15 & 0.91 & 3.62 & No & No & 0.03 & 2.22 & -5.55 & 2009.968 \\
S5-79 & 15.80 & 18.02 & Unknown Age & 99 & 18 & 0.56 & 1.06 & No & No & 0.01 & 4.68 & -2.46 & 2010.007 \\
S3-241 & 15.81 & 18.02 & Unknown Age & 76 & 18 & 1.21 & 2.42 & No & No & 0.00 & 2.47 & 2.68 & 2010.342 \\
S4-131 & 15.81 & 18.30 & Unknown Age & 99 & 18 & 1.54 & 0.62 & No & No & 0.01 & 1.47 & -4.04 & 2010.142 \\
S4-284 & 15.81 & 18.02 & Unknown Age & 98 & 16 & 1.03 & 3.12 & No & No & 0.06 & -0.95 & -4.70 & 2010.239 \\
S5-196 & 15.81 & 18.37 & Unknown Age & 65 & 16 & 5.26 & 1.40 & Yes & No & 0.00 & -4.59 & 3.59 & 2010.888 \\
S2-65 & 15.81 & 18.33 & Known Old & 96 & 17 & 12.88 & 43.80 & Yes & Yes & 0.00 & 2.36 & -1.07 & 2009.829 \\
S5-182 & 15.81 & 18.04 & Unknown Age & 47 & 5 & 3.45 & 0.03 & Yes & No & 0.00 & 5.00 & 2.86 & 2010.139 \\
S7-6 & 15.83 & 18.24 & Unknown Age & 76 & 17 & 3.81 & 2.72 & Yes & No & 0.02 & -4.07 & -6.25 & 2007.225 \\
S5-56 & 15.83 & 18.32 & Unknown Age & 45 & 11 & 1.40 & 1.69 & No & No & 0.01 & 3.62 & 3.73 & 2008.943 \\
S4-220 & 15.84 & \text{---} & Unknown Age & 34 & 0 & 1.17 & \text{---} & No & \text{---} & 0.00 & 1.95 & 4.16 & 2009.918 \\
S1-7 & 15.84 & 18.12 & Known Old & 70 & 11 & 2.24 & 4.48 & Yes & No & 0.05 & -1.05 & -0.58 & 2010.057 \\
S6-9 & 15.84 & 18.23 & Unknown Age & 97 & 16 & 5.17 & 9.10 & Yes & Yes & 0.04 & 2.59 & -5.48 & 2010.176 \\
S1-61 & 15.84 & 18.00 & Unknown Age & 46 & 18 & 0.50 & 2.94 & No & No & 0.03 & -1.54 & -0.97 & 2009.863 \\
S3-357 & 15.84 & 18.14 & Unknown Age & 84 & 16 & 0.57 & 0.27 & No & No & 0.09 & 3.14 & 2.32 & 2010.033 \\
S5-84 & 15.84 & 18.27 & Unknown Age & 99 & 18 & 2.88 & 1.56 & Yes & No & 0.03 & -2.74 & -4.53 & 2009.918 \\
S2-127 & 15.85 & 18.17 & Unknown Age & 82 & 6 & 4.30 & 4.38 & Yes & No & 0.03 & 0.20 & -2.21 & 2010.148 \\
S2-39 & 15.85 & 18.18 & Unknown Age & 100 & 18 & 0.75 & 3.35 & No & No & 0.04 & -1.94 & -0.72 & 2010.771 \\
S6-26 & 15.85 & 18.29 & Unknown Age & 92 & 16 & 4.81 & 3.23 & Yes & No & 0.01 & 2.52 & -5.68 & 2010.345 \\
S1-159 & 15.85 & \text{---} & Unknown Age & 82 & 0 & 5.65 & \text{---} & Yes & \text{---} & 0.01 & 1.32 & -1.43 & 2010.637 \\
S4-187 & 15.85 & 18.44 & Unknown Age & 99 & 17 & 7.05 & 36.12 & Yes & Yes & 0.02 & 0.43 & -4.48 & 2010.301 \\
S7-150 & 15.85 & 18.06 & Unknown Age & 43 & 11 & 4.03 & 1.52 & Yes & No & 0.01 & -5.00 & -5.26 & 2007.930 \\
S3-153 & 15.85 & 18.20 & Unknown Age & 100 & 18 & 2.46 & 4.09 & Yes & Yes & 0.09 & 1.60 & 2.98 & 2010.038 \\
S3-338 & 15.85 & 18.21 & Unknown Age & 98 & 18 & 2.11 & 4.55 & Yes & Yes & 0.01 & -3.82 & -0.46 & 2010.136 \\
S4-50 & 15.85 & 18.31 & Unknown Age & 99 & 18 & 1.66 & 1.46 & No & No & 0.07 & 3.08 & 2.76 & 2010.565 \\
S4-283 & 15.85 & 18.21 & Unknown Age & 100 & 18 & 1.80 & 5.49 & No & Yes & 0.04 & 4.38 & 1.85 & 2010.160 \\
S6-262 & 15.87 & 18.06 & Unknown Age & 48 & 11 & 1.13 & 3.49 & No & No & 0.03 & 2.49 & -6.46 & 2007.330 \\
S2-219 & 15.87 & 18.16 & Unknown Age & 56 & 8 & 6.15 & 6.45 & Yes & Yes & 0.01 & -1.57 & -2.09 & 2009.939 \\
S3-167 & 15.87 & 19.40 & Unknown Age & 50 & 8 & 97.12 & 171.31 & Yes & Yes & 0.00 & -3.07 & 1.41 & 2009.976 \\
S4-278 & 15.87 & 18.26 & Unknown Age & 99 & 18 & 1.15 & 1.78 & No & No & 0.08 & -2.52 & -4.02 & 2010.112 \\
S3-83 & 15.87 & 18.30 & Unknown Age & 65 & 15 & 5.28 & 4.23 & Yes & Yes & 0.01 & -2.32 & -2.12 & 2009.548 \\
S4-82 & 15.89 & 18.32 & Unknown Age & 88 & 16 & 9.42 & 9.11 & Yes & Yes & 0.03 & 2.62 & 3.27 & 2010.005 \\
S3-48 & 15.89 & 18.23 & Unknown Age & 94 & 18 & 2.05 & 2.23 & Yes & No & 0.03 & -2.97 & 0.36 & 2010.409 \\
S0-20 & 15.90 & 17.90 & Known Young & 67 & 16 & 3.78 & 1.78 & Yes & No & 0.01 & 0.05 & 0.14 & 2008.089 \\
S7-0 & 15.90 & 18.16 & Unknown Age & 88 & 18 & 1.34 & 1.60 & No & No & 0.10 & 4.05 & -5.79 & 2010.193 \\
S4-47 & 15.90 & 18.41 & Unknown Age & 95 & 16 & 7.27 & 14.88 & Yes & Yes & 0.02 & 2.57 & -3.21 & 2009.974 \\
S3-124 & 15.90 & 18.51 & Unknown Age & 100 & 18 & 20.86 & 41.31 & Yes & Yes & 0.01 & 1.85 & 2.72 & 2009.849 \\
S4-74 & 15.91 & 18.24 & Unknown Age & 99 & 17 & 1.23 & 2.25 & No & No & 0.10 & 0.12 & -4.16 & 2009.978 \\
S2-54 & 15.91 & 18.26 & Unknown Age & 64 & 13 & 5.24 & 11.23 & Yes & Yes & 0.02 & 2.29 & -0.68 & 2009.512 \\
S6-19 & 15.92 & 18.33 & Unknown Age & 62 & 11 & 0.99 & 3.35 & No & No & 0.02 & -4.53 & -4.15 & 2009.665 \\
S5-155 & 15.92 & 18.32 & Unknown Age & 64 & 18 & 2.01 & 1.90 & No & No & 0.02 & 4.72 & 3.02 & 2009.628 \\
S4-195 & 15.92 & 18.32 & Unknown Age & 65 & 14 & 2.60 & 3.60 & Yes & No & 0.01 & 2.42 & 3.81 & 2008.847 \\
S5-65 & 15.92 & 18.96 & Unknown Age & 59 & 15 & 31.56 & 6.19 & Yes & Yes & 0.02 & -3.81 & 3.60 & 2011.045 \\
S5-22 & 15.93 & 18.43 & Unknown Age & 89 & 17 & 4.09 & 1.59 & Yes & No & 0.04 & -3.06 & -4.05 & 2009.907 \\
S2-56 & 15.93 & 18.24 & Unknown Age & 97 & 18 & 2.03 & 2.38 & Yes & No & 0.05 & -0.26 & 2.39 & 2010.441 \\
S3-302 & 15.93 & 18.44 & Unknown Age & 90 & 15 & 7.21 & 14.54 & Yes & Yes & 0.00 & 0.09 & 3.77 & 2010.134 \\
S6-229 & 15.93 & 18.10 & Unknown Age & 53 & 8 & 2.08 & 1.64 & No & No & 0.01 & 5.56 & -3.51 & 2007.370 \\
S7-220 & 15.94 & 18.29 & Unknown Age & 71 & 7 & 2.57 & 2.11 & Yes & No & 0.01 & -4.98 & -6.12 & 2010.839 \\
S4-154 & 15.94 & 18.34 & Unknown Age & 70 & 17 & 3.89 & 9.40 & Yes & Yes & 0.00 & 2.67 & 3.49 & 2011.661 \\
S5-4 & 15.94 & 18.30 & Unknown Age & 100 & 18 & 1.15 & 0.80 & No & No & 0.03 & -2.39 & -4.42 & 2009.825 \\
S4-341 & 15.94 & 18.11 & Unknown Age & 98 & 18 & 1.04 & 1.82 & No & No & 0.06 & 4.18 & -2.62 & 2009.378 \\
S3-116 & 15.94 & 18.14 & Unknown Age & 84 & 18 & 0.83 & 1.84 & No & No & 0.07 & 2.24 & 2.34 & 2010.033 \\
S6-276 & 15.94 & 18.11 & Unknown Age & 77 & 13 & 6.79 & 2.20 & Yes & No & 0.05 & 5.00 & -4.73 & 2010.832 \\
S3-171 & 15.94 & 18.13 & Unknown Age & 33 & 18 & 0.45 & 0.18 & No & No & 0.07 & 2.44 & 2.40 & 2008.434 \\
S4-164 & 15.94 & 18.30 & Unknown Age & 44 & 18 & 1.13 & 6.39 & No & Yes & 0.00 & 3.75 & 2.33 & 2010.396 \\
S2-346 & 15.95 & \text{---} & Unknown Age & 32 & 0 & 15.20 & \text{---} & Yes & \text{---} & 0.00 & -1.96 & 0.78 & 2013.182 \\
S2-304 & 15.96 & 18.10 & Unknown Age & 84 & 12 & 3.51 & 2.91 & Yes & No & 0.00 & 2.52 & 1.46 & 2009.803 \\
S5-197 & 15.96 & 18.09 & Unknown Age & 54 & 8 & 2.44 & 0.34 & Yes & No & 0.07 & -1.09 & -5.73 & 2009.992 \\
S5-118 & 15.96 & 18.66 & Unknown Age & 89 & 15 & 1.19 & 1.11 & No & No & 0.11 & -4.85 & -2.44 & 2010.044 \\
S2-45 & 15.97 & 18.60 & Unknown Age & 96 & 15 & 5.59 & 6.39 & Yes & Yes & 0.02 & -2.15 & 0.57 & 2009.461 \\
S4-30 & 15.97 & 18.42 & Unknown Age & 69 & 6 & 39.78 & 39.87 & Yes & Yes & 0.00 & 2.52 & 3.23 & 2009.975 \\
S4-181 & 15.97 & 18.46 & Unknown Age & 92 & 16 & 2.53 & 10.42 & Yes & Yes & 0.06 & 0.96 & -4.40 & 2010.232 \\
S5-7 & 15.97 & 18.18 & Unknown Age & 90 & 18 & 1.21 & 1.22 & No & No & 0.16 & 1.04 & -4.89 & 2010.172 \\
S6-51 & 15.97 & \text{---} & Unknown Age & 31 & 0 & 2.16 & \text{---} & No & \text{---} & 0.00 & 4.99 & 4.08 & 2010.134 \\
S5-259 & 15.97 & 18.32 & Unknown Age & 92 & 16 & 1.83 & 3.06 & No & No & 0.14 & 5.26 & -1.88 & 2010.305 \\
S6-54 & 15.98 & 18.32 & Unknown Age & 81 & 10 & 3.48 & 16.57 & Yes & Yes & 0.00 & -1.92 & -6.18 & 2010.215 \\
S7-4 & 15.98 & 18.40 & Unknown Age & 90 & 17 & 1.90 & 5.04 & No & Yes & 0.06 & -4.27 & -6.00 & 2008.418 \\
S6-34 & 15.98 & 18.52 & Unknown Age & 66 & 16 & 5.63 & 14.98 & Yes & Yes & 0.02 & 5.28 & 3.32 & 2010.999 \\
S5-181 & 15.99 & 18.42 & Unknown Age & 47 & 13 & 3.42 & 15.81 & Yes & Yes & 0.00 & 5.06 & 2.76 & 2009.893 \\
S3-388 & 15.99 & 18.29 & Unknown Age & 96 & 16 & 1.05 & 0.72 & No & No & 0.03 & -2.43 & -3.16 & 2010.340 \\
S5-49 & 15.99 & 18.39 & Unknown Age & 98 & 18 & 2.87 & 5.79 & Yes & Yes & 0.00 & 4.90 & 1.61 & 2009.661 \\
S3-369 & 15.99 & 18.53 & Unknown Age & 97 & 17 & 4.99 & 2.53 & Yes & No & 0.05 & -1.97 & 3.42 & 2010.217 \\
S4-266 & 15.99 & 18.38 & Unknown Age & 90 & 17 & 7.80 & 22.46 & Yes & Yes & 0.08 & 0.48 & -4.67 & 2008.269 \\
S4-55 & 16.00 & 18.28 & Unknown Age & 99 & 18 & 1.32 & 1.25 & No & No & 0.15 & 4.10 & -0.58 & 2010.204 \\
S5-200 & 16.00 & 18.59 & Unknown Age & 75 & 8 & 3.37 & 2.48 & Yes & No & 0.01 & 4.36 & 3.92 & 2010.156 \\
S1-171 & 16.00 & 18.07 & Unknown Age & 68 & 12 & 3.52 & 2.15 & Yes & No & 0.02 & -0.76 & -1.73 & 2010.726 \\
S4-157 & 16.00 & 18.65 & Unknown Age & 99 & 17 & 56.49 & 44.06 & Yes & Yes & 0.00 & -3.32 & -2.90 & 2007.382 \\
S4-109 & 16.00 & 18.40 & Unknown Age & 98 & 18 & 0.46 & 0.54 & No & No & 0.19 & -2.49 & -3.44 & 2010.118 \\
S0-33 & 16.01 & 18.06 & Unknown Age & 57 & 14 & 6.43 & 5.74 & Yes & Yes & 0.00 & 0.65 & -0.53 & 2010.172 \\
S6-46 & 16.02 & 18.50 & Unknown Age & 78 & 10 & 4.31 & 10.79 & Yes & Yes & 0.00 & -4.00 & -4.99 & 2009.819 \\
S2-303 & 16.02 & 18.43 & Unknown Age & 77 & 13 & 8.90 & 6.57 & Yes & Yes & 0.02 & -2.91 & -0.23 & 2008.164 \\
S3-334 & 16.03 & 18.64 & Unknown Age & 76 & 11 & 5.75 & 8.56 & Yes & Yes & 0.00 & -0.60 & 3.82 & 2010.028 \\
S2-237 & 16.03 & 18.94 & Unknown Age & 75 & 14 & 5.44 & 9.94 & Yes & Yes & 0.00 & -0.44 & -2.67 & 2010.546 \\
S2-300 & 16.03 & 18.52 & Unknown Age & 97 & 17 & 2.73 & 2.88 & Yes & No & 0.03 & 0.26 & 2.88 & 2010.170 \\
S1-43 & 16.03 & 18.19 & Unknown Age & 89 & 12 & 3.27 & 2.38 & Yes & No & 0.01 & 1.11 & 1.21 & 2009.649 \\
S5-107 & 16.04 & 18.59 & Unknown Age & 90 & 17 & 1.77 & 0.78 & No & No & 0.02 & -4.60 & -2.76 & 2009.994 \\
S6-69 & 16.05 & 18.43 & Unknown Age & 89 & 16 & 4.00 & 3.23 & Yes & No & 0.03 & -4.25 & -5.20 & 2009.190 \\
S1-144 & 16.06 & \text{---} & Unknown Age & 70 & 0 & 2.51 & \text{---} & Yes & \text{---} & 0.01 & 1.63 & -0.94 & 2008.913 \\
S2-321 & 16.06 & 18.10 & Unknown Age & 95 & 16 & 1.00 & 2.29 & No & No & 0.09 & -2.43 & -1.69 & 2009.332 \\
S3-93 & 16.06 & 18.38 & Unknown Age & 59 & 8 & 5.58 & 4.78 & Yes & No & 0.00 & -2.40 & -2.11 & 2007.505 \\
S4-464 & 16.06 & 18.96 & Unknown Age & 67 & 15 & 3.83 & 6.94 & Yes & Yes & 0.01 & -4.33 & -1.23 & 2013.647 \\
S1-27 & 16.07 & 18.51 & Known Young & 56 & 12 & 58.04 & 4.02 & Yes & No & 0.01 & -1.03 & 0.19 & 2008.871 \\
S4-69 & 16.07 & 18.46 & Unknown Age & 78 & 9 & 8.88 & 7.58 & Yes & Yes & 0.00 & -3.00 & 2.83 & 2010.265 \\
S6-251 & 16.07 & 18.52 & Unknown Age & 92 & 16 & 1.82 & 2.35 & No & No & 0.05 & 3.35 & -5.99 & 2010.491 \\
S7-240 & 16.07 & 18.59 & Unknown Age & 78 & 14 & 2.86 & 2.30 & Yes & No & 0.01 & 4.78 & -6.36 & 2010.233 \\
S3-359 & 16.08 & 18.25 & Unknown Age & 95 & 16 & 2.77 & 5.39 & Yes & Yes & 0.02 & 3.75 & 1.16 & 2009.103 \\
S3-387 & 16.08 & 18.35 & Unknown Age & 74 & 12 & 3.50 & 6.05 & Yes & Yes & 0.02 & 0.63 & 3.90 & 2010.320 \\
S4-34 & 16.09 & 18.53 & Unknown Age & 78 & 17 & 3.32 & 3.36 & Yes & No & 0.06 & 1.60 & -3.77 & 2009.979 \\
S6-272 & 16.09 & 18.57 & Unknown Age & 75 & 16 & 1.54 & 4.29 & No & Yes & 0.04 & 3.60 & -5.99 & 2007.070 \\
S5-128 & 16.09 & \text{---} & Unknown Age & 84 & 0 & 4.67 & \text{---} & Yes & \text{---} & 0.00 & -5.00 & 2.25 & 2007.270 \\
S4-173 & 16.10 & 18.70 & Unknown Age & 100 & 17 & 7.20 & 12.82 & Yes & Yes & 0.06 & -3.20 & -3.10 & 2010.375 \\
S1-46 & 16.10 & 18.65 & Unknown Age & 89 & 16 & 10.94 & 6.72 & Yes & Yes & 0.00 & -0.10 & -1.60 & 2010.018 \\
S0-36 & 16.11 & 17.97 & Known Young & 39 & 18 & 2.42 & 1.84 & No & No & 0.01 & -0.54 & -0.73 & 2007.994 \\
S0-17 & 16.11 & 18.29 & Known Old & 89 & 16 & 10.88 & 1.14 & Yes & No & 0.01 & 0.05 & 0.01 & 2008.821 \\
S2-273 & 16.11 & 18.46 & Unknown Age & 99 & 17 & 5.53 & 6.47 & Yes & Yes & 0.04 & 0.43 & 2.81 & 2007.708 \\
S2-259 & 16.11 & 18.33 & Unknown Age & 99 & 18 & 1.10 & 1.85 & No & No & 0.11 & -2.13 & -1.77 & 2010.002 \\
S3-260 & 16.12 & 18.51 & Unknown Age & 79 & 15 & 8.37 & 7.31 & Yes & Yes & 0.02 & -3.56 & 0.88 & 2007.983 \\
S6-18 & 16.12 & 18.68 & Unknown Age & 78 & 11 & 2.84 & 1.35 & Yes & No & 0.00 & 4.73 & 3.95 & 2010.269 \\
S6-41 & 16.13 & 18.24 & Unknown Age & 85 & 16 & 2.09 & 2.86 & Yes & No & 0.02 & 1.04 & -6.25 & 2007.605 \\
S6-1 & 16.13 & 18.38 & Unknown Age & 90 & 14 & 1.39 & 2.23 & No & No & 0.10 & -0.60 & -5.98 & 2007.142 \\
S5-140 & 16.13 & \text{---} & Unknown Age & 31 & 0 & 273.16 & \text{---} & Yes & \text{---} & 0.00 & -4.21 & 3.58 & 2010.701 \\
S5-61 & 16.13 & 18.08 & Unknown Age & 98 & 15 & 1.20 & 10.35 & No & Yes & 0.08 & 4.18 & -3.13 & 2007.774 \\
S2-87 & 16.13 & 18.56 & Unknown Age & 88 & 17 & 3.47 & 10.77 & Yes & Yes & 0.01 & 2.30 & -1.40 & 2007.689 \\
S6-0 & 16.14 & 18.61 & Unknown Age & 74 & 15 & 1.82 & 1.20 & No & No & 0.03 & -4.83 & 3.57 & 2008.299 \\
S4-134 & 16.14 & 18.84 & Unknown Age & 91 & 15 & 3.35 & 2.63 & Yes & No & 0.02 & -3.70 & -2.26 & 2009.842 \\
S4-133 & 16.14 & 18.24 & Unknown Age & 87 & 12 & 8.68 & 14.57 & Yes & Yes & 0.00 & 4.30 & 0.33 & 2008.007 \\
S3-258 & 16.15 & 18.28 & Unknown Age & 84 & 16 & 3.98 & 2.53 & Yes & No & 0.02 & 2.69 & -2.51 & 2010.351 \\
S2-159 & 16.15 & 18.64 & Unknown Age & 92 & 18 & 1.37 & 1.73 & No & No & 0.08 & -0.84 & 2.10 & 2010.408 \\
S1-165 & 16.16 & 18.54 & Unknown Age & 92 & 13 & 3.77 & 6.12 & Yes & Yes & 0.01 & -0.25 & -1.97 & 2010.061 \\
S5-322 & 16.17 & \text{---} & Unknown Age & 43 & 0 & 4.92 & \text{---} & Yes & \text{---} & 0.00 & -5.29 & 0.15 & 2014.113 \\
S6-16 & 16.17 & 17.31 & Unknown Age & 57 & 16 & 9.69 & 1.97 & Yes & No & 0.01 & 4.12 & -4.53 & 2007.750 \\
S3-145 & 16.18 & 18.81 & Unknown Age & 41 & 15 & 24.69 & 26.63 & Yes & Yes & 0.00 & -3.00 & 1.50 & 2007.916 \\
S1-30 & 16.18 & 18.36 & Unknown Age & 76 & 10 & 2.99 & 2.28 & Yes & No & 0.00 & 0.53 & -0.97 & 2007.247 \\
S3-212 & 16.18 & 18.11 & Unknown Age & 72 & 16 & 4.94 & 2.62 & Yes & No & 0.02 & 2.57 & -2.46 & 2011.416 \\
S4-182 & 16.19 & 18.47 & Unknown Age & 91 & 18 & 2.06 & 1.88 & Yes & No & 0.10 & 3.66 & 2.60 & 2007.448 \\
S5-3 & 16.19 & 19.17 & Unknown Age & 62 & 7 & 4.97 & 18.60 & Yes & Yes & 0.02 & -3.94 & -3.10 & 2008.458 \\
S4-138 & 16.19 & 18.23 & Unknown Age & 95 & 16 & 3.24 & 3.81 & Yes & No & 0.02 & -0.53 & -4.31 & 2008.132 \\
S1-147 & 16.19 & \text{---} & Unknown Age & 63 & 0 & 3.59 & \text{---} & Yes & \text{---} & 0.00 & 1.19 & -1.47 & 2007.011 \\
S5-28 & 16.20 & 18.72 & Unknown Age & 52 & 16 & 6.27 & 9.62 & Yes & Yes & 0.00 & 3.54 & 3.71 & 2011.696 \\
S3-345 & 16.21 & 18.79 & Unknown Age & 92 & 14 & 4.52 & 6.01 & Yes & Yes & 0.03 & -2.82 & -2.68 & 2007.756 \\
S3-391 & 16.21 & 18.86 & Unknown Age & 67 & 17 & 2.89 & 2.88 & Yes & No & 0.01 & -2.79 & 2.82 & 2009.882 \\
S3-58 & 16.22 & 18.87 & Unknown Age & 80 & 12 & 20.75 & 2.70 & Yes & No & 0.00 & -2.85 & -1.11 & 2007.842 \\
S2-324 & 16.22 & 18.41 & Unknown Age & 78 & 11 & 2.15 & 2.53 & Yes & No & 0.00 & -0.11 & -2.98 & 2007.349 \\
S3-103 & 16.22 & 18.64 & Unknown Age & 90 & 17 & 5.35 & 4.96 & Yes & Yes & 0.00 & 0.22 & 3.21 & 2007.658 \\
S4-9 & 16.22 & 18.45 & Unknown Age & 92 & 17 & 1.45 & 0.87 & No & No & 0.07 & 3.99 & 0.53 & 2007.696 \\
S2-20 & 16.22 & 18.90 & Unknown Age & 67 & 9 & 3.96 & 40.00 & Yes & Yes & 0.00 & 1.65 & 1.57 & 2008.605 \\
S1-118 & 16.23 & \text{---} & Unknown Age & 33 & 0 & 3.52 & \text{---} & Yes & \text{---} & 0.00 & 0.55 & 1.38 & 2007.735 \\
S5-146 & 16.24 & 18.65 & Unknown Age & 82 & 11 & 6.51 & 1.21 & Yes & No & 0.05 & 5.00 & 2.49 & 2007.776 \\
S4-126 & 16.24 & 18.60 & Unknown Age & 57 & 16 & 3.84 & 10.61 & Yes & Yes & 0.01 & 3.25 & 2.82 & 2007.635 \\
S6-47 & 16.24 & 18.48 & Unknown Age & 72 & 16 & 2.73 & 2.60 & Yes & No & 0.07 & 3.69 & -5.22 & 2008.116 \\
S6-10 & 16.25 & 18.51 & Unknown Age & 56 & 5 & 5.21 & 0.28 & Yes & No & 0.00 & 4.94 & -3.55 & 2008.315 \\
S5-18 & 16.25 & 18.29 & Unknown Age & 69 & 18 & 0.79 & 1.31 & No & No & 0.10 & 0.46 & -5.05 & 2008.352 \\
S3-237 & 16.26 & 18.84 & Unknown Age & 94 & 16 & 1.80 & 6.15 & No & Yes & 0.02 & -3.60 & -0.42 & 2008.076 \\
S6-75 & 16.26 & 18.56 & Unknown Age & 56 & 10 & 1.17 & 2.47 & No & No & 0.06 & 3.67 & -5.79 & 2007.460 \\
S6-6 & 16.26 & 18.42 & Unknown Age & 91 & 18 & 2.23 & 3.49 & Yes & No & 0.03 & -0.85 & -5.99 & 2007.846 \\
S5-1 & 16.26 & 18.66 & Unknown Age & 73 & 8 & 8.55 & 3.66 & Yes & No & 0.00 & 3.07 & 3.97 & 2007.333 \\
S3-287 & 16.27 & 18.83 & Unknown Age & 98 & 18 & 5.28 & 5.75 & Yes & Yes & 0.00 & -3.56 & 1.20 & 2007.561 \\
S4-304 & 16.27 & 18.29 & Unknown Age & 78 & 12 & 4.04 & 1.50 & Yes & No & 0.00 & 4.79 & 0.68 & 2007.720 \\
S3-381 & 16.27 & 18.88 & Unknown Age & 95 & 15 & 3.65 & 1.31 & Yes & No & 0.01 & -3.71 & 1.38 & 2007.806 \\
S2-166 & 16.28 & 18.69 & Unknown Age & 96 & 12 & 6.21 & 6.11 & Yes & Yes & 0.01 & 0.11 & 2.33 & 2008.035 \\
S5-271 & 16.28 & 18.38 & Unknown Age & 49 & 10 & 3.90 & 5.49 & Yes & Yes & 0.00 & -2.00 & -5.18 & 2008.460 \\
S1-60 & 16.29 & 18.90 & Unknown Age & 66 & 9 & 3.91 & 3.91 & Yes & No & 0.00 & -0.92 & 1.54 & 2007.856 \\
S6-45 & 16.29 & 18.52 & Unknown Age & 85 & 15 & 2.49 & 2.84 & Yes & No & 0.03 & -1.40 & -6.25 & 2007.688 \\
S4-73 & 16.30 & 18.86 & Unknown Age & 78 & 16 & 2.56 & 5.53 & Yes & Yes & 0.01 & -4.15 & -0.00 & 2007.575 \\
S4-122 & 16.30 & 18.99 & Unknown Age & 89 & 16 & 3.54 & 1.92 & Yes & No & 0.01 & -4.28 & 0.24 & 2007.929 \\
S3-61 & 16.31 & 18.86 & Unknown Age & 68 & 17 & 6.63 & 3.02 & Yes & No & 0.00 & -3.06 & -0.08 & 2008.038 \\
S3-254 & 16.32 & 18.40 & Unknown Age & 93 & 16 & 2.02 & 4.80 & Yes & Yes & 0.01 & 3.23 & 1.72 & 2007.876 \\
S3-230 & 16.33 & 18.90 & Unknown Age & 84 & 5 & 1.83 & 5.88 & No & No & 0.00 & -2.90 & -2.15 & 2007.889 \\
S5-270 & 16.33 & 18.87 & Unknown Age & 98 & 16 & 1.66 & 1.78 & No & No & 0.05 & 2.00 & -4.98 & 2007.220 \\
S1-142 & 16.33 & 18.59 & Unknown Age & 93 & 12 & 3.38 & 0.73 & Yes & No & 0.02 & 0.01 & -1.84 & 2007.341 \\
S6-187 & 16.33 & \text{---} & Unknown Age & 47 & 0 & 14.59 & \text{---} & Yes & \text{---} & 0.00 & -5.20 & 3.00 & 2007.040 \\
S2-214 & 16.33 & 18.82 & Unknown Age & 53 & 10 & 6.77 & 35.77 & Yes & Yes & 0.01 & -1.48 & -2.14 & 2007.568 \\
S5-114 & 16.34 & 19.09 & Unknown Age & 67 & 16 & 3.25 & 7.83 & Yes & Yes & 0.00 & -4.50 & -3.04 & 2007.650 \\
S2-278 & 16.34 & 19.14 & Unknown Age & 57 & 13 & 7.59 & 8.85 & Yes & Yes & 0.00 & -2.21 & 1.76 & 2007.616 \\
S3-129 & 16.35 & 19.70 & Unknown Age & 41 & 7 & 85.09 & 107.55 & Yes & Yes & 0.00 & -2.94 & 1.51 & 2010.280 \\
S2-269 & 16.35 & 18.59 & Unknown Age & 50 & 11 & 3.51 & 7.85 & Yes & Yes & 0.00 & -0.48 & -2.79 & 2008.170 \\
S6-244 & 16.36 & 18.92 & Unknown Age & 30 & 5 & 5.92 & 0.22 & Yes & No & 0.00 & 5.65 & 3.77 & 2006.840 \\
S2-48 & 16.36 & 19.13 & Unknown Age & 72 & 15 & 12.29 & 19.52 & Yes & Yes & 0.00 & 0.96 & 2.07 & 2007.845 \\
S4-65 & 16.36 & 18.58 & Unknown Age & 76 & 18 & 0.64 & 1.51 & No & No & 0.04 & -1.71 & -3.77 & 2008.006 \\
S2-144 & 16.37 & 19.21 & Unknown Age & 85 & 8 & 3.86 & 5.57 & Yes & No & 0.02 & -1.13 & -1.97 & 2007.254 \\
S6-17 & 16.37 & 18.61 & Unknown Age & 44 & 11 & 2.10 & 1.57 & No & No & 0.01 & 0.48 & -6.11 & 2007.682 \\
S6-348 & 16.37 & 18.68 & Unknown Age & 88 & 8 & 2.36 & 4.72 & Yes & No & 0.06 & 1.60 & -6.04 & 2016.200 \\
S4-17 & 16.39 & 18.76 & Unknown Age & 95 & 17 & 1.41 & 2.05 & No & No & 0.04 & -1.88 & 3.56 & 2007.918 \\
S6-11 & 16.39 & 18.69 & Unknown Age & 71 & 14 & 6.30 & 5.79 & Yes & Yes & 0.00 & -4.76 & -3.81 & 2007.410 \\
S0-82 & 16.40 & 18.55 & Unknown Age & 39 & 5 & 8.83 & 7.12 & Yes & No & 0.00 & 0.42 & -0.68 & 2007.268 \\
S2-229 & 16.40 & 18.58 & Unknown Age & 74 & 15 & 2.02 & 3.65 & No & No & 0.00 & -0.41 & -2.61 & 2008.234 \\
S5-59 & 16.40 & 19.12 & Unknown Age & 67 & 7 & 2.63 & 4.29 & Yes & No & 0.00 & -5.15 & -0.69 & 2007.209 \\
S7-7 & 16.40 & 18.91 & Unknown Age & 90 & 15 & 3.27 & 2.58 & Yes & No & 0.01 & -4.38 & -6.07 & 2006.984 \\
S5-204 & 16.41 & 18.49 & Unknown Age & 97 & 16 & 1.33 & 0.82 & No & No & 0.02 & 1.53 & -5.67 & 2007.877 \\
S2-299 & 16.41 & 19.22 & Unknown Age & 65 & 15 & 8.19 & 5.40 & Yes & Yes & 0.00 & -2.05 & 2.03 & 2007.537 \\
S6-43 & 16.42 & 19.38 & Unknown Age & 56 & 9 & 75.75 & 87.19 & Yes & Yes & 0.00 & 5.13 & 3.82 & 2008.931 \\
S5-175 & 16.42 & 18.87 & Unknown Age & 60 & 10 & 1.15 & 2.63 & No & No & 0.03 & 4.84 & 3.06 & 2007.999 \\
S5-260 & 16.43 & 18.77 & Unknown Age & 34 & 6 & 2.35 & 1.70 & No & No & 0.00 & 5.60 & -2.01 & 2007.510 \\
S0-61 & 16.43 & 18.46 & Known Young & 63 & 7 & 8.09 & 2.28 & Yes & No & 0.00 & -0.20 & 0.44 & 2007.638 \\
S6-188 & 16.44 & 19.35 & Unknown Age & 73 & 8 & 2.89 & 2.72 & Yes & No & 0.01 & -5.07 & -3.22 & 2007.060 \\
S5-57 & 16.44 & 18.70 & Unknown Age & 97 & 16 & 3.38 & 7.12 & Yes & Yes & 0.01 & 0.15 & -5.20 & 2007.986 \\
S0-23 & 16.44 & \text{---} & Known Young & 39 & 0 & 10.54 & \text{---} & Yes & \text{---} & 0.00 & 0.25 & -0.29 & 2008.044 \\
S5-167 & 16.45 & \text{---} & Unknown Age & 48 & 0 & 14.97 & \text{---} & Yes & \text{---} & 0.00 & 4.42 & -3.55 & 2007.721 \\
S6-214 & 16.45 & \text{---} & Unknown Age & 40 & 0 & 3.34 & \text{---} & Yes & \text{---} & 0.00 & -5.04 & 3.98 & 2006.670 \\
S1-122 & 16.45 & 18.54 & Unknown Age & 98 & 16 & 2.31 & 1.13 & Yes & No & 0.01 & -1.52 & 0.22 & 2007.579 \\
S3-289 & 16.45 & 19.82 & Unknown Age & 85 & 15 & 16.72 & 90.93 & Yes & Yes & 0.00 & -2.27 & 2.99 & 2007.802 \\
S4-223 & 16.46 & 19.41 & Unknown Age & 89 & 15 & 4.05 & 6.41 & Yes & Yes & 0.02 & -4.61 & 0.10 & 2007.690 \\
S3-143 & 16.46 & 19.53 & Unknown Age & 63 & 15 & 6.70 & 9.69 & Yes & Yes & 0.01 & -3.22 & 0.91 & 2007.761 \\
S6-21 & 16.46 & 18.60 & Unknown Age & 92 & 16 & 0.85 & 1.70 & No & No & 0.02 & -1.20 & -6.03 & 2007.244 \\
S5-20 & 16.46 & 19.10 & Unknown Age & 81 & 15 & 3.48 & 3.86 & Yes & No & 0.00 & -4.86 & 1.46 & 2007.610 \\
S4-302 & 16.47 & 18.90 & Unknown Age & 96 & 17 & 1.25 & 1.69 & No & No & 0.04 & -2.82 & -3.92 & 2007.860 \\
S2-99 & 16.48 & 18.81 & Unknown Age & 59 & 5 & 3.79 & 1.31 & Yes & No & 0.00 & -1.91 & 0.69 & 2008.085 \\
S1-135 & 16.48 & 18.62 & Unknown Age & 62 & 12 & 3.23 & 5.91 & Yes & Yes & 0.01 & -0.25 & -1.75 & 2007.712 \\
S3-219 & 16.48 & 18.61 & Unknown Age & 44 & 12 & 1.35 & 0.67 & No & No & 0.02 & 2.80 & -2.23 & 2007.519 \\
S2-311 & 16.49 & 18.60 & Unknown Age & 47 & 15 & 4.22 & 5.12 & Yes & Yes & 0.00 & -2.74 & -1.04 & 2007.976 \\
S2-257 & 16.50 & 19.14 & Unknown Age & 97 & 15 & 4.96 & 2.88 & Yes & No & 0.00 & -2.73 & -0.48 & 2008.233 \\
S3-77 & 16.50 & 18.67 & Unknown Age & 89 & 18 & 1.73 & 1.91 & No & No & 0.00 & 2.32 & 2.07 & 2007.941 \\
S1-110 & 16.50 & \text{---} & Unknown Age & 35 & 0 & 22.61 & \text{---} & Yes & \text{---} & 0.00 & 1.36 & -0.51 & 2007.721 \\
S6-190 & 16.51 & 19.17 & Unknown Age & 96 & 13 & 1.71 & 5.35 & No & Yes & 0.00 & 3.79 & -4.68 & 2007.590 \\
S4-226 & 16.53 & 19.41 & Unknown Age & 47 & 15 & 2.22 & 2.19 & No & No & 0.00 & -4.61 & 0.21 & 2007.203 \\
S3-141 & 16.53 & 18.74 & Unknown Age & 96 & 16 & 3.94 & 1.46 & Yes & No & 0.00 & -0.71 & 3.27 & 2008.006 \\
S0-55 & 16.53 & 18.66 & Known Old & 81 & 17 & 2.37 & 2.03 & Yes & No & 0.00 & -0.34 & -0.36 & 2007.586 \\
S4-494 & 16.54 & 19.11 & Unknown Age & 35 & 12 & 2.62 & 4.38 & No & No & 0.00 & -4.13 & -2.51 & 2018.450 \\
S3-82 & 16.55 & 18.63 & Unknown Age & 65 & 12 & 2.40 & 2.82 & Yes & No & 0.00 & 2.81 & -1.38 & 2007.871 \\
S3-127 & 16.55 & 18.44 & Unknown Age & 70 & 12 & 5.59 & 3.91 & Yes & No & 0.00 & 2.92 & 1.62 & 2008.121 \\
S2-33 & 16.55 & 18.80 & Unknown Age & 64 & 18 & 0.88 & 1.62 & No & No & 0.00 & -1.99 & -0.17 & 2007.379 \\
S2-158 & 16.55 & 18.93 & Unknown Age & 91 & 15 & 3.39 & 2.04 & Yes & No & 0.00 & 0.62 & -2.22 & 2008.077 \\
S4-130 & 16.55 & 18.68 & Unknown Age & 88 & 17 & 1.16 & 2.31 & No & No & 0.00 & -1.29 & -4.12 & 2007.324 \\
S4-320 & 16.56 & 19.15 & Unknown Age & 36 & 12 & 3.94 & 1.77 & Yes & No & 0.00 & -4.12 & -2.63 & 2005.580 \\
S5-272 & 16.56 & 18.87 & Unknown Age & 50 & 9 & 6.02 & 2.75 & Yes & No & 0.00 & 5.58 & -0.26 & 2007.140 \\
S5-265 & 16.57 & 18.90 & Unknown Age & 99 & 16 & 2.37 & 1.16 & Yes & No & 0.00 & 2.68 & -4.50 & 2006.880 \\
S2-188 & 16.58 & 19.77 & Unknown Age & 97 & 12 & 12.86 & 20.13 & Yes & Yes & 0.00 & -1.34 & -2.09 & 2007.693 \\
S6-218 & 16.58 & 18.92 & Unknown Age & 36 & 6 & 2.67 & 7.39 & Yes & No & 0.00 & 5.68 & -3.11 & 2009.690 \\
S6-191 & 16.58 & 18.89 & Unknown Age & 87 & 14 & 10.38 & 4.01 & Yes & No & 0.00 & -4.23 & -4.29 & 2009.160 \\
S2-184 & 16.59 & 18.95 & Unknown Age & 76 & 5 & 11.52 & 12.30 & Yes & Yes & 0.00 & -2.23 & 1.00 & 2007.473 \\
S0-59 & 16.59 & 18.79 & Unknown Age & 65 & 12 & 4.05 & 6.54 & Yes & Yes & 0.00 & 0.31 & 0.41 & 2008.137 \\
S6-231 & 16.59 & 18.97 & Unknown Age & 90 & 15 & 2.98 & 1.70 & Yes & No & 0.00 & -2.58 & -6.07 & 2006.410 \\
S7-126 & 16.60 & 18.74 & Unknown Age & 97 & 16 & 1.76 & 1.57 & No & No & 0.00 & 5.00 & -5.03 & 2008.660 \\
S4-306 & 16.60 & 18.77 & Unknown Age & 72 & 14 & 5.19 & 4.42 & Yes & Yes & 0.00 & 4.84 & 0.19 & 2007.205 \\
S0-68 & 16.60 & 18.34 & Unknown Age & 54 & 6 & 5.85 & 6.63 & Yes & No & 0.00 & 0.43 & 0.49 & 2007.174 \\
S3-330 & 16.60 & 19.01 & Unknown Age & 96 & 16 & 2.56 & 1.69 & Yes & No & 0.00 & 1.63 & -3.50 & 2007.735 \\
S3-85 & 16.61 & \text{---} & Unknown Age & 58 & 0 & 1.87 & \text{---} & No & \text{---} & 0.00 & 1.24 & -2.88 & 2007.399 \\
S6-57 & 16.62 & 18.79 & Unknown Age & 95 & 16 & 1.98 & 0.77 & Yes & No & 0.00 & -3.38 & -5.56 & 2008.429 \\
S5-35 & 16.62 & 18.46 & Unknown Age & 93 & 12 & 0.66 & 0.38 & No & No & 0.00 & 3.84 & 3.39 & 2007.153 \\
S5-190 & 16.62 & \text{---} & Unknown Age & 32 & 0 & 13.92 & \text{---} & Yes & \text{---} & 0.00 & -5.34 & 2.28 & 2007.752 \\
S2-186 & 16.62 & 18.34 & Unknown Age & 91 & 16 & 3.77 & 3.58 & Yes & No & 0.00 & -2.35 & -0.74 & 2008.051 \\
S5-186 & 16.62 & 18.81 & Unknown Age & 76 & 16 & 2.59 & 3.43 & Yes & No & 0.00 & 4.02 & -4.15 & 2007.509 \\
S4-323 & 16.63 & \text{---} & Unknown Age & 30 & 0 & 1.73 & \text{---} & No & \text{---} & 0.00 & -0.76 & -4.84 & 2007.861 \\
S3-255 & 16.63 & 18.94 & Unknown Age & 91 & 9 & 5.50 & 9.18 & Yes & Yes & 0.00 & -2.81 & -2.34 & 2007.056 \\
S6-2 & 16.63 & 18.87 & Unknown Age & 90 & 16 & 3.13 & 5.27 & Yes & Yes & 0.00 & -1.65 & -5.79 & 2007.047 \\
S4-307 & 16.63 & 19.44 & Unknown Age & 88 & 15 & 2.99 & 3.32 & Yes & No & 0.00 & -4.78 & -0.71 & 2007.339 \\
S3-401 & 16.64 & 19.41 & Unknown Age & 43 & 11 & 4.14 & 3.58 & Yes & No & 0.00 & -3.12 & 2.35 & 2008.480 \\
S5-277 & 16.64 & 19.02 & Unknown Age & 56 & 11 & 4.25 & 2.57 & Yes & No & 0.00 & 5.51 & 1.50 & 2006.890 \\
S6-344 & 16.65 & 18.88 & Unknown Age & 99 & 15 & 1.36 & 1.01 & No & No & 0.00 & 3.56 & -4.88 & 2015.981 \\
S0-105 & 16.66 & \text{---} & Unknown Age & 43 & 0 & 13.54 & \text{---} & Yes & \text{---} & 0.00 & -0.24 & 0.08 & 2011.642 \\
S3-113 & 16.66 & 18.73 & Unknown Age & 59 & 8 & 5.92 & 9.69 & Yes & Yes & 0.00 & 0.21 & -3.25 & 2007.543 \\
S5-176 & 16.66 & 18.53 & Unknown Age & 33 & 16 & 2.82 & 3.94 & Yes & Yes & 0.00 & 3.53 & -4.49 & 2007.622 \\
S5-151 & 16.66 & 18.93 & Unknown Age & 99 & 16 & 7.42 & 29.96 & Yes & Yes & 0.00 & 3.56 & -4.32 & 2007.977 \\
S6-222 & 16.67 & \text{---} & Unknown Age & 70 & 0 & 4.83 & \text{---} & Yes & \text{---} & 0.00 & -2.94 & -5.81 & 2009.210 \\
S0-103 & 16.67 & 18.71 & Unknown Age & 49 & 8 & 10.27 & 12.25 & Yes & Yes & 0.00 & 0.00 & -0.13 & 2008.069 \\
S6-271 & 16.68 & 18.98 & Unknown Age & 89 & 15 & 1.90 & 3.43 & No & No & 0.00 & -3.53 & -6.03 & 2007.880 \\
S4-52 & 16.69 & 17.83 & Unknown Age & 95 & 18 & 1.50 & 0.46 & No & No & 0.00 & -0.17 & -4.12 & 2007.895 \\
S4-303 & 16.70 & 18.92 & Unknown Age & 55 & 16 & 13.15 & 11.47 & Yes & Yes & 0.00 & 4.34 & 2.14 & 2007.481 \\
S4-347 & 16.70 & 18.86 & Unknown Age & 48 & 11 & 1.79 & 4.71 & No & No & 0.00 & 4.59 & 1.87 & 2007.610 \\
S6-357 & 16.70 & 18.94 & Unknown Age & 69 & 10 & 3.76 & 0.99 & Yes & No & 0.00 & 5.27 & -3.28 & 2016.019 \\
S3-121 & 16.70 & 19.14 & Unknown Age & 65 & 16 & 3.64 & 4.34 & Yes & Yes & 0.00 & -0.06 & 3.28 & 2007.398 \\
S3-235 & 16.71 & 18.97 & Unknown Age & 66 & 5 & 4.30 & 0.89 & Yes & No & 0.00 & -0.57 & -3.57 & 2007.854 \\
S5-206 & 16.71 & 19.52 & Unknown Age & 82 & 10 & 4.13 & 4.65 & Yes & No & 0.00 & 5.30 & 2.59 & 2007.474 \\
S5-189 & 16.71 & 19.31 & Unknown Age & 87 & 11 & 6.29 & 10.54 & Yes & Yes & 0.00 & 2.93 & -5.01 & 2007.237 \\
S2-271 & 16.71 & 18.93 & Unknown Age & 89 & 9 & 3.74 & 17.97 & Yes & Yes & 0.00 & 0.73 & 2.74 & 2007.618 \\
S3-240 & 16.71 & 18.86 & Unknown Age & 45 & 12 & 15.00 & 6.08 & Yes & Yes & 0.00 & -1.27 & 3.39 & 2006.750 \\
S4-467 & 16.73 & 18.80 & Unknown Age & 81 & 14 & 1.64 & 0.44 & No & No & 0.00 & -1.19 & -3.99 & 2016.114 \\
S1-92 & 16.73 & 19.03 & Unknown Age & 86 & 17 & 2.79 & 3.06 & Yes & No & 0.00 & -1.14 & 0.49 & 2008.016 \\
S0-83 & 16.74 & 19.15 & Known Old & 87 & 13 & 3.63 & 14.38 & Yes & Yes & 0.00 & -0.36 & 0.70 & 2008.121 \\
S7-129 & 16.74 & 19.12 & Unknown Age & 32 & 14 & 2.51 & 1.47 & No & No & 0.00 & -4.80 & -5.28 & 2008.090 \\
S0-48 & 16.74 & \text{---} & Unknown Age & 36 & 0 & 85.48 & \text{---} & Yes & \text{---} & 0.00 & -0.18 & -0.30 & 2007.890 \\
S0-49 & 16.74 & 18.95 & Known Old & 91 & 7 & 4.32 & 5.81 & Yes & No & 0.00 & -0.35 & -0.12 & 2007.125 \\
S4-264 & 16.75 & 19.53 & Unknown Age & 84 & 14 & 8.08 & 9.78 & Yes & Yes & 0.00 & -4.20 & 2.09 & 2008.054 \\
S1-74 & 16.75 & 19.06 & Unknown Age & 61 & 8 & 4.55 & 2.21 & Yes & No & 0.00 & 0.98 & -0.34 & 2008.029 \\
S5-50 & 16.76 & 19.76 & Unknown Age & 93 & 16 & 12.49 & 39.82 & Yes & Yes & 0.00 & -3.99 & -3.31 & 2008.037 \\
S4-336 & 16.76 & 19.31 & Unknown Age & 97 & 15 & 5.49 & 5.00 & Yes & Yes & 0.00 & -3.66 & -3.31 & 2008.107 \\
S3-367 & 16.76 & 18.48 & Unknown Age & 96 & 16 & 1.54 & 1.35 & No & No & 0.00 & 3.39 & -1.99 & 2007.417 \\
S2-111 & 16.77 & 18.91 & Unknown Age & 86 & 14 & 17.67 & 37.67 & Yes & Yes & 0.00 & -2.09 & 0.14 & 2007.511 \\
S4-175 & 16.79 & 19.84 & Unknown Age & 84 & 15 & 2.85 & 6.59 & Yes & Yes & 0.00 & -4.40 & 0.79 & 2007.353 \\
S2-161 & 16.79 & 19.53 & Unknown Age & 32 & 7 & 4.79 & 15.09 & Yes & Yes & 0.00 & -1.47 & 1.82 & 2008.169 \\
S2-133 & 16.80 & 19.00 & Unknown Age & 59 & 10 & 2.23 & 10.07 & Yes & Yes & 0.00 & 0.52 & 2.15 & 2006.310 \\
S4-346 & 16.80 & 19.61 & Unknown Age & 83 & 11 & 3.86 & 10.34 & Yes & Yes & 0.00 & -4.95 & 0.02 & 2007.083 \\
S2-274 & 16.80 & 19.09 & Unknown Age & 77 & 12 & 3.40 & 4.77 & Yes & Yes & 0.00 & 1.27 & -2.54 & 2007.359 \\
S6-352 & 16.80 & 18.97 & Unknown Age & 76 & 15 & 1.63 & 3.11 & No & No & 0.00 & 3.25 & -5.20 & 2016.101 \\
S0-92 & 16.81 & 18.93 & Unknown Age & 53 & 11 & 10.27 & 5.63 & Yes & Yes & 0.00 & -0.79 & 0.48 & 2008.861 \\
S2-204 & 16.81 & \text{---} & Unknown Age & 68 & 0 & 3.10 & \text{---} & Yes & \text{---} & 0.00 & 0.33 & -2.54 & 2007.457 \\
S3-329 & 16.82 & \text{---} & Unknown Age & 44 & 0 & 4.09 & \text{---} & Yes & \text{---} & 0.00 & -3.20 & -2.14 & 2007.402 \\
S3-130 & 16.82 & \text{---} & Unknown Age & 34 & 0 & 5.73 & \text{---} & Yes & \text{---} & 0.00 & 3.22 & -0.84 & 2007.378 \\
S2-97 & 16.82 & 19.16 & Unknown Age & 88 & 15 & 4.80 & 8.40 & Yes & Yes & 0.00 & -2.04 & 0.29 & 2008.344 \\
S5-39 & 16.83 & 19.89 & Unknown Age & 85 & 13 & 4.39 & 1.40 & Yes & No & 0.00 & -4.73 & 1.99 & 2008.155 \\
S4-466 & 16.83 & 19.30 & Unknown Age & 95 & 16 & 5.43 & 4.86 & Yes & Yes & 0.00 & 1.95 & -4.59 & 2015.994 \\
S4-81 & 16.84 & 19.13 & Unknown Age & 59 & 12 & 4.89 & 1.24 & Yes & No & 0.00 & 2.23 & -3.52 & 2007.224 \\
S5-58 & 16.85 & 19.16 & Unknown Age & 50 & 16 & 3.58 & 2.13 & Yes & No & 0.00 & 5.01 & -1.40 & 2007.597 \\
S6-350 & 16.87 & 19.03 & Unknown Age & 84 & 12 & 3.91 & 0.79 & Yes & No & 0.00 & 2.78 & -5.34 & 2015.929 \\
S2-110 & 16.87 & 19.19 & Unknown Age & 71 & 15 & 19.46 & 51.63 & Yes & Yes & 0.00 & 1.15 & 1.75 & 2007.325 \\
S5-291 & 16.88 & 19.11 & Unknown Age & 93 & 15 & 3.17 & 3.73 & Yes & No & 0.00 & -1.97 & -5.64 & 2016.240 \\
S4-239 & 16.89 & 19.36 & Unknown Age & 90 & 15 & 1.67 & 1.04 & No & No & 0.00 & 4.61 & -0.55 & 2007.525 \\
S2-220 & 16.89 & 19.44 & Unknown Age & 92 & 15 & 3.34 & 5.43 & Yes & Yes & 0.00 & -2.48 & 0.79 & 2008.024 \\
S1-97 & 16.89 & 19.07 & Unknown Age & 37 & 15 & 4.95 & 12.39 & Yes & Yes & 0.00 & -1.00 & 0.83 & 2007.842 \\
S2-280 & 16.90 & 18.12 & Unknown Age & 80 & 16 & 1.93 & 2.00 & No & No & 0.00 & -2.52 & -1.35 & 2007.748 \\
S4-308 & 16.91 & 19.03 & Unknown Age & 62 & 8 & 3.57 & 9.96 & Yes & Yes & 0.00 & -2.91 & 3.85 & 2007.621 \\
S4-146 & 16.91 & 19.03 & Unknown Age & 59 & 12 & 4.64 & 8.75 & Yes & Yes & 0.00 & 4.09 & -1.49 & 2008.212 \\
S4-75 & 16.92 & 20.35 & Unknown Age & 88 & 12 & 21.11 & 4.92 & Yes & Yes & 0.00 & -4.05 & 0.89 & 2007.822 \\
S3-295 & 16.92 & 19.32 & Unknown Age & 47 & 15 & 3.14 & 6.18 & Yes & Yes & 0.00 & -2.42 & -2.90 & 2008.403 \\
S6-355 & 16.92 & \text{---} & Unknown Age & 73 & 0 & 1.81 & \text{---} & No & \text{---} & 0.00 & 2.09 & -5.93 & 2015.753 \\
S5-38 & 16.92 & 19.96 & Unknown Age & 87 & 13 & 3.54 & 4.70 & Yes & Yes & 0.00 & -4.77 & -1.89 & 2008.002 \\
S3-135 & 16.92 & 19.25 & Unknown Age & 56 & 13 & 2.18 & 4.52 & No & Yes & 0.00 & -0.83 & -3.23 & 2007.682 \\
S5-63 & 16.93 & 19.04 & Unknown Age & 43 & 12 & 2.35 & 5.23 & No & Yes & 0.00 & -2.11 & -4.77 & 2008.158 \\
S3-115 & 16.93 & 19.23 & Unknown Age & 65 & 11 & 2.54 & 1.42 & Yes & No & 0.00 & -3.23 & 0.49 & 2007.890 \\
S3-349 & 16.93 & 19.38 & Unknown Age & 86 & 15 & 1.81 & 3.63 & No & No & 0.00 & 1.86 & -3.42 & 2007.583 \\
S1-151 & 16.93 & 19.40 & Unknown Age & 88 & 12 & 4.94 & 8.03 & Yes & Yes & 0.00 & -1.87 & 0.25 & 2007.920 \\
S5-290 & 16.94 & 19.19 & Unknown Age & 96 & 15 & 2.71 & 5.90 & Yes & Yes & 0.00 & -2.78 & -4.65 & 2016.070 \\
S3-199 & 16.95 & 19.12 & Unknown Age & 44 & 12 & 1.97 & 1.14 & No & No & 0.00 & 2.81 & -2.14 & 2008.204 \\
S0-86 & 16.95 & 18.99 & Unknown Age & 67 & 10 & 1.75 & 0.72 & No & No & 0.00 & -0.10 & -0.85 & 2008.150 \\
S4-362 & 16.95 & 19.67 & Unknown Age & 87 & 15 & 2.15 & 9.57 & Yes & Yes & 0.00 & -4.63 & -1.90 & 2007.279 \\
S4-16 & 16.95 & 19.06 & Unknown Age & 75 & 10 & 3.29 & 2.75 & Yes & No & 0.00 & 3.41 & -2.17 & 2008.246 \\
S5-52 & 16.95 & 20.05 & Unknown Age & 88 & 11 & 4.87 & 6.99 & Yes & Yes & 0.00 & -4.68 & 2.22 & 2007.790 \\
S5-330 & 16.96 & \text{---} & Unknown Age & 38 & 0 & 6.92 & \text{---} & Yes & \text{---} & 0.00 & -5.29 & 2.73 & 2013.566 \\
S4-102 & 16.97 & 19.54 & Unknown Age & 93 & 15 & 2.81 & 5.89 & Yes & Yes & 0.00 & -3.21 & -2.74 & 2007.591 \\
S2-93 & 16.98 & 19.37 & Unknown Age & 88 & 15 & 3.85 & 6.83 & Yes & Yes & 0.00 & -1.98 & 0.37 & 2008.166 \\
S3-94 & 16.98 & 19.22 & Unknown Age & 31 & 16 & 1.01 & 4.45 & No & Yes & 0.00 & 2.08 & 2.43 & 2007.299 \\
S1-76 & 16.98 & 19.34 & Unknown Age & 37 & 11 & 4.48 & 4.80 & Yes & No & 0.00 & -0.79 & -0.73 & 2007.976 \\
S6-351 & 16.98 & 19.32 & Unknown Age & 81 & 15 & 1.97 & 2.85 & Yes & No & 0.00 & -0.90 & -6.25 & 2016.094 \\
S2-282 & 16.98 & 18.83 & Unknown Age & 97 & 17 & 1.55 & 1.45 & No & No & 0.00 & -0.49 & 2.81 & 2007.707 \\
S5-289 & 17.00 & 19.46 & Unknown Age & 98 & 15 & 1.82 & 3.96 & No & No & 0.00 & -2.44 & -5.07 & 2015.964 \\
S6-363 & 17.01 & 19.23 & Unknown Age & 64 & 10 & 2.36 & 2.34 & Yes & No & 0.00 & 5.39 & -3.27 & 2015.084 \\
S5-344 & 17.01 & 19.49 & Unknown Age & 31 & 15 & 1.89 & 3.15 & No & No & 0.00 & -4.64 & -3.51 & 2016.204 \\
S2-154 & 17.02 & 19.23 & Unknown Age & 38 & 13 & 2.32 & 6.94 & No & Yes & 0.00 & 2.27 & 0.24 & 2007.237 \\
S5-284 & 17.03 & \text{---} & Unknown Age & 69 & 0 & 34.86 & \text{---} & Yes & \text{---} & 0.00 & -5.14 & 3.08 & 2006.770 \\
S5-300 & 17.03 & 19.20 & Unknown Age & 73 & 15 & 2.79 & 2.42 & Yes & No & 0.00 & -2.99 & -5.14 & 2017.584 \\
S2-107 & 17.03 & \text{---} & Unknown Age & 58 & 0 & 3.05 & \text{---} & Yes & \text{---} & 0.00 & 0.47 & -2.03 & 2008.232 \\
S3-269 & 17.03 & 19.27 & Unknown Age & 81 & 15 & 1.59 & 1.89 & No & No & 0.00 & -0.02 & -3.70 & 2007.658 \\
S5-158 & 17.04 & 20.09 & Unknown Age & 68 & 7 & 2.05 & 1.69 & No & No & 0.00 & -5.07 & -2.46 & 2007.340 \\
S3-451 & 17.04 & 19.87 & Unknown Age & 33 & 14 & 6.65 & 2.65 & Yes & No & 0.00 & -2.90 & -0.78 & 2015.153 \\
S7-254 & 17.04 & 18.80 & Unknown Age & 30 & 10 & 2.21 & 2.01 & No & No & 0.00 & 4.44 & -6.46 & 2019.874 \\
S2-298 & 17.05 & 19.22 & Unknown Age & 68 & 10 & 3.44 & 3.08 & Yes & No & 0.00 & 2.81 & -0.74 & 2007.173 \\
S0-54 & 17.05 & 19.19 & Unknown Age & 35 & 5 & 6.20 & 1.76 & Yes & No & 0.00 & 0.01 & 0.47 & 2006.815 \\
S6-345 & 17.06 & 19.20 & Unknown Age & 93 & 16 & 1.05 & 0.64 & No & No & 0.00 & 4.65 & -4.41 & 2016.209 \\
S3-239 & 17.06 & 19.27 & Unknown Age & 52 & 16 & 5.75 & 12.94 & Yes & Yes & 0.00 & 2.74 & -2.37 & 2007.260 \\
S5-305 & 17.07 & 19.38 & Unknown Age & 70 & 13 & 2.57 & 6.92 & Yes & Yes & 0.00 & 2.15 & -5.60 & 2016.676 \\
S4-90 & 17.07 & \text{---} & Unknown Age & 53 & 0 & 2.72 & \text{---} & Yes & \text{---} & 0.00 & -1.17 & 4.01 & 2007.435 \\
S3-449 & 17.08 & 19.54 & Unknown Age & 35 & 11 & 10.58 & 12.56 & Yes & Yes & 0.00 & -1.16 & 2.79 & 2020.426 \\
S5-26 & 17.08 & 19.54 & Unknown Age & 79 & 10 & 2.48 & 1.69 & Yes & No & 0.00 & -3.36 & 3.81 & 2007.867 \\
S2-348 & 17.09 & 19.54 & Unknown Age & 47 & 10 & 5.23 & 22.79 & Yes & Yes & 0.00 & 1.32 & 2.40 & 2018.378 \\
S5-340 & 17.09 & 19.22 & Unknown Age & 33 & 11 & 1.60 & 0.37 & No & No & 0.00 & -2.14 & -4.81 & 2018.921 \\
S4-80 & 17.09 & 19.37 & Unknown Age & 31 & 15 & 1.85 & 5.15 & No & Yes & 0.00 & 2.17 & 3.56 & 2007.052 \\
S4-469 & 17.11 & 19.61 & Unknown Age & 78 & 9 & 3.65 & 3.42 & Yes & No & 0.00 & 3.16 & 3.71 & 2015.481 \\
S0-38 & 17.11 & \text{---} & Known Old & 37 & 0 & 7.06 & \text{---} & Yes & \text{---} & 0.00 & -0.18 & 0.05 & 2006.982 \\
S4-132 & 17.12 & 19.92 & Unknown Age & 74 & 15 & 3.01 & 6.79 & Yes & Yes & 0.00 & -4.24 & 0.79 & 2007.544 \\
S3-95 & 17.13 & 19.35 & Unknown Age & 95 & 15 & 4.29 & 2.84 & Yes & No & 0.00 & 1.70 & 2.70 & 2007.293 \\
S1-124 & 17.13 & 19.40 & Unknown Age & 57 & 11 & 6.46 & 1.17 & Yes & No & 0.00 & -0.56 & -1.47 & 2007.595 \\
S4-360 & 17.13 & \text{---} & Unknown Age & 49 & 0 & 120.41 & \text{---} & Yes & \text{---} & 0.00 & -4.03 & 2.92 & 2007.749 \\
S4-128 & 17.13 & 19.91 & Unknown Age & 86 & 15 & 6.13 & 18.01 & Yes & Yes & 0.00 & 1.27 & -4.12 & 2007.980 \\
S4-292 & 17.13 & 19.78 & Unknown Age & 73 & 15 & 2.15 & 2.67 & Yes & No & 0.00 & -3.89 & -2.80 & 2007.450 \\
S5-297 & 17.14 & 19.22 & Unknown Age & 78 & 16 & 1.47 & 1.68 & No & No & 0.00 & 1.17 & -5.27 & 2016.188 \\
S3-232 & 17.14 & 19.75 & Unknown Age & 97 & 15 & 2.98 & 12.44 & Yes & Yes & 0.00 & -3.56 & 0.66 & 2007.423 \\
S4-465 & 17.14 & 19.81 & Unknown Age & 96 & 15 & 1.95 & 2.00 & Yes & No & 0.00 & -2.92 & -3.65 & 2015.924 \\
S4-322 & 17.15 & 19.36 & Unknown Age & 64 & 7 & 5.61 & 2.51 & Yes & No & 0.00 & 4.29 & 2.36 & 2008.324 \\
S5-184 & 17.15 & 19.49 & Unknown Age & 85 & 11 & 4.82 & 1.31 & Yes & No & 0.00 & 4.47 & 3.68 & 2007.943 \\
S0-40 & 17.16 & 19.17 & Known Young & 82 & 15 & 7.51 & 4.46 & Yes & Yes & 0.00 & -0.23 & -0.10 & 2007.193 \\
S5-323 & 17.16 & 19.41 & Unknown Age & 43 & 15 & 2.70 & 2.36 & Yes & No & 0.00 & -2.29 & -5.14 & 2015.964 \\
S2-109 & 17.17 & 19.40 & Unknown Age & 46 & 9 & 2.28 & 2.19 & No & No & 0.00 & 1.62 & 1.36 & 2008.071 \\
S5-194 & 17.17 & 19.85 & Unknown Age & 84 & 13 & 11.66 & 20.24 & Yes & Yes & 0.00 & 4.77 & 3.39 & 2006.855 \\
S2-119 & 17.19 & 19.51 & Unknown Age & 30 & 13 & 1.88 & 5.29 & No & Yes & 0.00 & 1.68 & 1.34 & 2007.655 \\
S3-64 & 17.19 & \text{---} & Unknown Age & 31 & 0 & 6.22 & \text{---} & Yes & \text{---} & 0.00 & -2.90 & -1.00 & 2007.668 \\
S7-245 & 17.19 & 19.52 & Unknown Age & 62 & 13 & 4.23 & 4.58 & Yes & Yes & 0.00 & 5.22 & -4.72 & 2016.104 \\
S2-288 & 17.19 & 19.01 & Unknown Age & 60 & 10 & 4.26 & 3.78 & Yes & No & 0.00 & 0.12 & -2.87 & 2008.656 \\
S2-315 & 17.20 & 19.82 & Unknown Age & 72 & 14 & 15.49 & 24.96 & Yes & Yes & 0.00 & -0.73 & 2.85 & 2007.563 \\
S5-135 & 17.20 & 19.33 & Unknown Age & 66 & 12 & 5.87 & 0.64 & Yes & No & 0.00 & 3.99 & -3.80 & 2007.978 \\
S4-477 & 17.20 & 19.67 & Unknown Age & 54 & 15 & 3.96 & 10.57 & Yes & Yes & 0.00 & -3.45 & 2.43 & 2019.607 \\
S3-201 & 17.20 & 19.34 & Unknown Age & 95 & 15 & 2.00 & 3.93 & Yes & No & 0.00 & -1.12 & -3.35 & 2008.154 \\
S2-130 & 17.20 & 19.48 & Unknown Age & 62 & 11 & 5.99 & 6.97 & Yes & Yes & 0.00 & -1.59 & -1.53 & 2007.595 \\
S4-108 & 17.21 & 19.55 & Unknown Age & 53 & 8 & 7.30 & 5.14 & Yes & No & 0.00 & -3.92 & -1.57 & 2008.333 \\
S5-154 & 17.21 & 19.97 & Unknown Age & 76 & 7 & 1.89 & 3.24 & No & No & 0.00 & -5.00 & -2.55 & 2007.746 \\
S3-379 & 17.22 & 19.47 & Unknown Age & 72 & 11 & 3.38 & 1.07 & Yes & No & 0.00 & 3.74 & -1.32 & 2007.363 \\
S2-173 & 17.22 & 19.57 & Unknown Age & 76 & 15 & 2.45 & 3.87 & Yes & No & 0.00 & -0.38 & 2.36 & 2007.618 \\
S6-367 & 17.23 & 19.69 & Unknown Age & 57 & 6 & 4.95 & 2.55 & Yes & No & 0.00 & -3.13 & -5.80 & 2017.737 \\
S2-191 & 17.23 & \text{---} & Unknown Age & 51 & 0 & 5.77 & \text{---} & Yes & \text{---} & 0.00 & 0.30 & 2.46 & 2007.865 \\
S5-292 & 17.24 & 19.59 & Unknown Age & 91 & 15 & 2.41 & 6.79 & Yes & Yes & 0.00 & 0.86 & -5.71 & 2016.148 \\
S5-37 & 17.25 & 19.36 & Unknown Age & 52 & 8 & 2.97 & 3.00 & Yes & No & 0.00 & 5.00 & 1.19 & 2007.485 \\
S4-39 & 17.25 & 19.59 & Unknown Age & 44 & 5 & 2.61 & 3.01 & Yes & No & 0.00 & 3.69 & 1.82 & 2007.162 \\
S3-332 & 17.25 & 19.34 & Unknown Age & 33 & 5 & 7.59 & 3.34 & Yes & No & 0.00 & 0.78 & -3.77 & 2007.360 \\
S5-293 & 17.26 & 19.41 & Unknown Age & 87 & 15 & 6.65 & 5.93 & Yes & Yes & 0.00 & -1.44 & -5.04 & 2016.501 \\
S0-75 & 17.26 & 19.19 & Unknown Age & 59 & 13 & 2.33 & 4.28 & Yes & No & 0.00 & -0.14 & -0.73 & 2008.744 \\
S4-363 & 17.26 & 20.07 & Unknown Age & 72 & 7 & 3.16 & 4.76 & Yes & No & 0.00 & -4.98 & -0.52 & 2007.392 \\
S4-49 & 17.26 & 19.95 & Unknown Age & 82 & 14 & 4.99 & 4.86 & Yes & Yes & 0.00 & -4.11 & 0.41 & 2007.707 \\
S4-120 & 17.27 & \text{---} & Unknown Age & 33 & 0 & 6.03 & \text{---} & Yes & \text{---} & 0.00 & 1.18 & 4.10 & 2007.690 \\
S5-169 & 17.27 & 19.52 & Unknown Age & 60 & 10 & 4.48 & 7.01 & Yes & Yes & 0.00 & 4.84 & 3.00 & 2007.975 \\
S4-309 & 17.27 & 19.45 & Unknown Age & 39 & 7 & 3.70 & 1.21 & Yes & No & 0.00 & 4.76 & 0.93 & 2007.555 \\
S2-301 & 17.27 & 19.83 & Unknown Age & 74 & 15 & 4.51 & 8.70 & Yes & Yes & 0.00 & -2.30 & 1.75 & 2008.276 \\
S3-194 & 17.27 & 19.60 & Unknown Age & 82 & 15 & 2.67 & 1.56 & Yes & No & 0.00 & 2.12 & 2.79 & 2007.719 \\
S5-179 & 17.28 & 19.54 & Unknown Age & 63 & 11 & 3.54 & 2.53 & Yes & No & 0.00 & 3.86 & -4.24 & 2007.747 \\
S5-309 & 17.28 & \text{---} & Unknown Age & 60 & 0 & 9.50 & \text{---} & Yes & \text{---} & 0.00 & -1.83 & -5.43 & 2015.499 \\
S3-324 & 17.28 & \text{---} & Unknown Age & 52 & 0 & 6.99 & \text{---} & Yes & \text{---} & 0.00 & 3.55 & 1.47 & 2007.934 \\
S4-101 & 17.29 & 19.01 & Unknown Age & 70 & 10 & 1.82 & 3.49 & No & No & 0.00 & 1.52 & 3.94 & 2008.144 \\
S5-295 & 17.30 & \text{---} & Unknown Age & 81 & 0 & 11.75 & \text{---} & Yes & \text{---} & 0.00 & -4.91 & 2.71 & 2016.278 \\
S5-304 & 17.30 & 19.70 & Unknown Age & 71 & 6 & 61.77 & 23.77 & Yes & Yes & 0.00 & 5.11 & -1.20 & 2016.044 \\
S1-94 & 17.30 & 19.38 & Unknown Age & 74 & 14 & 2.69 & 2.73 & Yes & No & 0.00 & -0.98 & -0.80 & 2007.982 \\
S4-78 & 17.31 & 20.56 & Unknown Age & 78 & 6 & 16.49 & 31.10 & Yes & Yes & 0.00 & -4.03 & -1.05 & 2007.642 \\
S7-243 & 17.32 & 19.65 & Unknown Age & 77 & 9 & 4.39 & 2.79 & Yes & No & 0.00 & 5.06 & -5.20 & 2015.826 \\
S1-81 & 17.34 & 19.47 & Unknown Age & 33 & 9 & 4.42 & 47.11 & Yes & Yes & 0.00 & -0.88 & -0.79 & 2007.536 \\
S2-135 & 17.34 & 19.75 & Unknown Age & 72 & 14 & 4.41 & 4.10 & Yes & No & 0.00 & 1.49 & 1.64 & 2007.395 \\
S4-324 & 17.35 & 19.37 & Unknown Age & 91 & 15 & 2.26 & 0.57 & Yes & No & 0.00 & 4.90 & -0.14 & 2007.918 \\
S3-440 & 17.35 & 19.64 & Unknown Age & 91 & 15 & 13.66 & 9.46 & Yes & Yes & 0.00 & -0.81 & -3.88 & 2016.072 \\
S6-373 & 17.36 & \text{---} & Unknown Age & 52 & 0 & 1.75 & \text{---} & No & \text{---} & 0.00 & 1.42 & -6.32 & 2016.566 \\
S5-320 & 17.36 & \text{---} & Unknown Age & 49 & 0 & 5.29 & \text{---} & Yes & \text{---} & 0.00 & -0.17 & -5.59 & 2015.209 \\
S1-148 & 17.37 & 19.45 & Unknown Age & 35 & 12 & 2.74 & 2.66 & Yes & No & 0.00 & -0.34 & -1.85 & 2008.438 \\
S1-95 & 17.38 & 19.44 & Unknown Age & 76 & 15 & 2.66 & 4.96 & Yes & Yes & 0.00 & -1.23 & 0.27 & 2007.640 \\
S2-291 & 17.38 & 19.60 & Unknown Age & 89 & 15 & 1.26 & 0.97 & No & No & 0.00 & 2.04 & 2.04 & 2007.858 \\
S6-346 & 17.39 & 19.59 & Unknown Age & 91 & 15 & 1.42 & 1.85 & No & No & 0.00 & 3.85 & -5.10 & 2016.189 \\
S4-33 & 17.41 & 19.63 & Unknown Age & 62 & 14 & 2.78 & 1.36 & Yes & No & 0.00 & 3.61 & 1.93 & 2007.687 \\
S5-326 & 17.41 & 19.64 & Unknown Age & 39 & 15 & 2.29 & 5.79 & No & Yes & 0.00 & -1.60 & -5.19 & 2016.007 \\
S0-106 & 17.42 & 19.42 & Unknown Age & 42 & 11 & 3.69 & 2.46 & Yes & No & 0.00 & -0.20 & 0.23 & 2011.642 \\
S5-42 & 17.42 & 20.23 & Unknown Age & 60 & 13 & 22.64 & 6.29 & Yes & Yes & 0.00 & 2.69 & -4.36 & 2008.117 \\
S2-265 & 17.42 & 19.34 & Unknown Age & 52 & 15 & 2.92 & 8.39 & Yes & Yes & 0.00 & 2.26 & 1.65 & 2007.724 \\
S6-347 & 17.43 & 19.55 & Unknown Age & 90 & 15 & 6.50 & 5.23 & Yes & Yes & 0.00 & 4.73 & -4.70 & 2016.276 \\
S6-376 & 17.45 & \text{---} & Unknown Age & 48 & 0 & 6.14 & \text{---} & Yes & \text{---} & 0.00 & -2.81 & -6.30 & 2015.478 \\
S4-204 & 17.45 & 20.06 & Unknown Age & 93 & 13 & 5.85 & 7.13 & Yes & Yes & 0.00 & -3.15 & 3.27 & 2007.375 \\
S3-242 & 17.46 & 20.13 & Unknown Age & 78 & 7 & 7.07 & 3.10 & Yes & No & 0.00 & -3.04 & 1.95 & 2007.782 \\
S4-200 & 17.46 & 19.49 & Unknown Age & 95 & 15 & 7.60 & 0.82 & Yes & No & 0.00 & 4.40 & -1.10 & 2007.936 \\
S6-378 & 17.48 & 19.35 & Unknown Age & 46 & 7 & 3.85 & 5.26 & Yes & No & 0.00 & 4.82 & -4.20 & 2014.504 \\
S4-32 & 17.49 & 20.07 & Unknown Age & 69 & 13 & 2.96 & 3.22 & Yes & No & 0.00 & -2.31 & 3.36 & 2007.863 \\
S3-45 & 17.49 & 20.21 & Unknown Age & 57 & 13 & 2.96 & 5.96 & Yes & Yes & 0.00 & -2.10 & 2.16 & 2008.003 \\
S0-60 & 17.50 & 19.73 & Unknown Age & 92 & 14 & 3.93 & 1.81 & Yes & No & 0.00 & -0.48 & -0.12 & 2007.783 \\
S0-63 & 17.50 & 20.03 & Unknown Age & 93 & 14 & 4.96 & 9.60 & Yes & Yes & 0.00 & -0.45 & -0.28 & 2008.270 \\
S5-108 & 17.50 & \text{---} & Unknown Age & 71 & 0 & 2.43 & \text{---} & Yes & \text{---} & 0.00 & 4.03 & -3.57 & 2007.201 \\
S4-148 & 17.50 & 20.50 & Unknown Age & 47 & 8 & 4.83 & 12.34 & Yes & Yes & 0.00 & -3.79 & 2.14 & 2007.837 \\
S3-298 & 17.51 & 19.78 & Unknown Age & 90 & 14 & 4.72 & 1.65 & Yes & No & 0.00 & 2.92 & 2.40 & 2007.984 \\
S6-387 & 17.52 & 19.79 & Unknown Age & 34 & 10 & 2.70 & 2.93 & Yes & No & 0.00 & 5.49 & -4.11 & 2017.243 \\
S6-360 & 17.52 & 20.04 & Unknown Age & 64 & 5 & 4.19 & 3.87 & Yes & No & 0.00 & -5.08 & 3.42 & 2015.069 \\
S4-110 & 17.52 & \text{---} & Unknown Age & 42 & 0 & 2.24 & \text{---} & No & \text{---} & 0.00 & -1.22 & 4.05 & 2007.266 \\
S3-277 & 17.52 & 19.62 & Unknown Age & 82 & 14 & 8.44 & 5.19 & Yes & Yes & 0.00 & -2.08 & -3.08 & 2007.800 \\
S2-297 & 17.52 & 19.75 & Unknown Age & 87 & 12 & 1.51 & 2.11 & No & No & 0.00 & -1.06 & -2.70 & 2006.906 \\
S4-488 & 17.52 & 19.50 & Unknown Age & 40 & 10 & 1.16 & 0.41 & No & No & 0.00 & 4.05 & -1.53 & 2016.508 \\
S5-325 & 17.53 & 19.93 & Unknown Age & 40 & 6 & 3.03 & 6.50 & Yes & No & 0.00 & 5.62 & -1.80 & 2018.108 \\
S6-349 & 17.53 & 19.83 & Unknown Age & 85 & 14 & 7.44 & 4.43 & Yes & Yes & 0.00 & 3.45 & -5.78 & 2016.241 \\
S6-13 & 17.53 & \text{---} & Unknown Age & 42 & 0 & 3.76 & \text{---} & Yes & \text{---} & 0.00 & 4.23 & -4.41 & 2008.208 \\
S4-235 & 17.53 & 19.86 & Unknown Age & 84 & 13 & 3.69 & 6.53 & Yes & Yes & 0.00 & 4.32 & -1.66 & 2007.759 \\
S4-298 & 17.53 & 19.60 & Unknown Age & 87 & 15 & 3.52 & 1.42 & Yes & No & 0.00 & 4.82 & -0.11 & 2007.635 \\
S4-484 & 17.54 & \text{---} & Unknown Age & 42 & 0 & 3.10 & \text{---} & Yes & \text{---} & 0.00 & 1.03 & -4.25 & 2016.029 \\
S6-359 & 17.54 & 19.60 & Unknown Age & 66 & 13 & 3.37 & 4.67 & Yes & Yes & 0.00 & -3.36 & -5.34 & 2015.878 \\
S4-43 & 17.54 & 19.91 & Unknown Age & 65 & 14 & 2.25 & 1.35 & Yes & No & 0.00 & 1.68 & -3.77 & 2007.913 \\
S5-172 & 17.55 & 20.30 & Unknown Age & 89 & 9 & 3.88 & 7.61 & Yes & Yes & 0.00 & 5.30 & 2.13 & 2007.201 \\
S1-152 & 17.56 & 20.09 & Unknown Age & 52 & 11 & 5.42 & 31.24 & Yes & Yes & 0.00 & 1.09 & 1.55 & 2006.887 \\
S7-251 & 17.57 & \text{---} & Unknown Age & 39 & 0 & 11.41 & \text{---} & Yes & \text{---} & 0.00 & -4.87 & -5.23 & 2014.384 \\
S5-171 & 17.57 & \text{---} & Unknown Age & 34 & 0 & 5.03 & \text{---} & Yes & \text{---} & 0.00 & 4.10 & -3.96 & 2008.818 \\
S5-329 & 17.57 & 19.63 & Unknown Age & 39 & 11 & 3.15 & 2.52 & Yes & No & 0.00 & 0.26 & -5.26 & 2019.583 \\
S6-361 & 17.57 & \text{---} & Unknown Age & 64 & 0 & 3.35 & \text{---} & Yes & \text{---} & 0.00 & -5.06 & 3.53 & 2015.108 \\
S6-356 & 17.58 & 19.72 & Unknown Age & 70 & 11 & 2.80 & 3.23 & Yes & No & 0.00 & 5.48 & -3.86 & 2017.003 \\
S6-370 & 17.58 & 20.13 & Unknown Age & 54 & 5 & 3.74 & 33.64 & Yes & Yes & 0.00 & -3.16 & -5.93 & 2016.618 \\
S2-260 & 17.58 & \text{---} & Unknown Age & 34 & 0 & 3.89 & \text{---} & Yes & \text{---} & 0.00 & -2.37 & 1.48 & 2007.551 \\
S2-90 & 17.59 & 19.88 & Unknown Age & 35 & 5 & 4.90 & 0.90 & Yes & No & 0.00 & -1.32 & -1.51 & 2007.507 \\
S4-291 & 17.60 & 19.86 & Unknown Age & 94 & 15 & 3.68 & 8.59 & Yes & Yes & 0.00 & 4.40 & -1.91 & 2007.966 \\
S2-231 & 17.61 & 19.96 & Unknown Age & 77 & 14 & 4.51 & 2.54 & Yes & No & 0.00 & -2.58 & -0.63 & 2008.033 \\
S5-16 & 17.62 & 19.92 & Unknown Age & 79 & 9 & 2.49 & 6.52 & Yes & Yes & 0.00 & 3.33 & 3.81 & 2007.908 \\
S6-369 & 17.62 & 19.74 & Unknown Age & 56 & 10 & 5.78 & 6.34 & Yes & Yes & 0.00 & 3.60 & -5.78 & 2015.502 \\
S1-149 & 17.62 & \text{---} & Unknown Age & 44 & 0 & 2.19 & \text{---} & No & \text{---} & 0.00 & -1.65 & -0.91 & 2007.869 \\
S5-195 & 17.62 & 19.84 & Unknown Age & 63 & 9 & 4.62 & 2.68 & Yes & No & 0.00 & 3.88 & -4.37 & 2008.161 \\
S4-338 & 17.63 & 19.99 & Unknown Age & 92 & 14 & 2.09 & 2.09 & Yes & No & 0.00 & 3.46 & -3.49 & 2007.765 \\
S4-476 & 17.64 & \text{---} & Unknown Age & 55 & 0 & 2.19 & \text{---} & No & \text{---} & 0.00 & 0.52 & -4.35 & 2016.574 \\
S7-241 & 17.64 & 19.95 & Unknown Age & 84 & 15 & 4.00 & 9.31 & Yes & Yes & 0.00 & 4.43 & -5.80 & 2016.334 \\
S3-234 & 17.65 & 20.28 & Unknown Age & 76 & 11 & 6.43 & 4.34 & Yes & No & 0.00 & -3.52 & 0.86 & 2007.533 \\
S3-252 & 17.66 & 19.67 & Unknown Age & 42 & 12 & 2.66 & 2.90 & Yes & No & 0.00 & 2.74 & 2.41 & 2007.715 \\
S5-294 & 17.66 & 19.98 & Unknown Age & 83 & 15 & 4.03 & 4.80 & Yes & Yes & 0.00 & 0.58 & -5.30 & 2016.154 \\
S1-164 & 17.66 & 19.85 & Unknown Age & 75 & 12 & 2.00 & 1.75 & No & No & 0.00 & -1.98 & -0.01 & 2007.890 \\
S6-358 & 17.67 & 19.88 & Unknown Age & 69 & 13 & 3.94 & 5.48 & Yes & Yes & 0.00 & -3.07 & -5.24 & 2016.533 \\
S6-368 & 17.67 & 20.08 & Unknown Age & 56 & 10 & 8.53 & 13.68 & Yes & Yes & 0.00 & -3.05 & -5.65 & 2016.663 \\
S4-150 & 17.68 & 20.28 & Unknown Age & 82 & 9 & 11.53 & 23.62 & Yes & Yes & 0.00 & -2.95 & -3.24 & 2007.685 \\
S2-142 & 17.68 & 20.04 & Unknown Age & 33 & 13 & 5.57 & 5.70 & Yes & Yes & 0.00 & -2.16 & -0.63 & 2007.754 \\
S6-371 & 17.69 & \text{---} & Unknown Age & 53 & 0 & 4.30 & \text{---} & Yes & \text{---} & 0.00 & -4.68 & 3.92 & 2014.386 \\
S5-332 & 17.69 & 19.93 & Unknown Age & 37 & 6 & 6.08 & 7.70 & Yes & Yes & 0.00 & 5.54 & -0.44 & 2018.690 \\
S3-342 & 17.69 & 20.08 & Unknown Age & 90 & 14 & 1.77 & 2.25 & No & No & 0.00 & 1.59 & 3.55 & 2008.229 \\
S3-53 & 17.70 & 20.07 & Unknown Age & 39 & 8 & 3.89 & 14.33 & Yes & Yes & 0.00 & 2.99 & -0.54 & 2008.317 \\
S4-127 & 17.70 & 19.88 & Unknown Age & 40 & 10 & 4.39 & 7.13 & Yes & Yes & 0.00 & 4.14 & -1.21 & 2008.367 \\
S5-207 & 17.71 & 20.14 & Unknown Age & 92 & 14 & 1.47 & 5.26 & No & Yes & 0.00 & 4.88 & 3.35 & 2007.009 \\
S2-193 & 17.71 & 19.91 & Unknown Age & 58 & 15 & 2.40 & 5.08 & Yes & Yes & 0.00 & -2.22 & -1.13 & 2007.408 \\
S4-472 & 17.73 & 19.99 & Unknown Age & 71 & 9 & 3.11 & 5.77 & Yes & Yes & 0.00 & -1.55 & -4.42 & 2016.088 \\
S4-89 & 17.73 & 20.06 & Unknown Age & 47 & 6 & 9.98 & 15.16 & Yes & Yes & 0.00 & 3.18 & 2.73 & 2006.912 \\
S5-53 & 17.74 & 20.52 & Unknown Age & 67 & 8 & 11.23 & 26.50 & Yes & Yes & 0.00 & -3.63 & -3.70 & 2008.423 \\
S4-478 & 17.74 & 20.18 & Unknown Age & 52 & 8 & 3.30 & 2.06 & Yes & No & 0.00 & 1.39 & -4.65 & 2014.184 \\
S4-194 & 17.75 & 20.07 & Unknown Age & 66 & 11 & 4.98 & 12.01 & Yes & Yes & 0.00 & 4.26 & 1.50 & 2007.762 \\
S2-91 & 17.75 & 19.99 & Unknown Age & 55 & 9 & 1.72 & 0.88 & No & No & 0.00 & -1.95 & -0.49 & 2007.639 \\
S5-317 & 17.75 & 19.52 & Unknown Age & 52 & 15 & 5.12 & 1.74 & Yes & No & 0.00 & 1.41 & -5.83 & 2015.498 \\
S4-470 & 17.76 & 19.97 & Unknown Age & 77 & 15 & 4.80 & 1.75 & Yes & No & 0.00 & 0.45 & -4.73 & 2016.820 \\
S3-293 & 17.76 & 19.60 & Unknown Age & 94 & 11 & 6.27 & 3.71 & Yes & No & 0.00 & 2.25 & 3.03 & 2007.629 \\
S4-485 & 17.76 & 19.93 & Unknown Age & 41 & 6 & 5.94 & 5.98 & Yes & No & 0.00 & -0.53 & -4.56 & 2014.603 \\
S7-244 & 17.77 & 19.69 & Unknown Age & 64 & 10 & 2.46 & 11.95 & Yes & Yes & 0.00 & 4.57 & -5.73 & 2016.092 \\
S4-260 & 17.78 & 20.47 & Unknown Age & 36 & 7 & 3.81 & 4.35 & Yes & No & 0.00 & -4.67 & 0.24 & 2006.715 \\
S3-158 & 17.78 & 19.48 & Unknown Age & 78 & 15 & 2.43 & 2.02 & Yes & No & 0.00 & 0.95 & 3.26 & 2008.199 \\
S6-380 & 17.79 & \text{---} & Unknown Age & 44 & 0 & 6.25 & \text{---} & Yes & \text{---} & 0.00 & -2.29 & -5.76 & 2017.191 \\
S1-77 & 17.79 & 19.94 & Unknown Age & 32 & 12 & 3.22 & 1.27 & Yes & No & 0.00 & -1.00 & 0.51 & 2006.440 \\
S6-375 & 17.80 & 19.93 & Unknown Age & 51 & 10 & 2.22 & 3.02 & No & No & 0.00 & -3.17 & -5.69 & 2018.510 \\
S4-57 & 17.80 & 20.19 & Unknown Age & 55 & 15 & 2.12 & 1.41 & No & No & 0.00 & 3.47 & 2.25 & 2007.822 \\
S7-242 & 17.80 & 20.13 & Unknown Age & 82 & 11 & 2.85 & 3.16 & Yes & No & 0.00 & -4.82 & -5.84 & 2016.086 \\
S4-222 & 17.81 & 20.16 & Unknown Age & 51 & 15 & 2.09 & 0.97 & No & No & 0.00 & 1.97 & -4.16 & 2007.217 \\
S5-311 & 17.81 & 19.90 & Unknown Age & 57 & 10 & 3.50 & 2.02 & Yes & No & 0.00 & -0.04 & -5.18 & 2015.219 \\
S2-284 & 17.81 & 19.85 & Unknown Age & 34 & 14 & 5.13 & 2.35 & Yes & No & 0.00 & -2.80 & -0.63 & 2006.890 \\
S3-389 & 17.81 & 20.01 & Unknown Age & 59 & 5 & 3.61 & 1.41 & Yes & No & 0.00 & 3.58 & -1.74 & 2007.749 \\
S5-298 & 17.82 & 20.05 & Unknown Age & 76 & 14 & 4.11 & 1.28 & Yes & No & 0.00 & -2.52 & -4.59 & 2016.087 \\
S4-99 & 17.86 & 20.02 & Unknown Age & 93 & 15 & 2.20 & 1.40 & Yes & No & 0.00 & 3.40 & 2.51 & 2007.705 \\
S1-157 & 17.86 & 20.21 & Unknown Age & 34 & 7 & 5.45 & 6.53 & Yes & No & 0.00 & -1.56 & -1.11 & 2006.470 \\
S4-178 & 17.87 & 20.41 & Unknown Age & 94 & 14 & 4.58 & 3.09 & Yes & No & 0.00 & 3.59 & 2.69 & 2007.823 \\
S4-192 & 17.87 & 20.11 & Unknown Age & 84 & 15 & 3.68 & 3.10 & Yes & No & 0.00 & 1.70 & -4.18 & 2008.171 \\
S5-338 & 17.87 & 20.12 & Unknown Age & 34 & 15 & 1.81 & 7.95 & No & Yes & 0.00 & -2.20 & -5.54 & 2016.261 \\
S5-343 & 17.88 & 20.22 & Unknown Age & 31 & 6 & 2.88 & 8.36 & Yes & Yes & 0.00 & -4.61 & -3.53 & 2016.737 \\
S4-337 & 17.88 & 20.21 & Unknown Age & 86 & 10 & 2.66 & 2.19 & Yes & No & 0.00 & -3.34 & 3.61 & 2007.315 \\
S4-329 & 17.89 & \text{---} & Unknown Age & 48 & 0 & 5.06 & \text{---} & Yes & \text{---} & 0.00 & 2.73 & 4.09 & 2007.185 \\
S4-199 & 17.89 & 20.15 & Unknown Age & 51 & 8 & 6.93 & 6.79 & Yes & Yes & 0.00 & 4.54 & -0.09 & 2008.021 \\
S5-82 & 17.91 & 19.90 & Unknown Age & 55 & 6 & 2.25 & 4.79 & Yes & No & 0.00 & 3.96 & -3.50 & 2007.776 \\
S6-365 & 17.91 & \text{---} & Unknown Age & 58 & 0 & 3.67 & \text{---} & Yes & \text{---} & 0.00 & 4.04 & -5.03 & 2015.903 \\
S2-263 & 17.91 & 20.22 & Unknown Age & 95 & 14 & 4.81 & 10.74 & Yes & Yes & 0.00 & -2.80 & 0.15 & 2007.972 \\
S6-353 & 17.91 & 20.29 & Unknown Age & 73 & 9 & 7.35 & 8.67 & Yes & Yes & 0.00 & 4.95 & -4.52 & 2015.795 \\
S3-78 & 17.92 & \text{---} & Unknown Age & 45 & 0 & 3.75 & \text{---} & Yes & \text{---} & 0.00 & -2.08 & -2.33 & 2007.967 \\
S3-165 & 17.93 & 20.24 & Unknown Age & 37 & 8 & 5.03 & 6.26 & Yes & Yes & 0.00 & 0.78 & 3.31 & 2006.260 \\
S4-141 & 17.94 & 19.60 & Unknown Age & 81 & 15 & 2.99 & 1.94 & Yes & No & 0.00 & -4.32 & -0.60 & 2007.161 \\
S5-342 & 17.94 & \text{---} & Unknown Age & 32 & 0 & 10.20 & \text{---} & Yes & \text{---} & 0.00 & 1.82 & -4.95 & 2012.803 \\
S6-384 & 17.94 & 20.08 & Unknown Age & 36 & 6 & 1.53 & 3.35 & No & No & 0.00 & 0.41 & -6.16 & 2014.976 \\
S4-479 & 17.95 & 20.17 & Unknown Age & 52 & 10 & 7.90 & 5.73 & Yes & Yes & 0.00 & 2.34 & -3.78 & 2015.331 \\
S5-74 & 17.95 & 19.68 & Unknown Age & 48 & 6 & 3.02 & 1.36 & Yes & No & 0.00 & 4.02 & -3.36 & 2008.317 \\
S1-177 & 17.95 & \text{---} & Unknown Age & 41 & 0 & 8.47 & \text{---} & Yes & \text{---} & 0.00 & -1.31 & -0.96 & 2015.119 \\
S6-362 & 17.96 & 19.96 & Unknown Age & 64 & 8 & 1.94 & 2.72 & No & No & 0.00 & 4.45 & -4.83 & 2016.152 \\
S2-285 & 17.97 & \text{---} & Unknown Age & 35 & 0 & 3.76 & \text{---} & Yes & \text{---} & 0.00 & -2.04 & -2.02 & 2007.312 \\
S5-318 & 17.97 & 20.58 & Unknown Age & 50 & 11 & 4.21 & 6.68 & Yes & Yes & 0.00 & -4.43 & -3.35 & 2018.802 \\
S2-312 & 17.97 & 20.30 & Unknown Age & 46 & 10 & 3.15 & 12.25 & Yes & Yes & 0.00 & -2.54 & 1.47 & 2007.991 \\
S3-396 & 17.98 & 20.01 & Unknown Age & 72 & 6 & 1.80 & 3.54 & No & No & 0.00 & 0.94 & 3.89 & 2007.805 \\
S3-442 & 17.98 & 20.15 & Unknown Age & 60 & 9 & 7.83 & 2.51 & Yes & No & 0.00 & 0.49 & 2.98 & 2016.871 \\
S4-300 & 17.99 & 19.86 & Unknown Age & 81 & 12 & 4.43 & 2.44 & Yes & No & 0.00 & 4.67 & -1.21 & 2007.929 \\
S4-286 & 17.99 & 20.20 & Unknown Age & 83 & 14 & 3.37 & 2.85 & Yes & No & 0.00 & 4.77 & -0.35 & 2008.015 \\
S4-497 & 17.99 & \text{---} & Unknown Age & 31 & 0 & 12.12 & \text{---} & Yes & \text{---} & 0.00 & 3.11 & 2.57 & 2014.447 \\
S5-164 & 17.99 & 20.18 & Unknown Age & 77 & 12 & 1.53 & 1.62 & No & No & 0.00 & 4.66 & 3.22 & 2006.980 \\
S4-27 & 17.99 & 20.35 & Unknown Age & 88 & 5 & 14.68 & 4.52 & Yes & No & 0.00 & 2.73 & 3.04 & 2007.630 \\
S6-364 & 18.00 & 20.22 & Unknown Age & 60 & 13 & 2.62 & 2.69 & Yes & No & 0.00 & -4.53 & -5.15 & 2016.937 \\
S3-204 & 18.00 & 20.26 & Unknown Age & 92 & 13 & 3.77 & 1.73 & Yes & No & 0.00 & 2.45 & 2.56 & 2007.807 \\
S3-218 & 18.00 & 20.12 & Unknown Age & 30 & 12 & 2.17 & 1.37 & No & No & 0.00 & 2.92 & 2.07 & 2008.283 \\
S3-224 & 18.00 & 20.01 & Unknown Age & 89 & 15 & 2.14 & 1.81 & Yes & No & 0.00 & -2.86 & 2.16 & 2007.901 \\
S5-333 & 18.00 & 20.66 & Unknown Age & 36 & 5 & 5.13 & 1.13 & Yes & No & 0.00 & 2.62 & -4.84 & 2015.764 \\
S3-110 & 18.01 & 20.10 & Unknown Age & 53 & 15 & 2.66 & 1.38 & Yes & No & 0.00 & -2.09 & 2.46 & 2007.287 \\
S2-266 & 18.02 & 20.11 & Unknown Age & 34 & 6 & 7.81 & 6.59 & Yes & No & 0.00 & -0.79 & -2.70 & 2007.856 \\
S6-379 & 18.02 & 20.40 & Unknown Age & 45 & 10 & 3.45 & 4.67 & Yes & No & 0.00 & -4.23 & -5.41 & 2016.400 \\
S2-168 & 18.02 & 20.26 & Unknown Age & 56 & 11 & 2.62 & 0.98 & Yes & No & 0.00 & -2.33 & 0.31 & 2007.709 \\
S1-88 & 18.03 & 20.34 & Unknown Age & 40 & 11 & 3.75 & 5.55 & Yes & Yes & 0.00 & -0.43 & -1.18 & 2006.691 \\
S7-249 & 18.03 & \text{---} & Unknown Age & 41 & 0 & 3.32 & \text{---} & Yes & \text{---} & 0.00 & -5.03 & -5.06 & 2014.142 \\
S5-319 & 18.03 & 20.12 & Unknown Age & 49 & 14 & 2.98 & 2.61 & Yes & No & 0.00 & 1.34 & -5.35 & 2016.238 \\
S6-372 & 18.03 & 20.13 & Unknown Age & 52 & 15 & 3.12 & 1.61 & Yes & No & 0.00 & 4.17 & -5.52 & 2015.989 \\
S3-214 & 18.04 & \text{---} & Unknown Age & 38 & 0 & 6.58 & \text{---} & Yes & \text{---} & 0.00 & -1.88 & -3.04 & 2007.960 \\
S3-74 & 18.04 & \text{---} & Unknown Age & 59 & 0 & 9.34 & \text{---} & Yes & \text{---} & 0.00 & -3.09 & 0.02 & 2007.971 \\
S4-489 & 18.04 & 20.25 & Unknown Age & 40 & 5 & 7.75 & 2.84 & Yes & No & 0.00 & -0.05 & -4.79 & 2018.370 \\
S5-104 & 18.04 & \text{---} & Unknown Age & 61 & 0 & 17.32 & \text{---} & Yes & \text{---} & 0.00 & -3.71 & 3.87 & 2007.630 \\
S3-444 & 18.04 & 20.36 & Unknown Age & 41 & 8 & 3.61 & 3.76 & Yes & No & 0.00 & -1.66 & -3.45 & 2015.710 \\
S7-253 & 18.05 & \text{---} & Unknown Age & 30 & 0 & 2.47 & \text{---} & No & \text{---} & 0.00 & -4.80 & -6.30 & 2015.269 \\
S5-32 & 18.05 & \text{---} & Unknown Age & 60 & 0 & 3.97 & \text{---} & Yes & \text{---} & 0.00 & 3.28 & 3.93 & 2007.549 \\
S1-96 & 18.05 & 20.24 & Unknown Age & 36 & 11 & 3.55 & 2.08 & Yes & No & 0.00 & -0.06 & -1.28 & 2007.777 \\
S4-333 & 18.05 & 20.29 & Unknown Age & 54 & 6 & 6.42 & 5.07 & Yes & No & 0.00 & -2.99 & 3.88 & 2007.821 \\
S4-70 & 18.07 & \text{---} & Unknown Age & 32 & 0 & 8.51 & \text{---} & Yes & \text{---} & 0.00 & -2.37 & 3.38 & 2007.644 \\
S5-201 & 18.07 & \text{---} & Unknown Age & 44 & 0 & 6.51 & \text{---} & Yes & \text{---} & 0.00 & 5.06 & 2.98 & 2007.640 \\
S4-496 & 18.08 & 20.26 & Unknown Age & 31 & 8 & 10.50 & 15.10 & Yes & Yes & 0.00 & -1.98 & -4.12 & 2020.693 \\
S7-247 & 18.08 & \text{---} & Unknown Age & 44 & 0 & 2.48 & \text{---} & Yes & \text{---} & 0.00 & 3.65 & -6.33 & 2018.079 \\
S5-315 & 18.09 & 20.29 & Unknown Age & 53 & 7 & 1.66 & 3.73 & No & No & 0.00 & 3.83 & -4.24 & 2016.773 \\
S4-361 & 18.10 & \text{---} & Unknown Age & 59 & 0 & 3.95 & \text{---} & Yes & \text{---} & 0.00 & 4.57 & -2.04 & 2007.296 \\
S5-301 & 18.11 & 20.47 & Unknown Age & 72 & 12 & 3.50 & 2.07 & Yes & No & 0.00 & 5.09 & -0.41 & 2016.410 \\
S3-226 & 18.11 & 20.78 & Unknown Age & 40 & 8 & 9.31 & 7.79 & Yes & Yes & 0.00 & -3.56 & -0.61 & 2007.832 \\
S4-270 & 18.12 & 20.59 & Unknown Age & 43 & 6 & 3.60 & 9.45 & Yes & Yes & 0.00 & -3.81 & -2.79 & 2007.590 \\
S6-383 & 18.12 & \text{---} & Unknown Age & 38 & 0 & 4.51 & \text{---} & Yes & \text{---} & 0.00 & 4.68 & -5.18 & 2014.140 \\
S3-251 & 18.12 & \text{---} & Unknown Age & 30 & 0 & 7.30 & \text{---} & Yes & \text{---} & 0.00 & 3.57 & -0.67 & 2007.970 \\
S5-62 & 18.12 & 20.24 & Unknown Age & 59 & 6 & 2.51 & 2.15 & Yes & No & 0.00 & 4.40 & -2.80 & 2008.501 \\
S2-178 & 18.13 & 20.35 & Unknown Age & 40 & 13 & 8.13 & 0.99 & Yes & No & 0.00 & -2.12 & -1.13 & 2007.750 \\
S7-246 & 18.14 & \text{---} & Unknown Age & 59 & 0 & 3.08 & \text{---} & Yes & \text{---} & 0.00 & -3.89 & -6.19 & 2015.256 \\
S3-41 & 18.17 & 20.57 & Unknown Age & 71 & 12 & 3.52 & 2.03 & Yes & No & 0.00 & -2.93 & 0.63 & 2008.562 \\
S4-491 & 18.17 & 20.79 & Unknown Age & 39 & 8 & 5.06 & 4.92 & Yes & No & 0.00 & -4.39 & 0.38 & 2016.768 \\
S5-17 & 18.17 & 20.37 & Unknown Age & 70 & 15 & 3.31 & 4.52 & Yes & Yes & 0.00 & 2.84 & -4.19 & 2007.415 \\
S4-318 & 18.18 & \text{---} & Unknown Age & 45 & 0 & 3.58 & \text{---} & Yes & \text{---} & 0.00 & -4.85 & -0.47 & 2007.749 \\
S3-280 & 18.21 & 20.54 & Unknown Age & 34 & 7 & 3.82 & 15.23 & Yes & Yes & 0.00 & -2.39 & -2.87 & 2008.086 \\
S3-443 & 18.21 & 20.27 & Unknown Age & 46 & 11 & 2.44 & 1.36 & Yes & No & 0.00 & 2.94 & -2.04 & 2018.099 \\
S5-347 & 18.22 & \text{---} & Unknown Age & 30 & 0 & 6.55 & \text{---} & Yes & \text{---} & 0.00 & 5.61 & -1.90 & 2018.862 \\
S4-473 & 18.22 & 20.18 & Unknown Age & 63 & 12 & 5.33 & 5.04 & Yes & Yes & 0.00 & -1.38 & -4.25 & 2016.025 \\
S2-330 & 18.22 & 19.41 & Unknown Age & 59 & 14 & 2.32 & 1.21 & Yes & No & 0.00 & 0.71 & 2.91 & 2007.961 \\
S5-324 & 18.23 & 20.54 & Unknown Age & 41 & 7 & 3.96 & 1.79 & Yes & No & 0.00 & 4.21 & -2.81 & 2013.913 \\
S5-77 & 18.23 & 20.71 & Unknown Age & 85 & 12 & 5.11 & 8.67 & Yes & Yes & 0.00 & 2.98 & -4.33 & 2008.150 \\
S5-310 & 18.24 & 20.66 & Unknown Age & 59 & 7 & 2.56 & 9.97 & Yes & Yes & 0.00 & 5.28 & -2.61 & 2015.906 \\
S4-214 & 18.24 & \text{---} & Unknown Age & 57 & 0 & 5.48 & \text{---} & Yes & \text{---} & 0.00 & -3.77 & 2.54 & 2007.739 \\
S6-374 & 18.25 & 20.46 & Unknown Age & 51 & 9 & 5.32 & 0.61 & Yes & No & 0.00 & 5.29 & -3.98 & 2016.255 \\
S2-350 & 18.25 & 20.56 & Unknown Age & 36 & 10 & 1.22 & 6.22 & No & Yes & 0.00 & -2.39 & -0.20 & 2019.980 \\
S5-306 & 18.26 & 20.76 & Unknown Age & 62 & 9 & 3.89 & 0.75 & Yes & No & 0.00 & 5.10 & -2.18 & 2016.068 \\
S4-136 & 18.26 & 20.31 & Unknown Age & 81 & 13 & 3.68 & 1.90 & Yes & No & 0.00 & 4.27 & -0.68 & 2007.552 \\
S5-312 & 18.27 & 20.38 & Unknown Age & 55 & 13 & 3.69 & 2.88 & Yes & No & 0.00 & 0.41 & -5.23 & 2015.612 \\
S1-176 & 18.27 & \text{---} & Unknown Age & 52 & 0 & 4.34 & \text{---} & Yes & \text{---} & 0.00 & -1.40 & -1.17 & 2015.450 \\
S4-327 & 18.28 & \text{---} & Unknown Age & 51 & 0 & 3.80 & \text{---} & Yes & \text{---} & 0.00 & -3.60 & 3.33 & 2007.484 \\
S3-361 & 18.28 & 20.57 & Unknown Age & 49 & 5 & 3.71 & 2.75 & Yes & No & 0.00 & 2.91 & 2.63 & 2007.554 \\
S4-471 & 18.29 & 20.60 & Unknown Age & 76 & 13 & 2.29 & 3.49 & Yes & No & 0.00 & -1.74 & -3.68 & 2015.575 \\
S2-239 & 18.29 & 20.32 & Unknown Age & 77 & 10 & 2.30 & 4.21 & Yes & No & 0.00 & 1.43 & 2.30 & 2007.331 \\
S4-468 & 18.29 & 20.17 & Unknown Age & 79 & 15 & 1.69 & 1.99 & No & No & 0.00 & 2.00 & -4.32 & 2016.251 \\
S0-80 & 18.29 & 20.41 & Unknown Age & 36 & 10 & 2.03 & 1.65 & No & No & 0.00 & -0.74 & 0.24 & 2007.266 \\
S4-190 & 18.30 & \text{---} & Unknown Age & 65 & 0 & 5.16 & \text{---} & Yes & \text{---} & 0.00 & 4.41 & -0.98 & 2008.773 \\
S3-373 & 18.31 & 20.68 & Unknown Age & 77 & 5 & 6.53 & 1.15 & Yes & No & 0.00 & 1.77 & 3.52 & 2008.229 \\
S5-303 & 18.31 & 20.84 & Unknown Age & 71 & 6 & 5.32 & 0.91 & Yes & No & 0.00 & 5.35 & -0.86 & 2015.548 \\
S5-302 & 18.31 & 20.45 & Unknown Age & 72 & 12 & 1.81 & 0.74 & No & No & 0.00 & 1.28 & -5.13 & 2016.427 \\
S5-339 & 18.32 & \text{---} & Unknown Age & 33 & 0 & 2.20 & \text{---} & No & \text{---} & 0.00 & 3.46 & -4.54 & 2013.266 \\
S5-299 & 18.33 & 20.94 & Unknown Age & 73 & 5 & 3.41 & 9.55 & Yes & Yes & 0.00 & -4.81 & -3.29 & 2015.877 \\
S3-448 & 18.33 & \text{---} & Unknown Age & 36 & 0 & 5.27 & \text{---} & Yes & \text{---} & 0.00 & 0.10 & 3.12 & 2019.127 \\
S4-294 & 18.33 & 20.38 & Unknown Age & 42 & 13 & 1.38 & 5.68 & No & Yes & 0.00 & 4.71 & -0.94 & 2007.718 \\
S7-252 & 18.34 & \text{---} & Unknown Age & 31 & 0 & 3.73 & \text{---} & Yes & \text{---} & 0.00 & 5.36 & -4.89 & 2019.139 \\
S2-202 & 18.34 & 20.66 & Unknown Age & 66 & 9 & 3.43 & 1.98 & Yes & No & 0.00 & -2.51 & 0.32 & 2008.137 \\
S6-42 & 18.34 & \text{---} & Unknown Age & 64 & 0 & 3.33 & \text{---} & Yes & \text{---} & 0.00 & 5.32 & 3.48 & 2008.243 \\
S3-447 & 18.36 & \text{---} & Unknown Age & 37 & 0 & 4.32 & \text{---} & Yes & \text{---} & 0.00 & -0.04 & 3.32 & 2018.059 \\
S4-354 & 18.36 & 20.59 & Unknown Age & 77 & 7 & 10.75 & 7.97 & Yes & Yes & 0.00 & 4.32 & 2.49 & 2007.407 \\
S5-321 & 18.37 & 20.71 & Unknown Age & 47 & 10 & 4.32 & 3.55 & Yes & No & 0.00 & 1.87 & -5.13 & 2016.957 \\
S4-490 & 18.37 & \text{---} & Unknown Age & 39 & 0 & 5.82 & \text{---} & Yes & \text{---} & 0.00 & -3.15 & -3.22 & 2017.075 \\
S1-146 & 18.38 & \text{---} & Unknown Age & 32 & 0 & 7.51 & \text{---} & Yes & \text{---} & 0.00 & -1.75 & -0.71 & 2007.050 \\
S5-54 & 18.39 & \text{---} & Unknown Age & 31 & 0 & 4.34 & \text{---} & Yes & \text{---} & 0.00 & -5.03 & -1.27 & 2006.994 \\
S4-58 & 18.40 & \text{---} & Unknown Age & 33 & 0 & 4.83 & \text{---} & Yes & \text{---} & 0.00 & -1.48 & 3.85 & 2008.356 \\
S4-203 & 18.40 & 20.62 & Unknown Age & 75 & 14 & 6.07 & 1.77 & Yes & No & 0.00 & 4.51 & -0.56 & 2007.180 \\
S6-386 & 18.41 & 20.45 & Unknown Age & 35 & 5 & 2.09 & 1.71 & No & No & 0.00 & 4.55 & -4.74 & 2015.016 \\
S4-248 & 18.42 & \text{---} & Unknown Age & 41 & 0 & 1.96 & \text{---} & No & \text{---} & 0.00 & 3.83 & 2.67 & 2007.825 \\
S4-486 & 18.42 & 20.73 & Unknown Age & 41 & 7 & 2.79 & 2.33 & Yes & No & 0.00 & 1.65 & -4.42 & 2016.299 \\
S4-335 & 18.44 & 20.89 & Unknown Age & 80 & 10 & 2.89 & 3.35 & Yes & No & 0.00 & 2.40 & -4.29 & 2008.294 \\
S6-366 & 18.44 & 20.39 & Unknown Age & 58 & 5 & 5.45 & 3.15 & Yes & No & 0.00 & 3.68 & -4.95 & 2016.292 \\
S3-454 & 18.45 & \text{---} & Unknown Age & 31 & 0 & 1.28 & \text{---} & No & \text{---} & 0.00 & 2.05 & 2.34 & 2015.907 \\
S3-253 & 18.45 & 20.63 & Unknown Age & 55 & 5 & 5.14 & 0.80 & Yes & No & 0.00 & -0.20 & 3.63 & 2007.262 \\
S4-205 & 18.46 & 21.12 & Unknown Age & 73 & 5 & 2.47 & 6.38 & Yes & No & 0.00 & -4.50 & -0.65 & 2007.447 \\
S2-230 & 18.46 & 20.78 & Unknown Age & 74 & 12 & 2.28 & 2.91 & Yes & No & 0.00 & -2.64 & 0.16 & 2007.897 \\
S4-480 & 18.46 & 20.63 & Unknown Age & 49 & 12 & 2.01 & 3.77 & No & No & 0.00 & -1.34 & -3.99 & 2016.418 \\
S3-231 & 18.49 & 20.22 & Unknown Age & 67 & 14 & 2.92 & 3.70 & Yes & No & 0.00 & -0.44 & 3.58 & 2008.003 \\
S2-123 & 18.51 & 20.74 & Unknown Age & 33 & 7 & 3.29 & 1.87 & Yes & No & 0.00 & -2.15 & -0.18 & 2007.940 \\
S6-354 & 18.53 & 21.03 & Unknown Age & 73 & 7 & 2.89 & 3.33 & Yes & No & 0.00 & 3.78 & -5.39 & 2015.860 \\
S6-385 & 18.55 & \text{---} & Unknown Age & 35 & 0 & 4.24 & \text{---} & Yes & \text{---} & 0.00 & -2.35 & -6.15 & 2012.730 \\
S5-307 & 18.55 & 20.50 & Unknown Age & 61 & 10 & 5.68 & 5.03 & Yes & No & 0.00 & 1.17 & -5.52 & 2016.562 \\
S3-211 & 18.55 & \text{---} & Unknown Age & 42 & 0 & 7.21 & \text{---} & Yes & \text{---} & 0.00 & -0.96 & 3.41 & 2008.258 \\
S4-293 & 18.55 & \text{---} & Unknown Age & 32 & 0 & 2.70 & \text{---} & No & \text{---} & 0.00 & 4.27 & -2.18 & 2007.530 \\
S4-495 & 18.56 & \text{---} & Unknown Age & 33 & 0 & 2.97 & \text{---} & Yes & \text{---} & 0.00 & -1.88 & -4.02 & 2013.449 \\
S5-314 & 18.56 & 20.66 & Unknown Age & 54 & 9 & 2.17 & 1.41 & No & No & 0.00 & 1.46 & -5.30 & 2015.473 \\
S5-328 & 18.58 & \text{---} & Unknown Age & 39 & 0 & 4.41 & \text{---} & Yes & \text{---} & 0.00 & 2.13 & -5.08 & 2017.292 \\
S6-388 & 18.58 & 20.65 & Unknown Age & 33 & 7 & 2.09 & 1.59 & No & No & 0.00 & 1.08 & -5.94 & 2016.708 \\
S4-482 & 18.59 & \text{---} & Unknown Age & 43 & 0 & 3.46 & \text{---} & Yes & \text{---} & 0.00 & 2.69 & 3.60 & 2016.197 \\
S3-446 & 18.59 & 20.88 & Unknown Age & 41 & 8 & 3.14 & 2.69 & Yes & No & 0.00 & -1.72 & -3.54 & 2019.551 \\
S3-445 & 18.59 & \text{---} & Unknown Age & 41 & 0 & 6.89 & \text{---} & Yes & \text{---} & 0.00 & -1.96 & -3.35 & 2013.836 \\
S3-170 & 18.59 & 20.60 & Unknown Age & 43 & 10 & 7.23 & 5.76 & Yes & Yes & 0.00 & -3.26 & 1.00 & 2008.606 \\
S4-501 & 18.60 & 21.12 & Unknown Age & 30 & 7 & 8.68 & 1.94 & Yes & No & 0.00 & -2.77 & -4.06 & 2016.955 \\
S5-308 & 18.62 & 20.51 & Unknown Age & 60 & 13 & 2.93 & 0.80 & Yes & No & 0.00 & 1.42 & -5.48 & 2016.124 \\
S4-475 & 18.63 & 20.90 & Unknown Age & 57 & 8 & 3.08 & 2.51 & Yes & No & 0.00 & -2.09 & -4.30 & 2015.891 \\
S3-244 & 18.63 & \text{---} & Unknown Age & 52 & 0 & 3.64 & \text{---} & Yes & \text{---} & 0.00 & -2.04 & 3.00 & 2007.694 \\
S5-331 & 18.64 & 20.76 & Unknown Age & 37 & 7 & 5.24 & 10.14 & Yes & Yes & 0.00 & 1.58 & -5.54 & 2017.002 \\
S5-73 & 18.64 & \text{---} & Unknown Age & 47 & 0 & 2.88 & \text{---} & Yes & \text{---} & 0.00 & -4.84 & -2.02 & 2007.155 \\
S4-500 & 18.64 & \text{---} & Unknown Age & 30 & 0 & 2.20 & \text{---} & No & \text{---} & 0.00 & -1.90 & -4.61 & 2016.582 \\
S6-377 & 18.65 & \text{---} & Unknown Age & 47 & 0 & 4.21 & \text{---} & Yes & \text{---} & 0.00 & 4.80 & -4.48 & 2014.517 \\
S5-13 & 18.65 & \text{---} & Unknown Age & 36 & 0 & 6.50 & \text{---} & Yes & \text{---} & 0.00 & -4.92 & -1.11 & 2007.696 \\
S3-311 & 18.65 & 20.29 & Unknown Age & 46 & 12 & 17.91 & 2.90 & Yes & No & 0.00 & 1.08 & 3.65 & 2007.411 \\
S4-250 & 18.65 & \text{---} & Unknown Age & 52 & 0 & 5.57 & \text{---} & Yes & \text{---} & 0.00 & -3.17 & 3.41 & 2008.123 \\
S5-188 & 18.66 & \text{---} & Unknown Age & 56 & 0 & 4.59 & \text{---} & Yes & \text{---} & 0.00 & 5.31 & 2.37 & 2007.169 \\
S3-301 & 18.67 & \text{---} & Unknown Age & 36 & 0 & 7.29 & \text{---} & Yes & \text{---} & 0.00 & -3.16 & 2.06 & 2007.793 \\
S5-337 & 18.68 & \text{---} & Unknown Age & 34 & 0 & 4.85 & \text{---} & Yes & \text{---} & 0.00 & 3.91 & -3.14 & 2013.532 \\
S2-245 & 18.69 & 21.49 & Unknown Age & 45 & 5 & 4.11 & 8.56 & Yes & No & 0.00 & -0.56 & 2.66 & 2006.948 \\
S3-206 & 18.69 & 20.59 & Unknown Age & 42 & 6 & 2.05 & 4.32 & No & No & 0.00 & -0.18 & 3.54 & 2007.710 \\
S4-351 & 18.69 & 20.57 & Unknown Age & 43 & 13 & 4.27 & 2.24 & Yes & No & 0.00 & 3.41 & -3.60 & 2007.732 \\
S4-499 & 18.71 & 20.90 & Unknown Age & 30 & 7 & 4.79 & 2.06 & Yes & No & 0.00 & -0.01 & -4.37 & 2016.785 \\
S4-493 & 18.72 & \text{---} & Unknown Age & 37 & 0 & 3.30 & \text{---} & Yes & \text{---} & 0.00 & -2.20 & -4.33 & 2015.283 \\
S5-341 & 18.72 & \text{---} & Unknown Age & 32 & 0 & 2.54 & \text{---} & No & \text{---} & 0.00 & -4.86 & -2.56 & 2015.004 \\
S7-248 & 18.73 & 21.07 & Unknown Age & 42 & 5 & 1.67 & 4.40 & No & No & 0.00 & -4.49 & -5.78 & 2015.608 \\
S5-327 & 18.73 & 20.62 & Unknown Age & 39 & 6 & 1.71 & 6.87 & No & No & 0.00 & 1.32 & -5.59 & 2017.260 \\
S5-336 & 18.73 & \text{---} & Unknown Age & 34 & 0 & 6.35 & \text{---} & Yes & \text{---} & 0.00 & 0.93 & -5.92 & 2018.448 \\
S5-335 & 18.73 & \text{---} & Unknown Age & 34 & 0 & 3.78 & \text{---} & Yes & \text{---} & 0.00 & -4.56 & 3.77 & 2015.320 \\
S4-163 & 18.73 & \text{---} & Unknown Age & 72 & 0 & 3.68 & \text{---} & Yes & \text{---} & 0.00 & 3.30 & 2.96 & 2008.290 \\
S6-389 & 18.74 & 20.76 & Unknown Age & 32 & 10 & 1.59 & 2.54 & No & No & 0.00 & 3.97 & -5.31 & 2015.842 \\
S6-382 & 18.74 & \text{---} & Unknown Age & 39 & 0 & 2.13 & \text{---} & No & \text{---} & 0.00 & 3.76 & -5.27 & 2019.327 \\
S3-453 & 18.75 & \text{---} & Unknown Age & 31 & 0 & 6.05 & \text{---} & Yes & \text{---} & 0.00 & -3.26 & 0.85 & 2017.142 \\
S4-41 & 18.76 & 20.47 & Unknown Age & 60 & 6 & 1.79 & 3.51 & No & No & 0.00 & 1.57 & 3.81 & 2007.825 \\
S4-481 & 18.77 & 20.97 & Unknown Age & 45 & 11 & 3.82 & 3.11 & Yes & No & 0.00 & -2.07 & -3.74 & 2016.370 \\
S5-313 & 18.78 & 21.00 & Unknown Age & 54 & 8 & 2.97 & 1.43 & Yes & No & 0.00 & 5.13 & -1.46 & 2016.319 \\
S2-163 & 18.79 & 20.49 & Unknown Age & 50 & 13 & 7.55 & 3.16 & Yes & No & 0.00 & -2.28 & -0.42 & 2006.992 \\
S3-441 & 18.79 & 21.04 & Unknown Age & 63 & 6 & 3.67 & 2.17 & Yes & No & 0.00 & 2.25 & 2.46 & 2016.072 \\
S2-349 & 18.80 & 21.26 & Unknown Age & 44 & 6 & 3.06 & 12.57 & Yes & Yes & 0.00 & -0.63 & 2.81 & 2018.247 \\
S4-151 & 18.81 & \text{---} & Unknown Age & 47 & 0 & 4.72 & \text{---} & Yes & \text{---} & 0.00 & -3.00 & 3.17 & 2007.699 \\
S6-381 & 18.82 & \text{---} & Unknown Age & 41 & 0 & 6.76 & \text{---} & Yes & \text{---} & 0.00 & 4.01 & -5.62 & 2013.928 \\
S5-100 & 18.83 & \text{---} & Unknown Age & 46 & 0 & 4.74 & \text{---} & Yes & \text{---} & 0.00 & 3.53 & -4.02 & 2008.669 \\
S3-210 & 18.84 & \text{---} & Unknown Age & 40 & 0 & 7.58 & \text{---} & Yes & \text{---} & 0.00 & 1.72 & 3.10 & 2007.865 \\
S4-474 & 18.87 & 21.20 & Unknown Age & 60 & 5 & 5.12 & 1.96 & Yes & No & 0.00 & 4.89 & -0.98 & 2015.759 \\
S7-250 & 18.87 & 21.08 & Unknown Age & 40 & 5 & 6.24 & 4.78 & Yes & No & 0.00 & 3.85 & -5.98 & 2014.230 \\
S3-336 & 18.89 & \text{---} & Unknown Age & 31 & 0 & 10.13 & \text{---} & Yes & \text{---} & 0.00 & 2.70 & 2.76 & 2008.486 \\
S5-316 & 18.90 & \text{---} & Unknown Age & 53 & 0 & 3.83 & \text{---} & Yes & \text{---} & 0.00 & 2.15 & -4.62 & 2015.298 \\
S3-177 & 18.92 & 20.86 & Unknown Age & 51 & 9 & 2.37 & 2.83 & Yes & No & 0.00 & -0.60 & 3.39 & 2007.621 \\
S5-0 & 18.93 & 20.84 & Unknown Age & 58 & 8 & 3.30 & 0.60 & Yes & No & 0.00 & 4.30 & 2.58 & 2008.012 \\
S5-334 & 18.95 & \text{---} & Unknown Age & 34 & 0 & 2.37 & \text{---} & No & \text{---} & 0.00 & -2.26 & -5.54 & 2014.586 \\
S3-228 & 19.02 & \text{---} & Unknown Age & 45 & 0 & 3.09 & \text{---} & Yes & \text{---} & 0.00 & -3.60 & -0.11 & 2007.941 \\
S3-321 & 19.03 & \text{---} & Unknown Age & 55 & 0 & 2.50 & \text{---} & Yes & \text{---} & 0.00 & 1.38 & 3.57 & 2008.127 \\
S4-483 & 19.04 & 21.08 & Unknown Age & 43 & 6 & 4.12 & 4.35 & Yes & No & 0.00 & -2.19 & -4.18 & 2015.382 \\
S3-325 & 19.06 & 21.14 & Unknown Age & 31 & 5 & 3.17 & 1.59 & Yes & No & 0.00 & 2.88 & 2.55 & 2007.666 \\
S3-452 & 19.07 & \text{---} & Unknown Age & 32 & 0 & 3.77 & \text{---} & Yes & \text{---} & 0.00 & -3.23 & 1.96 & 2015.644 \\
S5-45 & 19.07 & \text{---} & Unknown Age & 33 & 0 & 3.94 & \text{---} & Yes & \text{---} & 0.00 & 4.32 & 2.82 & 2008.084 \\
S5-87 & 19.10 & \text{---} & Unknown Age & 66 & 0 & 6.08 & \text{---} & Yes & \text{---} & 0.00 & 4.70 & 2.50 & 2007.733 \\
S4-348 & 19.18 & \text{---} & Unknown Age & 46 & 0 & 3.43 & \text{---} & Yes & \text{---} & 0.00 & 4.55 & 1.98 & 2007.118 \\
S5-346 & 19.18 & \text{---} & Unknown Age & 30 & 0 & 3.32 & \text{---} & Yes & \text{---} & 0.00 & -2.18 & -4.61 & 2013.778 \\
S4-492 & 19.20 & \text{---} & Unknown Age & 37 & 0 & 2.80 & \text{---} & Yes & \text{---} & 0.00 & 1.85 & -4.27 & 2015.725 \\
S4-487 & 19.23 & \text{---} & Unknown Age & 40 & 0 & 5.96 & \text{---} & Yes & \text{---} & 0.00 & 2.00 & 3.68 & 2015.235 \\
S3-450 & 19.29 & \text{---} & Unknown Age & 33 & 0 & 6.30 & \text{---} & Yes & \text{---} & 0.00 & -0.70 & 3.57 & 2016.411 \\
S4-498 & 19.29 & \text{---} & Unknown Age & 33 & 0 & 5.33 & \text{---} & Yes & \text{---} & 0.00 & 2.87 & 2.83 & 2018.983 \\
S5-78 & 19.30 & \text{---} & Unknown Age & 32 & 0 & 3.51 & \text{---} & Yes & \text{---} & 0.00 & 3.59 & 3.89 & 2007.656 \\
S5-345 & 19.36 & \text{---} & Unknown Age & 30 & 0 & 1.37 & \text{---} & No & \text{---} & 0.00 & 5.20 & -1.34 & 2015.582
\enddata
\end{deluxetable}
\end{longrotatetable}

==> Tables/Sample/samp_cat_orig.tex <==
%    /\_/\
%   ( o.o )
%    > ^ <
% Samp Cat (Sample Catalog)

\begin{longrotatetable}
\begin{deluxetable}{l|DD|r|rr|DD|cc|D|DDD}
    \tablehead{
        \colhead{Star} &
        \multicolumn2c{$\overline{m}_{K'}$} & \multicolumn2c{$\overline{m}_{H}$} &
        \colhead{Star Age} &
        \colhead{$K'$} & \colhead{$H$} &
        \multicolumn2c{$\chi^2_{\text{red, }K'}$} & \multicolumn2c{$\chi^2_{\text{red, }H}$} &
        \colhead{$K'$} & \colhead{$H$} &
        \multicolumn2c{Injected Binary} &
        \multicolumn2c{$x_0$} & \multicolumn2c{$y_0$} & \multicolumn2c{$t_0$} \\
        \colhead{} &
        \multicolumn2c{} & \multicolumn2c{} &
        \colhead{} &
        \colhead{Nights} & \colhead{Nights} &
        \multicolumn2c{} & \multicolumn2c{} &
        \colhead{Var.?} & \colhead{Var.?} &
        \multicolumn2c{Recovery Fraction} &
        \multicolumn2c{$x_0$} & \multicolumn2c{$y_0$} & \multicolumn2c{$t_0$}
    }
    \tablecaption{Stellar sample\label{tab:stellar_sample}}
\decimals
\startdata
IRS 16C & 10.03 & 12.07 & Known Young & 100 & 19 & 4.20 & 3.48 & Yes & No & 0.11 & 1.05 & 0.55 & 2009.989 \\
IRS 16SW & 10.08 & 12.16 & Known Young & 100 & 19 & 16.02 & 26.02 & Yes & Yes & 0.02 & 1.11 & -0.95 & 2009.820 \\
IRS 16NW & 10.28 & 12.34 & Known Young & 100 & 19 & 1.89 & 0.71 & Yes & No & 0.06 & 0.08 & 1.22 & 2010.047 \\
IRS 33E & 10.29 & 12.51 & Known Young & 100 & 19 & 1.22 & 0.61 & No & No & 0.10 & 0.71 & -3.14 & 2010.182 \\
S2-17 & 10.69 & 12.74 & Known Young & 100 & 19 & 1.10 & 2.48 & No & No & 0.01 & 1.34 & -1.88 & 2010.154 \\
S5-89 & 10.90 & 13.30 & Known Old & 99 & 19 & 1.23 & 1.27 & No & No & 0.04 & -0.79 & -5.25 & 2010.162 \\
IRS 16CC & 10.99 & 13.46 & Known Young & 100 & 19 & 80.36 & 67.19 & Yes & Yes & 0.00 & 1.98 & 0.60 & 2010.135 \\
S3-22 & 11.12 & 13.46 & Known Old & 100 & 19 & 0.38 & 0.53 & No & No & 0.09 & -0.34 & -3.21 & 2010.201 \\
IRS 16SW-E & 11.22 & 14.36 & Known Young & 92 & 19 & 5.61 & 12.51 & Yes & Yes & 0.00 & 1.90 & -1.12 & 2010.045 \\
S6-12 & 11.27 & 13.74 & Unknown Age & 93 & 19 & 3.49 & 3.39 & Yes & No & 0.01 & -0.21 & -6.08 & 2010.161 \\
IRS 33N & 11.29 & 13.48 & Known Young & 100 & 19 & 3.59 & 3.98 & Yes & Yes & 0.04 & -0.03 & -2.24 & 2010.161 \\
S6-63 & 11.31 & 13.44 & Known Young & 87 & 17 & 2.06 & 2.26 & Yes & No & 0.03 & 1.87 & -6.31 & 2011.057 \\
S4-207 & 11.32 & 14.31 & Known Old & 99 & 18 & 6.32 & 10.38 & Yes & Yes & 0.02 & -4.05 & -2.08 & 2009.835 \\
IRS 29S & 11.38 & 13.75 & Known Old & 100 & 19 & 0.60 & 1.05 & No & No & 0.04 & -1.84 & 0.96 & 2010.201 \\
S1-24 & 11.42 & 13.62 & Known Young & 73 & 19 & 1.78 & 4.01 & No & Yes & 0.02 & 0.74 & -1.65 & 2010.125 \\
S5-183 & 11.59 & 13.49 & Known Young & 100 & 19 & 1.13 & 0.39 & No & No & 0.01 & 4.59 & -3.44 & 2010.024 \\
S1-23 & 11.67 & 14.01 & Known Old & 100 & 19 & 2.66 & 2.04 & Yes & No & 0.02 & -0.90 & -1.50 & 2010.144 \\
IRS 34W & 11.67 & 14.85 & Known Young & 70 & 8 & 18.46 & 38.68 & Yes & Yes & 0.00 & -4.07 & 1.55 & 2010.189 \\
S2-11 & 11.78 & 13.88 & Known Old & 100 & 19 & 1.83 & 1.14 & No & No & 0.03 & 1.97 & -0.61 & 2009.813 \\
S6-343 & 11.81 & 14.10 & Unknown Age & 63 & 15 & 2.27 & 4.23 & Yes & Yes & 0.01 & -1.80 & -6.41 & 2017.086 \\
S2-6 & 11.90 & 14.11 & Known Young & 100 & 19 & 6.59 & 7.16 & Yes & Yes & 0.03 & 1.66 & -1.33 & 2010.067 \\
S3-5 & 11.93 & 14.25 & Known Young & 100 & 19 & 1.81 & 1.02 & No & No & 0.02 & 2.96 & -1.15 & 2009.910 \\
S2-4 & 12.04 & 14.39 & Known Young & 99 & 19 & 7.85 & 5.77 & Yes & Yes & 0.00 & 1.52 & -1.46 & 2010.007 \\
S4-129 & 12.06 & 14.42 & Known Old & 100 & 18 & 17.20 & 1.35 & Yes & No & 0.00 & 3.69 & -2.22 & 2009.999 \\
S3-291 & 12.12 & \text{---} & Known Old & 31 & 0 & 2.10 & \text{---} & No & \text{---} & 0.02 & -3.53 & -1.25 & 2010.064 \\
S3-10 & 12.13 & 14.09 & Known Young & 100 & 19 & 0.74 & 0.41 & No & No & 0.01 & 3.34 & -1.11 & 2009.944 \\
S4-4 & 12.13 & 14.90 & Known Old & 100 & 19 & 15.81 & 7.07 & Yes & Yes & 0.01 & 3.61 & -2.44 & 2009.973 \\
S3-2 & 12.16 & 14.36 & Known Young & 100 & 19 & 3.90 & 7.86 & Yes & Yes & 0.01 & 3.09 & 0.55 & 2010.014 \\
IRS 9W & 12.19 & 14.59 & Known Young & 99 & 19 & 3.74 & 4.63 & Yes & Yes & 0.03 & 2.90 & -5.59 & 2010.247 \\
S1-3 & 12.20 & 14.31 & Known Young & 98 & 19 & 1.13 & 0.82 & No & No & 0.03 & 0.32 & 0.88 & 2010.207 \\
S2-8 & 12.23 & 14.09 & Known Old & 96 & 17 & 1.01 & 0.35 & No & No & 0.01 & -1.96 & 0.89 & 2010.183 \\
S1-17 & 12.24 & 14.67 & Known Old & 85 & 13 & 1.19 & 2.00 & No & No & 0.01 & 0.48 & -1.53 & 2010.070 \\
S6-89 & 12.30 & 14.61 & Known Young & 44 & 9 & 5.49 & 3.22 & Yes & No & 0.02 & 5.45 & 3.00 & 2009.877 \\
S2-32 & 12.32 & 14.49 & Known Old & 100 & 18 & 1.03 & 0.57 & No & No & 0.01 & 1.13 & 2.78 & 2009.937 \\
S7-5 & 12.33 & 14.63 & Known Young & 99 & 18 & 4.13 & 4.43 & Yes & Yes & 0.00 & 4.86 & -5.52 & 2010.523 \\
S6-27 & 12.33 & 14.60 & Known Old & 100 & 19 & 0.32 & 0.74 & No & No & 0.02 & 4.08 & -4.68 & 2010.175 \\
S2-16 & 12.34 & 15.76 & Known Young & 100 & 19 & 13.35 & 4.92 & Yes & Yes & 0.00 & -1.07 & 2.06 & 2010.201 \\
S4-71 & 12.38 & 14.57 & Known Young & 100 & 19 & 0.80 & 0.49 & No & No & 0.01 & 0.77 & -4.09 & 2010.194 \\
S3-26 & 12.38 & 14.48 & Known Young & 100 & 19 & 2.31 & 2.77 & Yes & No & 0.00 & -2.57 & -2.07 & 2010.133 \\
S2-85 & 12.40 & 15.42 & Known Old & 84 & 18 & 30.39 & 121.75 & Yes & Yes & 0.01 & -1.29 & 2.67 & 2010.210 \\
S6-35 & 12.43 & 14.95 & Known Old & 85 & 16 & 3.23 & 2.99 & Yes & No & 0.02 & -4.91 & -3.96 & 2009.226 \\
S1-20 & 12.43 & 14.73 & Known Old & 100 & 19 & 32.68 & 10.65 & Yes & Yes & 0.00 & 0.45 & 1.60 & 2010.147 \\
S3-30 & 12.46 & 14.74 & Known Young & 69 & 19 & 2.64 & 3.75 & Yes & Yes & 0.01 & 1.66 & -2.94 & 2010.064 \\
S8-11 & 12.50 & 15.00 & Unknown Age & 77 & 17 & 14.35 & 39.61 & Yes & Yes & 0.01 & 5.38 & -5.97 & 2011.241 \\
S3-374 & 12.55 & 15.23 & Known Young & 100 & 19 & 19.80 & 75.68 & Yes & Yes & 0.00 & -2.76 & -2.85 & 2010.080 \\
S1-4 & 12.57 & 14.77 & Known Young & 100 & 19 & 2.99 & 1.91 & Yes & No & 0.01 & 0.88 & -0.66 & 2010.057 \\
S1-5 & 12.58 & 14.98 & Known Old & 80 & 18 & 2.37 & 8.23 & Yes & Yes & 0.00 & 0.32 & -0.89 & 2010.094 \\
S1-22 & 12.62 & 14.73 & Known Young & 51 & 19 & 0.85 & 4.41 & No & Yes & 0.01 & -1.57 & -0.52 & 2010.135 \\
S5-233 & 12.64 & 14.73 & Known Young & 33 & 10 & 2.20 & 4.55 & No & No & 0.00 & 5.59 & 0.67 & 2010.312 \\
S4-344 & 12.65 & 15.13 & Known Old & 100 & 19 & 0.80 & 2.64 & No & No & 0.03 & -1.43 & -4.72 & 2010.131 \\
S4-2 & 12.67 & 15.03 & Known Old & 100 & 19 & 1.37 & 2.30 & No & No & 0.04 & 3.76 & 1.65 & 2009.789 \\
S2-19 & 12.71 & 14.83 & Known Young & 100 & 19 & 1.85 & 3.76 & No & Yes & 0.00 & 0.38 & 2.31 & 2010.075 \\
S4-6 & 12.73 & 15.25 & Known Old & 100 & 19 & 4.67 & 17.15 & Yes & Yes & 0.01 & 3.28 & -2.75 & 2010.123 \\
S5-234 & 12.79 & \text{---} & Known Old & 34 & 0 & 2.59 & \text{---} & No & \text{---} & 0.01 & 5.71 & 0.56 & 2010.134 \\
S1-14 & 12.80 & 14.78 & Known Young & 84 & 18 & 0.96 & 3.43 & No & No & 0.02 & -1.32 & -0.37 & 2009.666 \\
S3-6 & 12.81 & 15.22 & Known Old & 42 & 19 & 0.65 & 3.42 & No & No & 0.04 & 3.23 & -0.05 & 2010.040 \\
S4-36 & 12.82 & 15.29 & Known Young & 83 & 11 & 5.93 & 5.13 & Yes & Yes & 0.00 & -3.69 & 1.78 & 2009.810 \\
S5-213 & 12.86 & 15.07 & Known Old & 99 & 19 & 0.86 & 1.38 & No & No & 0.01 & 4.98 & -3.26 & 2010.066 \\
S5-191 & 12.87 & 14.91 & Known Young & 100 & 19 & 0.58 & 1.15 & No & No & 0.03 & 3.18 & -4.89 & 2010.357 \\
S2-22 & 12.96 & 15.01 & Known Young & 100 & 19 & 0.85 & 1.43 & No & No & 0.03 & 2.30 & -0.21 & 2010.168 \\
S4-3 & 12.99 & 15.15 & Known Old & 100 & 18 & 0.16 & 0.38 & No & No & 0.01 & 4.22 & 0.12 & 2009.959 \\
S2-31 & 12.99 & 15.44 & Known Old & 100 & 18 & 3.93 & 5.61 & Yes & Yes & 0.03 & 2.76 & -0.19 & 2010.061 \\
S3-34 & 13.00 & 15.09 & Known Old & 100 & 19 & 179.80 & 30.85 & Yes & Yes & 0.00 & 3.24 & -1.26 & 2010.374 \\
S1-34 & 13.00 & 14.74 & Known Old & 94 & 19 & 0.35 & 0.15 & No & No & 0.02 & 0.87 & -0.99 & 2010.145 \\
S3-178 & 13.06 & 15.36 & Known Old & 31 & 19 & 0.53 & 1.79 & No & No & 0.04 & -0.51 & -3.39 & 2009.953 \\
S1-1 & 13.10 & 15.11 & Known Young & 100 & 19 & 0.67 & 0.33 & No & No & 0.03 & 1.04 & 0.03 & 2009.895 \\
S4-258 & 13.11 & 16.37 & Known Young & 91 & 18 & 142.99 & 398.75 & Yes & Yes & 0.00 & -4.40 & -1.63 & 2009.761 \\
S2-18 & 13.18 & 15.70 & Known Old & 100 & 19 & 17.33 & 92.74 & Yes & Yes & 0.01 & -1.00 & -2.15 & 2010.123 \\
S4-180 & 13.19 & 15.87 & Known Young & 41 & 18 & 2.59 & 1.57 & Yes & No & 0.01 & -4.29 & -1.33 & 2011.094 \\
IRS 7SE & 13.24 & 15.91 & Known Young & 99 & 18 & 34.40 & 3.84 & Yes & Yes & 0.00 & 2.99 & 3.46 & 2009.595 \\
S2-5 & 13.27 & 15.39 & Known Young & 99 & 19 & 1.36 & 0.90 & No & No & 0.00 & 1.94 & -0.79 & 2010.021 \\
S3-149 & 13.27 & 15.74 & Known Old & 100 & 19 & 7.03 & 4.10 & Yes & Yes & 0.01 & -2.90 & 1.71 & 2010.286 \\
S6-58 & 13.28 & 15.68 & Unknown Age & 99 & 19 & 1.38 & 4.32 & No & Yes & 0.02 & 3.22 & -5.65 & 2010.151 \\
S5-237 & 13.28 & 15.33 & Known Young & 63 & 14 & 8.20 & 2.40 & Yes & No & 0.00 & 5.49 & 1.02 & 2012.046 \\
S5-187 & 13.29 & 15.27 & Known Young & 99 & 19 & 1.79 & 1.64 & No & No & 0.03 & -1.71 & -5.55 & 2009.655 \\
S4-1 & 13.29 & 15.59 & Known Old & 100 & 19 & 0.61 & 0.78 & No & No & 0.02 & 4.00 & -0.36 & 2009.980 \\
S1-68 & 13.30 & 15.55 & Known Old & 99 & 19 & 1.04 & 1.73 & No & No & 0.00 & 1.83 & -0.65 & 2010.023 \\
S2-74 & 13.30 & 15.59 & Known Young & 100 & 18 & 4.26 & 3.25 & Yes & No & 0.01 & 0.11 & 2.78 & 2010.109 \\
S5-211 & 13.30 & 15.00 & Known Old & 100 & 19 & 0.29 & 0.39 & No & No & 0.02 & 4.46 & -3.90 & 2010.061 \\
S1-21 & 13.31 & 15.32 & Known Young & 100 & 19 & 0.96 & 0.60 & No & No & 0.02 & -1.64 & 0.09 & 2010.177 \\
S2-21 & 13.33 & 15.42 & Known Young & 100 & 19 & 1.40 & 0.89 & No & No & 0.00 & -1.62 & -1.67 & 2010.222 \\
S5-95 & 13.33 & 15.63 & Known Old & 86 & 16 & 1.99 & 1.05 & Yes & No & 0.01 & -1.94 & -4.99 & 2010.143 \\
S0-13 & 13.33 & 15.48 & Known Old & 49 & 13 & 0.57 & 1.46 & No & No & 0.01 & 0.56 & -0.41 & 2010.122 \\
S1-25 & 13.39 & 15.69 & Known Old & 97 & 19 & 0.64 & 0.46 & No & No & 0.01 & 1.68 & -0.61 & 2010.098 \\
S5-134 & 13.39 & 15.80 & Known Old & 94 & 18 & 3.64 & 2.21 & Yes & No & 0.00 & -0.53 & -5.46 & 2009.951 \\
S2-67 & 13.40 & 15.79 & Known Old & 98 & 19 & 3.37 & 2.23 & Yes & No & 0.01 & -2.47 & -0.88 & 2010.171 \\
S2-36 & 13.43 & 15.61 & Known Young & 98 & 19 & 8.85 & 9.81 & Yes & Yes & 0.00 & 1.99 & 0.44 & 2009.947 \\
S4-143 & 13.47 & 16.03 & Known Old & 94 & 18 & 0.39 & 0.41 & No & No & 0.01 & 2.90 & -3.25 & 2010.331 \\
S1-12 & 13.53 & 15.58 & Known Young & 100 & 19 & 0.50 & 0.75 & No & No & 0.01 & -0.75 & -1.03 & 2010.234 \\
S2-78 & 13.55 & 16.01 & Known Old & 89 & 13 & 1.74 & 2.93 & No & No & 0.00 & -2.82 & -0.28 & 2010.204 \\
S3-13 & 13.57 & 15.86 & Known Old & 100 & 19 & 0.64 & 0.79 & No & No & 0.01 & 3.84 & 0.98 & 2009.952 \\
S2-77 & 13.58 & 15.85 & Known Old & 36 & 19 & 1.57 & 11.95 & No & Yes & 0.02 & -1.76 & -2.21 & 2008.709 \\
S1-19 & 13.58 & 15.68 & Known Young & 83 & 13 & 0.93 & 0.64 & No & No & 0.00 & 0.43 & -1.64 & 2010.024 \\
S3-39 & 13.59 & 15.91 & Known Old & 99 & 18 & 1.23 & 1.37 & No & No & 0.02 & 3.56 & 1.08 & 2009.733 \\
S3-7 & 13.61 & 16.02 & Known Old & 100 & 19 & 1.91 & 6.93 & Yes & Yes & 0.02 & 1.92 & -2.61 & 2010.088 \\
S3-29 & 13.61 & 15.67 & Known Old & 97 & 19 & 2.58 & 1.14 & Yes & No & 0.00 & 1.44 & -3.08 & 2010.219 \\
S3-370 & 13.63 & 15.84 & Known Old & 95 & 19 & 0.47 & 0.19 & No & No & 0.03 & -0.29 & -3.91 & 2010.136 \\
S4-169 & 13.64 & 15.57 & Known Young & 100 & 12 & 0.43 & 0.36 & No & No & 0.00 & 4.41 & 0.28 & 2009.872 \\
S2-24 & 13.67 & 16.08 & Known Old & 94 & 17 & 0.71 & 1.06 & No & No & 0.00 & -2.34 & -0.89 & 2009.893 \\
S6-76 & 13.68 & 16.02 & Known Old & 100 & 19 & 0.91 & 1.27 & No & No & 0.00 & 5.18 & -4.52 & 2010.291 \\
S0-14 & 13.69 & 15.73 & Known Young & 96 & 18 & 0.98 & 2.41 & No & No & 0.00 & -0.76 & -0.29 & 2010.316 \\
S0-15 & 13.70 & 15.86 & Known Young & 56 & 17 & 9.32 & 49.61 & Yes & Yes & 0.00 & -0.97 & 0.18 & 2009.722 \\
IRS 34NW & 13.71 & 16.90 & Known Young & 90 & 18 & 29.56 & 40.95 & Yes & Yes & 0.00 & -3.78 & 2.83 & 2010.283 \\
S3-198 & 13.71 & 16.36 & Unknown Age & 99 & 18 & 3.87 & 10.81 & Yes & Yes & 0.01 & 0.65 & 3.45 & 2009.959 \\
S4-287 & 13.73 & 15.87 & Known Young & 100 & 19 & 0.42 & 0.25 & No & No & 0.01 & 0.13 & -4.77 & 2010.188 \\
S7-27 & 13.73 & 16.05 & Unknown Age & 77 & 17 & 2.06 & 3.41 & Yes & No & 0.01 & 3.26 & -6.36 & 2011.875 \\
S5-34 & 13.73 & 16.18 & Known Young & 89 & 18 & 1.46 & 2.76 & No & No & 0.01 & -4.33 & -2.74 & 2010.071 \\
S2-26 & 13.74 & 16.11 & Known Old & 100 & 19 & 59.39 & 6.19 & Yes & Yes & 0.00 & 0.79 & 2.31 & 2010.167 \\
S4-161 & 13.74 & 16.18 & Known Old & 100 & 19 & 0.50 & 1.17 & No & No & 0.01 & 4.42 & -0.26 & 2009.943 \\
S3-331 & 13.75 & 15.85 & Known Young & 95 & 18 & 2.16 & 1.82 & Yes & No & 0.00 & -1.22 & 3.65 & 2010.150 \\
S6-25 & 13.77 & 16.10 & Unknown Age & 92 & 18 & 1.23 & 4.21 & No & Yes & 0.02 & 0.71 & -6.17 & 2010.070 \\
S2-25 & 13.78 & 16.17 & Known Old & 100 & 19 & 1.14 & 1.23 & No & No & 0.01 & 0.76 & -2.42 & 2010.330 \\
S5-185 & 13.79 & 16.08 & Unknown Age & 100 & 18 & 1.55 & 1.46 & No & No & 0.01 & 3.00 & -4.92 & 2010.475 \\
S4-112 & 13.79 & 16.15 & Known Old & 96 & 19 & 4.35 & 5.04 & Yes & Yes & 0.01 & 2.24 & -3.61 & 2010.251 \\
S3-134 & 13.79 & 16.10 & Known Old & 100 & 19 & 0.36 & 0.28 & No & No & 0.00 & -1.39 & -3.01 & 2010.208 \\
S5-115 & 13.80 & 16.54 & Unknown Age & 68 & 8 & 4.45 & 3.25 & Yes & No & 0.02 & -5.17 & -1.55 & 2010.148 \\
S3-17 & 13.81 & 16.43 & Known Young & 34 & 18 & 8.09 & 63.40 & Yes & Yes & 0.00 & -1.41 & 2.85 & 2009.185 \\
S3-14 & 13.84 & 16.41 & Known Old & 79 & 18 & 11.05 & 28.40 & Yes & Yes & 0.00 & 0.18 & 3.07 & 2009.981 \\
S4-59 & 13.84 & 15.93 & Known Old & 72 & 7 & 0.82 & 0.32 & No & No & 0.02 & -3.15 & 2.65 & 2010.023 \\
S3-35 & 13.87 & 16.60 & Unknown Age & 99 & 18 & 3.71 & 2.72 & Yes & No & 0.00 & -1.21 & 3.28 & 2010.167 \\
S5-71 & 13.88 & 16.12 & Known Old & 100 & 19 & 0.44 & 0.25 & No & No & 0.02 & -1.75 & -4.94 & 2009.691 \\
S6-31 & 13.88 & 16.21 & Known Old & 93 & 18 & 1.23 & 0.46 & No & No & 0.03 & -2.12 & -5.85 & 2010.015 \\
S2-7 & 13.91 & 16.17 & Known Young & 100 & 18 & 46.48 & 12.53 & Yes & Yes & 0.00 & 0.93 & 1.85 & 2010.257 \\
S4-342 & 13.92 & 16.39 & Unknown Age & 74 & 14 & 16.73 & 6.33 & Yes & Yes & 0.01 & 3.07 & 3.86 & 2010.650 \\
S3-28 & 13.93 & 16.40 & Unknown Age & 99 & 18 & 2.68 & 1.06 & Yes & No & 0.00 & -0.83 & 3.23 & 2010.134 \\
S3-27 & 13.96 & 16.33 & Unknown Age & 99 & 18 & 9.21 & 0.76 & Yes & No & 0.00 & -0.33 & 3.32 & 2010.092 \\
S3-284 & 13.97 & 17.13 & Known Old & 100 & 18 & 9.82 & 8.53 & Yes & Yes & 0.00 & -2.57 & 2.71 & 2010.347 \\
S4-84 & 13.99 & 16.80 & Known Old & 35 & 9 & 4.39 & 7.07 & Yes & Yes & 0.00 & -3.36 & 2.52 & 2009.984 \\
S5-145 & 13.99 & 15.96 & Unknown Age & 90 & 18 & 1.61 & 0.93 & No & No & 0.00 & -0.57 & -5.54 & 2010.081 \\
S4-24 & 14.02 & 16.75 & Unknown Age & 68 & 5 & 5.63 & 6.02 & Yes & No & 0.01 & -0.72 & 4.00 & 2010.423 \\
S3-25 & 14.04 & 16.13 & Known Young & 100 & 18 & 1.76 & 3.76 & No & Yes & 0.00 & 1.41 & 2.95 & 2009.923 \\
S0-6 & 14.04 & 16.32 & Known Old & 100 & 19 & 1.27 & 6.06 & No & Yes & 0.03 & 0.02 & -0.36 & 2010.779 \\
S2-58 & 14.05 & 16.27 & Known Young & 94 & 18 & 3.12 & 6.02 & Yes & Yes & 0.01 & 2.14 & -1.13 & 2010.157 \\
S6-66 & 14.06 & 16.59 & Known Old & 39 & 15 & 2.52 & 2.24 & No & No & 0.00 & -4.71 & -4.66 & 2009.332 \\
S3-207 & 14.06 & 16.33 & Unknown Age & 99 & 18 & 0.61 & 0.53 & No & No & 0.00 & 1.55 & 3.21 & 2009.989 \\
S2-2 & 14.06 & 15.78 & Known Old & 100 & 19 & 0.20 & 0.24 & No & No & 0.01 & -0.52 & 2.09 & 2010.141 \\
S4-158 & 14.08 & 16.20 & Known Old & 100 & 19 & 0.40 & 0.92 & No & No & 0.02 & -0.86 & -4.33 & 2010.174 \\
S1-13 & 14.08 & 16.41 & Known Old & 76 & 19 & 0.82 & 3.02 & No & No & 0.01 & -1.14 & -0.97 & 2010.185 \\
S4-197 & 14.09 & 16.62 & Known Old & 100 & 19 & 2.12 & 3.62 & Yes & Yes & 0.01 & -2.55 & -3.71 & 2010.272 \\
S5-205 & 14.09 & 16.39 & Known Old & 93 & 19 & 3.42 & 10.93 & Yes & Yes & 0.00 & -0.91 & -5.81 & 2010.004 \\
S7-29 & 14.12 & 16.58 & Known Old & 72 & 16 & 1.98 & 2.34 & No & No & 0.00 & -3.66 & -6.38 & 2010.986 \\
S0-2 & 14.12 & 16.13 & Known Young & 89 & 18 & 1.92 & 3.86 & No & Yes & 0.02 & -0.01 & 0.17 & 2007.893 \\
S6-39 & 14.13 & 16.47 & Unknown Age & 93 & 18 & 5.95 & 2.93 & Yes & No & 0.00 & 2.51 & -5.79 & 2009.801 \\
S5-202 & 14.14 & 16.12 & Unknown Age & 93 & 19 & 0.74 & 2.76 & No & No & 0.00 & -0.51 & -5.85 & 2010.094 \\
S5-199 & 14.16 & 16.68 & Known Old & 83 & 18 & 1.34 & 4.54 & No & Yes & 0.01 & -4.20 & -4.08 & 2009.569 \\
S3-146 & 14.17 & 16.38 & Probable Old & 89 & 17 & 5.50 & 6.03 & Yes & Yes & 0.00 & -0.29 & -3.35 & 2010.110 \\
S4-319 & 14.17 & 16.42 & Known Old & 86 & 19 & 1.29 & 0.88 & No & No & 0.00 & 4.68 & -1.38 & 2010.042 \\
S0-32 & 14.19 & 15.05 & Probable Young & 90 & 18 & 0.81 & 0.26 & No & No & 0.02 & 0.32 & 0.79 & 2010.090 \\
S4-229 & 14.20 & 17.03 & Unknown Age & 66 & 10 & 4.28 & 13.93 & Yes & Yes & 0.00 & -4.19 & 1.94 & 2010.123 \\
S2-57 & 14.22 & 16.47 & Known Old & 71 & 14 & 1.71 & 0.89 & No & No & 0.00 & -1.15 & -2.09 & 2010.273 \\
S4-170 & 14.22 & 16.40 & Known Old & 99 & 19 & 1.57 & 0.49 & No & No & 0.01 & -0.57 & -4.41 & 2010.181 \\
S1-8 & 14.22 & 16.48 & Known Young & 99 & 19 & 2.86 & 2.68 & Yes & No & 0.00 & -0.58 & -0.92 & 2010.185 \\
S0-4 & 14.23 & 16.25 & Known Young & 39 & 13 & 2.14 & 1.31 & No & No & 0.00 & 0.45 & -0.33 & 2010.008 \\
S2-3 & 14.23 & 16.63 & Known Old & 58 & 18 & 0.74 & 1.26 & No & No & 0.00 & -1.51 & -1.41 & 2010.300 \\
S3-88 & 14.24 & 16.42 & Known Old & 100 & 19 & 0.36 & 0.11 & No & No & 0.00 & -0.85 & -3.00 & 2010.102 \\
S2-344 & 14.25 & 16.57 & Unknown Age & 36 & 9 & 1.74 & 1.05 & No & No & 0.01 & -1.73 & -2.20 & 2012.518 \\
S5-43 & 14.26 & 16.79 & Known Old & 100 & 19 & 3.54 & 5.42 & Yes & Yes & 0.00 & 1.84 & -4.80 & 2010.260 \\
S5-240 & 14.26 & 16.45 & Probable Old & 76 & 16 & 1.78 & 1.27 & No & No & 0.01 & 5.36 & 0.08 & 2011.220 \\
S2-47 & 14.26 & 16.61 & Known Old & 100 & 19 & 1.39 & 1.27 & No & No & 0.01 & 2.19 & -0.52 & 2010.214 \\
S4-221 & 14.27 & 16.70 & Known Old & 100 & 19 & 2.83 & 9.74 & Yes & Yes & 0.00 & 2.69 & -3.77 & 2010.222 \\
S0-9 & 14.28 & 16.27 & Known Young & 82 & 18 & 3.21 & 6.85 & Yes & Yes & 0.00 & 0.22 & -0.60 & 2009.769 \\
S7-3 & 14.30 & 16.63 & Unknown Age & 87 & 18 & 0.84 & 1.87 & No & No & 0.02 & 4.17 & -5.80 & 2010.379 \\
S6-49 & 14.31 & 16.67 & Known Old & 88 & 19 & 1.30 & 3.37 & No & No & 0.00 & -2.85 & -5.77 & 2010.422 \\
S4-196 & 14.32 & 16.56 & Known Young & 100 & 19 & 5.62 & 7.76 & Yes & Yes & 0.00 & 2.24 & -3.93 & 2010.135 \\
S3-288 & 14.32 & 17.58 & Known Old & 100 & 18 & 11.95 & 6.10 & Yes & Yes & 0.00 & -2.77 & 2.54 & 2010.339 \\
S3-190 & 14.33 & 17.12 & Known Young & 100 & 19 & 11.22 & 22.72 & Yes & Yes & 0.00 & -3.19 & 1.41 & 2010.223 \\
S5-170 & 14.33 & 16.54 & Unknown Age & 34 & 16 & 16.45 & 2.76 & Yes & No & 0.00 & 4.23 & 3.84 & 2009.509 \\
S5-174 & 14.37 & 16.84 & Known Old & 90 & 18 & 1.61 & 2.80 & No & No & 0.00 & -4.16 & -3.94 & 2010.073 \\
S6-77 & 14.38 & 16.60 & Known Old & 78 & 15 & 1.53 & 1.75 & No & No & 0.00 & 5.06 & -4.75 & 2010.476 \\
S0-12 & 14.39 & 16.66 & Known Old & 100 & 19 & 1.29 & 2.14 & No & No & 0.00 & -0.55 & 0.41 & 2009.012 \\
S4-168 & 14.40 & 16.90 & Unknown Age & 76 & 9 & 4.20 & 1.57 & Yes & No & 0.00 & -1.91 & 3.97 & 2010.678 \\
S4-139 & 14.41 & 16.65 & Known Old & 99 & 18 & 5.03 & 1.77 & Yes & No & 0.00 & 2.40 & -3.62 & 2010.074 \\
S1-49 & 14.41 & 16.46 & Probable Old & 98 & 19 & 5.57 & 5.68 & Yes & Yes & 0.01 & -1.72 & 0.15 & 2010.287 \\
S2-75 & 14.43 & 16.73 & Known Old & 100 & 19 & 0.43 & 0.91 & No & No & 0.00 & 2.63 & -0.85 & 2010.082 \\
S2-70 & 14.45 & 17.25 & Known Old & 100 & 19 & 14.15 & 103.90 & Yes & Yes & 0.00 & -2.68 & 0.39 & 2010.154 \\
S3-20 & 14.45 & 16.97 & Known Old & 98 & 19 & 3.04 & 8.68 & Yes & Yes & 0.00 & 1.58 & -2.79 & 2009.965 \\
S3-208 & 14.47 & 16.36 & Known Young & 100 & 19 & 1.41 & 1.54 & No & No & 0.00 & -0.98 & -3.41 & 2010.198 \\
S2-23 & 14.47 & 17.07 & Known Old & 100 & 19 & 2.50 & 8.38 & Yes & Yes & 0.00 & 1.65 & 1.74 & 2010.053 \\
S4-352 & 14.48 & 17.34 & Unknown Age & 90 & 16 & 4.87 & 8.33 & Yes & Yes & 0.00 & -4.88 & -0.88 & 2009.519 \\
S6-70 & 14.49 & 16.88 & Known Old & 84 & 19 & 1.44 & 3.29 & No & No & 0.01 & -2.80 & -6.15 & 2011.881 \\
S5-168 & 14.51 & 16.96 & Unknown Age & 52 & 8 & 1.61 & 1.56 & No & No & 0.00 & 4.37 & 3.62 & 2010.149 \\
S6-64 & 14.53 & 16.34 & Known Young & 74 & 18 & 1.28 & 0.69 & No & No & 0.00 & -3.05 & -5.86 & 2010.405 \\
S3-187 & 14.55 & 17.09 & Known Old & 100 & 19 & 7.19 & 7.15 & Yes & Yes & 0.00 & -3.40 & -0.75 & 2010.032 \\
S3-96 & 14.56 & 17.14 & Known Young & 68 & 12 & 1.15 & 1.45 & No & No & 0.01 & -3.13 & -0.63 & 2010.217 \\
S3-364 & 14.59 & 16.72 & Unknown Age & 86 & 14 & 3.04 & 7.10 & Yes & Yes & 0.00 & -0.96 & 3.80 & 2010.143 \\
S4-236 & 14.59 & 16.84 & Known Old & 65 & 19 & 0.43 & 0.76 & No & No & 0.01 & -1.91 & -4.22 & 2009.747 \\
S3-36 & 14.62 & 16.70 & Known Old & 100 & 19 & 0.20 & 0.73 & No & No & 0.01 & 3.47 & -0.81 & 2010.145 \\
S5-198 & 14.62 & 16.85 & Unknown Age & 93 & 19 & 0.91 & 2.28 & No & No & 0.00 & 0.51 & -5.82 & 2010.297 \\
S3-4 & 14.63 & 17.76 & Probable Old & 98 & 19 & 9.62 & 5.09 & Yes & Yes & 0.00 & 3.07 & -0.48 & 2010.182 \\
S0-3 & 14.65 & 16.74 & Known Young & 98 & 19 & 1.46 & 5.31 & No & Yes & 0.00 & 0.34 & 0.12 & 2008.393 \\
S5-83 & 14.69 & 16.86 & Known Old & 100 & 19 & 0.60 & 0.89 & No & No & 0.01 & 5.20 & -0.94 & 2010.125 \\
S6-62 & 14.71 & 17.12 & Known Old & 36 & 15 & 3.51 & 3.65 & Yes & No & 0.00 & -4.70 & -4.60 & 2009.407 \\
S2-277 & 14.73 & 16.86 & Probable Old & 100 & 18 & 1.25 & 2.06 & No & No & 0.00 & -2.44 & -1.44 & 2010.286 \\
S4-46 & 14.76 & 16.61 & Known Old & 99 & 19 & 0.82 & 0.32 & No & No & 0.01 & 3.84 & -1.48 & 2010.066 \\
S1-10 & 14.77 & 16.57 & Known Old & 89 & 15 & 0.43 & 1.06 & No & No & 0.00 & -1.10 & -0.02 & 2010.139 \\
S1-2 & 14.78 & 16.82 & Known Young & 100 & 19 & 2.06 & 1.22 & Yes & No & 0.00 & 0.08 & -1.02 & 2009.985 \\
S0-1 & 14.78 & 16.92 & Known Young & 67 & 18 & 9.03 & 7.40 & Yes & Yes & 0.00 & 0.04 & -0.26 & 2006.300 \\
S3-249 & 14.80 & 18.51 & Known Old & 100 & 13 & 60.47 & 278.63 & Yes & Yes & 0.00 & -3.38 & 1.28 & 2010.016 \\
S4-98 & 14.80 & 17.13 & Unknown Age & 94 & 12 & 5.64 & 2.98 & Yes & No & 0.00 & -4.12 & -0.90 & 2009.807 \\
S5-12 & 14.82 & 17.45 & Known Old & 88 & 18 & 0.55 & 1.07 & No & No & 0.00 & -4.28 & -2.63 & 2010.189 \\
S2-69 & 14.82 & 17.84 & Unknown Age & 99 & 18 & 13.76 & 90.06 & Yes & Yes & 0.00 & -0.88 & 2.56 & 2010.273 \\
S5-112 & 14.83 & \text{---} & Unknown Age & 40 & 0 & 7.99 & \text{---} & Yes & \text{---} & 0.00 & -5.27 & 1.23 & 2009.265 \\
S4-12 & 14.83 & 17.45 & Known Young & 70 & 18 & 18.53 & 20.45 & Yes & Yes & 0.00 & -2.86 & 2.84 & 2010.034 \\
S5-133 & 14.83 & 16.85 & Unknown Age & 88 & 16 & 9.58 & 3.50 & Yes & No & 0.00 & -0.75 & -5.45 & 2009.873 \\
S3-403 & 14.84 & 17.10 & Probable Old & 57 & 16 & 4.07 & 5.30 & Yes & Yes & 0.00 & -0.12 & -3.38 & 2009.561 \\
S2-72 & 14.84 & 17.22 & Known Old & 56 & 12 & 2.95 & 4.99 & Yes & Yes & 0.00 & -1.50 & -2.24 & 2010.007 \\
S6-123 & 14.84 & 17.13 & Unknown Age & 47 & 15 & 1.11 & 3.35 & No & No & 0.00 & -0.11 & -6.45 & 2010.778 \\
S7-43 & 14.86 & 17.42 & Unknown Age & 72 & 15 & 2.44 & 3.44 & Yes & No & 0.01 & 4.09 & -6.40 & 2011.383 \\
S1-18 & 14.87 & 17.13 & Known Young & 69 & 19 & 2.98 & 4.90 & Yes & Yes & 0.00 & -0.79 & 1.50 & 2009.682 \\
S5-243 & 14.90 & 17.21 & Known Old & 48 & 10 & 3.80 & 5.61 & Yes & Yes & 0.00 & 5.52 & 1.45 & 2007.596 \\
S2-73 & 14.91 & 17.13 & Known Old & 100 & 19 & 2.04 & 5.56 & Yes & Yes & 0.00 & 2.13 & -1.66 & 2009.926 \\
S5-99 & 14.91 & 17.15 & Known Old & 100 & 19 & 0.53 & 0.77 & No & No & 0.02 & 4.61 & -2.74 & 2010.082 \\
S3-223 & 14.92 & 17.37 & Probable Old & 63 & 12 & 4.18 & 14.31 & Yes & Yes & 0.00 & 1.28 & -3.37 & 2009.821 \\
S6-37 & 14.96 & 17.58 & Known Old & 93 & 19 & 3.89 & 0.92 & Yes & No & 0.00 & -2.31 & -5.87 & 2010.256 \\
S3-11 & 14.99 & 17.46 & Known Old & 91 & 18 & 2.30 & 5.57 & Yes & Yes & 0.00 & 2.96 & -1.90 & 2011.181 \\
S1-51 & 15.01 & 17.29 & Probable Old & 100 & 19 & 1.35 & 0.44 & No & No & 0.00 & -1.66 & -0.17 & 2010.270 \\
S5-31 & 15.02 & 16.95 & Unknown Age & 43 & 10 & 1.30 & 1.27 & No & No & 0.00 & -4.34 & 2.65 & 2011.201 \\
S0-5 & 15.03 & 17.13 & Known Young & 72 & 12 & 4.49 & 1.31 & Yes & No & 0.00 & 0.17 & -0.36 & 2009.636 \\
S0-53 & 15.03 & \text{---} & Unknown Age & 81 & 0 & 37.75 & \text{---} & Yes & \text{---} & 0.00 & 0.35 & 0.20 & 2005.892 \\
S1-33 & 15.04 & 17.13 & Known Young & 100 & 19 & 1.01 & 0.65 & No & No & 0.00 & -1.25 & -0.00 & 2009.977 \\
S3-16 & 15.04 & 17.27 & Known Old & 93 & 17 & 9.38 & 3.57 & Yes & No & 0.00 & 2.97 & -0.95 & 2009.811 \\
S6-128 & 15.06 & 17.59 & Known Old & 38 & 8 & 2.86 & 2.16 & Yes & No & 0.00 & 5.70 & -2.54 & 2010.873 \\
S3-438 & 15.06 & 17.16 & Unknown Age & 31 & 8 & 4.23 & 3.45 & Yes & No & 0.00 & -0.52 & -3.41 & 2016.818 \\
S4-172 & 15.08 & 17.39 & Known Old & 92 & 17 & 16.83 & 22.94 & Yes & Yes & 0.00 & 3.09 & -3.17 & 2010.358 \\
S2-62 & 15.08 & 17.43 & Known Old & 99 & 19 & 0.92 & 2.03 & No & No & 0.00 & -1.03 & -2.32 & 2010.009 \\
S3-37 & 15.09 & 16.96 & Known Old & 95 & 17 & 1.14 & 1.45 & No & No & 0.01 & 3.42 & 1.36 & 2010.050 \\
S3-216 & 15.10 & 17.16 & Probable Old & 72 & 18 & 0.55 & 0.94 & No & No & 0.00 & -3.14 & 1.67 & 2009.725 \\
S0-31 & 15.10 & 17.10 & Known Young & 88 & 11 & 2.41 & 8.33 & Yes & Yes & 0.00 & 0.57 & 0.45 & 2009.906 \\
S5-193 & 15.11 & 16.84 & Probable Old & 59 & 19 & 0.77 & 1.09 & No & No & 0.01 & -1.16 & -5.73 & 2009.874 \\
S3-3 & 15.13 & 17.20 & Known Young & 100 & 19 & 1.27 & 2.23 & No & No & 0.00 & 3.09 & -0.64 & 2010.081 \\
S0-18 & 15.14 & 17.34 & Known Old & 32 & 19 & 1.29 & 4.82 & No & Yes & 0.00 & -0.12 & -0.42 & 2009.454 \\
S5-159 & 15.15 & 17.31 & Unknown Age & 98 & 19 & 0.54 & 0.60 & No & No & 0.01 & 0.43 & -5.60 & 2010.221 \\
S0-7 & 15.17 & 17.26 & Known Young & 97 & 17 & 3.42 & 3.53 & Yes & No & 0.00 & 0.51 & 0.10 & 2010.379 \\
S4-315 & 15.18 & 17.40 & Known Old & 85 & 16 & 6.00 & 1.77 & Yes & No & 0.00 & 4.81 & 0.85 & 2009.738 \\
S3-155 & 15.18 & 17.03 & Known Young & 99 & 18 & 0.47 & 0.41 & No & No & 0.00 & -1.84 & -2.83 & 2010.185 \\
S2-12 & 15.18 & 17.39 & Known Old & 99 & 18 & 1.79 & 1.57 & No & No & 0.00 & 1.64 & 1.14 & 2010.272 \\
S0-11 & 15.19 & 17.27 & Known Young & 98 & 18 & 1.68 & 1.03 & No & No & 0.00 & 0.49 & -0.06 & 2010.011 \\
S2-55 & 15.19 & 17.48 & Known Old & 98 & 17 & 2.30 & 1.87 & Yes & No & 0.00 & 0.90 & -2.19 & 2009.600 \\
S2-50 & 15.20 & 17.34 & Known Young & 85 & 16 & 5.50 & 7.82 & Yes & Yes & 0.00 & 1.70 & -1.51 & 2009.533 \\
S4-188 & 15.20 & 17.80 & Unknown Age & 91 & 17 & 24.07 & 18.82 & Yes & Yes & 0.00 & -4.14 & -1.77 & 2010.496 \\
S2-49 & 15.20 & 17.41 & Known Old & 100 & 19 & 1.60 & 1.41 & No & No & 0.00 & -0.80 & -2.14 & 2010.126 \\
S2-71 & 15.21 & 17.35 & Known Old & 100 & 19 & 0.79 & 0.96 & No & No & 0.01 & -0.88 & -2.52 & 2010.060 \\
S3-262 & 15.22 & 18.78 & Known Old & 100 & 16 & 27.50 & 158.86 & Yes & Yes & 0.00 & -2.35 & 2.81 & 2010.084 \\
S4-277 & 15.22 & 17.38 & Known Old & 75 & 16 & 1.46 & 1.71 & No & No & 0.01 & 4.75 & 0.21 & 2009.665 \\
S5-98 & 15.22 & 17.32 & Probable Young & 99 & 18 & 0.59 & 0.53 & No & No & 0.01 & 1.04 & -5.24 & 2010.354 \\
S5-156 & 15.22 & 17.54 & Known Old & 98 & 19 & 1.91 & 2.33 & Yes & No & 0.00 & -1.42 & -5.45 & 2010.209 \\
S6-44 & 15.22 & 17.43 & Known Young & 92 & 19 & 5.26 & 6.17 & Yes & Yes & 0.00 & -2.15 & -6.00 & 2010.113 \\
S3-227 & 15.22 & 17.45 & Probable Old & 98 & 17 & 1.63 & 0.54 & No & No & 0.00 & 0.03 & -3.60 & 2010.028 \\
S1-53 & 15.22 & 17.42 & Known Old & 98 & 19 & 1.58 & 1.76 & No & No & 0.00 & 1.67 & -0.10 & 2009.524 \\
S3-51 & 15.23 & 17.34 & Probable Old & 99 & 18 & 0.64 & 0.84 & No & No & 0.01 & -0.15 & 3.02 & 2010.104 \\
S3-385 & 15.24 & 17.36 & Known Old & 90 & 16 & 0.84 & 0.94 & No & No & 0.00 & 3.69 & -1.46 & 2009.997 \\
S3-32 & 15.24 & 17.48 & Known Old & 99 & 19 & 2.23 & 5.08 & Yes & Yes & 0.00 & 2.87 & -1.77 & 2010.163 \\
S6-14 & 15.25 & 17.61 & Known Old & 85 & 19 & 1.30 & 0.33 & No & No & 0.01 & -3.24 & -5.16 & 2009.107 \\
S2-84 & 15.25 & 17.54 & Probable Old & 99 & 18 & 1.56 & 1.50 & No & No & 0.00 & 1.66 & -2.47 & 2010.187 \\
S3-192 & 15.25 & 17.55 & Probable Old & 94 & 10 & 1.93 & 3.78 & Yes & No & 0.02 & 0.50 & -3.47 & 2009.890 \\
S1-39 & 15.25 & 17.53 & Known Old & 76 & 19 & 1.50 & 1.82 & No & No & 0.01 & -0.54 & -1.38 & 2009.934 \\
S4-86 & 15.25 & 17.32 & Known Old & 100 & 19 & 0.65 & 0.28 & No & No & 0.00 & -0.66 & -4.12 & 2009.691 \\
S1-32 & 15.27 & 17.55 & Known Old & 71 & 11 & 1.33 & 1.98 & No & No & 0.00 & -0.99 & -0.66 & 2010.144 \\
S1-63 & 15.27 & 17.94 & Probable Old & 66 & 11 & 7.08 & 54.15 & Yes & Yes & 0.00 & -1.22 & 1.41 & 2008.658 \\
S2-316 & 15.27 & 17.77 & Unknown Age & 54 & 18 & 7.66 & 3.52 & Yes & No & 0.00 & -2.43 & 1.64 & 2009.665 \\
S2-306 & 15.28 & 17.89 & Known Young & 52 & 11 & 6.16 & 9.79 & Yes & Yes & 0.00 & -0.49 & -2.89 & 2010.382 \\
S1-52 & 15.28 & 17.36 & Probable Old & 38 & 6 & 0.97 & 4.88 & No & No & 0.00 & 0.01 & 1.68 & 2007.924 \\
S2-29 & 15.29 & 17.43 & Known Young & 87 & 17 & 2.30 & 1.68 & Yes & No & 0.00 & 1.95 & -2.16 & 2010.009 \\
S2-82 & 15.29 & 17.53 & Probable Old & 36 & 17 & 1.92 & 7.18 & No & Yes & 0.00 & 2.86 & 0.06 & 2009.160 \\
S4-375 & 15.29 & 17.58 & Unknown Age & 47 & 13 & 3.02 & 3.29 & Yes & No & 0.00 & 3.94 & 1.62 & 2010.282 \\
S3-268 & 15.29 & 17.56 & Known Young & 87 & 19 & 1.44 & 2.20 & No & No & 0.00 & -2.15 & -3.03 & 2010.422 \\
S3-43 & 15.29 & 17.44 & Probable Old & 84 & 13 & 3.01 & 1.43 & Yes & No & 0.00 & -0.16 & -3.02 & 2009.661 \\
S3-344 & 15.29 & 17.47 & Unknown Age & 100 & 18 & 1.24 & 0.81 & No & No & 0.00 & 3.07 & 2.41 & 2010.234 \\
S4-45 & 15.29 & 17.57 & Probable Old & 93 & 18 & 0.97 & 0.57 & No & No & 0.02 & 4.11 & -0.41 & 2009.981 \\
S3-348 & 15.30 & 17.42 & Probable Old & 95 & 18 & 0.63 & 0.26 & No & No & 0.00 & 3.91 & 0.23 & 2009.944 \\
S3-286 & 15.30 & 17.44 & Known Old & 100 & 19 & 0.78 & 0.59 & No & No & 0.00 & 3.41 & -1.52 & 2010.090 \\
S3-327 & 15.30 & 17.40 & Known Old & 45 & 16 & 9.07 & 5.17 & Yes & Yes & 0.00 & 2.50 & -2.92 & 2010.243 \\
S2-345 & 15.30 & 17.68 & Unknown Age & 32 & 6 & 13.10 & 12.32 & Yes & Yes & 0.00 & 1.78 & -1.18 & 2015.482 \\
S6-78 & 15.31 & 17.56 & Unknown Age & 88 & 18 & 1.07 & 3.76 & No & Yes & 0.00 & 4.38 & -5.38 & 2009.990 \\
S2-61 & 15.31 & 17.47 & Known Old & 65 & 13 & 4.60 & 1.45 & Yes & No & 0.00 & 2.36 & -0.65 & 2009.705 \\
S6-135 & 15.31 & 17.67 & Unknown Age & 54 & 14 & 5.75 & 2.17 & Yes & No & 0.00 & 5.49 & 2.56 & 2008.759 \\
S5-60 & 15.32 & 17.45 & Probable Old & 86 & 15 & 2.44 & 2.43 & Yes & No & 0.00 & 5.22 & 0.12 & 2009.817 \\
S3-33 & 15.33 & 17.53 & Probable Old & 36 & 17 & 1.66 & 4.75 & No & Yes & 0.01 & 3.32 & -0.83 & 2010.120 \\
S0-35 & 15.33 & 17.61 & Probable Old & 39 & 16 & 3.13 & 5.86 & Yes & Yes & 0.00 & 0.02 & 0.88 & 2009.499 \\
S1-29 & 15.34 & 17.63 & Known Young & 82 & 11 & 2.63 & 3.98 & Yes & No & 0.00 & 1.07 & 0.16 & 2010.071 \\
S4-312 & 15.34 & 17.56 & Known Old & 99 & 19 & 0.74 & 0.67 & No & No & 0.00 & 4.60 & -1.54 & 2010.231 \\
S6-4 & 15.35 & 17.57 & Unknown Age & 92 & 18 & 1.52 & 2.03 & No & No & 0.01 & 1.72 & -5.79 & 2010.138 \\
S1-48 & 15.35 & 17.56 & Known Old & 96 & 17 & 4.20 & 2.39 & Yes & No & 0.00 & -0.63 & -1.55 & 2009.947 \\
S3-319 & 15.35 & 17.48 & Probable Old & 98 & 19 & 0.67 & 1.08 & No & No & 0.01 & 3.57 & -1.44 & 2010.045 \\
S3-62 & 15.35 & 17.56 & Unknown Age & 33 & 11 & 0.78 & 1.20 & No & No & 0.00 & 2.70 & -1.53 & 2011.039 \\
S4-8 & 15.35 & 17.54 & Known Young & 99 & 19 & 0.64 & 1.44 & No & No & 0.00 & -0.45 & -3.97 & 2010.186 \\
S4-176 & 15.36 & 17.55 & Probable Old & 100 & 18 & 1.02 & 1.03 & No & No & 0.01 & 4.26 & 1.40 & 2010.293 \\
S5-113 & 15.36 & 17.66 & Known Old & 100 & 19 & 1.19 & 1.07 & No & No & 0.00 & -2.55 & -4.80 & 2009.454 \\
S5-178 & 15.37 & 17.54 & Known Old & 98 & 17 & 1.39 & 4.17 & No & Yes & 0.00 & 4.85 & -3.04 & 2010.330 \\
S2-41 & 15.37 & 17.58 & Known Old & 99 & 19 & 3.35 & 2.36 & Yes & No & 0.00 & -0.47 & -2.09 & 2010.303 \\
S5-212 & 15.37 & 17.50 & Known Old & 95 & 18 & 3.23 & 1.50 & Yes & No & 0.01 & 4.03 & -4.39 & 2010.182 \\
S2-59 & 15.37 & 17.79 & Known Old & 74 & 14 & 2.50 & 4.83 & Yes & Yes & 0.00 & 0.82 & -2.33 & 2009.842 \\
S3-31 & 15.38 & 17.40 & Probable Young & 59 & 17 & 2.25 & 2.43 & Yes & No & 0.00 & 3.39 & 0.39 & 2009.878 \\
S5-141 & 15.38 & 17.50 & Probable Old & 96 & 15 & 1.63 & 4.30 & No & Yes & 0.00 & 4.34 & -3.41 & 2010.171 \\
S4-279 & 15.38 & 17.65 & Unknown Age & 40 & 18 & 0.52 & 1.68 & No & No & 0.01 & 4.00 & 2.59 & 2010.027 \\
S3-21 & 15.38 & 17.58 & Probable Old & 39 & 9 & 8.06 & 58.05 & Yes & Yes & 0.00 & 3.20 & -0.21 & 2009.590 \\
S6-80 & 15.38 & 17.68 & Known Old & 72 & 18 & 1.54 & 2.20 & No & No & 0.00 & 5.03 & -4.86 & 2010.739 \\
S1-45 & 15.38 & 17.83 & Probable Old & 40 & 1 & 4.65 & \text{---} & Yes & No & 0.00 & -1.28 & 1.10 & 2009.660 \\
S5-131 & 15.39 & 17.76 & Known Old & 98 & 18 & 1.47 & 2.90 & No & No & 0.00 & 4.87 & -2.55 & 2010.240 \\
S3-159 & 15.39 & 17.85 & Probable Young & 96 & 18 & 2.66 & 1.03 & Yes & No & 0.00 & -1.29 & 3.13 & 2010.052 \\
S3-23 & 15.39 & 17.77 & Probable Old & 68 & 12 & 1.90 & 2.09 & No & No & 0.00 & 2.91 & -1.37 & 2009.964 \\
S2-81 & 15.39 & 17.78 & Known Old & 98 & 17 & 2.49 & 1.97 & Yes & No & 0.00 & 1.98 & -2.04 & 2010.068 \\
S2-68 & 15.40 & 18.12 & Probable Old & 97 & 18 & 12.94 & 4.92 & Yes & Yes & 0.00 & -1.81 & 1.95 & 2010.217 \\
S4-314 & 15.41 & 17.60 & Known Young & 99 & 19 & 0.59 & 1.97 & No & No & 0.02 & 4.41 & -2.03 & 2010.075 \\
S6-48 & 15.42 & 17.67 & Known Old & 46 & 10 & 2.18 & 3.41 & No & No & 0.01 & 4.88 & -4.16 & 2009.975 \\
S1-50 & 15.42 & 17.73 & Probable Old & 88 & 7 & 4.67 & 9.32 & Yes & Yes & 0.00 & 1.48 & 0.66 & 2009.664 \\
S0-19 & 15.43 & 17.52 & Known Young & 79 & 17 & 5.90 & 5.08 & Yes & Yes & 0.00 & -0.01 & 0.40 & 2009.642 \\
S0-28 & 15.43 & \text{---} & Known Old & 45 & 0 & 12.00 & \text{---} & Yes & \text{---} & 0.00 & -0.14 & -0.49 & 2007.822 \\
S5-165 & 15.44 & 17.65 & Known Old & 100 & 18 & 0.59 & 0.80 & No & No & 0.01 & 4.88 & -2.86 & 2010.181 \\
S2-40 & 15.44 & 17.62 & Known Young & 34 & 18 & 1.06 & 1.24 & No & No & 0.00 & 1.74 & 1.27 & 2009.828 \\
S1-175 & 15.46 & 17.66 & Unknown Age & 82 & 16 & 4.53 & 7.59 & Yes & Yes & 0.00 & -1.41 & -0.34 & 2014.063 \\
S3-314 & 15.46 & 17.56 & Known Young & 79 & 19 & 1.39 & 1.82 & No & No & 0.01 & 3.84 & -0.09 & 2010.262 \\
S4-295 & 15.46 & 17.92 & Unknown Age & 51 & 12 & 1.59 & 4.17 & No & No & 0.01 & -3.09 & 3.67 & 2010.626 \\
S0-62 & 15.46 & 17.69 & Known Old & 80 & 17 & 2.42 & 4.70 & Yes & Yes & 0.00 & 0.16 & -0.54 & 2010.228 \\
S1-6 & 15.46 & 17.77 & Known Old & 37 & 15 & 2.97 & 3.22 & Yes & No & 0.00 & -0.96 & 0.74 & 2008.886 \\
S3-383 & 15.47 & 17.74 & Known Old & 99 & 19 & 1.08 & 1.79 & No & No & 0.00 & 3.92 & -0.56 & 2010.082 \\
S2-63 & 15.47 & 17.73 & Probable Old & 100 & 18 & 1.92 & 2.44 & Yes & No & 0.00 & -0.65 & 2.47 & 2010.227 \\
S3-437 & 15.47 & 17.82 & Unknown Age & 51 & 17 & 1.38 & 1.02 & No & No & 0.00 & 2.69 & -1.38 & 2013.944 \\
S1-64 & 15.47 & 17.90 & Probable Old & 97 & 16 & 7.18 & 31.30 & Yes & Yes & 0.00 & 0.66 & 1.82 & 2010.079 \\
S6-142 & 15.47 & 17.75 & Known Old & 63 & 15 & 1.32 & 2.37 & No & No & 0.01 & 5.47 & -3.56 & 2011.172 \\
S1-66 & 15.47 & 17.72 & Known Old & 68 & 12 & 6.18 & 2.69 & Yes & No & 0.02 & -0.81 & -1.74 & 2009.970 \\
S2-308 & 15.48 & 17.64 & Known Old & 36 & 12 & 1.13 & 1.00 & No & No & 0.00 & -0.64 & -2.85 & 2010.059 \\
S5-24 & 15.48 & 18.27 & Unknown Age & 79 & 10 & 3.47 & 2.57 & Yes & No & 0.00 & -5.00 & -0.89 & 2010.110 \\
S1-26 & 15.49 & 17.71 & Known Old & 98 & 18 & 2.34 & 0.46 & Yes & No & 0.01 & -0.88 & 0.39 & 2010.306 \\
S1-62 & 15.49 & 17.88 & Probable Old & 98 & 13 & 6.02 & 9.08 & Yes & Yes & 0.01 & 0.44 & 1.80 & 2010.021 \\
S2-34 & 15.49 & 17.81 & Known Old & 95 & 16 & 1.07 & 1.60 & No & No & 0.01 & 1.84 & 1.00 & 2009.058 \\
S2-134 & 15.49 & 17.69 & Known Old & 70 & 14 & 2.98 & 3.18 & Yes & No & 0.00 & -0.99 & -2.00 & 2010.568 \\
S2-46 & 15.49 & 17.71 & Probable Young & 94 & 17 & 1.69 & 5.30 & No & Yes & 0.00 & 2.17 & -0.71 & 2010.099 \\
S3-209 & 15.50 & 17.23 & Unknown Age & 90 & 17 & 1.71 & 1.83 & No & No & 0.00 & -2.93 & -1.98 & 2010.310 \\
S5-123 & 15.50 & 18.29 & Known Old & 63 & 14 & 7.77 & 2.09 & Yes & No & 0.01 & -4.34 & -3.30 & 2009.664 \\
S1-56 & 15.50 & 18.00 & Known Old & 85 & 14 & 28.05 & 16.48 & Yes & Yes & 0.00 & -1.11 & 1.32 & 2009.763 \\
S7-2 & 15.51 & 17.81 & Unknown Age & 74 & 14 & 4.55 & 5.41 & Yes & Yes & 0.00 & 3.37 & -6.31 & 2010.793 \\
S1-55 & 15.51 & 17.89 & Probable Old & 95 & 15 & 2.51 & 7.28 & Yes & Yes & 0.00 & 1.59 & 0.64 & 2008.856 \\
S5-252 & 15.51 & 17.77 & Known Old & 80 & 15 & 3.19 & 1.33 & Yes & No & 0.01 & 5.50 & -1.23 & 2012.288 \\
S4-105 & 15.51 & 18.24 & Known Old & 100 & 18 & 1.39 & 2.26 & No & No & 0.00 & -2.82 & -3.18 & 2010.228 \\
S4-56 & 15.52 & 17.88 & Unknown Age & 71 & 10 & 1.95 & 3.62 & No & No & 0.00 & -0.99 & 3.99 & 2010.465 \\
S3-24 & 15.52 & 17.82 & Probable Young & 59 & 6 & 3.65 & 1.14 & Yes & No & 0.00 & 3.29 & 0.45 & 2009.493 \\
S3-109 & 15.52 & 17.89 & Known Old & 65 & 11 & 1.76 & 4.19 & No & No & 0.02 & -3.19 & 0.42 & 2010.197 \\
S1-47 & 15.52 & 17.74 & Probable Young & 99 & 18 & 1.85 & 9.55 & No & Yes & 0.00 & -1.61 & 0.43 & 2010.417 \\
S1-67 & 15.53 & 17.85 & Known Old & 91 & 17 & 1.64 & 3.15 & No & No & 0.00 & -1.43 & -1.32 & 2010.456 \\
S3-125 & 15.53 & 18.05 & Probable Old & 35 & 6 & 2.02 & 0.57 & No & No & 0.00 & -3.07 & -1.22 & 2010.010 \\
S5-106 & 15.53 & 17.96 & Known Young & 86 & 18 & 3.68 & 1.16 & Yes & No & 0.02 & -4.35 & -3.20 & 2010.067 \\
S2-198 & 15.54 & 17.90 & Known Old & 96 & 17 & 2.25 & 4.93 & Yes & Yes & 0.01 & 0.41 & -2.48 & 2009.978 \\
S3-377 & 15.54 & 18.01 & Unknown Age & 85 & 16 & 107.61 & 51.03 & Yes & Yes & 0.00 & 2.56 & -3.03 & 2008.170 \\
S0-67 & 15.54 & 17.79 & Known Old & 79 & 17 & 3.45 & 5.77 & Yes & Yes & 0.00 & 0.25 & -0.54 & 2009.197 \\
S5-288 & 15.55 & 17.73 & Unknown Age & 68 & 15 & 2.36 & 2.70 & Yes & No & 0.00 & 5.33 & 0.16 & 2011.188 \\
S0-29 & 15.56 & 17.60 & Known Old & 34 & 12 & 1.23 & 3.35 & No & No & 0.02 & 0.37 & -0.44 & 2009.722 \\
S3-169 & 15.56 & 17.86 & Probable Old & 100 & 18 & 0.69 & 0.87 & No & No & 0.03 & -3.39 & 0.37 & 2010.038 \\
S5-124 & 15.56 & 17.76 & Probable Young & 50 & 10 & 1.53 & 0.96 & No & No & 0.01 & -1.85 & -5.16 & 2009.615 \\
S3-92 & 15.56 & 18.11 & Probable Young & 34 & 5 & 10.00 & 12.80 & Yes & Yes & 0.00 & -1.35 & 2.88 & 2009.116 \\
S6-8 & 15.57 & 17.81 & Known Old & 91 & 18 & 1.03 & 3.75 & No & Yes & 0.00 & -0.76 & -6.01 & 2009.881 \\
S5-94 & 15.57 & 18.01 & Probable Old & 83 & 18 & 1.39 & 1.69 & No & No & 0.02 & 4.92 & 2.12 & 2008.726 \\
S1-36 & 15.57 & 17.79 & Known Old & 49 & 18 & 2.40 & 4.63 & Yes & Yes & 0.00 & -0.53 & -1.21 & 2010.227 \\
S2-83 & 15.57 & 17.89 & Known Old & 68 & 10 & 2.00 & 3.61 & No & No & 0.01 & 2.86 & -0.69 & 2009.982 \\
S2-175 & 15.58 & 18.03 & Probable Old & 51 & 13 & 10.83 & 4.06 & Yes & No & 0.00 & 2.07 & -1.21 & 2009.495 \\
S2-212 & 15.58 & 17.81 & Known Old & 95 & 17 & 2.65 & 5.41 & Yes & Yes & 0.00 & 0.17 & -2.59 & 2009.949 \\
S6-28 & 15.58 & 17.80 & Known Old & 58 & 14 & 1.02 & 0.98 & No & No & 0.02 & 5.01 & -3.66 & 2010.052 \\
S5-210 & 15.58 & 17.76 & Unknown Age & 95 & 15 & 5.88 & 8.72 & Yes & Yes & 0.00 & -1.82 & -5.66 & 2009.694 \\
S4-97 & 15.58 & 17.68 & Known Old & 100 & 19 & 0.74 & 0.41 & No & No & 0.02 & -0.95 & -4.12 & 2010.207 \\
S4-67 & 15.58 & 18.30 & Probable Old & 89 & 14 & 5.36 & 9.74 & Yes & Yes & 0.00 & 2.82 & -3.04 & 2010.016 \\
S0-27 & 15.58 & 17.79 & Known Old & 84 & 13 & 1.40 & 2.90 & No & No & 0.00 & 0.15 & 0.55 & 2009.841 \\
S5-6 & 15.58 & 18.35 & Unknown Age & 89 & 16 & 3.31 & 3.84 & Yes & No & 0.00 & -4.81 & -1.46 & 2009.544 \\
S2-80 & 15.58 & 17.78 & Known Old & 98 & 18 & 1.74 & 1.42 & No & No & 0.02 & 2.20 & 1.81 & 2010.224 \\
S6-55 & 15.58 & 17.81 & Known Old & 61 & 10 & 1.45 & 1.07 & No & No & 0.00 & 5.00 & -4.11 & 2010.196 \\
S5-80 & 15.59 & 17.78 & Unknown Age & 55 & 18 & 0.87 & 1.73 & No & No & 0.02 & 0.24 & -5.30 & 2009.782 \\
S4-280 & 15.59 & 18.05 & Probable Old & 56 & 18 & 2.28 & 1.94 & Yes & No & 0.00 & 1.23 & -4.60 & 2010.339 \\
S2-64 & 15.59 & 17.80 & Known Old & 91 & 12 & 2.05 & 4.74 & Yes & Yes & 0.01 & 2.63 & 0.25 & 2010.053 \\
S3-50 & 15.59 & 17.85 & Probable Young & 98 & 19 & 2.60 & 9.46 & Yes & Yes & 0.00 & -1.88 & -2.33 & 2010.312 \\
S2-205 & 15.59 & 17.81 & Known Old & 98 & 17 & 22.28 & 18.23 & Yes & Yes & 0.00 & 0.48 & 2.49 & 2010.052 \\
S3-108 & 15.60 & 17.80 & Unknown Age & 96 & 18 & 1.72 & 1.45 & No & No & 0.01 & -0.89 & 3.12 & 2010.133 \\
S2-317 & 15.60 & 17.89 & Known Old & 62 & 14 & 3.47 & 12.80 & Yes & Yes & 0.01 & -0.71 & -2.87 & 2010.148 \\
S4-107 & 15.60 & 17.68 & Unknown Age & 44 & 13 & 2.04 & 3.46 & No & No & 0.01 & 3.93 & 1.54 & 2011.962 \\
S1-54 & 15.61 & 18.03 & Probable Old & 89 & 15 & 4.20 & 2.64 & Yes & No & 0.01 & -1.51 & 0.75 & 2009.661 \\
S2-195 & 15.61 & 18.07 & Probable Young & 92 & 16 & 9.66 & 2.90 & Yes & No & 0.01 & -2.03 & 1.45 & 2008.883 \\
S2-42 & 15.61 & 17.98 & Probable Old & 60 & 17 & 5.04 & 3.21 & Yes & No & 0.00 & 0.49 & 2.15 & 2009.692 \\
S1-59 & 15.61 & 17.17 & Probable Old & 38 & 10 & 5.87 & 11.57 & Yes & Yes & 0.00 & 0.02 & 1.78 & 2007.241 \\
S4-40 & 15.62 & 17.93 & Known Old & 100 & 18 & 1.19 & 1.70 & No & No & 0.00 & -1.97 & -3.61 & 2010.232 \\
S1-58 & 15.62 & 17.99 & Probable Old & 76 & 15 & 3.62 & 3.77 & Yes & No & 0.01 & -1.49 & 0.97 & 2010.095 \\
S1-65 & 15.62 & 17.71 & Probable Young & 97 & 16 & 1.49 & 1.66 & No & No & 0.02 & 1.48 & 1.28 & 2009.943 \\
S2-76 & 15.62 & 18.18 & Known Young & 68 & 17 & 11.59 & 21.94 & Yes & Yes & 0.01 & -0.22 & 2.81 & 2011.550 \\
S5-44 & 15.62 & 17.83 & Known Old & 99 & 19 & 0.95 & 0.38 & No & No & 0.00 & 3.52 & -3.74 & 2010.094 \\
S4-273 & 15.62 & 17.88 & Probable Old & 100 & 19 & 1.08 & 0.71 & No & No & 0.03 & -1.15 & -4.61 & 2009.965 \\
S5-203 & 15.62 & 17.92 & Unknown Age & 50 & 10 & 4.75 & 6.71 & Yes & Yes & 0.00 & -0.23 & -5.87 & 2009.735 \\
S5-126 & 15.64 & 16.81 & Unknown Age & 98 & 19 & 1.43 & 0.80 & No & No & 0.02 & -0.04 & -5.47 & 2009.751 \\
S4-167 & 15.64 & 17.91 & Unknown Age & 96 & 18 & 1.74 & 3.14 & No & No & 0.00 & 3.73 & 2.42 & 2010.133 \\
S6-40 & 15.64 & 17.90 & Unknown Age & 79 & 14 & 3.84 & 4.12 & Yes & No & 0.01 & 0.09 & -6.34 & 2009.538 \\
S6-33 & 15.64 & 18.01 & Unknown Age & 90 & 15 & 2.92 & 4.49 & Yes & Yes & 0.02 & -3.61 & -5.09 & 2009.762 \\
S0-16 & 15.64 & 17.75 & Known Young & 44 & 11 & 19.66 & 6.28 & Yes & Yes & 0.00 & 0.23 & 0.17 & 2007.593 \\
S3-91 & 15.64 & 17.87 & Probable Young & 95 & 16 & 4.75 & 4.14 & Yes & Yes & 0.02 & -1.71 & -2.67 & 2010.365 \\
S6-53 & 15.65 & \text{---} & Unknown Age & 42 & 0 & 3.53 & \text{---} & Yes & \text{---} & 0.00 & -3.69 & -5.33 & 2009.250 \\
S3-229 & 15.65 & 18.33 & Probable Old & 84 & 16 & 5.98 & 3.84 & Yes & No & 0.00 & 1.56 & -3.22 & 2010.224 \\
S5-25 & 15.65 & 17.98 & Probable Old & 100 & 18 & 0.54 & 0.47 & No & No & 0.01 & -2.58 & -4.37 & 2010.133 \\
S3-160 & 15.66 & \text{---} & Probable Old & 36 & 0 & 3.22 & \text{---} & Yes & \text{---} & 0.00 & 3.30 & 0.79 & 2009.133 \\
S4-140 & 15.66 & 17.97 & Unknown Age & 100 & 18 & 0.66 & 0.31 & No & No & 0.00 & 3.17 & 2.98 & 2010.071 \\
S6-181 & 15.66 & 17.93 & Known Old & 94 & 16 & 1.98 & 3.17 & Yes & No & 0.02 & 5.31 & -4.21 & 2010.492 \\
S5-209 & 15.66 & 17.87 & Unknown Age & 74 & 18 & 0.77 & 0.82 & No & No & 0.02 & -2.93 & -5.15 & 2008.589 \\
S0-24 & 15.66 & 17.75 & Known Old & 71 & 17 & 5.62 & 1.68 & Yes & No & 0.00 & 0.20 & 0.09 & 2008.557 \\
S4-31 & 15.67 & 17.93 & Probable Young & 100 & 18 & 7.92 & 0.99 & Yes & No & 0.01 & -2.21 & -3.43 & 2010.415 \\
S3-263 & 15.67 & 17.85 & Probable Young & 94 & 15 & 2.41 & 0.95 & Yes & No & 0.01 & -0.40 & -3.64 & 2010.140 \\
S6-30 & 15.67 & 17.90 & Unknown Age & 82 & 16 & 1.78 & 10.22 & No & Yes & 0.03 & 0.58 & -6.20 & 2009.828 \\
S4-51 & 15.67 & 17.78 & Unknown Age & 43 & 18 & 2.68 & 8.71 & Yes & Yes & 0.01 & 3.17 & 2.63 & 2011.116 \\
S3-225 & 15.67 & 18.02 & Probable Old & 94 & 16 & 2.14 & 2.43 & Yes & No & 0.01 & 1.45 & -3.26 & 2009.856 \\
S1-40 & 15.68 & \text{---} & Probable Young & 43 & 0 & 5.89 & \text{---} & Yes & \text{---} & 0.00 & -1.41 & -0.61 & 2010.207 \\
S2-268 & 15.69 & 18.17 & Probable Old & 83 & 14 & 9.64 & 22.18 & Yes & Yes & 0.01 & -2.78 & 0.48 & 2010.071 \\
S2-319 & 15.69 & \text{---} & Known Old & 89 & 0 & 2.51 & \text{---} & Yes & \text{---} & 0.01 & 0.99 & -2.78 & 2009.644 \\
S3-256 & 15.70 & 18.19 & Probable Old & 73 & 18 & 9.27 & 12.65 & Yes & Yes & 0.00 & -1.85 & -3.18 & 2009.353 \\
S5-160 & 15.70 & \text{---} & Unknown Age & 34 & 0 & 132.84 & \text{---} & Yes & \text{---} & 0.00 & 4.23 & 3.76 & 2009.530 \\
S1-31 & 15.70 & 18.00 & Known Old & 83 & 17 & 2.00 & 3.38 & Yes & No & 0.01 & -0.99 & 0.54 & 2010.569 \\
S5-127 & 15.70 & 17.78 & Known Old & 93 & 18 & 0.81 & 1.29 & No & No & 0.03 & 4.79 & -2.64 & 2010.228 \\
S4-262 & 15.71 & 17.77 & Known Young & 98 & 18 & 11.27 & 5.79 & Yes & Yes & 0.01 & 4.28 & -1.96 & 2010.562 \\
S3-65 & 15.71 & 18.01 & Known Young & 98 & 16 & 1.27 & 2.30 & No & No & 0.03 & -1.24 & -2.80 & 2009.687 \\
S1-170 & 15.71 & \text{---} & Unknown Age & 64 & 0 & 3.67 & \text{---} & Yes & \text{---} & 0.00 & 1.57 & -1.19 & 2009.609 \\
S2-86 & 15.71 & 18.09 & Probable Old & 55 & 13 & 4.87 & 6.67 & Yes & Yes & 0.00 & 2.66 & -1.36 & 2007.744 \\
S2-208 & 15.72 & 18.44 & Probable Old & 75 & 13 & 12.12 & 10.31 & Yes & Yes & 0.00 & -2.05 & 1.58 & 2010.131 \\
S2-200 & 15.72 & 18.06 & Probable Old & 36 & 18 & 2.84 & 0.94 & Yes & No & 0.02 & -2.53 & 0.01 & 2009.425 \\
S3-59 & 15.72 & 17.89 & Probable Old & 94 & 15 & 4.12 & 1.83 & Yes & No & 0.01 & -2.42 & -1.88 & 2010.347 \\
S0-108 & 15.72 & 17.76 & Unknown Age & 54 & 10 & 3.04 & 3.77 & Yes & No & 0.00 & 0.45 & -0.90 & 2015.921 \\
S2-261 & 15.72 & 18.22 & Probable Young & 99 & 18 & 3.52 & 1.36 & Yes & No & 0.01 & -2.60 & 1.01 & 2009.671 \\
S6-36 & 15.73 & 18.18 & Known Old & 66 & 11 & 1.70 & 3.69 & No & No & 0.00 & -4.60 & -4.28 & 2009.482 \\
S6-52 & 15.74 & 17.94 & Unknown Age & 83 & 14 & 3.73 & 3.93 & Yes & No & 0.00 & -1.61 & -6.24 & 2012.171 \\
S2-51 & 15.74 & 18.12 & Known Old & 99 & 18 & 2.09 & 3.34 & Yes & No & 0.02 & 0.74 & 2.14 & 2009.837 \\
S4-123 & 15.75 & 18.10 & Unknown Age & 98 & 18 & 1.10 & 2.07 & No & No & 0.03 & 2.27 & 3.63 & 2010.065 \\
S2-128 & 15.75 & 18.16 & Probable Old & 81 & 6 & 4.47 & 13.89 & Yes & Yes & 0.00 & 1.09 & -1.89 & 2010.052 \\
S2-44 & 15.75 & 18.17 & Unknown Age & 98 & 16 & 3.20 & 16.43 & Yes & Yes & 0.01 & 0.52 & -2.14 & 2009.503 \\
S5-162 & 15.75 & 17.98 & Probable Old & 99 & 19 & 1.88 & 1.84 & Yes & No & 0.03 & 5.17 & -2.25 & 2010.076 \\
S3-151 & 15.75 & 18.06 & Known Old & 93 & 16 & 3.29 & 4.46 & Yes & Yes & 0.01 & 1.91 & -2.78 & 2009.954 \\
S3-104 & 15.75 & 18.43 & Probable Young & 68 & 12 & 11.56 & 44.77 & Yes & Yes & 0.00 & -3.17 & -0.66 & 2010.439 \\
S3-215 & 15.76 & 18.18 & Probable Old & 63 & 12 & 1.72 & 4.97 & No & Yes & 0.00 & 1.33 & -3.30 & 2010.030 \\
S2-89 & 15.76 & 18.27 & Probable Young & 90 & 9 & 4.13 & 3.38 & Yes & No & 0.02 & 1.06 & -1.69 & 2010.077 \\
S1-41 & 15.76 & 17.95 & Probable Young & 74 & 6 & 3.47 & 4.13 & Yes & No & 0.00 & 0.96 & 1.14 & 2010.300 \\
S3-176 & 15.78 & \text{---} & Probable Young & 65 & 0 & 3.62 & \text{---} & Yes & \text{---} & 0.00 & 3.09 & 1.43 & 2009.859 \\
S1-42 & 15.78 & 18.10 & Probable Old & 74 & 8 & 4.70 & 4.94 & Yes & No & 0.00 & 0.92 & 1.23 & 2010.216 \\
S5-217 & 15.78 & 18.13 & Unknown Age & 97 & 17 & 0.81 & 0.82 & No & No & 0.02 & 2.45 & -5.46 & 2010.004 \\
S3-123 & 15.79 & 17.97 & Unknown Age & 99 & 17 & 0.93 & 0.87 & No & No & 0.01 & -1.14 & -3.10 & 2009.922 \\
S0-8 & 15.79 & 17.81 & Known Young & 88 & 16 & 8.72 & 5.25 & Yes & Yes & 0.00 & -0.23 & 0.16 & 2008.370 \\
S5-150 & 15.79 & 18.22 & Known Old & 91 & 18 & 4.80 & 2.96 & Yes & No & 0.02 & -3.91 & -4.02 & 2009.922 \\
S2-14 & 15.79 & 18.16 & Probable Old & 75 & 13 & 3.59 & 2.81 & Yes & No & 0.02 & -1.56 & -1.41 & 2010.393 \\
S4-66 & 15.79 & 18.24 & Unknown Age & 80 & 15 & 8.64 & 19.29 & Yes & Yes & 0.03 & 2.73 & -3.13 & 2010.371 \\
S3-294 & 15.79 & 18.22 & Unknown Age & 87 & 13 & 2.75 & 3.51 & Yes & No & 0.01 & 0.52 & 3.75 & 2010.542 \\
S6-50 & 15.80 & 18.13 & Probable Old & 62 & 18 & 1.51 & 1.29 & No & No & 0.02 & -3.13 & -5.61 & 2008.044 \\
S4-23 & 15.80 & 18.17 & Probable Old & 98 & 18 & 4.79 & 4.60 & Yes & Yes & 0.01 & 1.47 & -3.78 & 2009.563 \\
S5-250 & 15.80 & 18.17 & Probable Old & 43 & 7 & 3.90 & 2.14 & Yes & No & 0.01 & 5.65 & -1.08 & 2011.116 \\
S5-137 & 15.80 & \text{---} & Unknown Age & 33 & 0 & 5.90 & \text{---} & Yes & \text{---} & 0.00 & 3.59 & 4.19 & 2009.603 \\
S5-216 & 15.80 & 18.22 & Unknown Age & 72 & 15 & 0.91 & 3.62 & No & No & 0.03 & 2.22 & -5.55 & 2009.968 \\
S5-79 & 15.80 & 18.02 & Probable Old & 99 & 18 & 0.56 & 1.06 & No & No & 0.01 & 4.68 & -2.46 & 2010.007 \\
S3-241 & 15.81 & 18.02 & Unknown Age & 76 & 18 & 1.21 & 2.42 & No & No & 0.00 & 2.47 & 2.68 & 2010.342 \\
S4-131 & 15.81 & 18.30 & Probable Old & 99 & 18 & 1.54 & 0.62 & No & No & 0.01 & 1.47 & -4.04 & 2010.142 \\
S4-284 & 15.81 & 18.02 & Probable Young & 98 & 16 & 1.03 & 3.12 & No & No & 0.06 & -0.95 & -4.70 & 2010.239 \\
S5-196 & 15.81 & 18.37 & Unknown Age & 65 & 16 & 5.26 & 1.40 & Yes & No & 0.00 & -4.59 & 3.59 & 2010.888 \\
S2-65 & 15.81 & 18.33 & Known Old & 96 & 17 & 12.88 & 43.80 & Yes & Yes & 0.00 & 2.36 & -1.07 & 2009.829 \\
S5-182 & 15.81 & 18.04 & Unknown Age & 47 & 5 & 3.45 & 0.03 & Yes & No & 0.00 & 5.00 & 2.86 & 2010.139 \\
S7-6 & 15.83 & 18.24 & Unknown Age & 76 & 17 & 3.81 & 2.72 & Yes & No & 0.02 & -4.07 & -6.25 & 2007.225 \\
S5-56 & 15.83 & 18.32 & Unknown Age & 45 & 11 & 1.40 & 1.69 & No & No & 0.01 & 3.62 & 3.73 & 2008.943 \\
S4-220 & 15.84 & \text{---} & Unknown Age & 34 & 0 & 1.17 & \text{---} & No & \text{---} & 0.00 & 1.95 & 4.16 & 2009.918 \\
S1-7 & 15.84 & 18.12 & Known Old & 70 & 11 & 2.24 & 4.48 & Yes & No & 0.05 & -1.05 & -0.58 & 2010.057 \\
S6-9 & 15.84 & 18.23 & Unknown Age & 97 & 16 & 5.17 & 9.10 & Yes & Yes & 0.04 & 2.59 & -5.48 & 2010.176 \\
S1-61 & 15.84 & 18.00 & Probable Old & 46 & 18 & 0.50 & 2.94 & No & No & 0.03 & -1.54 & -0.97 & 2009.863 \\
S3-357 & 15.84 & 18.14 & Unknown Age & 84 & 16 & 0.57 & 0.27 & No & No & 0.09 & 3.14 & 2.32 & 2010.033 \\
S5-84 & 15.84 & 18.27 & Probable Young & 99 & 18 & 2.88 & 1.56 & Yes & No & 0.03 & -2.74 & -4.53 & 2009.918 \\
S2-127 & 15.85 & 18.17 & Probable Old & 82 & 6 & 4.30 & 4.38 & Yes & No & 0.03 & 0.20 & -2.21 & 2010.148 \\
S2-39 & 15.85 & 18.18 & Probable Old & 100 & 18 & 0.75 & 3.35 & No & No & 0.04 & -1.94 & -0.72 & 2010.771 \\
S6-26 & 15.85 & 18.29 & Unknown Age & 92 & 16 & 4.81 & 3.23 & Yes & No & 0.01 & 2.52 & -5.68 & 2010.345 \\
S1-159 & 15.85 & \text{---} & Probable Old & 82 & 0 & 5.65 & \text{---} & Yes & \text{---} & 0.01 & 1.32 & -1.43 & 2010.637 \\
S4-187 & 15.85 & 18.44 & Probable Young & 99 & 17 & 7.05 & 36.12 & Yes & Yes & 0.02 & 0.43 & -4.48 & 2010.301 \\
S7-150 & 15.85 & 18.06 & Unknown Age & 43 & 11 & 4.03 & 1.52 & Yes & No & 0.01 & -5.00 & -5.26 & 2007.930 \\
S3-153 & 15.85 & 18.20 & Unknown Age & 100 & 18 & 2.46 & 4.09 & Yes & Yes & 0.09 & 1.60 & 2.98 & 2010.038 \\
S3-338 & 15.85 & 18.21 & Probable Old & 98 & 18 & 2.11 & 4.55 & Yes & Yes & 0.01 & -3.82 & -0.46 & 2010.136 \\
S4-50 & 15.85 & 18.31 & Unknown Age & 99 & 18 & 1.66 & 1.46 & No & No & 0.07 & 3.08 & 2.76 & 2010.565 \\
S4-283 & 15.85 & 18.21 & Probable Old & 100 & 18 & 1.80 & 5.49 & No & Yes & 0.04 & 4.38 & 1.85 & 2010.160 \\
S6-262 & 15.87 & 18.06 & Unknown Age & 48 & 11 & 1.13 & 3.49 & No & No & 0.03 & 2.49 & -6.46 & 2007.330 \\
S2-219 & 15.87 & 18.16 & Probable Old & 56 & 8 & 6.15 & 6.45 & Yes & Yes & 0.01 & -1.57 & -2.09 & 2009.939 \\
S3-167 & 15.87 & 19.40 & Probable Old & 50 & 8 & 97.12 & 171.31 & Yes & Yes & 0.00 & -3.07 & 1.41 & 2009.976 \\
S4-278 & 15.87 & 18.26 & Probable Old & 99 & 18 & 1.15 & 1.78 & No & No & 0.08 & -2.52 & -4.02 & 2010.112 \\
S3-83 & 15.87 & 18.30 & Unknown Age & 65 & 15 & 5.28 & 4.23 & Yes & Yes & 0.01 & -2.32 & -2.12 & 2009.548 \\
S4-82 & 15.89 & 18.32 & Unknown Age & 88 & 16 & 9.42 & 9.11 & Yes & Yes & 0.03 & 2.62 & 3.27 & 2010.005 \\
S3-48 & 15.89 & 18.23 & Probable Young & 94 & 18 & 2.05 & 2.23 & Yes & No & 0.03 & -2.97 & 0.36 & 2010.409 \\
S0-20 & 15.90 & 17.90 & Known Young & 67 & 16 & 3.78 & 1.78 & Yes & No & 0.01 & 0.05 & 0.14 & 2008.089 \\
S7-0 & 15.90 & 18.16 & Unknown Age & 88 & 18 & 1.34 & 1.60 & No & No & 0.10 & 4.05 & -5.79 & 2010.193 \\
S4-47 & 15.90 & 18.41 & Probable Old & 95 & 16 & 7.27 & 14.88 & Yes & Yes & 0.02 & 2.57 & -3.21 & 2009.974 \\
S3-124 & 15.90 & 18.51 & Unknown Age & 100 & 18 & 20.86 & 41.31 & Yes & Yes & 0.01 & 1.85 & 2.72 & 2009.849 \\
S4-74 & 15.91 & 18.24 & Probable Old & 99 & 17 & 1.23 & 2.25 & No & No & 0.10 & 0.12 & -4.16 & 2009.978 \\
S2-54 & 15.91 & 18.26 & Probable Old & 64 & 13 & 5.24 & 11.23 & Yes & Yes & 0.02 & 2.29 & -0.68 & 2009.512 \\
S6-19 & 15.92 & 18.33 & Probable Old & 62 & 11 & 0.99 & 3.35 & No & No & 0.02 & -4.53 & -4.15 & 2009.665 \\
S5-155 & 15.92 & 18.32 & Unknown Age & 64 & 18 & 2.01 & 1.90 & No & No & 0.02 & 4.72 & 3.02 & 2009.628 \\
S4-195 & 15.92 & 18.32 & Unknown Age & 65 & 14 & 2.60 & 3.60 & Yes & No & 0.01 & 2.42 & 3.81 & 2008.847 \\
S5-65 & 15.92 & 18.96 & Unknown Age & 59 & 15 & 31.56 & 6.19 & Yes & Yes & 0.02 & -3.81 & 3.60 & 2011.045 \\
S5-22 & 15.93 & 18.43 & Probable Young & 89 & 17 & 4.09 & 1.59 & Yes & No & 0.04 & -3.06 & -4.05 & 2009.907 \\
S2-56 & 15.93 & 18.24 & Unknown Age & 97 & 18 & 2.03 & 2.38 & Yes & No & 0.05 & -0.26 & 2.39 & 2010.441 \\
S3-302 & 15.93 & 18.44 & Unknown Age & 90 & 15 & 7.21 & 14.54 & Yes & Yes & 0.00 & 0.09 & 3.77 & 2010.134 \\
S6-229 & 15.93 & 18.10 & Probable Young & 53 & 8 & 2.08 & 1.64 & No & No & 0.01 & 5.56 & -3.51 & 2007.370 \\
S7-220 & 15.94 & 18.29 & Probable Old & 71 & 7 & 2.57 & 2.11 & Yes & No & 0.01 & -4.98 & -6.12 & 2010.839 \\
S4-154 & 15.94 & 18.34 & Unknown Age & 70 & 17 & 3.89 & 9.40 & Yes & Yes & 0.00 & 2.67 & 3.49 & 2011.661 \\
S5-4 & 15.94 & 18.30 & Probable Old & 100 & 18 & 1.15 & 0.80 & No & No & 0.03 & -2.39 & -4.42 & 2009.825 \\
S4-341 & 15.94 & 18.11 & Probable Old & 98 & 18 & 1.04 & 1.82 & No & No & 0.06 & 4.18 & -2.62 & 2009.378 \\
S3-116 & 15.94 & 18.14 & Unknown Age & 84 & 18 & 0.83 & 1.84 & No & No & 0.07 & 2.24 & 2.34 & 2010.033 \\
S6-276 & 15.94 & 18.11 & Unknown Age & 77 & 13 & 6.79 & 2.20 & Yes & No & 0.05 & 5.00 & -4.73 & 2010.832 \\
S3-171 & 15.94 & 18.13 & Unknown Age & 33 & 18 & 0.45 & 0.18 & No & No & 0.07 & 2.44 & 2.40 & 2008.434 \\
S4-164 & 15.94 & 18.30 & Unknown Age & 44 & 18 & 1.13 & 6.39 & No & Yes & 0.00 & 3.75 & 2.33 & 2010.396 \\
S2-346 & 15.95 & \text{---} & Unknown Age & 32 & 0 & 15.20 & \text{---} & Yes & \text{---} & 0.00 & -1.96 & 0.78 & 2013.182 \\
S2-304 & 15.96 & 18.10 & Probable Old & 84 & 12 & 3.51 & 2.91 & Yes & No & 0.00 & 2.52 & 1.46 & 2009.803 \\
S5-197 & 15.96 & 18.09 & Unknown Age & 54 & 8 & 2.44 & 0.34 & Yes & No & 0.07 & -1.09 & -5.73 & 2009.992 \\
S5-118 & 15.96 & 18.66 & Unknown Age & 89 & 15 & 1.19 & 1.11 & No & No & 0.11 & -4.85 & -2.44 & 2010.044 \\
S2-45 & 15.97 & 18.60 & Probable Old & 96 & 15 & 5.59 & 6.39 & Yes & Yes & 0.02 & -2.15 & 0.57 & 2009.461 \\
S4-30 & 15.97 & 18.42 & Unknown Age & 69 & 6 & 39.78 & 39.87 & Yes & Yes & 0.00 & 2.52 & 3.23 & 2009.975 \\
S4-181 & 15.97 & 18.46 & Probable Old & 92 & 16 & 2.53 & 10.42 & Yes & Yes & 0.06 & 0.96 & -4.40 & 2010.232 \\
S5-7 & 15.97 & 18.18 & Probable Old & 90 & 18 & 1.21 & 1.22 & No & No & 0.16 & 1.04 & -4.89 & 2010.172 \\
S6-51 & 15.97 & \text{---} & Unknown Age & 31 & 0 & 2.16 & \text{---} & No & \text{---} & 0.00 & 4.99 & 4.08 & 2010.134 \\
S5-259 & 15.97 & 18.32 & Probable Old & 92 & 16 & 1.83 & 3.06 & No & No & 0.14 & 5.26 & -1.88 & 2010.305 \\
S6-54 & 15.98 & 18.32 & Unknown Age & 81 & 10 & 3.48 & 16.57 & Yes & Yes & 0.00 & -1.92 & -6.18 & 2010.215 \\
S7-4 & 15.98 & 18.40 & Unknown Age & 90 & 17 & 1.90 & 5.04 & No & Yes & 0.06 & -4.27 & -6.00 & 2008.418 \\
S6-34 & 15.98 & 18.52 & Unknown Age & 66 & 16 & 5.63 & 14.98 & Yes & Yes & 0.02 & 5.28 & 3.32 & 2010.999 \\
S5-181 & 15.99 & 18.42 & Unknown Age & 47 & 13 & 3.42 & 15.81 & Yes & Yes & 0.00 & 5.06 & 2.76 & 2009.893 \\
S3-388 & 15.99 & 18.29 & Probable Young & 96 & 16 & 1.05 & 0.72 & No & No & 0.03 & -2.43 & -3.16 & 2010.340 \\
S5-49 & 15.99 & 18.39 & Probable Old & 98 & 18 & 2.87 & 5.79 & Yes & Yes & 0.00 & 4.90 & 1.61 & 2009.661 \\
S3-369 & 15.99 & 18.53 & Unknown Age & 97 & 17 & 4.99 & 2.53 & Yes & No & 0.05 & -1.97 & 3.42 & 2010.217 \\
S4-266 & 15.99 & 18.38 & Probable Young & 90 & 17 & 7.80 & 22.46 & Yes & Yes & 0.08 & 0.48 & -4.67 & 2008.269 \\
S4-55 & 16.00 & 18.28 & Unknown Age & 99 & 18 & 1.32 & 1.25 & No & No & 0.15 & 4.10 & -0.58 & 2010.204 \\
S5-200 & 16.00 & 18.59 & Unknown Age & 75 & 8 & 3.37 & 2.48 & Yes & No & 0.01 & 4.36 & 3.92 & 2010.156 \\
S1-171 & 16.00 & 18.07 & Unknown Age & 68 & 12 & 3.52 & 2.15 & Yes & No & 0.02 & -0.76 & -1.73 & 2010.726 \\
S4-157 & 16.00 & 18.65 & Unknown Age & 99 & 17 & 56.49 & 44.06 & Yes & Yes & 0.00 & -3.32 & -2.90 & 2007.382 \\
S4-109 & 16.00 & 18.40 & Probable Young & 98 & 18 & 0.46 & 0.54 & No & No & 0.19 & -2.49 & -3.44 & 2010.118 \\
S0-33 & 16.01 & 18.06 & Probable Old & 57 & 14 & 6.43 & 5.74 & Yes & Yes & 0.00 & 0.65 & -0.53 & 2010.172 \\
S6-46 & 16.02 & 18.50 & Probable Old & 78 & 10 & 4.31 & 10.79 & Yes & Yes & 0.00 & -4.00 & -4.99 & 2009.819 \\
S2-303 & 16.02 & 18.43 & Unknown Age & 77 & 13 & 8.90 & 6.57 & Yes & Yes & 0.02 & -2.91 & -0.23 & 2008.164 \\
S3-334 & 16.03 & 18.64 & Unknown Age & 76 & 11 & 5.75 & 8.56 & Yes & Yes & 0.00 & -0.60 & 3.82 & 2010.028 \\
S2-237 & 16.03 & 18.94 & Probable Old & 75 & 14 & 5.44 & 9.94 & Yes & Yes & 0.00 & -0.44 & -2.67 & 2010.546 \\
S2-300 & 16.03 & 18.52 & Unknown Age & 97 & 17 & 2.73 & 2.88 & Yes & No & 0.03 & 0.26 & 2.88 & 2010.170 \\
S1-43 & 16.03 & 18.19 & Probable Old & 89 & 12 & 3.27 & 2.38 & Yes & No & 0.01 & 1.11 & 1.21 & 2009.649 \\
S5-107 & 16.04 & 18.59 & Probable Old & 90 & 17 & 1.77 & 0.78 & No & No & 0.02 & -4.60 & -2.76 & 2009.994 \\
S6-69 & 16.05 & 18.43 & Unknown Age & 89 & 16 & 4.00 & 3.23 & Yes & No & 0.03 & -4.25 & -5.20 & 2009.190 \\
S1-144 & 16.06 & \text{---} & Probable Young & 70 & 0 & 2.51 & \text{---} & Yes & \text{---} & 0.01 & 1.63 & -0.94 & 2008.913 \\
S2-321 & 16.06 & 18.10 & Unknown Age & 95 & 16 & 1.00 & 2.29 & No & No & 0.09 & -2.43 & -1.69 & 2009.332 \\
S3-93 & 16.06 & 18.38 & Unknown Age & 59 & 8 & 5.58 & 4.78 & Yes & No & 0.00 & -2.40 & -2.11 & 2007.505 \\
S4-464 & 16.06 & 18.96 & Unknown Age & 67 & 15 & 3.83 & 6.94 & Yes & Yes & 0.01 & -4.33 & -1.23 & 2013.647 \\
S1-27 & 16.07 & 18.51 & Known Young & 56 & 12 & 58.04 & 4.02 & Yes & No & 0.01 & -1.03 & 0.19 & 2008.871 \\
S4-69 & 16.07 & 18.46 & Unknown Age & 78 & 9 & 8.88 & 7.58 & Yes & Yes & 0.00 & -3.00 & 2.83 & 2010.265 \\
S6-251 & 16.07 & 18.52 & Unknown Age & 92 & 16 & 1.82 & 2.35 & No & No & 0.05 & 3.35 & -5.99 & 2010.491 \\
S7-240 & 16.07 & 18.59 & Unknown Age & 78 & 14 & 2.86 & 2.30 & Yes & No & 0.01 & 4.78 & -6.36 & 2010.233 \\
S3-359 & 16.08 & 18.25 & Unknown Age & 95 & 16 & 2.77 & 5.39 & Yes & Yes & 0.02 & 3.75 & 1.16 & 2009.103 \\
S3-387 & 16.08 & 18.35 & Unknown Age & 74 & 12 & 3.50 & 6.05 & Yes & Yes & 0.02 & 0.63 & 3.90 & 2010.320 \\
S4-34 & 16.09 & 18.53 & Probable Young & 78 & 17 & 3.32 & 3.36 & Yes & No & 0.06 & 1.60 & -3.77 & 2009.979 \\
S6-272 & 16.09 & 18.57 & Unknown Age & 75 & 16 & 1.54 & 4.29 & No & Yes & 0.04 & 3.60 & -5.99 & 2007.070 \\
S5-128 & 16.09 & \text{---} & Unknown Age & 84 & 0 & 4.67 & \text{---} & Yes & \text{---} & 0.00 & -5.00 & 2.25 & 2007.270 \\
S4-173 & 16.10 & 18.70 & Probable Young & 100 & 17 & 7.20 & 12.82 & Yes & Yes & 0.06 & -3.20 & -3.10 & 2010.375 \\
S1-46 & 16.10 & 18.65 & Unknown Age & 89 & 16 & 10.94 & 6.72 & Yes & Yes & 0.00 & -0.10 & -1.60 & 2010.018 \\
S0-36 & 16.11 & 17.97 & Known Young & 39 & 18 & 2.42 & 1.84 & No & No & 0.01 & -0.54 & -0.73 & 2007.994 \\
S0-17 & 16.11 & 18.29 & Known Old & 89 & 16 & 10.88 & 1.14 & Yes & No & 0.01 & 0.05 & 0.01 & 2008.821 \\
S2-273 & 16.11 & 18.46 & Unknown Age & 99 & 17 & 5.53 & 6.47 & Yes & Yes & 0.04 & 0.43 & 2.81 & 2007.708 \\
S2-259 & 16.11 & 18.33 & Unknown Age & 99 & 18 & 1.10 & 1.85 & No & No & 0.11 & -2.13 & -1.77 & 2010.002 \\
S3-260 & 16.12 & 18.51 & Probable Young & 79 & 15 & 8.37 & 7.31 & Yes & Yes & 0.02 & -3.56 & 0.88 & 2007.983 \\
S6-18 & 16.12 & 18.68 & Unknown Age & 78 & 11 & 2.84 & 1.35 & Yes & No & 0.00 & 4.73 & 3.95 & 2010.269 \\
S6-41 & 16.13 & 18.24 & Unknown Age & 85 & 16 & 2.09 & 2.86 & Yes & No & 0.02 & 1.04 & -6.25 & 2007.605 \\
S6-1 & 16.13 & 18.38 & Unknown Age & 90 & 14 & 1.39 & 2.23 & No & No & 0.10 & -0.60 & -5.98 & 2007.142 \\
S5-140 & 16.13 & \text{---} & Unknown Age & 31 & 0 & 273.16 & \text{---} & Yes & \text{---} & 0.00 & -4.21 & 3.58 & 2010.701 \\
S5-61 & 16.13 & 18.08 & Unknown Age & 98 & 15 & 1.20 & 10.35 & No & Yes & 0.08 & 4.18 & -3.13 & 2007.774 \\
S2-87 & 16.13 & 18.56 & Unknown Age & 88 & 17 & 3.47 & 10.77 & Yes & Yes & 0.01 & 2.30 & -1.40 & 2007.689 \\
S6-0 & 16.14 & 18.61 & Unknown Age & 74 & 15 & 1.82 & 1.20 & No & No & 0.03 & -4.83 & 3.57 & 2008.299 \\
S4-134 & 16.14 & 18.84 & Unknown Age & 91 & 15 & 3.35 & 2.63 & Yes & No & 0.02 & -3.70 & -2.26 & 2009.842 \\
S4-133 & 16.14 & 18.24 & Unknown Age & 87 & 12 & 8.68 & 14.57 & Yes & Yes & 0.00 & 4.30 & 0.33 & 2008.007 \\
S3-258 & 16.15 & 18.28 & Unknown Age & 84 & 16 & 3.98 & 2.53 & Yes & No & 0.02 & 2.69 & -2.51 & 2010.351 \\
S2-159 & 16.15 & 18.64 & Unknown Age & 92 & 18 & 1.37 & 1.73 & No & No & 0.08 & -0.84 & 2.10 & 2010.408 \\
S1-165 & 16.16 & 18.54 & Unknown Age & 92 & 13 & 3.77 & 6.12 & Yes & Yes & 0.01 & -0.25 & -1.97 & 2010.061 \\
S5-322 & 16.17 & \text{---} & Unknown Age & 43 & 0 & 4.92 & \text{---} & Yes & \text{---} & 0.00 & -5.29 & 0.15 & 2014.113 \\
S6-16 & 16.17 & 17.31 & Unknown Age & 57 & 16 & 9.69 & 1.97 & Yes & No & 0.01 & 4.12 & -4.53 & 2007.750 \\
S3-145 & 16.18 & 18.81 & Unknown Age & 41 & 15 & 24.69 & 26.63 & Yes & Yes & 0.00 & -3.00 & 1.50 & 2007.916 \\
S1-30 & 16.18 & 18.36 & Unknown Age & 76 & 10 & 2.99 & 2.28 & Yes & No & 0.00 & 0.53 & -0.97 & 2007.247 \\
S3-212 & 16.18 & 18.11 & Unknown Age & 72 & 16 & 4.94 & 2.62 & Yes & No & 0.02 & 2.57 & -2.46 & 2011.416 \\
S4-182 & 16.19 & 18.47 & Unknown Age & 91 & 18 & 2.06 & 1.88 & Yes & No & 0.10 & 3.66 & 2.60 & 2007.448 \\
S5-3 & 16.19 & 19.17 & Probable Old & 62 & 7 & 4.97 & 18.60 & Yes & Yes & 0.02 & -3.94 & -3.10 & 2008.458 \\
S4-138 & 16.19 & 18.23 & Unknown Age & 95 & 16 & 3.24 & 3.81 & Yes & No & 0.02 & -0.53 & -4.31 & 2008.132 \\
S1-147 & 16.19 & \text{---} & Probable Young & 63 & 0 & 3.59 & \text{---} & Yes & \text{---} & 0.00 & 1.19 & -1.47 & 2007.011 \\
S5-28 & 16.20 & 18.72 & Unknown Age & 52 & 16 & 6.27 & 9.62 & Yes & Yes & 0.00 & 3.54 & 3.71 & 2011.696 \\
S3-345 & 16.21 & 18.79 & Unknown Age & 92 & 14 & 4.52 & 6.01 & Yes & Yes & 0.03 & -2.82 & -2.68 & 2007.756 \\
S3-391 & 16.21 & 18.86 & Unknown Age & 67 & 17 & 2.89 & 2.88 & Yes & No & 0.01 & -2.79 & 2.82 & 2009.882 \\
S3-58 & 16.22 & 18.87 & Unknown Age & 80 & 12 & 20.75 & 2.70 & Yes & No & 0.00 & -2.85 & -1.11 & 2007.842 \\
S2-324 & 16.22 & 18.41 & Unknown Age & 78 & 11 & 2.15 & 2.53 & Yes & No & 0.00 & -0.11 & -2.98 & 2007.349 \\
S3-103 & 16.22 & 18.64 & Unknown Age & 90 & 17 & 5.35 & 4.96 & Yes & Yes & 0.00 & 0.22 & 3.21 & 2007.658 \\
S4-9 & 16.22 & 18.45 & Unknown Age & 92 & 17 & 1.45 & 0.87 & No & No & 0.07 & 3.99 & 0.53 & 2007.696 \\
S2-20 & 16.22 & 18.90 & Unknown Age & 67 & 9 & 3.96 & 40.00 & Yes & Yes & 0.00 & 1.65 & 1.57 & 2008.605 \\
S1-118 & 16.23 & \text{---} & Unknown Age & 33 & 0 & 3.52 & \text{---} & Yes & \text{---} & 0.00 & 0.55 & 1.38 & 2007.735 \\
S5-146 & 16.24 & 18.65 & Unknown Age & 82 & 11 & 6.51 & 1.21 & Yes & No & 0.05 & 5.00 & 2.49 & 2007.776 \\
S4-126 & 16.24 & 18.60 & Unknown Age & 57 & 16 & 3.84 & 10.61 & Yes & Yes & 0.01 & 3.25 & 2.82 & 2007.635 \\
S6-47 & 16.24 & 18.48 & Unknown Age & 72 & 16 & 2.73 & 2.60 & Yes & No & 0.07 & 3.69 & -5.22 & 2008.116 \\
S6-10 & 16.25 & 18.51 & Unknown Age & 56 & 5 & 5.21 & 0.28 & Yes & No & 0.00 & 4.94 & -3.55 & 2008.315 \\
S5-18 & 16.25 & 18.29 & Unknown Age & 69 & 18 & 0.79 & 1.31 & No & No & 0.10 & 0.46 & -5.05 & 2008.352 \\
S3-237 & 16.26 & 18.84 & Unknown Age & 94 & 16 & 1.80 & 6.15 & No & Yes & 0.02 & -3.60 & -0.42 & 2008.076 \\
S6-75 & 16.26 & 18.56 & Unknown Age & 56 & 10 & 1.17 & 2.47 & No & No & 0.06 & 3.67 & -5.79 & 2007.460 \\
S6-6 & 16.26 & 18.42 & Unknown Age & 91 & 18 & 2.23 & 3.49 & Yes & No & 0.03 & -0.85 & -5.99 & 2007.846 \\
S5-1 & 16.26 & 18.66 & Unknown Age & 73 & 8 & 8.55 & 3.66 & Yes & No & 0.00 & 3.07 & 3.97 & 2007.333 \\
S3-287 & 16.27 & 18.83 & Unknown Age & 98 & 18 & 5.28 & 5.75 & Yes & Yes & 0.00 & -3.56 & 1.20 & 2007.561 \\
S4-304 & 16.27 & 18.29 & Unknown Age & 78 & 12 & 4.04 & 1.50 & Yes & No & 0.00 & 4.79 & 0.68 & 2007.720 \\
S3-381 & 16.27 & 18.88 & Unknown Age & 95 & 15 & 3.65 & 1.31 & Yes & No & 0.01 & -3.71 & 1.38 & 2007.806 \\
S2-166 & 16.28 & 18.69 & Unknown Age & 96 & 12 & 6.21 & 6.11 & Yes & Yes & 0.01 & 0.11 & 2.33 & 2008.035 \\
S5-271 & 16.28 & 18.38 & Unknown Age & 49 & 10 & 3.90 & 5.49 & Yes & Yes & 0.00 & -2.00 & -5.18 & 2008.460 \\
S1-60 & 16.29 & 18.90 & Unknown Age & 66 & 9 & 3.91 & 3.91 & Yes & No & 0.00 & -0.92 & 1.54 & 2007.856 \\
S6-45 & 16.29 & 18.52 & Unknown Age & 85 & 15 & 2.49 & 2.84 & Yes & No & 0.03 & -1.40 & -6.25 & 2007.688 \\
S4-73 & 16.30 & 18.86 & Unknown Age & 78 & 16 & 2.56 & 5.53 & Yes & Yes & 0.01 & -4.15 & -0.00 & 2007.575 \\
S4-122 & 16.30 & 18.99 & Unknown Age & 89 & 16 & 3.54 & 1.92 & Yes & No & 0.01 & -4.28 & 0.24 & 2007.929 \\
S3-61 & 16.31 & 18.86 & Unknown Age & 68 & 17 & 6.63 & 3.02 & Yes & No & 0.00 & -3.06 & -0.08 & 2008.038 \\
S3-254 & 16.32 & 18.40 & Unknown Age & 93 & 16 & 2.02 & 4.80 & Yes & Yes & 0.01 & 3.23 & 1.72 & 2007.876 \\
S3-230 & 16.33 & 18.90 & Unknown Age & 84 & 5 & 1.83 & 5.88 & No & No & 0.00 & -2.90 & -2.15 & 2007.889 \\
S5-270 & 16.33 & 18.87 & Unknown Age & 98 & 16 & 1.66 & 1.78 & No & No & 0.05 & 2.00 & -4.98 & 2007.220 \\
S1-142 & 16.33 & 18.59 & Unknown Age & 93 & 12 & 3.38 & 0.73 & Yes & No & 0.02 & 0.01 & -1.84 & 2007.341 \\
S6-187 & 16.33 & \text{---} & Unknown Age & 47 & 0 & 14.59 & \text{---} & Yes & \text{---} & 0.00 & -5.20 & 3.00 & 2007.040 \\
S2-214 & 16.33 & 18.82 & Unknown Age & 53 & 10 & 6.77 & 35.77 & Yes & Yes & 0.01 & -1.48 & -2.14 & 2007.568 \\
S5-114 & 16.34 & 19.09 & Probable Old & 67 & 16 & 3.25 & 7.83 & Yes & Yes & 0.00 & -4.50 & -3.04 & 2007.650 \\
S2-278 & 16.34 & 19.14 & Unknown Age & 57 & 13 & 7.59 & 8.85 & Yes & Yes & 0.00 & -2.21 & 1.76 & 2007.616 \\
S3-129 & 16.35 & 19.70 & Probable Old & 41 & 7 & 85.09 & 107.55 & Yes & Yes & 0.00 & -2.94 & 1.51 & 2010.280 \\
S2-269 & 16.35 & 18.59 & Unknown Age & 50 & 11 & 3.51 & 7.85 & Yes & Yes & 0.00 & -0.48 & -2.79 & 2008.170 \\
S6-244 & 16.36 & 18.92 & Unknown Age & 30 & 5 & 5.92 & 0.22 & Yes & No & 0.00 & 5.65 & 3.77 & 2006.840 \\
S2-48 & 16.36 & 19.13 & Unknown Age & 72 & 15 & 12.29 & 19.52 & Yes & Yes & 0.00 & 0.96 & 2.07 & 2007.845 \\
S4-65 & 16.36 & 18.58 & Unknown Age & 76 & 18 & 0.64 & 1.51 & No & No & 0.04 & -1.71 & -3.77 & 2008.006 \\
S2-144 & 16.37 & 19.21 & Unknown Age & 85 & 8 & 3.86 & 5.57 & Yes & No & 0.02 & -1.13 & -1.97 & 2007.254 \\
S6-17 & 16.37 & 18.61 & Unknown Age & 44 & 11 & 2.10 & 1.57 & No & No & 0.01 & 0.48 & -6.11 & 2007.682 \\
S6-348 & 16.37 & 18.68 & Unknown Age & 88 & 8 & 2.36 & 4.72 & Yes & No & 0.06 & 1.60 & -6.04 & 2016.200 \\
S4-17 & 16.39 & 18.76 & Unknown Age & 95 & 17 & 1.41 & 2.05 & No & No & 0.04 & -1.88 & 3.56 & 2007.918 \\
S6-11 & 16.39 & 18.69 & Unknown Age & 71 & 14 & 6.30 & 5.79 & Yes & Yes & 0.00 & -4.76 & -3.81 & 2007.410 \\
S0-82 & 16.40 & 18.55 & Unknown Age & 39 & 5 & 8.83 & 7.12 & Yes & No & 0.00 & 0.42 & -0.68 & 2007.268 \\
S2-229 & 16.40 & 18.58 & Unknown Age & 74 & 15 & 2.02 & 3.65 & No & No & 0.00 & -0.41 & -2.61 & 2008.234 \\
S5-59 & 16.40 & 19.12 & Unknown Age & 67 & 7 & 2.63 & 4.29 & Yes & No & 0.00 & -5.15 & -0.69 & 2007.209 \\
S7-7 & 16.40 & 18.91 & Unknown Age & 90 & 15 & 3.27 & 2.58 & Yes & No & 0.01 & -4.38 & -6.07 & 2006.984 \\
S5-204 & 16.41 & 18.49 & Unknown Age & 97 & 16 & 1.33 & 0.82 & No & No & 0.02 & 1.53 & -5.67 & 2007.877 \\
S2-299 & 16.41 & 19.22 & Unknown Age & 65 & 15 & 8.19 & 5.40 & Yes & Yes & 0.00 & -2.05 & 2.03 & 2007.537 \\
S6-43 & 16.42 & 19.38 & Unknown Age & 56 & 9 & 75.75 & 87.19 & Yes & Yes & 0.00 & 5.13 & 3.82 & 2008.931 \\
S5-175 & 16.42 & 18.87 & Unknown Age & 60 & 10 & 1.15 & 2.63 & No & No & 0.03 & 4.84 & 3.06 & 2007.999 \\
S5-260 & 16.43 & 18.77 & Unknown Age & 34 & 6 & 2.35 & 1.70 & No & No & 0.00 & 5.60 & -2.01 & 2007.510 \\
S0-61 & 16.43 & 18.46 & Known Young & 63 & 7 & 8.09 & 2.28 & Yes & No & 0.00 & -0.20 & 0.44 & 2007.638 \\
S6-188 & 16.44 & 19.35 & Unknown Age & 73 & 8 & 2.89 & 2.72 & Yes & No & 0.01 & -5.07 & -3.22 & 2007.060 \\
S5-57 & 16.44 & 18.70 & Unknown Age & 97 & 16 & 3.38 & 7.12 & Yes & Yes & 0.01 & 0.15 & -5.20 & 2007.986 \\
S0-23 & 16.44 & \text{---} & Known Young & 39 & 0 & 10.54 & \text{---} & Yes & \text{---} & 0.00 & 0.25 & -0.29 & 2008.044 \\
S5-167 & 16.45 & \text{---} & Unknown Age & 48 & 0 & 14.97 & \text{---} & Yes & \text{---} & 0.00 & 4.42 & -3.55 & 2007.721 \\
S6-214 & 16.45 & \text{---} & Unknown Age & 40 & 0 & 3.34 & \text{---} & Yes & \text{---} & 0.00 & -5.04 & 3.98 & 2006.670 \\
S1-122 & 16.45 & 18.54 & Unknown Age & 98 & 16 & 2.31 & 1.13 & Yes & No & 0.01 & -1.52 & 0.22 & 2007.579 \\
S3-289 & 16.45 & 19.82 & Unknown Age & 85 & 15 & 16.72 & 90.93 & Yes & Yes & 0.00 & -2.27 & 2.99 & 2007.802 \\
S4-223 & 16.46 & 19.41 & Unknown Age & 89 & 15 & 4.05 & 6.41 & Yes & Yes & 0.02 & -4.61 & 0.10 & 2007.690 \\
S3-143 & 16.46 & 19.53 & Probable Young & 63 & 15 & 6.70 & 9.69 & Yes & Yes & 0.01 & -3.22 & 0.91 & 2007.761 \\
S6-21 & 16.46 & 18.60 & Unknown Age & 92 & 16 & 0.85 & 1.70 & No & No & 0.02 & -1.20 & -6.03 & 2007.244 \\
S5-20 & 16.46 & 19.10 & Unknown Age & 81 & 15 & 3.48 & 3.86 & Yes & No & 0.00 & -4.86 & 1.46 & 2007.610 \\
S4-302 & 16.47 & 18.90 & Unknown Age & 96 & 17 & 1.25 & 1.69 & No & No & 0.04 & -2.82 & -3.92 & 2007.860 \\
S2-99 & 16.48 & 18.81 & Unknown Age & 59 & 5 & 3.79 & 1.31 & Yes & No & 0.00 & -1.91 & 0.69 & 2008.085 \\
S1-135 & 16.48 & 18.62 & Unknown Age & 62 & 12 & 3.23 & 5.91 & Yes & Yes & 0.01 & -0.25 & -1.75 & 2007.712 \\
S3-219 & 16.48 & 18.61 & Unknown Age & 44 & 12 & 1.35 & 0.67 & No & No & 0.02 & 2.80 & -2.23 & 2007.519 \\
S2-311 & 16.49 & 18.60 & Unknown Age & 47 & 15 & 4.22 & 5.12 & Yes & Yes & 0.00 & -2.74 & -1.04 & 2007.976 \\
S2-257 & 16.50 & 19.14 & Unknown Age & 97 & 15 & 4.96 & 2.88 & Yes & No & 0.00 & -2.73 & -0.48 & 2008.233 \\
S3-77 & 16.50 & 18.67 & Unknown Age & 89 & 18 & 1.73 & 1.91 & No & No & 0.00 & 2.32 & 2.07 & 2007.941 \\
S1-110 & 16.50 & \text{---} & Unknown Age & 35 & 0 & 22.61 & \text{---} & Yes & \text{---} & 0.00 & 1.36 & -0.51 & 2007.721 \\
S6-190 & 16.51 & 19.17 & Unknown Age & 96 & 13 & 1.71 & 5.35 & No & Yes & 0.00 & 3.79 & -4.68 & 2007.590 \\
S4-226 & 16.53 & 19.41 & Unknown Age & 47 & 15 & 2.22 & 2.19 & No & No & 0.00 & -4.61 & 0.21 & 2007.203 \\
S3-141 & 16.53 & 18.74 & Unknown Age & 96 & 16 & 3.94 & 1.46 & Yes & No & 0.00 & -0.71 & 3.27 & 2008.006 \\
S0-55 & 16.53 & 18.66 & Known Old & 81 & 17 & 2.37 & 2.03 & Yes & No & 0.00 & -0.34 & -0.36 & 2007.586 \\
S4-494 & 16.54 & 19.11 & Unknown Age & 35 & 12 & 2.62 & 4.38 & No & No & 0.00 & -4.13 & -2.51 & 2018.450 \\
S3-82 & 16.55 & 18.63 & Unknown Age & 65 & 12 & 2.40 & 2.82 & Yes & No & 0.00 & 2.81 & -1.38 & 2007.871 \\
S3-127 & 16.55 & 18.44 & Unknown Age & 70 & 12 & 5.59 & 3.91 & Yes & No & 0.00 & 2.92 & 1.62 & 2008.121 \\
S2-33 & 16.55 & 18.80 & Unknown Age & 64 & 18 & 0.88 & 1.62 & No & No & 0.00 & -1.99 & -0.17 & 2007.379 \\
S2-158 & 16.55 & 18.93 & Unknown Age & 91 & 15 & 3.39 & 2.04 & Yes & No & 0.00 & 0.62 & -2.22 & 2008.077 \\
S4-130 & 16.55 & 18.68 & Unknown Age & 88 & 17 & 1.16 & 2.31 & No & No & 0.00 & -1.29 & -4.12 & 2007.324 \\
S4-320 & 16.56 & 19.15 & Unknown Age & 36 & 12 & 3.94 & 1.77 & Yes & No & 0.00 & -4.12 & -2.63 & 2005.580 \\
S5-272 & 16.56 & 18.87 & Unknown Age & 50 & 9 & 6.02 & 2.75 & Yes & No & 0.00 & 5.58 & -0.26 & 2007.140 \\
S5-265 & 16.57 & 18.90 & Unknown Age & 99 & 16 & 2.37 & 1.16 & Yes & No & 0.00 & 2.68 & -4.50 & 2006.880 \\
S2-188 & 16.58 & 19.77 & Unknown Age & 97 & 12 & 12.86 & 20.13 & Yes & Yes & 0.00 & -1.34 & -2.09 & 2007.693 \\
S6-218 & 16.58 & 18.92 & Unknown Age & 36 & 6 & 2.67 & 7.39 & Yes & No & 0.00 & 5.68 & -3.11 & 2009.690 \\
S6-191 & 16.58 & 18.89 & Unknown Age & 87 & 14 & 10.38 & 4.01 & Yes & No & 0.00 & -4.23 & -4.29 & 2009.160 \\
S2-184 & 16.59 & 18.95 & Unknown Age & 76 & 5 & 11.52 & 12.30 & Yes & Yes & 0.00 & -2.23 & 1.00 & 2007.473 \\
S0-59 & 16.59 & 18.79 & Unknown Age & 65 & 12 & 4.05 & 6.54 & Yes & Yes & 0.00 & 0.31 & 0.41 & 2008.137 \\
S6-231 & 16.59 & 18.97 & Unknown Age & 90 & 15 & 2.98 & 1.70 & Yes & No & 0.00 & -2.58 & -6.07 & 2006.410 \\
S7-126 & 16.60 & 18.74 & Unknown Age & 97 & 16 & 1.76 & 1.57 & No & No & 0.00 & 5.00 & -5.03 & 2008.660 \\
S4-306 & 16.60 & 18.77 & Unknown Age & 72 & 14 & 5.19 & 4.42 & Yes & Yes & 0.00 & 4.84 & 0.19 & 2007.205 \\
S0-68 & 16.60 & 18.34 & Unknown Age & 54 & 6 & 5.85 & 6.63 & Yes & No & 0.00 & 0.43 & 0.49 & 2007.174 \\
S3-330 & 16.60 & 19.01 & Unknown Age & 96 & 16 & 2.56 & 1.69 & Yes & No & 0.00 & 1.63 & -3.50 & 2007.735 \\
S3-85 & 16.61 & \text{---} & Unknown Age & 58 & 0 & 1.87 & \text{---} & No & \text{---} & 0.00 & 1.24 & -2.88 & 2007.399 \\
S6-57 & 16.62 & 18.79 & Unknown Age & 95 & 16 & 1.98 & 0.77 & Yes & No & 0.00 & -3.38 & -5.56 & 2008.429 \\
S5-35 & 16.62 & 18.46 & Unknown Age & 93 & 12 & 0.66 & 0.38 & No & No & 0.00 & 3.84 & 3.39 & 2007.153 \\
S5-190 & 16.62 & \text{---} & Unknown Age & 32 & 0 & 13.92 & \text{---} & Yes & \text{---} & 0.00 & -5.34 & 2.28 & 2007.752 \\
S2-186 & 16.62 & 18.34 & Unknown Age & 91 & 16 & 3.77 & 3.58 & Yes & No & 0.00 & -2.35 & -0.74 & 2008.051 \\
S5-186 & 16.62 & 18.81 & Unknown Age & 76 & 16 & 2.59 & 3.43 & Yes & No & 0.00 & 4.02 & -4.15 & 2007.509 \\
S4-323 & 16.63 & \text{---} & Unknown Age & 30 & 0 & 1.73 & \text{---} & No & \text{---} & 0.00 & -0.76 & -4.84 & 2007.861 \\
S3-255 & 16.63 & 18.94 & Unknown Age & 91 & 9 & 5.50 & 9.18 & Yes & Yes & 0.00 & -2.81 & -2.34 & 2007.056 \\
S6-2 & 16.63 & 18.87 & Unknown Age & 90 & 16 & 3.13 & 5.27 & Yes & Yes & 0.00 & -1.65 & -5.79 & 2007.047 \\
S4-307 & 16.63 & 19.44 & Unknown Age & 88 & 15 & 2.99 & 3.32 & Yes & No & 0.00 & -4.78 & -0.71 & 2007.339 \\
S3-401 & 16.64 & 19.41 & Unknown Age & 43 & 11 & 4.14 & 3.58 & Yes & No & 0.00 & -3.12 & 2.35 & 2008.480 \\
S5-277 & 16.64 & 19.02 & Unknown Age & 56 & 11 & 4.25 & 2.57 & Yes & No & 0.00 & 5.51 & 1.50 & 2006.890 \\
S6-344 & 16.65 & 18.88 & Unknown Age & 99 & 15 & 1.36 & 1.01 & No & No & 0.00 & 3.56 & -4.88 & 2015.981 \\
S0-105 & 16.66 & \text{---} & Unknown Age & 43 & 0 & 13.54 & \text{---} & Yes & \text{---} & 0.00 & -0.24 & 0.08 & 2011.642 \\
S3-113 & 16.66 & 18.73 & Unknown Age & 59 & 8 & 5.92 & 9.69 & Yes & Yes & 0.00 & 0.21 & -3.25 & 2007.543 \\
S5-176 & 16.66 & 18.53 & Unknown Age & 33 & 16 & 2.82 & 3.94 & Yes & Yes & 0.00 & 3.53 & -4.49 & 2007.622 \\
S5-151 & 16.66 & 18.93 & Unknown Age & 99 & 16 & 7.42 & 29.96 & Yes & Yes & 0.00 & 3.56 & -4.32 & 2007.977 \\
S6-222 & 16.67 & \text{---} & Unknown Age & 70 & 0 & 4.83 & \text{---} & Yes & \text{---} & 0.00 & -2.94 & -5.81 & 2009.210 \\
S0-103 & 16.67 & 18.71 & Unknown Age & 49 & 8 & 10.27 & 12.25 & Yes & Yes & 0.00 & 0.00 & -0.13 & 2008.069 \\
S6-271 & 16.68 & 18.98 & Unknown Age & 89 & 15 & 1.90 & 3.43 & No & No & 0.00 & -3.53 & -6.03 & 2007.880 \\
S4-52 & 16.69 & 17.83 & Unknown Age & 95 & 18 & 1.50 & 0.46 & No & No & 0.00 & -0.17 & -4.12 & 2007.895 \\
S4-303 & 16.70 & 18.92 & Unknown Age & 55 & 16 & 13.15 & 11.47 & Yes & Yes & 0.00 & 4.34 & 2.14 & 2007.481 \\
S4-347 & 16.70 & 18.86 & Unknown Age & 48 & 11 & 1.79 & 4.71 & No & No & 0.00 & 4.59 & 1.87 & 2007.610 \\
S6-357 & 16.70 & 18.94 & Unknown Age & 69 & 10 & 3.76 & 0.99 & Yes & No & 0.00 & 5.27 & -3.28 & 2016.019 \\
S3-121 & 16.70 & 19.14 & Unknown Age & 65 & 16 & 3.64 & 4.34 & Yes & Yes & 0.00 & -0.06 & 3.28 & 2007.398 \\
S3-235 & 16.71 & 18.97 & Unknown Age & 66 & 5 & 4.30 & 0.89 & Yes & No & 0.00 & -0.57 & -3.57 & 2007.854 \\
S5-206 & 16.71 & 19.52 & Unknown Age & 82 & 10 & 4.13 & 4.65 & Yes & No & 0.00 & 5.30 & 2.59 & 2007.474 \\
S5-189 & 16.71 & 19.31 & Unknown Age & 87 & 11 & 6.29 & 10.54 & Yes & Yes & 0.00 & 2.93 & -5.01 & 2007.237 \\
S2-271 & 16.71 & 18.93 & Unknown Age & 89 & 9 & 3.74 & 17.97 & Yes & Yes & 0.00 & 0.73 & 2.74 & 2007.618 \\
S3-240 & 16.71 & 18.86 & Unknown Age & 45 & 12 & 15.00 & 6.08 & Yes & Yes & 0.00 & -1.27 & 3.39 & 2006.750 \\
S4-467 & 16.73 & 18.80 & Unknown Age & 81 & 14 & 1.64 & 0.44 & No & No & 0.00 & -1.19 & -3.99 & 2016.114 \\
S1-92 & 16.73 & 19.03 & Unknown Age & 86 & 17 & 2.79 & 3.06 & Yes & No & 0.00 & -1.14 & 0.49 & 2008.016 \\
S0-83 & 16.74 & 19.15 & Known Old & 87 & 13 & 3.63 & 14.38 & Yes & Yes & 0.00 & -0.36 & 0.70 & 2008.121 \\
S7-129 & 16.74 & 19.12 & Unknown Age & 32 & 14 & 2.51 & 1.47 & No & No & 0.00 & -4.80 & -5.28 & 2008.090 \\
S0-48 & 16.74 & \text{---} & Unknown Age & 36 & 0 & 85.48 & \text{---} & Yes & \text{---} & 0.00 & -0.18 & -0.30 & 2007.890 \\
S0-49 & 16.74 & 18.95 & Known Old & 91 & 7 & 4.32 & 5.81 & Yes & No & 0.00 & -0.35 & -0.12 & 2007.125 \\
S4-264 & 16.75 & 19.53 & Unknown Age & 84 & 14 & 8.08 & 9.78 & Yes & Yes & 0.00 & -4.20 & 2.09 & 2008.054 \\
S1-74 & 16.75 & 19.06 & Unknown Age & 61 & 8 & 4.55 & 2.21 & Yes & No & 0.00 & 0.98 & -0.34 & 2008.029 \\
S5-50 & 16.76 & 19.76 & Unknown Age & 93 & 16 & 12.49 & 39.82 & Yes & Yes & 0.00 & -3.99 & -3.31 & 2008.037 \\
S4-336 & 16.76 & 19.31 & Unknown Age & 97 & 15 & 5.49 & 5.00 & Yes & Yes & 0.00 & -3.66 & -3.31 & 2008.107 \\
S3-367 & 16.76 & 18.48 & Unknown Age & 96 & 16 & 1.54 & 1.35 & No & No & 0.00 & 3.39 & -1.99 & 2007.417 \\
S2-111 & 16.77 & 18.91 & Unknown Age & 86 & 14 & 17.67 & 37.67 & Yes & Yes & 0.00 & -2.09 & 0.14 & 2007.511 \\
S4-175 & 16.79 & 19.84 & Unknown Age & 84 & 15 & 2.85 & 6.59 & Yes & Yes & 0.00 & -4.40 & 0.79 & 2007.353 \\
S2-161 & 16.79 & 19.53 & Unknown Age & 32 & 7 & 4.79 & 15.09 & Yes & Yes & 0.00 & -1.47 & 1.82 & 2008.169 \\
S2-133 & 16.80 & 19.00 & Unknown Age & 59 & 10 & 2.23 & 10.07 & Yes & Yes & 0.00 & 0.52 & 2.15 & 2006.310 \\
S4-346 & 16.80 & 19.61 & Unknown Age & 83 & 11 & 3.86 & 10.34 & Yes & Yes & 0.00 & -4.95 & 0.02 & 2007.083 \\
S2-274 & 16.80 & 19.09 & Unknown Age & 77 & 12 & 3.40 & 4.77 & Yes & Yes & 0.00 & 1.27 & -2.54 & 2007.359 \\
S6-352 & 16.80 & 18.97 & Unknown Age & 76 & 15 & 1.63 & 3.11 & No & No & 0.00 & 3.25 & -5.20 & 2016.101 \\
S0-92 & 16.81 & 18.93 & Unknown Age & 53 & 11 & 10.27 & 5.63 & Yes & Yes & 0.00 & -0.79 & 0.48 & 2008.861 \\
S2-204 & 16.81 & \text{---} & Unknown Age & 68 & 0 & 3.10 & \text{---} & Yes & \text{---} & 0.00 & 0.33 & -2.54 & 2007.457 \\
S3-329 & 16.82 & \text{---} & Unknown Age & 44 & 0 & 4.09 & \text{---} & Yes & \text{---} & 0.00 & -3.20 & -2.14 & 2007.402 \\
S3-130 & 16.82 & \text{---} & Unknown Age & 34 & 0 & 5.73 & \text{---} & Yes & \text{---} & 0.00 & 3.22 & -0.84 & 2007.378 \\
S2-97 & 16.82 & 19.16 & Unknown Age & 88 & 15 & 4.80 & 8.40 & Yes & Yes & 0.00 & -2.04 & 0.29 & 2008.344 \\
S5-39 & 16.83 & 19.89 & Unknown Age & 85 & 13 & 4.39 & 1.40 & Yes & No & 0.00 & -4.73 & 1.99 & 2008.155 \\
S4-466 & 16.83 & 19.30 & Unknown Age & 95 & 16 & 5.43 & 4.86 & Yes & Yes & 0.00 & 1.95 & -4.59 & 2015.994 \\
S4-81 & 16.84 & 19.13 & Unknown Age & 59 & 12 & 4.89 & 1.24 & Yes & No & 0.00 & 2.23 & -3.52 & 2007.224 \\
S5-58 & 16.85 & 19.16 & Unknown Age & 50 & 16 & 3.58 & 2.13 & Yes & No & 0.00 & 5.01 & -1.40 & 2007.597 \\
S6-350 & 16.87 & 19.03 & Unknown Age & 84 & 12 & 3.91 & 0.79 & Yes & No & 0.00 & 2.78 & -5.34 & 2015.929 \\
S2-110 & 16.87 & 19.19 & Unknown Age & 71 & 15 & 19.46 & 51.63 & Yes & Yes & 0.00 & 1.15 & 1.75 & 2007.325 \\
S5-291 & 16.88 & 19.11 & Unknown Age & 93 & 15 & 3.17 & 3.73 & Yes & No & 0.00 & -1.97 & -5.64 & 2016.240 \\
S4-239 & 16.89 & 19.36 & Unknown Age & 90 & 15 & 1.67 & 1.04 & No & No & 0.00 & 4.61 & -0.55 & 2007.525 \\
S2-220 & 16.89 & 19.44 & Unknown Age & 92 & 15 & 3.34 & 5.43 & Yes & Yes & 0.00 & -2.48 & 0.79 & 2008.024 \\
S1-97 & 16.89 & 19.07 & Unknown Age & 37 & 15 & 4.95 & 12.39 & Yes & Yes & 0.00 & -1.00 & 0.83 & 2007.842 \\
S2-280 & 16.90 & 18.12 & Unknown Age & 80 & 16 & 1.93 & 2.00 & No & No & 0.00 & -2.52 & -1.35 & 2007.748 \\
S4-308 & 16.91 & 19.03 & Unknown Age & 62 & 8 & 3.57 & 9.96 & Yes & Yes & 0.00 & -2.91 & 3.85 & 2007.621 \\
S4-146 & 16.91 & 19.03 & Unknown Age & 59 & 12 & 4.64 & 8.75 & Yes & Yes & 0.00 & 4.09 & -1.49 & 2008.212 \\
S4-75 & 16.92 & 20.35 & Unknown Age & 88 & 12 & 21.11 & 4.92 & Yes & Yes & 0.00 & -4.05 & 0.89 & 2007.822 \\
S3-295 & 16.92 & 19.32 & Unknown Age & 47 & 15 & 3.14 & 6.18 & Yes & Yes & 0.00 & -2.42 & -2.90 & 2008.403 \\
S6-355 & 16.92 & \text{---} & Unknown Age & 73 & 0 & 1.81 & \text{---} & No & \text{---} & 0.00 & 2.09 & -5.93 & 2015.753 \\
S5-38 & 16.92 & 19.96 & Unknown Age & 87 & 13 & 3.54 & 4.70 & Yes & Yes & 0.00 & -4.77 & -1.89 & 2008.002 \\
S3-135 & 16.92 & 19.25 & Unknown Age & 56 & 13 & 2.18 & 4.52 & No & Yes & 0.00 & -0.83 & -3.23 & 2007.682 \\
S5-63 & 16.93 & 19.04 & Unknown Age & 43 & 12 & 2.35 & 5.23 & No & Yes & 0.00 & -2.11 & -4.77 & 2008.158 \\
S3-115 & 16.93 & 19.23 & Unknown Age & 65 & 11 & 2.54 & 1.42 & Yes & No & 0.00 & -3.23 & 0.49 & 2007.890 \\
S3-349 & 16.93 & 19.38 & Unknown Age & 86 & 15 & 1.81 & 3.63 & No & No & 0.00 & 1.86 & -3.42 & 2007.583 \\
S1-151 & 16.93 & 19.40 & Unknown Age & 88 & 12 & 4.94 & 8.03 & Yes & Yes & 0.00 & -1.87 & 0.25 & 2007.920 \\
S5-290 & 16.94 & 19.19 & Unknown Age & 96 & 15 & 2.71 & 5.90 & Yes & Yes & 0.00 & -2.78 & -4.65 & 2016.070 \\
S3-199 & 16.95 & 19.12 & Unknown Age & 44 & 12 & 1.97 & 1.14 & No & No & 0.00 & 2.81 & -2.14 & 2008.204 \\
S0-86 & 16.95 & 18.99 & Unknown Age & 67 & 10 & 1.75 & 0.72 & No & No & 0.00 & -0.10 & -0.85 & 2008.150 \\
S4-362 & 16.95 & 19.67 & Unknown Age & 87 & 15 & 2.15 & 9.57 & Yes & Yes & 0.00 & -4.63 & -1.90 & 2007.279 \\
S4-16 & 16.95 & 19.06 & Unknown Age & 75 & 10 & 3.29 & 2.75 & Yes & No & 0.00 & 3.41 & -2.17 & 2008.246 \\
S5-52 & 16.95 & 20.05 & Unknown Age & 88 & 11 & 4.87 & 6.99 & Yes & Yes & 0.00 & -4.68 & 2.22 & 2007.790 \\
S5-330 & 16.96 & \text{---} & Unknown Age & 38 & 0 & 6.92 & \text{---} & Yes & \text{---} & 0.00 & -5.29 & 2.73 & 2013.566 \\
S4-102 & 16.97 & 19.54 & Unknown Age & 93 & 15 & 2.81 & 5.89 & Yes & Yes & 0.00 & -3.21 & -2.74 & 2007.591 \\
S2-93 & 16.98 & 19.37 & Unknown Age & 88 & 15 & 3.85 & 6.83 & Yes & Yes & 0.00 & -1.98 & 0.37 & 2008.166 \\
S3-94 & 16.98 & 19.22 & Unknown Age & 31 & 16 & 1.01 & 4.45 & No & Yes & 0.00 & 2.08 & 2.43 & 2007.299 \\
S1-76 & 16.98 & 19.34 & Unknown Age & 37 & 11 & 4.48 & 4.80 & Yes & No & 0.00 & -0.79 & -0.73 & 2007.976 \\
S6-351 & 16.98 & 19.32 & Unknown Age & 81 & 15 & 1.97 & 2.85 & Yes & No & 0.00 & -0.90 & -6.25 & 2016.094 \\
S2-282 & 16.98 & 18.83 & Unknown Age & 97 & 17 & 1.55 & 1.45 & No & No & 0.00 & -0.49 & 2.81 & 2007.707 \\
S5-289 & 17.00 & 19.46 & Unknown Age & 98 & 15 & 1.82 & 3.96 & No & No & 0.00 & -2.44 & -5.07 & 2015.964 \\
S6-363 & 17.01 & 19.23 & Unknown Age & 64 & 10 & 2.36 & 2.34 & Yes & No & 0.00 & 5.39 & -3.27 & 2015.084 \\
S5-344 & 17.01 & 19.49 & Unknown Age & 31 & 15 & 1.89 & 3.15 & No & No & 0.00 & -4.64 & -3.51 & 2016.204 \\
S2-154 & 17.02 & 19.23 & Unknown Age & 38 & 13 & 2.32 & 6.94 & No & Yes & 0.00 & 2.27 & 0.24 & 2007.237 \\
S5-284 & 17.03 & \text{---} & Unknown Age & 69 & 0 & 34.86 & \text{---} & Yes & \text{---} & 0.00 & -5.14 & 3.08 & 2006.770 \\
S5-300 & 17.03 & 19.20 & Unknown Age & 73 & 15 & 2.79 & 2.42 & Yes & No & 0.00 & -2.99 & -5.14 & 2017.584 \\
S2-107 & 17.03 & \text{---} & Unknown Age & 58 & 0 & 3.05 & \text{---} & Yes & \text{---} & 0.00 & 0.47 & -2.03 & 2008.232 \\
S3-269 & 17.03 & 19.27 & Unknown Age & 81 & 15 & 1.59 & 1.89 & No & No & 0.00 & -0.02 & -3.70 & 2007.658 \\
S5-158 & 17.04 & 20.09 & Unknown Age & 68 & 7 & 2.05 & 1.69 & No & No & 0.00 & -5.07 & -2.46 & 2007.340 \\
S3-451 & 17.04 & 19.87 & Unknown Age & 33 & 14 & 6.65 & 2.65 & Yes & No & 0.00 & -2.90 & -0.78 & 2015.153 \\
S7-254 & 17.04 & 18.80 & Unknown Age & 30 & 10 & 2.21 & 2.01 & No & No & 0.00 & 4.44 & -6.46 & 2019.874 \\
S2-298 & 17.05 & 19.22 & Unknown Age & 68 & 10 & 3.44 & 3.08 & Yes & No & 0.00 & 2.81 & -0.74 & 2007.173 \\
S0-54 & 17.05 & 19.19 & Unknown Age & 35 & 5 & 6.20 & 1.76 & Yes & No & 0.00 & 0.01 & 0.47 & 2006.815 \\
S6-345 & 17.06 & 19.20 & Unknown Age & 93 & 16 & 1.05 & 0.64 & No & No & 0.00 & 4.65 & -4.41 & 2016.209 \\
S3-239 & 17.06 & 19.27 & Unknown Age & 52 & 16 & 5.75 & 12.94 & Yes & Yes & 0.00 & 2.74 & -2.37 & 2007.260 \\
S5-305 & 17.07 & 19.38 & Unknown Age & 70 & 13 & 2.57 & 6.92 & Yes & Yes & 0.00 & 2.15 & -5.60 & 2016.676 \\
S4-90 & 17.07 & \text{---} & Unknown Age & 53 & 0 & 2.72 & \text{---} & Yes & \text{---} & 0.00 & -1.17 & 4.01 & 2007.435 \\
S3-449 & 17.08 & 19.54 & Unknown Age & 35 & 11 & 10.58 & 12.56 & Yes & Yes & 0.00 & -1.16 & 2.79 & 2020.426 \\
S5-26 & 17.08 & 19.54 & Unknown Age & 79 & 10 & 2.48 & 1.69 & Yes & No & 0.00 & -3.36 & 3.81 & 2007.867 \\
S2-348 & 17.09 & 19.54 & Unknown Age & 47 & 10 & 5.23 & 22.79 & Yes & Yes & 0.00 & 1.32 & 2.40 & 2018.378 \\
S5-340 & 17.09 & 19.22 & Unknown Age & 33 & 11 & 1.60 & 0.37 & No & No & 0.00 & -2.14 & -4.81 & 2018.921 \\
S4-80 & 17.09 & 19.37 & Unknown Age & 31 & 15 & 1.85 & 5.15 & No & Yes & 0.00 & 2.17 & 3.56 & 2007.052 \\
S4-469 & 17.11 & 19.61 & Unknown Age & 78 & 9 & 3.65 & 3.42 & Yes & No & 0.00 & 3.16 & 3.71 & 2015.481 \\
S0-38 & 17.11 & \text{---} & Known Old & 37 & 0 & 7.06 & \text{---} & Yes & \text{---} & 0.00 & -0.18 & 0.05 & 2006.982 \\
S4-132 & 17.12 & 19.92 & Unknown Age & 74 & 15 & 3.01 & 6.79 & Yes & Yes & 0.00 & -4.24 & 0.79 & 2007.544 \\
S3-95 & 17.13 & 19.35 & Unknown Age & 95 & 15 & 4.29 & 2.84 & Yes & No & 0.00 & 1.70 & 2.70 & 2007.293 \\
S1-124 & 17.13 & 19.40 & Unknown Age & 57 & 11 & 6.46 & 1.17 & Yes & No & 0.00 & -0.56 & -1.47 & 2007.595 \\
S4-360 & 17.13 & \text{---} & Unknown Age & 49 & 0 & 120.41 & \text{---} & Yes & \text{---} & 0.00 & -4.03 & 2.92 & 2007.749 \\
S4-128 & 17.13 & 19.91 & Unknown Age & 86 & 15 & 6.13 & 18.01 & Yes & Yes & 0.00 & 1.27 & -4.12 & 2007.980 \\
S4-292 & 17.13 & 19.78 & Unknown Age & 73 & 15 & 2.15 & 2.67 & Yes & No & 0.00 & -3.89 & -2.80 & 2007.450 \\
S5-297 & 17.14 & 19.22 & Unknown Age & 78 & 16 & 1.47 & 1.68 & No & No & 0.00 & 1.17 & -5.27 & 2016.188 \\
S3-232 & 17.14 & 19.75 & Unknown Age & 97 & 15 & 2.98 & 12.44 & Yes & Yes & 0.00 & -3.56 & 0.66 & 2007.423 \\
S4-465 & 17.14 & 19.81 & Unknown Age & 96 & 15 & 1.95 & 2.00 & Yes & No & 0.00 & -2.92 & -3.65 & 2015.924 \\
S4-322 & 17.15 & 19.36 & Unknown Age & 64 & 7 & 5.61 & 2.51 & Yes & No & 0.00 & 4.29 & 2.36 & 2008.324 \\
S5-184 & 17.15 & 19.49 & Unknown Age & 85 & 11 & 4.82 & 1.31 & Yes & No & 0.00 & 4.47 & 3.68 & 2007.943 \\
S0-40 & 17.16 & 19.17 & Known Young & 82 & 15 & 7.51 & 4.46 & Yes & Yes & 0.00 & -0.23 & -0.10 & 2007.193 \\
S5-323 & 17.16 & 19.41 & Unknown Age & 43 & 15 & 2.70 & 2.36 & Yes & No & 0.00 & -2.29 & -5.14 & 2015.964 \\
S2-109 & 17.17 & 19.40 & Unknown Age & 46 & 9 & 2.28 & 2.19 & No & No & 0.00 & 1.62 & 1.36 & 2008.071 \\
S5-194 & 17.17 & 19.85 & Unknown Age & 84 & 13 & 11.66 & 20.24 & Yes & Yes & 0.00 & 4.77 & 3.39 & 2006.855 \\
S2-119 & 17.19 & 19.51 & Unknown Age & 30 & 13 & 1.88 & 5.29 & No & Yes & 0.00 & 1.68 & 1.34 & 2007.655 \\
S3-64 & 17.19 & \text{---} & Unknown Age & 31 & 0 & 6.22 & \text{---} & Yes & \text{---} & 0.00 & -2.90 & -1.00 & 2007.668 \\
S7-245 & 17.19 & 19.52 & Unknown Age & 62 & 13 & 4.23 & 4.58 & Yes & Yes & 0.00 & 5.22 & -4.72 & 2016.104 \\
S2-288 & 17.19 & 19.01 & Unknown Age & 60 & 10 & 4.26 & 3.78 & Yes & No & 0.00 & 0.12 & -2.87 & 2008.656 \\
S2-315 & 17.20 & 19.82 & Unknown Age & 72 & 14 & 15.49 & 24.96 & Yes & Yes & 0.00 & -0.73 & 2.85 & 2007.563 \\
S5-135 & 17.20 & 19.33 & Unknown Age & 66 & 12 & 5.87 & 0.64 & Yes & No & 0.00 & 3.99 & -3.80 & 2007.978 \\
S4-477 & 17.20 & 19.67 & Unknown Age & 54 & 15 & 3.96 & 10.57 & Yes & Yes & 0.00 & -3.45 & 2.43 & 2019.607 \\
S3-201 & 17.20 & 19.34 & Unknown Age & 95 & 15 & 2.00 & 3.93 & Yes & No & 0.00 & -1.12 & -3.35 & 2008.154 \\
S2-130 & 17.20 & 19.48 & Unknown Age & 62 & 11 & 5.99 & 6.97 & Yes & Yes & 0.00 & -1.59 & -1.53 & 2007.595 \\
S4-108 & 17.21 & 19.55 & Unknown Age & 53 & 8 & 7.30 & 5.14 & Yes & No & 0.00 & -3.92 & -1.57 & 2008.333 \\
S5-154 & 17.21 & 19.97 & Unknown Age & 76 & 7 & 1.89 & 3.24 & No & No & 0.00 & -5.00 & -2.55 & 2007.746 \\
S3-379 & 17.22 & 19.47 & Unknown Age & 72 & 11 & 3.38 & 1.07 & Yes & No & 0.00 & 3.74 & -1.32 & 2007.363 \\
S2-173 & 17.22 & 19.57 & Unknown Age & 76 & 15 & 2.45 & 3.87 & Yes & No & 0.00 & -0.38 & 2.36 & 2007.618 \\
S6-367 & 17.23 & 19.69 & Unknown Age & 57 & 6 & 4.95 & 2.55 & Yes & No & 0.00 & -3.13 & -5.80 & 2017.737 \\
S2-191 & 17.23 & \text{---} & Unknown Age & 51 & 0 & 5.77 & \text{---} & Yes & \text{---} & 0.00 & 0.30 & 2.46 & 2007.865 \\
S5-292 & 17.24 & 19.59 & Unknown Age & 91 & 15 & 2.41 & 6.79 & Yes & Yes & 0.00 & 0.86 & -5.71 & 2016.148 \\
S5-37 & 17.25 & 19.36 & Unknown Age & 52 & 8 & 2.97 & 3.00 & Yes & No & 0.00 & 5.00 & 1.19 & 2007.485 \\
S4-39 & 17.25 & 19.59 & Unknown Age & 44 & 5 & 2.61 & 3.01 & Yes & No & 0.00 & 3.69 & 1.82 & 2007.162 \\
S3-332 & 17.25 & 19.34 & Unknown Age & 33 & 5 & 7.59 & 3.34 & Yes & No & 0.00 & 0.78 & -3.77 & 2007.360 \\
S5-293 & 17.26 & 19.41 & Unknown Age & 87 & 15 & 6.65 & 5.93 & Yes & Yes & 0.00 & -1.44 & -5.04 & 2016.501 \\
S0-75 & 17.26 & 19.19 & Unknown Age & 59 & 13 & 2.33 & 4.28 & Yes & No & 0.00 & -0.14 & -0.73 & 2008.744 \\
S4-363 & 17.26 & 20.07 & Unknown Age & 72 & 7 & 3.16 & 4.76 & Yes & No & 0.00 & -4.98 & -0.52 & 2007.392 \\
S4-49 & 17.26 & 19.95 & Unknown Age & 82 & 14 & 4.99 & 4.86 & Yes & Yes & 0.00 & -4.11 & 0.41 & 2007.707 \\
S4-120 & 17.27 & \text{---} & Unknown Age & 33 & 0 & 6.03 & \text{---} & Yes & \text{---} & 0.00 & 1.18 & 4.10 & 2007.690 \\
S5-169 & 17.27 & 19.52 & Unknown Age & 60 & 10 & 4.48 & 7.01 & Yes & Yes & 0.00 & 4.84 & 3.00 & 2007.975 \\
S4-309 & 17.27 & 19.45 & Unknown Age & 39 & 7 & 3.70 & 1.21 & Yes & No & 0.00 & 4.76 & 0.93 & 2007.555 \\
S2-301 & 17.27 & 19.83 & Unknown Age & 74 & 15 & 4.51 & 8.70 & Yes & Yes & 0.00 & -2.30 & 1.75 & 2008.276 \\
S3-194 & 17.27 & 19.60 & Unknown Age & 82 & 15 & 2.67 & 1.56 & Yes & No & 0.00 & 2.12 & 2.79 & 2007.719 \\
S5-179 & 17.28 & 19.54 & Unknown Age & 63 & 11 & 3.54 & 2.53 & Yes & No & 0.00 & 3.86 & -4.24 & 2007.747 \\
S5-309 & 17.28 & \text{---} & Unknown Age & 60 & 0 & 9.50 & \text{---} & Yes & \text{---} & 0.00 & -1.83 & -5.43 & 2015.499 \\
S3-324 & 17.28 & \text{---} & Unknown Age & 52 & 0 & 6.99 & \text{---} & Yes & \text{---} & 0.00 & 3.55 & 1.47 & 2007.934 \\
S4-101 & 17.29 & 19.01 & Unknown Age & 70 & 10 & 1.82 & 3.49 & No & No & 0.00 & 1.52 & 3.94 & 2008.144 \\
S5-295 & 17.30 & \text{---} & Unknown Age & 81 & 0 & 11.75 & \text{---} & Yes & \text{---} & 0.00 & -4.91 & 2.71 & 2016.278 \\
S5-304 & 17.30 & 19.70 & Unknown Age & 71 & 6 & 61.77 & 23.77 & Yes & Yes & 0.00 & 5.11 & -1.20 & 2016.044 \\
S1-94 & 17.30 & 19.38 & Unknown Age & 74 & 14 & 2.69 & 2.73 & Yes & No & 0.00 & -0.98 & -0.80 & 2007.982 \\
S4-78 & 17.31 & 20.56 & Unknown Age & 78 & 6 & 16.49 & 31.10 & Yes & Yes & 0.00 & -4.03 & -1.05 & 2007.642 \\
S7-243 & 17.32 & 19.65 & Unknown Age & 77 & 9 & 4.39 & 2.79 & Yes & No & 0.00 & 5.06 & -5.20 & 2015.826 \\
S1-81 & 17.34 & 19.47 & Unknown Age & 33 & 9 & 4.42 & 47.11 & Yes & Yes & 0.00 & -0.88 & -0.79 & 2007.536 \\
S2-135 & 17.34 & 19.75 & Unknown Age & 72 & 14 & 4.41 & 4.10 & Yes & No & 0.00 & 1.49 & 1.64 & 2007.395 \\
S4-324 & 17.35 & 19.37 & Unknown Age & 91 & 15 & 2.26 & 0.57 & Yes & No & 0.00 & 4.90 & -0.14 & 2007.918 \\
S3-440 & 17.35 & 19.64 & Unknown Age & 91 & 15 & 13.66 & 9.46 & Yes & Yes & 0.00 & -0.81 & -3.88 & 2016.072 \\
S6-373 & 17.36 & \text{---} & Unknown Age & 52 & 0 & 1.75 & \text{---} & No & \text{---} & 0.00 & 1.42 & -6.32 & 2016.566 \\
S5-320 & 17.36 & \text{---} & Unknown Age & 49 & 0 & 5.29 & \text{---} & Yes & \text{---} & 0.00 & -0.17 & -5.59 & 2015.209 \\
S1-148 & 17.37 & 19.45 & Unknown Age & 35 & 12 & 2.74 & 2.66 & Yes & No & 0.00 & -0.34 & -1.85 & 2008.438 \\
S1-95 & 17.38 & 19.44 & Unknown Age & 76 & 15 & 2.66 & 4.96 & Yes & Yes & 0.00 & -1.23 & 0.27 & 2007.640 \\
S2-291 & 17.38 & 19.60 & Unknown Age & 89 & 15 & 1.26 & 0.97 & No & No & 0.00 & 2.04 & 2.04 & 2007.858 \\
S6-346 & 17.39 & 19.59 & Unknown Age & 91 & 15 & 1.42 & 1.85 & No & No & 0.00 & 3.85 & -5.10 & 2016.189 \\
S4-33 & 17.41 & 19.63 & Unknown Age & 62 & 14 & 2.78 & 1.36 & Yes & No & 0.00 & 3.61 & 1.93 & 2007.687 \\
S5-326 & 17.41 & 19.64 & Unknown Age & 39 & 15 & 2.29 & 5.79 & No & Yes & 0.00 & -1.60 & -5.19 & 2016.007 \\
S0-106 & 17.42 & 19.42 & Unknown Age & 42 & 11 & 3.69 & 2.46 & Yes & No & 0.00 & -0.20 & 0.23 & 2011.642 \\
S5-42 & 17.42 & 20.23 & Unknown Age & 60 & 13 & 22.64 & 6.29 & Yes & Yes & 0.00 & 2.69 & -4.36 & 2008.117 \\
S2-265 & 17.42 & 19.34 & Unknown Age & 52 & 15 & 2.92 & 8.39 & Yes & Yes & 0.00 & 2.26 & 1.65 & 2007.724 \\
S6-347 & 17.43 & 19.55 & Unknown Age & 90 & 15 & 6.50 & 5.23 & Yes & Yes & 0.00 & 4.73 & -4.70 & 2016.276 \\
S6-376 & 17.45 & \text{---} & Unknown Age & 48 & 0 & 6.14 & \text{---} & Yes & \text{---} & 0.00 & -2.81 & -6.30 & 2015.478 \\
S4-204 & 17.45 & 20.06 & Unknown Age & 93 & 13 & 5.85 & 7.13 & Yes & Yes & 0.00 & -3.15 & 3.27 & 2007.375 \\
S3-242 & 17.46 & 20.13 & Unknown Age & 78 & 7 & 7.07 & 3.10 & Yes & No & 0.00 & -3.04 & 1.95 & 2007.782 \\
S4-200 & 17.46 & 19.49 & Unknown Age & 95 & 15 & 7.60 & 0.82 & Yes & No & 0.00 & 4.40 & -1.10 & 2007.936 \\
S6-378 & 17.48 & 19.35 & Unknown Age & 46 & 7 & 3.85 & 5.26 & Yes & No & 0.00 & 4.82 & -4.20 & 2014.504 \\
S4-32 & 17.49 & 20.07 & Unknown Age & 69 & 13 & 2.96 & 3.22 & Yes & No & 0.00 & -2.31 & 3.36 & 2007.863 \\
S3-45 & 17.49 & 20.21 & Unknown Age & 57 & 13 & 2.96 & 5.96 & Yes & Yes & 0.00 & -2.10 & 2.16 & 2008.003 \\
S0-60 & 17.50 & 19.73 & Unknown Age & 92 & 14 & 3.93 & 1.81 & Yes & No & 0.00 & -0.48 & -0.12 & 2007.783 \\
S0-63 & 17.50 & 20.03 & Unknown Age & 93 & 14 & 4.96 & 9.60 & Yes & Yes & 0.00 & -0.45 & -0.28 & 2008.270 \\
S5-108 & 17.50 & \text{---} & Unknown Age & 71 & 0 & 2.43 & \text{---} & Yes & \text{---} & 0.00 & 4.03 & -3.57 & 2007.201 \\
S4-148 & 17.50 & 20.50 & Unknown Age & 47 & 8 & 4.83 & 12.34 & Yes & Yes & 0.00 & -3.79 & 2.14 & 2007.837 \\
S3-298 & 17.51 & 19.78 & Unknown Age & 90 & 14 & 4.72 & 1.65 & Yes & No & 0.00 & 2.92 & 2.40 & 2007.984 \\
S6-387 & 17.52 & 19.79 & Unknown Age & 34 & 10 & 2.70 & 2.93 & Yes & No & 0.00 & 5.49 & -4.11 & 2017.243 \\
S6-360 & 17.52 & 20.04 & Unknown Age & 64 & 5 & 4.19 & 3.87 & Yes & No & 0.00 & -5.08 & 3.42 & 2015.069 \\
S4-110 & 17.52 & \text{---} & Unknown Age & 42 & 0 & 2.24 & \text{---} & No & \text{---} & 0.00 & -1.22 & 4.05 & 2007.266 \\
S3-277 & 17.52 & 19.62 & Unknown Age & 82 & 14 & 8.44 & 5.19 & Yes & Yes & 0.00 & -2.08 & -3.08 & 2007.800 \\
S2-297 & 17.52 & 19.75 & Unknown Age & 87 & 12 & 1.51 & 2.11 & No & No & 0.00 & -1.06 & -2.70 & 2006.906 \\
S4-488 & 17.52 & 19.50 & Unknown Age & 40 & 10 & 1.16 & 0.41 & No & No & 0.00 & 4.05 & -1.53 & 2016.508 \\
S5-325 & 17.53 & 19.93 & Unknown Age & 40 & 6 & 3.03 & 6.50 & Yes & No & 0.00 & 5.62 & -1.80 & 2018.108 \\
S6-349 & 17.53 & 19.83 & Unknown Age & 85 & 14 & 7.44 & 4.43 & Yes & Yes & 0.00 & 3.45 & -5.78 & 2016.241 \\
S6-13 & 17.53 & \text{---} & Unknown Age & 42 & 0 & 3.76 & \text{---} & Yes & \text{---} & 0.00 & 4.23 & -4.41 & 2008.208 \\
S4-235 & 17.53 & 19.86 & Unknown Age & 84 & 13 & 3.69 & 6.53 & Yes & Yes & 0.00 & 4.32 & -1.66 & 2007.759 \\
S4-298 & 17.53 & 19.60 & Unknown Age & 87 & 15 & 3.52 & 1.42 & Yes & No & 0.00 & 4.82 & -0.11 & 2007.635 \\
S4-484 & 17.54 & \text{---} & Unknown Age & 42 & 0 & 3.10 & \text{---} & Yes & \text{---} & 0.00 & 1.03 & -4.25 & 2016.029 \\
S6-359 & 17.54 & 19.60 & Unknown Age & 66 & 13 & 3.37 & 4.67 & Yes & Yes & 0.00 & -3.36 & -5.34 & 2015.878 \\
S4-43 & 17.54 & 19.91 & Unknown Age & 65 & 14 & 2.25 & 1.35 & Yes & No & 0.00 & 1.68 & -3.77 & 2007.913 \\
S5-172 & 17.55 & 20.30 & Unknown Age & 89 & 9 & 3.88 & 7.61 & Yes & Yes & 0.00 & 5.30 & 2.13 & 2007.201 \\
S1-152 & 17.56 & 20.09 & Unknown Age & 52 & 11 & 5.42 & 31.24 & Yes & Yes & 0.00 & 1.09 & 1.55 & 2006.887 \\
S7-251 & 17.57 & \text{---} & Unknown Age & 39 & 0 & 11.41 & \text{---} & Yes & \text{---} & 0.00 & -4.87 & -5.23 & 2014.384 \\
S5-171 & 17.57 & \text{---} & Unknown Age & 34 & 0 & 5.03 & \text{---} & Yes & \text{---} & 0.00 & 4.10 & -3.96 & 2008.818 \\
S5-329 & 17.57 & 19.63 & Unknown Age & 39 & 11 & 3.15 & 2.52 & Yes & No & 0.00 & 0.26 & -5.26 & 2019.583 \\
S6-361 & 17.57 & \text{---} & Unknown Age & 64 & 0 & 3.35 & \text{---} & Yes & \text{---} & 0.00 & -5.06 & 3.53 & 2015.108 \\
S6-356 & 17.58 & 19.72 & Unknown Age & 70 & 11 & 2.80 & 3.23 & Yes & No & 0.00 & 5.48 & -3.86 & 2017.003 \\
S6-370 & 17.58 & 20.13 & Unknown Age & 54 & 5 & 3.74 & 33.64 & Yes & Yes & 0.00 & -3.16 & -5.93 & 2016.618 \\
S2-260 & 17.58 & \text{---} & Unknown Age & 34 & 0 & 3.89 & \text{---} & Yes & \text{---} & 0.00 & -2.37 & 1.48 & 2007.551 \\
S2-90 & 17.59 & 19.88 & Unknown Age & 35 & 5 & 4.90 & 0.90 & Yes & No & 0.00 & -1.32 & -1.51 & 2007.507 \\
S4-291 & 17.60 & 19.86 & Unknown Age & 94 & 15 & 3.68 & 8.59 & Yes & Yes & 0.00 & 4.40 & -1.91 & 2007.966 \\
S2-231 & 17.61 & 19.96 & Unknown Age & 77 & 14 & 4.51 & 2.54 & Yes & No & 0.00 & -2.58 & -0.63 & 2008.033 \\
S5-16 & 17.62 & 19.92 & Unknown Age & 79 & 9 & 2.49 & 6.52 & Yes & Yes & 0.00 & 3.33 & 3.81 & 2007.908 \\
S6-369 & 17.62 & 19.74 & Unknown Age & 56 & 10 & 5.78 & 6.34 & Yes & Yes & 0.00 & 3.60 & -5.78 & 2015.502 \\
S1-149 & 17.62 & \text{---} & Unknown Age & 44 & 0 & 2.19 & \text{---} & No & \text{---} & 0.00 & -1.65 & -0.91 & 2007.869 \\
S5-195 & 17.62 & 19.84 & Unknown Age & 63 & 9 & 4.62 & 2.68 & Yes & No & 0.00 & 3.88 & -4.37 & 2008.161 \\
S4-338 & 17.63 & 19.99 & Unknown Age & 92 & 14 & 2.09 & 2.09 & Yes & No & 0.00 & 3.46 & -3.49 & 2007.765 \\
S4-476 & 17.64 & \text{---} & Unknown Age & 55 & 0 & 2.19 & \text{---} & No & \text{---} & 0.00 & 0.52 & -4.35 & 2016.574 \\
S7-241 & 17.64 & 19.95 & Unknown Age & 84 & 15 & 4.00 & 9.31 & Yes & Yes & 0.00 & 4.43 & -5.80 & 2016.334 \\
S3-234 & 17.65 & 20.28 & Unknown Age & 76 & 11 & 6.43 & 4.34 & Yes & No & 0.00 & -3.52 & 0.86 & 2007.533 \\
S3-252 & 17.66 & 19.67 & Unknown Age & 42 & 12 & 2.66 & 2.90 & Yes & No & 0.00 & 2.74 & 2.41 & 2007.715 \\
S5-294 & 17.66 & 19.98 & Unknown Age & 83 & 15 & 4.03 & 4.80 & Yes & Yes & 0.00 & 0.58 & -5.30 & 2016.154 \\
S1-164 & 17.66 & 19.85 & Unknown Age & 75 & 12 & 2.00 & 1.75 & No & No & 0.00 & -1.98 & -0.01 & 2007.890 \\
S6-358 & 17.67 & 19.88 & Unknown Age & 69 & 13 & 3.94 & 5.48 & Yes & Yes & 0.00 & -3.07 & -5.24 & 2016.533 \\
S6-368 & 17.67 & 20.08 & Unknown Age & 56 & 10 & 8.53 & 13.68 & Yes & Yes & 0.00 & -3.05 & -5.65 & 2016.663 \\
S4-150 & 17.68 & 20.28 & Unknown Age & 82 & 9 & 11.53 & 23.62 & Yes & Yes & 0.00 & -2.95 & -3.24 & 2007.685 \\
S2-142 & 17.68 & 20.04 & Unknown Age & 33 & 13 & 5.57 & 5.70 & Yes & Yes & 0.00 & -2.16 & -0.63 & 2007.754 \\
S6-371 & 17.69 & \text{---} & Unknown Age & 53 & 0 & 4.30 & \text{---} & Yes & \text{---} & 0.00 & -4.68 & 3.92 & 2014.386 \\
S5-332 & 17.69 & 19.93 & Unknown Age & 37 & 6 & 6.08 & 7.70 & Yes & Yes & 0.00 & 5.54 & -0.44 & 2018.690 \\
S3-342 & 17.69 & 20.08 & Unknown Age & 90 & 14 & 1.77 & 2.25 & No & No & 0.00 & 1.59 & 3.55 & 2008.229 \\
S3-53 & 17.70 & 20.07 & Unknown Age & 39 & 8 & 3.89 & 14.33 & Yes & Yes & 0.00 & 2.99 & -0.54 & 2008.317 \\
S4-127 & 17.70 & 19.88 & Unknown Age & 40 & 10 & 4.39 & 7.13 & Yes & Yes & 0.00 & 4.14 & -1.21 & 2008.367 \\
S5-207 & 17.71 & 20.14 & Unknown Age & 92 & 14 & 1.47 & 5.26 & No & Yes & 0.00 & 4.88 & 3.35 & 2007.009 \\
S2-193 & 17.71 & 19.91 & Unknown Age & 58 & 15 & 2.40 & 5.08 & Yes & Yes & 0.00 & -2.22 & -1.13 & 2007.408 \\
S4-472 & 17.73 & 19.99 & Unknown Age & 71 & 9 & 3.11 & 5.77 & Yes & Yes & 0.00 & -1.55 & -4.42 & 2016.088 \\
S4-89 & 17.73 & 20.06 & Unknown Age & 47 & 6 & 9.98 & 15.16 & Yes & Yes & 0.00 & 3.18 & 2.73 & 2006.912 \\
S5-53 & 17.74 & 20.52 & Unknown Age & 67 & 8 & 11.23 & 26.50 & Yes & Yes & 0.00 & -3.63 & -3.70 & 2008.423 \\
S4-478 & 17.74 & 20.18 & Unknown Age & 52 & 8 & 3.30 & 2.06 & Yes & No & 0.00 & 1.39 & -4.65 & 2014.184 \\
S4-194 & 17.75 & 20.07 & Unknown Age & 66 & 11 & 4.98 & 12.01 & Yes & Yes & 0.00 & 4.26 & 1.50 & 2007.762 \\
S2-91 & 17.75 & 19.99 & Unknown Age & 55 & 9 & 1.72 & 0.88 & No & No & 0.00 & -1.95 & -0.49 & 2007.639 \\
S5-317 & 17.75 & 19.52 & Unknown Age & 52 & 15 & 5.12 & 1.74 & Yes & No & 0.00 & 1.41 & -5.83 & 2015.498 \\
S4-470 & 17.76 & 19.97 & Unknown Age & 77 & 15 & 4.80 & 1.75 & Yes & No & 0.00 & 0.45 & -4.73 & 2016.820 \\
S3-293 & 17.76 & 19.60 & Unknown Age & 94 & 11 & 6.27 & 3.71 & Yes & No & 0.00 & 2.25 & 3.03 & 2007.629 \\
S4-485 & 17.76 & 19.93 & Unknown Age & 41 & 6 & 5.94 & 5.98 & Yes & No & 0.00 & -0.53 & -4.56 & 2014.603 \\
S7-244 & 17.77 & 19.69 & Unknown Age & 64 & 10 & 2.46 & 11.95 & Yes & Yes & 0.00 & 4.57 & -5.73 & 2016.092 \\
S4-260 & 17.78 & 20.47 & Unknown Age & 36 & 7 & 3.81 & 4.35 & Yes & No & 0.00 & -4.67 & 0.24 & 2006.715 \\
S3-158 & 17.78 & 19.48 & Unknown Age & 78 & 15 & 2.43 & 2.02 & Yes & No & 0.00 & 0.95 & 3.26 & 2008.199 \\
S6-380 & 17.79 & \text{---} & Unknown Age & 44 & 0 & 6.25 & \text{---} & Yes & \text{---} & 0.00 & -2.29 & -5.76 & 2017.191 \\
S1-77 & 17.79 & 19.94 & Unknown Age & 32 & 12 & 3.22 & 1.27 & Yes & No & 0.00 & -1.00 & 0.51 & 2006.440 \\
S6-375 & 17.80 & 19.93 & Unknown Age & 51 & 10 & 2.22 & 3.02 & No & No & 0.00 & -3.17 & -5.69 & 2018.510 \\
S4-57 & 17.80 & 20.19 & Unknown Age & 55 & 15 & 2.12 & 1.41 & No & No & 0.00 & 3.47 & 2.25 & 2007.822 \\
S7-242 & 17.80 & 20.13 & Unknown Age & 82 & 11 & 2.85 & 3.16 & Yes & No & 0.00 & -4.82 & -5.84 & 2016.086 \\
S4-222 & 17.81 & 20.16 & Unknown Age & 51 & 15 & 2.09 & 0.97 & No & No & 0.00 & 1.97 & -4.16 & 2007.217 \\
S5-311 & 17.81 & 19.90 & Unknown Age & 57 & 10 & 3.50 & 2.02 & Yes & No & 0.00 & -0.04 & -5.18 & 2015.219 \\
S2-284 & 17.81 & 19.85 & Unknown Age & 34 & 14 & 5.13 & 2.35 & Yes & No & 0.00 & -2.80 & -0.63 & 2006.890 \\
S3-389 & 17.81 & 20.01 & Unknown Age & 59 & 5 & 3.61 & 1.41 & Yes & No & 0.00 & 3.58 & -1.74 & 2007.749 \\
S5-298 & 17.82 & 20.05 & Unknown Age & 76 & 14 & 4.11 & 1.28 & Yes & No & 0.00 & -2.52 & -4.59 & 2016.087 \\
S4-99 & 17.86 & 20.02 & Unknown Age & 93 & 15 & 2.20 & 1.40 & Yes & No & 0.00 & 3.40 & 2.51 & 2007.705 \\
S1-157 & 17.86 & 20.21 & Unknown Age & 34 & 7 & 5.45 & 6.53 & Yes & No & 0.00 & -1.56 & -1.11 & 2006.470 \\
S4-178 & 17.87 & 20.41 & Unknown Age & 94 & 14 & 4.58 & 3.09 & Yes & No & 0.00 & 3.59 & 2.69 & 2007.823 \\
S4-192 & 17.87 & 20.11 & Unknown Age & 84 & 15 & 3.68 & 3.10 & Yes & No & 0.00 & 1.70 & -4.18 & 2008.171 \\
S5-338 & 17.87 & 20.12 & Unknown Age & 34 & 15 & 1.81 & 7.95 & No & Yes & 0.00 & -2.20 & -5.54 & 2016.261 \\
S5-343 & 17.88 & 20.22 & Unknown Age & 31 & 6 & 2.88 & 8.36 & Yes & Yes & 0.00 & -4.61 & -3.53 & 2016.737 \\
S4-337 & 17.88 & 20.21 & Unknown Age & 86 & 10 & 2.66 & 2.19 & Yes & No & 0.00 & -3.34 & 3.61 & 2007.315 \\
S4-329 & 17.89 & \text{---} & Unknown Age & 48 & 0 & 5.06 & \text{---} & Yes & \text{---} & 0.00 & 2.73 & 4.09 & 2007.185 \\
S4-199 & 17.89 & 20.15 & Unknown Age & 51 & 8 & 6.93 & 6.79 & Yes & Yes & 0.00 & 4.54 & -0.09 & 2008.021 \\
S5-82 & 17.91 & 19.90 & Unknown Age & 55 & 6 & 2.25 & 4.79 & Yes & No & 0.00 & 3.96 & -3.50 & 2007.776 \\
S6-365 & 17.91 & \text{---} & Unknown Age & 58 & 0 & 3.67 & \text{---} & Yes & \text{---} & 0.00 & 4.04 & -5.03 & 2015.903 \\
S2-263 & 17.91 & 20.22 & Unknown Age & 95 & 14 & 4.81 & 10.74 & Yes & Yes & 0.00 & -2.80 & 0.15 & 2007.972 \\
S6-353 & 17.91 & 20.29 & Unknown Age & 73 & 9 & 7.35 & 8.67 & Yes & Yes & 0.00 & 4.95 & -4.52 & 2015.795 \\
S3-78 & 17.92 & \text{---} & Unknown Age & 45 & 0 & 3.75 & \text{---} & Yes & \text{---} & 0.00 & -2.08 & -2.33 & 2007.967 \\
S3-165 & 17.93 & 20.24 & Unknown Age & 37 & 8 & 5.03 & 6.26 & Yes & Yes & 0.00 & 0.78 & 3.31 & 2006.260 \\
S4-141 & 17.94 & 19.60 & Unknown Age & 81 & 15 & 2.99 & 1.94 & Yes & No & 0.00 & -4.32 & -0.60 & 2007.161 \\
S5-342 & 17.94 & \text{---} & Unknown Age & 32 & 0 & 10.20 & \text{---} & Yes & \text{---} & 0.00 & 1.82 & -4.95 & 2012.803 \\
S6-384 & 17.94 & 20.08 & Unknown Age & 36 & 6 & 1.53 & 3.35 & No & No & 0.00 & 0.41 & -6.16 & 2014.976 \\
S4-479 & 17.95 & 20.17 & Unknown Age & 52 & 10 & 7.90 & 5.73 & Yes & Yes & 0.00 & 2.34 & -3.78 & 2015.331 \\
S5-74 & 17.95 & 19.68 & Unknown Age & 48 & 6 & 3.02 & 1.36 & Yes & No & 0.00 & 4.02 & -3.36 & 2008.317 \\
S1-177 & 17.95 & \text{---} & Unknown Age & 41 & 0 & 8.47 & \text{---} & Yes & \text{---} & 0.00 & -1.31 & -0.96 & 2015.119 \\
S6-362 & 17.96 & 19.96 & Unknown Age & 64 & 8 & 1.94 & 2.72 & No & No & 0.00 & 4.45 & -4.83 & 2016.152 \\
S2-285 & 17.97 & \text{---} & Unknown Age & 35 & 0 & 3.76 & \text{---} & Yes & \text{---} & 0.00 & -2.04 & -2.02 & 2007.312 \\
S5-318 & 17.97 & 20.58 & Unknown Age & 50 & 11 & 4.21 & 6.68 & Yes & Yes & 0.00 & -4.43 & -3.35 & 2018.802 \\
S2-312 & 17.97 & 20.30 & Unknown Age & 46 & 10 & 3.15 & 12.25 & Yes & Yes & 0.00 & -2.54 & 1.47 & 2007.991 \\
S3-396 & 17.98 & 20.01 & Unknown Age & 72 & 6 & 1.80 & 3.54 & No & No & 0.00 & 0.94 & 3.89 & 2007.805 \\
S3-442 & 17.98 & 20.15 & Unknown Age & 60 & 9 & 7.83 & 2.51 & Yes & No & 0.00 & 0.49 & 2.98 & 2016.871 \\
S4-300 & 17.99 & 19.86 & Unknown Age & 81 & 12 & 4.43 & 2.44 & Yes & No & 0.00 & 4.67 & -1.21 & 2007.929 \\
S4-286 & 17.99 & 20.20 & Unknown Age & 83 & 14 & 3.37 & 2.85 & Yes & No & 0.00 & 4.77 & -0.35 & 2008.015 \\
S4-497 & 17.99 & \text{---} & Unknown Age & 31 & 0 & 12.12 & \text{---} & Yes & \text{---} & 0.00 & 3.11 & 2.57 & 2014.447 \\
S5-164 & 17.99 & 20.18 & Unknown Age & 77 & 12 & 1.53 & 1.62 & No & No & 0.00 & 4.66 & 3.22 & 2006.980 \\
S4-27 & 17.99 & 20.35 & Unknown Age & 88 & 5 & 14.68 & 4.52 & Yes & No & 0.00 & 2.73 & 3.04 & 2007.630 \\
S6-364 & 18.00 & 20.22 & Unknown Age & 60 & 13 & 2.62 & 2.69 & Yes & No & 0.00 & -4.53 & -5.15 & 2016.937 \\
S3-204 & 18.00 & 20.26 & Unknown Age & 92 & 13 & 3.77 & 1.73 & Yes & No & 0.00 & 2.45 & 2.56 & 2007.807 \\
S3-218 & 18.00 & 20.12 & Unknown Age & 30 & 12 & 2.17 & 1.37 & No & No & 0.00 & 2.92 & 2.07 & 2008.283 \\
S3-224 & 18.00 & 20.01 & Unknown Age & 89 & 15 & 2.14 & 1.81 & Yes & No & 0.00 & -2.86 & 2.16 & 2007.901 \\
S5-333 & 18.00 & 20.66 & Unknown Age & 36 & 5 & 5.13 & 1.13 & Yes & No & 0.00 & 2.62 & -4.84 & 2015.764 \\
S3-110 & 18.01 & 20.10 & Unknown Age & 53 & 15 & 2.66 & 1.38 & Yes & No & 0.00 & -2.09 & 2.46 & 2007.287 \\
S2-266 & 18.02 & 20.11 & Unknown Age & 34 & 6 & 7.81 & 6.59 & Yes & No & 0.00 & -0.79 & -2.70 & 2007.856 \\
S6-379 & 18.02 & 20.40 & Unknown Age & 45 & 10 & 3.45 & 4.67 & Yes & No & 0.00 & -4.23 & -5.41 & 2016.400 \\
S2-168 & 18.02 & 20.26 & Unknown Age & 56 & 11 & 2.62 & 0.98 & Yes & No & 0.00 & -2.33 & 0.31 & 2007.709 \\
S1-88 & 18.03 & 20.34 & Unknown Age & 40 & 11 & 3.75 & 5.55 & Yes & Yes & 0.00 & -0.43 & -1.18 & 2006.691 \\
S7-249 & 18.03 & \text{---} & Unknown Age & 41 & 0 & 3.32 & \text{---} & Yes & \text{---} & 0.00 & -5.03 & -5.06 & 2014.142 \\
S5-319 & 18.03 & 20.12 & Unknown Age & 49 & 14 & 2.98 & 2.61 & Yes & No & 0.00 & 1.34 & -5.35 & 2016.238 \\
S6-372 & 18.03 & 20.13 & Unknown Age & 52 & 15 & 3.12 & 1.61 & Yes & No & 0.00 & 4.17 & -5.52 & 2015.989 \\
S3-214 & 18.04 & \text{---} & Unknown Age & 38 & 0 & 6.58 & \text{---} & Yes & \text{---} & 0.00 & -1.88 & -3.04 & 2007.960 \\
S3-74 & 18.04 & \text{---} & Unknown Age & 59 & 0 & 9.34 & \text{---} & Yes & \text{---} & 0.00 & -3.09 & 0.02 & 2007.971 \\
S4-489 & 18.04 & 20.25 & Unknown Age & 40 & 5 & 7.75 & 2.84 & Yes & No & 0.00 & -0.05 & -4.79 & 2018.370 \\
S5-104 & 18.04 & \text{---} & Unknown Age & 61 & 0 & 17.32 & \text{---} & Yes & \text{---} & 0.00 & -3.71 & 3.87 & 2007.630 \\
S3-444 & 18.04 & 20.36 & Unknown Age & 41 & 8 & 3.61 & 3.76 & Yes & No & 0.00 & -1.66 & -3.45 & 2015.710 \\
S7-253 & 18.05 & \text{---} & Unknown Age & 30 & 0 & 2.47 & \text{---} & No & \text{---} & 0.00 & -4.80 & -6.30 & 2015.269 \\
S5-32 & 18.05 & \text{---} & Unknown Age & 60 & 0 & 3.97 & \text{---} & Yes & \text{---} & 0.00 & 3.28 & 3.93 & 2007.549 \\
S1-96 & 18.05 & 20.24 & Unknown Age & 36 & 11 & 3.55 & 2.08 & Yes & No & 0.00 & -0.06 & -1.28 & 2007.777 \\
S4-333 & 18.05 & 20.29 & Unknown Age & 54 & 6 & 6.42 & 5.07 & Yes & No & 0.00 & -2.99 & 3.88 & 2007.821 \\
S4-70 & 18.07 & \text{---} & Unknown Age & 32 & 0 & 8.51 & \text{---} & Yes & \text{---} & 0.00 & -2.37 & 3.38 & 2007.644 \\
S5-201 & 18.07 & \text{---} & Unknown Age & 44 & 0 & 6.51 & \text{---} & Yes & \text{---} & 0.00 & 5.06 & 2.98 & 2007.640 \\
S4-496 & 18.08 & 20.26 & Unknown Age & 31 & 8 & 10.50 & 15.10 & Yes & Yes & 0.00 & -1.98 & -4.12 & 2020.693 \\
S7-247 & 18.08 & \text{---} & Unknown Age & 44 & 0 & 2.48 & \text{---} & Yes & \text{---} & 0.00 & 3.65 & -6.33 & 2018.079 \\
S5-315 & 18.09 & 20.29 & Unknown Age & 53 & 7 & 1.66 & 3.73 & No & No & 0.00 & 3.83 & -4.24 & 2016.773 \\
S4-361 & 18.10 & \text{---} & Unknown Age & 59 & 0 & 3.95 & \text{---} & Yes & \text{---} & 0.00 & 4.57 & -2.04 & 2007.296 \\
S5-301 & 18.11 & 20.47 & Unknown Age & 72 & 12 & 3.50 & 2.07 & Yes & No & 0.00 & 5.09 & -0.41 & 2016.410 \\
S3-226 & 18.11 & 20.78 & Unknown Age & 40 & 8 & 9.31 & 7.79 & Yes & Yes & 0.00 & -3.56 & -0.61 & 2007.832 \\
S4-270 & 18.12 & 20.59 & Unknown Age & 43 & 6 & 3.60 & 9.45 & Yes & Yes & 0.00 & -3.81 & -2.79 & 2007.590 \\
S6-383 & 18.12 & \text{---} & Unknown Age & 38 & 0 & 4.51 & \text{---} & Yes & \text{---} & 0.00 & 4.68 & -5.18 & 2014.140 \\
S3-251 & 18.12 & \text{---} & Unknown Age & 30 & 0 & 7.30 & \text{---} & Yes & \text{---} & 0.00 & 3.57 & -0.67 & 2007.970 \\
S5-62 & 18.12 & 20.24 & Unknown Age & 59 & 6 & 2.51 & 2.15 & Yes & No & 0.00 & 4.40 & -2.80 & 2008.501 \\
S2-178 & 18.13 & 20.35 & Unknown Age & 40 & 13 & 8.13 & 0.99 & Yes & No & 0.00 & -2.12 & -1.13 & 2007.750 \\
S7-246 & 18.14 & \text{---} & Unknown Age & 59 & 0 & 3.08 & \text{---} & Yes & \text{---} & 0.00 & -3.89 & -6.19 & 2015.256 \\
S3-41 & 18.17 & 20.57 & Unknown Age & 71 & 12 & 3.52 & 2.03 & Yes & No & 0.00 & -2.93 & 0.63 & 2008.562 \\
S4-491 & 18.17 & 20.79 & Unknown Age & 39 & 8 & 5.06 & 4.92 & Yes & No & 0.00 & -4.39 & 0.38 & 2016.768 \\
S5-17 & 18.17 & 20.37 & Unknown Age & 70 & 15 & 3.31 & 4.52 & Yes & Yes & 0.00 & 2.84 & -4.19 & 2007.415 \\
S4-318 & 18.18 & \text{---} & Unknown Age & 45 & 0 & 3.58 & \text{---} & Yes & \text{---} & 0.00 & -4.85 & -0.47 & 2007.749 \\
S3-280 & 18.21 & 20.54 & Unknown Age & 34 & 7 & 3.82 & 15.23 & Yes & Yes & 0.00 & -2.39 & -2.87 & 2008.086 \\
S3-443 & 18.21 & 20.27 & Unknown Age & 46 & 11 & 2.44 & 1.36 & Yes & No & 0.00 & 2.94 & -2.04 & 2018.099 \\
S5-347 & 18.22 & \text{---} & Unknown Age & 30 & 0 & 6.55 & \text{---} & Yes & \text{---} & 0.00 & 5.61 & -1.90 & 2018.862 \\
S4-473 & 18.22 & 20.18 & Unknown Age & 63 & 12 & 5.33 & 5.04 & Yes & Yes & 0.00 & -1.38 & -4.25 & 2016.025 \\
S2-330 & 18.22 & 19.41 & Unknown Age & 59 & 14 & 2.32 & 1.21 & Yes & No & 0.00 & 0.71 & 2.91 & 2007.961 \\
S5-324 & 18.23 & 20.54 & Unknown Age & 41 & 7 & 3.96 & 1.79 & Yes & No & 0.00 & 4.21 & -2.81 & 2013.913 \\
S5-77 & 18.23 & 20.71 & Unknown Age & 85 & 12 & 5.11 & 8.67 & Yes & Yes & 0.00 & 2.98 & -4.33 & 2008.150 \\
S5-310 & 18.24 & 20.66 & Unknown Age & 59 & 7 & 2.56 & 9.97 & Yes & Yes & 0.00 & 5.28 & -2.61 & 2015.906 \\
S4-214 & 18.24 & \text{---} & Unknown Age & 57 & 0 & 5.48 & \text{---} & Yes & \text{---} & 0.00 & -3.77 & 2.54 & 2007.739 \\
S6-374 & 18.25 & 20.46 & Unknown Age & 51 & 9 & 5.32 & 0.61 & Yes & No & 0.00 & 5.29 & -3.98 & 2016.255 \\
S2-350 & 18.25 & 20.56 & Unknown Age & 36 & 10 & 1.22 & 6.22 & No & Yes & 0.00 & -2.39 & -0.20 & 2019.980 \\
S5-306 & 18.26 & 20.76 & Unknown Age & 62 & 9 & 3.89 & 0.75 & Yes & No & 0.00 & 5.10 & -2.18 & 2016.068 \\
S4-136 & 18.26 & 20.31 & Unknown Age & 81 & 13 & 3.68 & 1.90 & Yes & No & 0.00 & 4.27 & -0.68 & 2007.552 \\
S5-312 & 18.27 & 20.38 & Unknown Age & 55 & 13 & 3.69 & 2.88 & Yes & No & 0.00 & 0.41 & -5.23 & 2015.612 \\
S1-176 & 18.27 & \text{---} & Unknown Age & 52 & 0 & 4.34 & \text{---} & Yes & \text{---} & 0.00 & -1.40 & -1.17 & 2015.450 \\
S4-327 & 18.28 & \text{---} & Unknown Age & 51 & 0 & 3.80 & \text{---} & Yes & \text{---} & 0.00 & -3.60 & 3.33 & 2007.484 \\
S3-361 & 18.28 & 20.57 & Unknown Age & 49 & 5 & 3.71 & 2.75 & Yes & No & 0.00 & 2.91 & 2.63 & 2007.554 \\
S4-471 & 18.29 & 20.60 & Unknown Age & 76 & 13 & 2.29 & 3.49 & Yes & No & 0.00 & -1.74 & -3.68 & 2015.575 \\
S2-239 & 18.29 & 20.32 & Unknown Age & 77 & 10 & 2.30 & 4.21 & Yes & No & 0.00 & 1.43 & 2.30 & 2007.331 \\
S4-468 & 18.29 & 20.17 & Unknown Age & 79 & 15 & 1.69 & 1.99 & No & No & 0.00 & 2.00 & -4.32 & 2016.251 \\
S0-80 & 18.29 & 20.41 & Unknown Age & 36 & 10 & 2.03 & 1.65 & No & No & 0.00 & -0.74 & 0.24 & 2007.266 \\
S4-190 & 18.30 & \text{---} & Unknown Age & 65 & 0 & 5.16 & \text{---} & Yes & \text{---} & 0.00 & 4.41 & -0.98 & 2008.773 \\
S3-373 & 18.31 & 20.68 & Unknown Age & 77 & 5 & 6.53 & 1.15 & Yes & No & 0.00 & 1.77 & 3.52 & 2008.229 \\
S5-303 & 18.31 & 20.84 & Unknown Age & 71 & 6 & 5.32 & 0.91 & Yes & No & 0.00 & 5.35 & -0.86 & 2015.548 \\
S5-302 & 18.31 & 20.45 & Unknown Age & 72 & 12 & 1.81 & 0.74 & No & No & 0.00 & 1.28 & -5.13 & 2016.427 \\
S5-339 & 18.32 & \text{---} & Unknown Age & 33 & 0 & 2.20 & \text{---} & No & \text{---} & 0.00 & 3.46 & -4.54 & 2013.266 \\
S5-299 & 18.33 & 20.94 & Unknown Age & 73 & 5 & 3.41 & 9.55 & Yes & Yes & 0.00 & -4.81 & -3.29 & 2015.877 \\
S3-448 & 18.33 & \text{---} & Unknown Age & 36 & 0 & 5.27 & \text{---} & Yes & \text{---} & 0.00 & 0.10 & 3.12 & 2019.127 \\
S4-294 & 18.33 & 20.38 & Unknown Age & 42 & 13 & 1.38 & 5.68 & No & Yes & 0.00 & 4.71 & -0.94 & 2007.718 \\
S7-252 & 18.34 & \text{---} & Unknown Age & 31 & 0 & 3.73 & \text{---} & Yes & \text{---} & 0.00 & 5.36 & -4.89 & 2019.139 \\
S2-202 & 18.34 & 20.66 & Unknown Age & 66 & 9 & 3.43 & 1.98 & Yes & No & 0.00 & -2.51 & 0.32 & 2008.137 \\
S6-42 & 18.34 & \text{---} & Unknown Age & 64 & 0 & 3.33 & \text{---} & Yes & \text{---} & 0.00 & 5.32 & 3.48 & 2008.243 \\
S3-447 & 18.36 & \text{---} & Unknown Age & 37 & 0 & 4.32 & \text{---} & Yes & \text{---} & 0.00 & -0.04 & 3.32 & 2018.059 \\
S4-354 & 18.36 & 20.59 & Unknown Age & 77 & 7 & 10.75 & 7.97 & Yes & Yes & 0.00 & 4.32 & 2.49 & 2007.407 \\
S5-321 & 18.37 & 20.71 & Unknown Age & 47 & 10 & 4.32 & 3.55 & Yes & No & 0.00 & 1.87 & -5.13 & 2016.957 \\
S4-490 & 18.37 & \text{---} & Unknown Age & 39 & 0 & 5.82 & \text{---} & Yes & \text{---} & 0.00 & -3.15 & -3.22 & 2017.075 \\
S1-146 & 18.38 & \text{---} & Unknown Age & 32 & 0 & 7.51 & \text{---} & Yes & \text{---} & 0.00 & -1.75 & -0.71 & 2007.050 \\
S5-54 & 18.39 & \text{---} & Unknown Age & 31 & 0 & 4.34 & \text{---} & Yes & \text{---} & 0.00 & -5.03 & -1.27 & 2006.994 \\
S4-58 & 18.40 & \text{---} & Unknown Age & 33 & 0 & 4.83 & \text{---} & Yes & \text{---} & 0.00 & -1.48 & 3.85 & 2008.356 \\
S4-203 & 18.40 & 20.62 & Unknown Age & 75 & 14 & 6.07 & 1.77 & Yes & No & 0.00 & 4.51 & -0.56 & 2007.180 \\
S6-386 & 18.41 & 20.45 & Unknown Age & 35 & 5 & 2.09 & 1.71 & No & No & 0.00 & 4.55 & -4.74 & 2015.016 \\
S4-248 & 18.42 & \text{---} & Unknown Age & 41 & 0 & 1.96 & \text{---} & No & \text{---} & 0.00 & 3.83 & 2.67 & 2007.825 \\
S4-486 & 18.42 & 20.73 & Unknown Age & 41 & 7 & 2.79 & 2.33 & Yes & No & 0.00 & 1.65 & -4.42 & 2016.299 \\
S4-335 & 18.44 & 20.89 & Unknown Age & 80 & 10 & 2.89 & 3.35 & Yes & No & 0.00 & 2.40 & -4.29 & 2008.294 \\
S6-366 & 18.44 & 20.39 & Unknown Age & 58 & 5 & 5.45 & 3.15 & Yes & No & 0.00 & 3.68 & -4.95 & 2016.292 \\
S3-454 & 18.45 & \text{---} & Unknown Age & 31 & 0 & 1.28 & \text{---} & No & \text{---} & 0.00 & 2.05 & 2.34 & 2015.907 \\
S3-253 & 18.45 & 20.63 & Unknown Age & 55 & 5 & 5.14 & 0.80 & Yes & No & 0.00 & -0.20 & 3.63 & 2007.262 \\
S4-205 & 18.46 & 21.12 & Unknown Age & 73 & 5 & 2.47 & 6.38 & Yes & No & 0.00 & -4.50 & -0.65 & 2007.447 \\
S2-230 & 18.46 & 20.78 & Unknown Age & 74 & 12 & 2.28 & 2.91 & Yes & No & 0.00 & -2.64 & 0.16 & 2007.897 \\
S4-480 & 18.46 & 20.63 & Unknown Age & 49 & 12 & 2.01 & 3.77 & No & No & 0.00 & -1.34 & -3.99 & 2016.418 \\
S3-231 & 18.49 & 20.22 & Unknown Age & 67 & 14 & 2.92 & 3.70 & Yes & No & 0.00 & -0.44 & 3.58 & 2008.003 \\
S2-123 & 18.51 & 20.74 & Unknown Age & 33 & 7 & 3.29 & 1.87 & Yes & No & 0.00 & -2.15 & -0.18 & 2007.940 \\
S6-354 & 18.53 & 21.03 & Unknown Age & 73 & 7 & 2.89 & 3.33 & Yes & No & 0.00 & 3.78 & -5.39 & 2015.860 \\
S6-385 & 18.55 & \text{---} & Unknown Age & 35 & 0 & 4.24 & \text{---} & Yes & \text{---} & 0.00 & -2.35 & -6.15 & 2012.730 \\
S5-307 & 18.55 & 20.50 & Unknown Age & 61 & 10 & 5.68 & 5.03 & Yes & No & 0.00 & 1.17 & -5.52 & 2016.562 \\
S3-211 & 18.55 & \text{---} & Unknown Age & 42 & 0 & 7.21 & \text{---} & Yes & \text{---} & 0.00 & -0.96 & 3.41 & 2008.258 \\
S4-293 & 18.55 & \text{---} & Unknown Age & 32 & 0 & 2.70 & \text{---} & No & \text{---} & 0.00 & 4.27 & -2.18 & 2007.530 \\
S4-495 & 18.56 & \text{---} & Unknown Age & 33 & 0 & 2.97 & \text{---} & Yes & \text{---} & 0.00 & -1.88 & -4.02 & 2013.449 \\
S5-314 & 18.56 & 20.66 & Unknown Age & 54 & 9 & 2.17 & 1.41 & No & No & 0.00 & 1.46 & -5.30 & 2015.473 \\
S5-328 & 18.58 & \text{---} & Unknown Age & 39 & 0 & 4.41 & \text{---} & Yes & \text{---} & 0.00 & 2.13 & -5.08 & 2017.292 \\
S6-388 & 18.58 & 20.65 & Unknown Age & 33 & 7 & 2.09 & 1.59 & No & No & 0.00 & 1.08 & -5.94 & 2016.708 \\
S4-482 & 18.59 & \text{---} & Unknown Age & 43 & 0 & 3.46 & \text{---} & Yes & \text{---} & 0.00 & 2.69 & 3.60 & 2016.197 \\
S3-446 & 18.59 & 20.88 & Unknown Age & 41 & 8 & 3.14 & 2.69 & Yes & No & 0.00 & -1.72 & -3.54 & 2019.551 \\
S3-445 & 18.59 & \text{---} & Unknown Age & 41 & 0 & 6.89 & \text{---} & Yes & \text{---} & 0.00 & -1.96 & -3.35 & 2013.836 \\
S3-170 & 18.59 & 20.60 & Unknown Age & 43 & 10 & 7.23 & 5.76 & Yes & Yes & 0.00 & -3.26 & 1.00 & 2008.606 \\
S4-501 & 18.60 & 21.12 & Unknown Age & 30 & 7 & 8.68 & 1.94 & Yes & No & 0.00 & -2.77 & -4.06 & 2016.955 \\
S5-308 & 18.62 & 20.51 & Unknown Age & 60 & 13 & 2.93 & 0.80 & Yes & No & 0.00 & 1.42 & -5.48 & 2016.124 \\
S4-475 & 18.63 & 20.90 & Unknown Age & 57 & 8 & 3.08 & 2.51 & Yes & No & 0.00 & -2.09 & -4.30 & 2015.891 \\
S3-244 & 18.63 & \text{---} & Unknown Age & 52 & 0 & 3.64 & \text{---} & Yes & \text{---} & 0.00 & -2.04 & 3.00 & 2007.694 \\
S5-331 & 18.64 & 20.76 & Unknown Age & 37 & 7 & 5.24 & 10.14 & Yes & Yes & 0.00 & 1.58 & -5.54 & 2017.002 \\
S5-73 & 18.64 & \text{---} & Unknown Age & 47 & 0 & 2.88 & \text{---} & Yes & \text{---} & 0.00 & -4.84 & -2.02 & 2007.155 \\
S4-500 & 18.64 & \text{---} & Unknown Age & 30 & 0 & 2.20 & \text{---} & No & \text{---} & 0.00 & -1.90 & -4.61 & 2016.582 \\
S6-377 & 18.65 & \text{---} & Unknown Age & 47 & 0 & 4.21 & \text{---} & Yes & \text{---} & 0.00 & 4.80 & -4.48 & 2014.517 \\
S5-13 & 18.65 & \text{---} & Unknown Age & 36 & 0 & 6.50 & \text{---} & Yes & \text{---} & 0.00 & -4.92 & -1.11 & 2007.696 \\
S3-311 & 18.65 & 20.29 & Unknown Age & 46 & 12 & 17.91 & 2.90 & Yes & No & 0.00 & 1.08 & 3.65 & 2007.411 \\
S4-250 & 18.65 & \text{---} & Unknown Age & 52 & 0 & 5.57 & \text{---} & Yes & \text{---} & 0.00 & -3.17 & 3.41 & 2008.123 \\
S5-188 & 18.66 & \text{---} & Unknown Age & 56 & 0 & 4.59 & \text{---} & Yes & \text{---} & 0.00 & 5.31 & 2.37 & 2007.169 \\
S3-301 & 18.67 & \text{---} & Unknown Age & 36 & 0 & 7.29 & \text{---} & Yes & \text{---} & 0.00 & -3.16 & 2.06 & 2007.793 \\
S5-337 & 18.68 & \text{---} & Unknown Age & 34 & 0 & 4.85 & \text{---} & Yes & \text{---} & 0.00 & 3.91 & -3.14 & 2013.532 \\
S2-245 & 18.69 & 21.49 & Unknown Age & 45 & 5 & 4.11 & 8.56 & Yes & No & 0.00 & -0.56 & 2.66 & 2006.948 \\
S3-206 & 18.69 & 20.59 & Unknown Age & 42 & 6 & 2.05 & 4.32 & No & No & 0.00 & -0.18 & 3.54 & 2007.710 \\
S4-351 & 18.69 & 20.57 & Unknown Age & 43 & 13 & 4.27 & 2.24 & Yes & No & 0.00 & 3.41 & -3.60 & 2007.732 \\
S4-499 & 18.71 & 20.90 & Unknown Age & 30 & 7 & 4.79 & 2.06 & Yes & No & 0.00 & -0.01 & -4.37 & 2016.785 \\
S4-493 & 18.72 & \text{---} & Unknown Age & 37 & 0 & 3.30 & \text{---} & Yes & \text{---} & 0.00 & -2.20 & -4.33 & 2015.283 \\
S5-341 & 18.72 & \text{---} & Unknown Age & 32 & 0 & 2.54 & \text{---} & No & \text{---} & 0.00 & -4.86 & -2.56 & 2015.004 \\
S7-248 & 18.73 & 21.07 & Unknown Age & 42 & 5 & 1.67 & 4.40 & No & No & 0.00 & -4.49 & -5.78 & 2015.608 \\
S5-327 & 18.73 & 20.62 & Unknown Age & 39 & 6 & 1.71 & 6.87 & No & No & 0.00 & 1.32 & -5.59 & 2017.260 \\
S5-336 & 18.73 & \text{---} & Unknown Age & 34 & 0 & 6.35 & \text{---} & Yes & \text{---} & 0.00 & 0.93 & -5.92 & 2018.448 \\
S5-335 & 18.73 & \text{---} & Unknown Age & 34 & 0 & 3.78 & \text{---} & Yes & \text{---} & 0.00 & -4.56 & 3.77 & 2015.320 \\
S4-163 & 18.73 & \text{---} & Unknown Age & 72 & 0 & 3.68 & \text{---} & Yes & \text{---} & 0.00 & 3.30 & 2.96 & 2008.290 \\
S6-389 & 18.74 & 20.76 & Unknown Age & 32 & 10 & 1.59 & 2.54 & No & No & 0.00 & 3.97 & -5.31 & 2015.842 \\
S6-382 & 18.74 & \text{---} & Unknown Age & 39 & 0 & 2.13 & \text{---} & No & \text{---} & 0.00 & 3.76 & -5.27 & 2019.327 \\
S3-453 & 18.75 & \text{---} & Unknown Age & 31 & 0 & 6.05 & \text{---} & Yes & \text{---} & 0.00 & -3.26 & 0.85 & 2017.142 \\
S4-41 & 18.76 & 20.47 & Unknown Age & 60 & 6 & 1.79 & 3.51 & No & No & 0.00 & 1.57 & 3.81 & 2007.825 \\
S4-481 & 18.77 & 20.97 & Unknown Age & 45 & 11 & 3.82 & 3.11 & Yes & No & 0.00 & -2.07 & -3.74 & 2016.370 \\
S5-313 & 18.78 & 21.00 & Unknown Age & 54 & 8 & 2.97 & 1.43 & Yes & No & 0.00 & 5.13 & -1.46 & 2016.319 \\
S2-163 & 18.79 & 20.49 & Unknown Age & 50 & 13 & 7.55 & 3.16 & Yes & No & 0.00 & -2.28 & -0.42 & 2006.992 \\
S3-441 & 18.79 & 21.04 & Unknown Age & 63 & 6 & 3.67 & 2.17 & Yes & No & 0.00 & 2.25 & 2.46 & 2016.072 \\
S2-349 & 18.80 & 21.26 & Unknown Age & 44 & 6 & 3.06 & 12.57 & Yes & Yes & 0.00 & -0.63 & 2.81 & 2018.247 \\
S4-151 & 18.81 & \text{---} & Unknown Age & 47 & 0 & 4.72 & \text{---} & Yes & \text{---} & 0.00 & -3.00 & 3.17 & 2007.699 \\
S6-381 & 18.82 & \text{---} & Unknown Age & 41 & 0 & 6.76 & \text{---} & Yes & \text{---} & 0.00 & 4.01 & -5.62 & 2013.928 \\
S5-100 & 18.83 & \text{---} & Unknown Age & 46 & 0 & 4.74 & \text{---} & Yes & \text{---} & 0.00 & 3.53 & -4.02 & 2008.669 \\
S3-210 & 18.84 & \text{---} & Unknown Age & 40 & 0 & 7.58 & \text{---} & Yes & \text{---} & 0.00 & 1.72 & 3.10 & 2007.865 \\
S4-474 & 18.87 & 21.20 & Unknown Age & 60 & 5 & 5.12 & 1.96 & Yes & No & 0.00 & 4.89 & -0.98 & 2015.759 \\
S7-250 & 18.87 & 21.08 & Unknown Age & 40 & 5 & 6.24 & 4.78 & Yes & No & 0.00 & 3.85 & -5.98 & 2014.230 \\
S3-336 & 18.89 & \text{---} & Unknown Age & 31 & 0 & 10.13 & \text{---} & Yes & \text{---} & 0.00 & 2.70 & 2.76 & 2008.486 \\
S5-316 & 18.90 & \text{---} & Unknown Age & 53 & 0 & 3.83 & \text{---} & Yes & \text{---} & 0.00 & 2.15 & -4.62 & 2015.298 \\
S3-177 & 18.92 & 20.86 & Unknown Age & 51 & 9 & 2.37 & 2.83 & Yes & No & 0.00 & -0.60 & 3.39 & 2007.621 \\
S5-0 & 18.93 & 20.84 & Unknown Age & 58 & 8 & 3.30 & 0.60 & Yes & No & 0.00 & 4.30 & 2.58 & 2008.012 \\
S5-334 & 18.95 & \text{---} & Unknown Age & 34 & 0 & 2.37 & \text{---} & No & \text{---} & 0.00 & -2.26 & -5.54 & 2014.586 \\
S3-228 & 19.02 & \text{---} & Unknown Age & 45 & 0 & 3.09 & \text{---} & Yes & \text{---} & 0.00 & -3.60 & -0.11 & 2007.941 \\
S3-321 & 19.03 & \text{---} & Unknown Age & 55 & 0 & 2.50 & \text{---} & Yes & \text{---} & 0.00 & 1.38 & 3.57 & 2008.127 \\
S4-483 & 19.04 & 21.08 & Unknown Age & 43 & 6 & 4.12 & 4.35 & Yes & No & 0.00 & -2.19 & -4.18 & 2015.382 \\
S3-325 & 19.06 & 21.14 & Unknown Age & 31 & 5 & 3.17 & 1.59 & Yes & No & 0.00 & 2.88 & 2.55 & 2007.666 \\
S3-452 & 19.07 & \text{---} & Unknown Age & 32 & 0 & 3.77 & \text{---} & Yes & \text{---} & 0.00 & -3.23 & 1.96 & 2015.644 \\
S5-45 & 19.07 & \text{---} & Unknown Age & 33 & 0 & 3.94 & \text{---} & Yes & \text{---} & 0.00 & 4.32 & 2.82 & 2008.084 \\
S5-87 & 19.10 & \text{---} & Unknown Age & 66 & 0 & 6.08 & \text{---} & Yes & \text{---} & 0.00 & 4.70 & 2.50 & 2007.733 \\
S4-348 & 19.18 & \text{---} & Unknown Age & 46 & 0 & 3.43 & \text{---} & Yes & \text{---} & 0.00 & 4.55 & 1.98 & 2007.118 \\
S5-346 & 19.18 & \text{---} & Unknown Age & 30 & 0 & 3.32 & \text{---} & Yes & \text{---} & 0.00 & -2.18 & -4.61 & 2013.778 \\
S4-492 & 19.20 & \text{---} & Unknown Age & 37 & 0 & 2.80 & \text{---} & Yes & \text{---} & 0.00 & 1.85 & -4.27 & 2015.725 \\
S4-487 & 19.23 & \text{---} & Unknown Age & 40 & 0 & 5.96 & \text{---} & Yes & \text{---} & 0.00 & 2.00 & 3.68 & 2015.235 \\
S3-450 & 19.29 & \text{---} & Unknown Age & 33 & 0 & 6.30 & \text{---} & Yes & \text{---} & 0.00 & -0.70 & 3.57 & 2016.411 \\
S4-498 & 19.29 & \text{---} & Unknown Age & 33 & 0 & 5.33 & \text{---} & Yes & \text{---} & 0.00 & 2.87 & 2.83 & 2018.983 \\
S5-78 & 19.30 & \text{---} & Unknown Age & 32 & 0 & 3.51 & \text{---} & Yes & \text{---} & 0.00 & 3.59 & 3.89 & 2007.656 \\
S5-345 & 19.36 & \text{---} & Unknown Age & 30 & 0 & 1.37 & \text{---} & No & \text{---} & 0.00 & 5.20 & -1.34 & 2015.582
\enddata
\end{deluxetable}
\end{longrotatetable}
